Data Consistency in Transactional Storage Systems: a Centralised Approach

We introduce an interleaving operational semantics for describing the client-observable behaviour of atomic transactions on distributed key-value stores. Our semantics builds on abstract states comprising centralised, global key-value stores and partial client views. We provide operational definitions of consistency models for our key-value stores which are shown to be equivalent to the well-known declarative definitions of consistency model for execution graphs. We explore two immediate applications of our semantics: specific protocols of geo-replicated databases (e.g. COPS) and partitioned databases (e.g. Clock-SI) can be shown to be correct for a specific consistency model by embedding them in our centralised semantics; programs can be directly shown to have invariant properties such as robustness results against a weak consistency model.

==> aexec/anarchic-model.tex <==
\subsection{Anarchic Model}

To justify this semantics capture all the possible abstract executions under certain consistency model,
we introduce \emph{anarchic model}.
Then by \cref{thm:consistency-intersect-anarchic},
the operational semantics captures all possible behaviours of a program \( \prog \) under certain consistency model.


\begin{definition}[Anarchic Model]
\label{def:anarchic-model}
The anarchic resolution policy $\RP_{\anarchic}$ is defined as 
$\RP_{\anarchic}(\_, \_) = \Snapshots$. The \emph{anarchic consistency model} is 
defined axiomatically by the pair $\anarchicCM = (\RP_{\anarchic}, \emptyset)$.
\end{definition}

Under the anarchic model, the initial snapshot of a transaction \( \txid \) is non-deterministic 
and does not depend on its observable transactions \( \txidset \).
When committing, the transaction \( \txid \) is always allowed to do so no matter the state of visibility relation.
Suppose a client $\cl$ has the transactional code below:
\[
\begin{session}
    \begin{transaction}
    \plookup{\pvar{a}}{\key}; \\
    \pifs{\pvar{a} = \val_{1}} \pmutate{\key'}{\val_1} \pife
    \end{transaction}
\end{session}
\]

Let consider executing the transaction under initial state with all keys set to the same initial value \( \val_0 \).
Under $\anarchicCM$, because the snapshot is chosen non-deterministically, 
the transaction might start with an initial snapshot where all keys have the value \( \val_1 \),
which are not necessary equal to \( \val_0 \).
Since there is no constraint on the visibility relation,
such transaction is always allowed to commit.
Consequently, the abstract execution after is the following: 
\begin{center}
\begin{tikzpicture}[scale=0.85, every node/.style={transform shape}]

\node[rounded corners,draw](t0rx) {$(\otR, \key, \val_1)$ \quad $(\otW, \key', \val_1)$}; 

\end{tikzpicture}
\end{center}

It is important to note, however, that the set of abstract executions generated by $\prog$ 
is still bound to the structure of the program.
For example, executing $\prog$ under the anarchic execution model will never lead to 
an abstract execution with multiple transactions, 
or to an abstract execution where a transaction writes a key other than $\key'$ is written.

The \cref{def:axiom-to-cm} defines all the possible abstract executions 
induced by a axiomatic definition $(\RP, \Ax)$.

\begin{definition}[Programs under axiomatic definition]
\label{def:axiom-to-cm}
\label{def:axiom-to-prog}
The semantics of a program $\prog$ under a consistency model with axiomatic definition 
$(\RP, \Ax)$ is given by 
\[
\interpr{\prog}_{(\RP, \Ax)} = \Set{ \aexec }[ (\aexec_{0}, \thdenv_{0}, \prog) \toAEXEC{\_}_{(\RP, \Ax)}^{\ast} (\aexec, \stub, \prog_{f}) ]
\]
where $\thdenv_{0} = \lambda \cl \in \dom(\prog) \ldotp \lambda \vx \ldotp 0$ and $\prog_{f} = \lambda \cl \in \dom(\prog).\pskip$.
\end{definition}

We define the set of all the possible behaviours of a program $\prog$ to be $\interpr{\prog}_{\anarchic}$. 
One may argue that the axiomatic definition $\anarchicCM$ does not truly represent an anarchic consistency model. 
Consider the following code:
\[
\begin{session}
\begin{transaction}
\plookup{\pvar{a}}{\key}; \\
\plookup{\pvar{b}}{\key};\\
\pifs{\pvar{a} != \pvar{b}} \pmutate{\key'}{\val_1} \pife
\end{transaction}
\end{session}
\]
Under a even weaker anarchic consistency model, 
it would be possible for program $\prog'$ to write the value $\val_1$ for key $\key'$. 
However, this never happens if $\prog'$ is executed under our $\anarchicCM$.
Because we embedded into abstract execution the assumption that 
transactions only read at most one value for each key.

We can weaken the anarchic behaviours further by lifting this limitation 
and still retain the validity of all the results contained in this report.
However, the constraint that an object is never read twice in transactions is enforced by atomic visibility, 
so it is unnecessary to lift such limitation of our $\anarchicCM$.

The set of all possible behaviours exhibited by a program $\prog$ under a consistency model $(\RP, \Ax)$ 
can be defined by intersecting the set of executions that $\prog$ exhibits under the anarchic consistency model,
with the set of all executions allowed by the axiomatic definition $(\RP, \Ax)$ (\cref{thm:consistency-intersect-anarchic}).

\begin{theorem}
\label{thm:consistency-intersect-anarchic}
For any program $\prog$ and axiomatic definition $(\RP, \Ax)$:
\[
\interpr{\prog}_{(\RP, \Ax)} = \interpr{\prog}_{\anarchic} \cap \CMa(\RP, \Ax)
\]
\end{theorem}
\begin{proof}
    It is easy to see \( \interpr{\prog}_{(\RP, \Ax)} \subseteq \CMa(\RP, \Ax) \) by \cref{def:axiom-to-cm} 
    so \( \interpr{\prog}_{(\RP, \Ax)} \subseteq \interpr{\prog}_{\anarchic} \cap \CMa(\RP, \Ax) \).
    For another way, by \cref{prop:aexec-semantics-mono}, 
    we know \( \interpr{\prog}_{\anarchic} \subseteq \interpr{\prog}_{(\RP, \Ax)} \).
    Then, by the definition of \( \interpr{\prog}_{\stub} \), it follows
    \( \interpr{\prog}_{\anarchic} \cap \CMa(\RP, \Ax) \subseteq \interpr{\prog}_{(\RP, \Ax)} \).
\end{proof}


\begin{proposition}[Monotonic axiomatic definition]
\label{prop:aexec-semantics-mono}
Let define \( (\RP_1, \Ax_1) \sqsubseteq (\RP_2, \Ax_2) \) as the following:
\[
    \fora{\aexec,\txidset} \RP_2(\aexec,\txidset) \subseteq \RP_1(\aexec,\txidset)
\]
and,
\[
    \fora{\aexec} \bigcup_{\A_1 \in \Ax_1}\A_1(\aexec) \subseteq \bigcup_{\A_2 \in \Ax_2}\A_2(\aexec)
\]
then
\[ \interpr{\prog}_{(\RP, \Ax)} \subseteq \interpr{\prog}_{\anarchic} \]
\end{proposition}
\begin{proof}
    Since \( \anarchic \sqsubseteq (\RP, \Ax) \),
    We prove stronger result that for \( (\RP_1, \Ax_1) \sqsubseteq  (\RP_2, \Ax_2)\),
    the following  hold:
    \[
        \begin{array}{@{}l@{}}
            \fora{\cl, \aexec, \aexec', \prog, \prog', \stk, \stk'} 
            \cl \vdash ( \aexec, \stk ), \prog \toAEXEC{\stub}_{(\RP_1, \Ax_1)} ( \aexec', \stk' ), \prog' 
            \implies \cl \vdash ( \aexec, \stk ), \prog \toAEXEC{\stub}_{(\RP_2, \Ax_2)} ( \aexec', \stk' ), \prog' \\
        \end{array}
    \]
    We prove it by induction on the derivations.
    The only interesting case is the \rl{PAtomicTrans} rule.
    Given an initial runtime abstract execution \( \aexec \),
    a set of observable transactions \( \txidset \),
    a new transaction identifier \( \txid \),
    by the \rl{AAtomicTrans} rule, it is sufficient to prove, 
    first, all the snapshot under the stronger consistency model is also a valid snapshot under the weaker one:
    \begin{equation}
        \label{equ:obs-state-included}
        \fora{\aexec,\txidset} \RP_2(\aexec,\txidset) \subseteq  \RP_1(\aexec,\txidset)
    \end{equation}
    and second if it is valid  to commit a new transition with the observable set \( \txidset \) under stronger consistency model,
    it is able to do so under weaker consistency model:
    \begin{equation}
        \label{equ:consis-both-exist}
        \bigcup_{\A_1 \in \Ax_1}\A_1(\aexec')^{-1}(\txid) \subseteq \bigcup_{\A_2 \in \Ax_2}\A_2(\aexec')^{-1}(\txid)
    \end{equation}
    The \cref{equ:obs-state-included,equ:consis-both-exist} can be proven by \( (\RP_1, \Ax_1) \sqsubseteq  (\RP_2, \Ax_2) \).

    \caseB{\rl{PAssign}, \rl{PAssume}, \rl{PChoice}, \rl{PLoop}, \rl{PSeqSkipS}, \rl{PPar}, \rl{PWait}}
    These base cases do not depend on the consistency model, so they trivial hold because of the hypothesis.
    \caseI{\rl{PSeq}}
    It is proved directly by applying the \ih
\end{proof}


==> appdix-compositionality.tex <==
\section{Proof of \cref{thm:ettraces2sem}}
\label{app:compositionality}
\label{app:exec-test-and-traces}
%\input{\RootPath/composition-et/et-mono.tex}
%\input{\RootPath/composition-et/et-mono-new.tex}
\input{\RootPath/composition-et/normal-trace.tex}
%\input{\RootPath/composition-et/counterexamples-for-mr-ryw.tex}
%\input{\RootPath/composition-et/counterexamples-for-composition.tex}
%\input{\RootPath/composition-et/et-comm.tex}


==> appdix-logic.tex <==
\section{Logic}


\sx{
    Parametrised by CM.

    Generalise CAP by generalise the meaning of box assertions, stable and atomic update rule.

    Two example write skew and long fork.

    Discussion: our first step. For each consistency models, we want to build specific pattern to use the capabilities
    so to provide a more syntactic rules.

    Cite: FCSL(for the idea that recording some history in the assertions), 
    CAP,
    Iris (they have powerful framework, whether it also fits in the weaker consistency world?)
    TaDA
    Relaxed SL (The first separation logic that deal with weaker behaviour)

    Alexey, Reaon about ..... in Dis. Sys. A proof system to verify if 
    a system (a set of operations that might be installed with tokens to specify synchronisation ) satisfies invariant.
}

We present a logic that is parametrised by consistency models that have strong session guarantees.
The logic has syntax that similar to concurrent abstract predicate (CAP),
but we generalise \emph{assertions} and \emph{atomic update rule} so it is parametrised by consistency models.


We motivate the logic by the \emph{write skew} example under snapshot isolation (\cref{fig:write-skew-si-proof}).
This example distinguishes snapshot isolation (SI) from serialisability.
For serialisability that transactions appear one after another, only one key, \( \vx \) or \( \vy \), will be 1 at the end.
While for SI, transactions take a snapshot when they start, and concurrent transactions can commit as long as they write to different keys.
In \cref{fig:write-skew-si-proof}, both transactions may take snapshots where \( \vx \) and \( \vy \) are 0, and can commit, 
which yields result that \( \vx \) and \( \vy \) are 1.

\begin{figure}[!t]
\hrule
\[
\intass :
\begin{array}[t]{@{} c @{\quad} c @{\quad}  @{} }
\begin{rclarray}[t]
    \CB{L} & : & \vx \fpW 1 \sep \vy \fpR 0 \sep \null \fpA \cass{\CB{L}}{\lrid} \\
\end{rclarray}
&
\begin{rclarray}[t]
    \CB{R} & : & \vx \fpR 0 \sep \vy \fpW 1 \sep \null \fpA \cass{\CB{R}}{\lrid} \\
\end{rclarray}
\\
\begin{rclarray}[t]
    \CB{U} & : & \exsts{\V n} \vx \fpR \V{n} \\
\end{rclarray} 
&
\begin{rclarray}[t]
    \CB{U} & : & \exsts{\V n} \vy \fpR \V{n} \\
\end{rclarray} \\
\end{array}
\]
\[
\CB{L} \composeK \CB{L} \ \text{is undefined} \quad  \CB{R} \composeK \CB{R} \ \text{is undefined} \quad \CB{U} \ \text{is the unit}
\]
\hrule\vspace{5pt}
\[
\begin{session}
{\color{blue}P : } \specline{ \cass{\CB{L}}{\lrid} \sep \cass{\CB{R}}{\lrid} \sep \boxass{\vx \pt 0 \sep \vy \pt 0 }{\lrid}{\intass}  } \\
\begin{parl}
\begin{session}
    {\color{blue}P1 : } \specline{\cass{\CB{L}}{\lrid} \sep 
            \boxass{\vx \pt 0 \sep \vy \pt 0 }{\lrid}{\intass} \\
            {} \lor \boxass{\vx \pt 0 \sep ( \vy \pt 0 \lor \vy \pt 1 ) \sep \cass{\CB{R}}{\lrid} }{\lrid}{\intass} 
    } \\
    \txid_1 : \begin{transaction}
        {\color{blue}p1 : } \specline{\vx \fpI 0 \sep ( \vy \fpI 0 \lor \vy \fpI 1 )} \\
        \plookup{\pvar{b}}{\vy} ; 
        \quad \pifs{\pvar{b} = 0} 
        \pmutate{\vx}{1} ;
        \pife \\
        {\color{blue}q1 : } \specline{\vx \fpW 1 \sep  \vy \fpR 0 \lor {}\\
        \quad \vx \fpI 0 \sep \vy \fpR 1 )} \\
    \end{transaction} \\
    {\color{blue}Q1 : } \specline{ 
            \boxass{ \vx \pt 1 \sep \vy \pt 0 \sep \cass{\CB{L}}{\lrid} }{\lrid}{\intass} \\
            {} \lor \boxass{\vx \pt 1 \sep ( \vy \pt 0 \lor \vy \pt 1 ) \sep {} \\
            \cass{\CB{R}}{\lrid} \sep \cass{\CB{L}}{\lrid} }{\lrid}{\intass}  \\
            {} \lor \cass{\CB{L}}{\lrid} \sep \boxass{\vx \pt 0 \sep \vy \pt 1 \sep \cass{\CB{R}}{\lrid} }{\lrid}{\intass}  \\
    } \\
\end{session}
&
\begin{session}
    {\color{blue}P2 : } \specline{\cass{\CB{R}}{\lrid} \sep 
            \boxass{ ( \vx \pt 0 \sep \vy \pt 0 }{\lrid}{\intass} \\
            {} \lor \boxass{ ( \vx \pt 0 \lor \vx \pt 1 ) \sep \vy \pt 0 \sep \cass{\CB{L}}{\lrid} }{\lrid}{\intass} 
    } \\
    \txid_2 : \begin{transaction}
        {\color{blue}p2 : } \specline{ ( \vx \fpI 0 \lor \vx \fpI 1 ) \sep \vy \fpI 0 )} \\
        \plookup{\pvar{a}}{\vx} ; 
        \quad \pifs{\pvar{a} = 0} 
        \pmutate{\vy}{1} ; 
        \pife \\
        {\color{blue}q2 : } \specline{ \vx \fpR 0 \sep \vy \fpW 1 \lor {} \\
        \quad \vx \fpR 1 \sep \vy \fpI 0 )} \\
    \end{transaction} \\
    {\color{blue}Q2 : } \specline{ 
            \boxass{ \vx \pt 0 \sep \vy \pt 1 \sep \cass{\CB{R}}{\lrid} }{\lrid}{\intass} \\
            {} \lor \boxass{ ( \vx \pt 0 \lor \vx \pt 1 ) \sep \vy \pt 1 \sep {} \\
            \cass{\CB{L}}{\lrid} \sep \cass{\CB{R}}{\lrid} }{\lrid}{\intass}  \\
            {} \lor \cass{\CB{R}}{\lrid} \sep \boxass{\vx \pt 1 \sep \vy \pt 0 \sep \cass{\CB{L}}{\lrid} }{\lrid}{\intass}  \\
    } \\
\end{session}
\end{parl} \\
{\color{blue}Q : } \specline{ 
        \cass{\CB{L}}{\lrid} \sep \boxass{ \vx \pt 0 \sep \vy \pt 1 \sep \cass{\CB{R}}{\lrid} }{\lrid}{\intass} 
        \lor \cass{\CB{R}}{\lrid} \sep \boxass{\vx \pt 1 \sep \vy \pt 0 \sep \cass{\CB{L}}{\lrid} }{\lrid}{\intass}
        \lor \boxass{ \vx \pt 1 \sep \vy \pt 1 \sep \cass{\CB{L}}{\lrid} \sep \cass{\CB{R}}{\lrid} }{\lrid}{\intass}  \\
} \\
\end{session}
\]
\hrule
\caption{Interference (the top) and the sketch proof (the bottom) for write skew under snapshot isolation}
\label{fig:write-skew-si-proof}
\end{figure}

We often use \( \lpre, \lpost \) to denote \emph{transactional assertions} and \( \gpre, \gpost \) for \emph{program assertions}.
The transactional assertions, such as \( p1 \) in \cref{fig:write-skew-si-proof}, 
describe the state of local snapshots for transactions and more importantly the fingerprints.
The fingerprint is the transaction's contribution to the key-value store, that is, \emph{the first read preceding any write} and \emph{last write} of each key.
The transactional assertions for individual keys have the following forms: \( \vx \fpI 0 \), \( \vx \fpR 0\), \( \vx \fpW 0\), and \( \vx \fpRW (0,1) \),
where \( \otR \) and \( \otW \) are read and write labels respectively.
The first three asserts the only key \( \vx \) in the local snapshot has value 0 and it has not been touched (no label), 
has been read (\(\otR\)) and has been written (\(\otW\)) respectively.
The last one asserts that the key \( \vx \) currently has value 1, 
\emph{the first read preceding any write} fetched 0 and the \emph{the last write} updated the key to \( 1 \).
We extend the standard sequential separation logic rules in a ways that the first read to a key adds a read label to the assertion; 
and a write to a key adds a write label to assertion and updates the value.
It is easy to see that transactional assertions are interpreted as pairs of snapshots and fingerprints.
We use \( (\sn,\fp) \in \evalLS{\lpre} \) to denote the snapshot \( \sn \) and fingerprint \( \fp \) satisfy 
the assertion \( \lpre \) under the stack \( \stk \) and logical environment \( \lenv \).
All the detail is in \cref{sec:reasoning-transaction}.

The program assertions, such as \( P1 \) in \cref{fig:write-skew-si-proof}, 
describe clients' views on key-value stores, together with some capabilities for the purpose of reasoning.
The assertion in the form of \( \boxass{\bar{\lpre}}{\lrid}{\intass}\),
for example \( \boxass{\vx \pt 1 \sep \vy \pt 1}{\lrid}{\intass} \) in \( \gpre_1 \),
is called the \emph{shared region assertions} also know as \emph{boxed assertions},
where \( \lrid \) is a unique \emph{region identifier},  \( \intass \) is \emph{interference},
and \( \lpre \) describes the views on key-value stores.
Region are shareable and indivisible, \ie 
\( \boxass{\bar{\lpre}}{\lrid}{\intass} \sep \boxass{\bar{\lpost}}{\lrid}{\intass} \iff \boxass{\bar{\lpre} \land \bar{\lpost}}{\lrid}{\intass}\).

Interference is a set of actions to specify what transactions are allowed by the region.
Each action has the form \( \kap : \assfp \),
where \( \kap \) is the \emph{client-specified capability} and \( \assfp \) is the \emph{fingerprint},
describes that if a client holds the capability \( \kap \), 
it is allowed to execute a transaction with the fingerprint \( \assfp \).
For instance in \cref{fig:write-skew-si-proof}, 
the \( \CB{L}\) allows a client to read \( \vy \) when it is 0 (\(\vy \fpR 0\)) and write 1 to \( \vx \) (\(\vx \fpW 1\)),
and similarly \( \CB{R} \) allows a client to read \( \vx \) when it is 0 and write 1 to \( \vy \).
The fingerprint \( \assfp \) in an action also specifies capabilities transformation.
For example, \( \null \fpA \cass{\CB{L}}{\lrid} \) means that \( \CB{L} \) needs to return to the shared region after the transaction is committed.
Last, the capabilities forms \emph{a partial commutative monoid (PCM)} where \( \composeK \) denotes the composition function.
In the write skew example (\cref{fig:write-skew-si-proof}), 
both \( \CB{L} \) and \( \CB{R} \) are unique as the compositions are undefined and \( \CB{U} \) is the unit.

Interference induces a label transitions system upon states \( (\mkvs, \vi, \ca) \)
where the labels are actions from the interference.
Then the \emph{invariant} of a region \( \func{inv}{\lrid} \) is the set of states reachable from 
the initial states of the regions provided by the function \( \func{init}{\lrid}\).

Given the invariant, a state \( (\mkvs, \vi, \ca) \) satisfies the assertion \( \boxass{\bar{\lpre}}{\lrid}{\intass} \),
if it is in the invariant of the region \( (\mkvs, \vi, \ca) \in \func{inv}{\lrid} \) and the snapshot induced by the view \( \snapshot[\mkvs, \vi] \) and 
the shared capabilities satisfy \( \bar{\lpre} \) (details in \cref{def:prog-assertion}).

Now let discuss the sketch proof in \cref{fig:write-skew-si-proof}, 
especially the \(\rl{PRCommit} \) rule for committing a transaction (other rules are standard and can be found in \cref{sec:reasoning-prog}):
\[
    \inferrule[\rl{PRCommit}]{%
        \tripleL{\lpre}{\trans}{\lpost} 
        \\ \repartition{\gpre}{\gpost}{\lpre}{\lpost}
        \\\\ \stable{\gpre, \ET} 
        \\ \stable{\gpost, \ET} 
    }{%
        \tripleG{\gpre}{ \ptrans{\trans} }{\gpost}
    }
\]
An assertion \( \gpre \) is \emph{stable} under execution test \( \ET \), written \( \stable{\gpre, \ET} \), if it is true against the interference.
Stabilisation needs to takes the following two situations into account: 
\textbf{(i)} the environment might interfere and change the state of key-value stores, 
note that, but not the views of the current client since the views are local; 
\textbf{(ii)} consequentially, the client might advance the views.
For example, \( P1 \) is stable as it describes the states that 
either the environment does nothing \( \boxass{\vx \pt 0 \sep \vy \pt 0 }{\lrid}{\intass} \),
or the environment has performed the action associated with \( \cass{\CB{R}}{\lrid}\), 
after which the environment cannot do any further action since the capabilities \( \cass{\CB{R}}{\lrid}\) is in the shared region,
\ie \( \boxass{\vx \pt 0 \sep ( \vy \pt 0 \lor \vy \pt 1 ) \sep \cass{\CB{R}}{\lrid} }{\lrid}{\intass}  \).
Let discuss further the assertions \( \vx \pt 0 \sep ( \vy \pt 0 \lor \vy \pt 1 ) \sep \cass{\CB{R}}{\lrid} \).
The environment returns the capability \( \cass{\CB{R}}{\lrid} \), 
it means the environment commits a transaction that writes 1 to \( \vy \) and the capability \( \cass{\CB{R}}{\lrid} \), 
yet since the current client still have the \( \vy \pt 0 \) as its view on the \( \vy \).
Afterword, the view might be advanced so we get an more up-to-date view with \( \vy \pt 1 \).

We generalise the \emph{repartitioning} \( \repartition{\gpre}{\gpost}{\lpre}{\lpost} \) from CAP \cite{cap}:
\begin{definition}[Repartitioning]
The repartitioning  \( \repartition{\gpre}{\gpost}{\lpre}{\lpost} \) is defined as that 
given any key-value store, view and capabilities, \( (\mkvs, \vi, \ca) \) that satisfy the precondition \( \gpre \):
\begin{itemize}
    \item the snapshot \( \snapshot[\mkvs,\vi] \) together with empty fingerprint satisfies the transactional precondition \( \lpre \); and
    \item for any snapshot and fingerprint \( \fp \) satisfy the transactional postcondition \( \lpost \), if
        there exists a new key-value store \( \mkvs' \), a new view \( \vi' \) and new capabilities \( \ca' \) such that 
    \begin{itemize}
        \item the new key-value store \( \mkvs' \in \updateKV(\mkvs, \vi, \stub, \fp) \),
        \item the update is allowed by the execution test, \ie \( (\mkvs, \vi) \csat \fp : \vi' \), and
        \item the transition from \( (\mkvs, \vi, \ca) \) to \( (\mkvs', \vi', \ca') \) is allowed by guarantee, \ie some local capabilities,
    \end{itemize} 
\end{itemize}
then the state \( (\mkvs', \vi', \ca') \) satisfies the postcondition \( \gpost \).
\end{definition}

For example,  let consider the transaction \( \txid_1 \) in \cref{fig:write-skew-si-proof}.
The precondition \( P1 \) asserts following views:

%\begin{center}
%\begin{tikzpicture}
%\begin{pgfonlayer}{foreground}
%%\draw[help lines] grid(5,4);

%%Location x
%\node(locx) {$\vx \mapsto$};

%\matrix(versionx) [version list]
    %at ([xshift=\tikzkvspace]locx.east) {
    %{a} \& $\txid_0$ \\
    %{a} \& $\emptyset $ \\
%};
%\tikzvalue{versionx-1-1}{versionx-2-1}{locx-v0}{$0$};

%%Location y
%\path (locx.south) + (0,\tikzkeyspace) node (locy) {$\vy \mapsto$};
%\matrix(versiony) [version list]
   %at ([xshift=\tikzkvspace]locy.east) {
  %{a} \& $\txid_0$  \\
  %{a} \& $\emptyset $ \\
%};

%\tikzvalue{versiony-1-1}{versiony-2-1}{locy-v0}{$0$};

%\end{pgfonlayer}
%\end{tikzpicture}
%%
%\quad
%%
%\begin{tikzpicture}
%\begin{pgfonlayer}{foreground}
%%\draw[help lines] grid(5,4);

%%Location x
%\node(locx) {$\vx \mapsto$};

%\matrix(versionx) [version list]
    %at ([xshift=\tikzkvspace]locx.east) {
    %{a} \& $\txid_0$ \\
    %{a} \& $\Set{\txid}$  \\
%};
%\tikzvalue{versionx-1-1}{versionx-2-1}{locx-v0}{$0$};

%%Location y
%\path (locx.south) + (0,\tikzkeyspace) node (locy) {$\vy \mapsto$};
%\matrix(versiony) [version list, column 3/.style={dotted}, column 4/.style={dotted}]
   %at ([xshift=\tikzkvspace]locy.east) {
       %{a} \& $\txid_0$ \& {a} \& \color{gray}$\txid$ \\
  %{a} \& $\emptyset$ \& {a} \&  \color{gray} $\emptyset$\\
%};

%\tikzvalue{versiony-1-1}{versiony-2-1}{locy-v0}{$0$};
%\node[version node,draw=none,fit=(versiony-1-3) (versiony-2-3),fill=white, inner sep=0pt] (locx-v1) {\color{gray}$1$};

%\end{pgfonlayer}
%\end{tikzpicture}
%%
%\quad
%%
%\begin{tikzpicture}
%\begin{pgfonlayer}{foreground}
%%\draw[help lines] grid(5,4);

%%Location x
%\node(locx) {$\vx \mapsto$};

%\matrix(versionx) [version list]
    %at ([xshift=\tikzkvspace]locx.east) {
    %{a} \& $\txid_0$ \\
    %{a} \& $\Set{\txid}$  \\
%};
%\tikzvalue{versionx-1-1}{versionx-2-1}{locx-v0}{$0$};

%%Location y
%\path (locx.south) + (0,\tikzkeyspace) node (locy) {$\vy \mapsto$};
%\matrix(versiony) [version list]
   %at ([xshift=\tikzkvspace]locy.east) {
 %{a} \& $\txid_0$ \& {a} \& $\txid$ \\
  %{a} \& $\emptyset$ \& {a} \& $\emptyset$\\
%};

%\tikzvalue{versiony-1-1}{versiony-2-1}{locy-v0}{$0$};
%\tikzvalue{versiony-1-3}{versiony-2-3}{locy-v1}{$1$};

%\end{pgfonlayer}
%\end{tikzpicture}
%\end{center}
%Note that the they must satisfy the invariant of the region \( \lrid \).
%The transactional precondition \( p1 \) describes exactly the snapshots given the views above.
%The transaction \( \txid_1 \) has the fingerprints \( \Set{(\otW, \vx, 1), (\otR, \vy, 0)} \) or  
%\( \Set{(\otR, \vx, 1)} \) by the transactional postcondition \( \lpost \).
%The repartitioning asserts that any new key-value stores \( \mkvs' \) and new views \( \vi' \)
%by committing the fingerprint under snapshot isolation \( \SI \):
%\begin{center}
%\begin{tikzpicture}
%\begin{pgfonlayer}{foreground}
%%\draw[help lines] grid(5,4);

%%Location x
%\node(locx) {$\vx \mapsto$};

%\matrix(versionx) [version list, column 2/.style={text width=7mm}]
    %at ([xshift=\tikzkvspace]locx.east) {
        %{a} \& $\txid_0$ \& {a} \& $\txid'$ \\
        %{a} \& $\emptyset$ \& {a} \& $\emptyset$ \\
%};
%\tikzvalue{versionx-1-1}{versionx-2-1}{locx-v0}{$0$};
%\tikzvalue{versionx-1-3}{versionx-2-3}{locx-v1}{$1$};

%%Location y
%\path (locx.south) + (0,\tikzkeyspace) node (locy) {$\vy \mapsto$};
%\matrix(versiony) [version list, column 2/.style={text width=7mm}]
   %at ([xshift=\tikzkvspace]locy.east) {
  %{a} \& $\txid_0$  \\
  %{a} \& $\Set{\txid'}$ \\
%};

%\tikzvalue{versiony-1-1}{versiony-2-1}{locy-v0}{$0$};

%\end{pgfonlayer}
%\end{tikzpicture}
%%
%\quad
%%
%\begin{tikzpicture}
%\begin{pgfonlayer}{foreground}
%%\draw[help lines] grid(5,4);

%%Location x
%\node(locx) {$\vx \mapsto$};

%\matrix(versionx) [version list, column 2/.style={text width=7mm}]
    %at ([xshift=\tikzkvspace]locx.east) {
        %{a} \& $\txid_0$ \& {a} \& $\txid'$ \\
        %{a} \& $\Set{\txid}$ \& {a} \& $\emptyset$ \\
%};
%\tikzvalue{versionx-1-1}{versionx-2-1}{locx-v0}{$0$};
%\tikzvalue{versionx-1-3}{versionx-2-3}{locx-v1}{$1$};

%%Location y
%\path (locx.south) + (0,\tikzkeyspace) node (locy) {$\vy \mapsto$};
%\matrix(versiony) [version list, column 2/.style={text width=7mm}, column 3/.style={dotted}, column 4/.style={dotted}]
   %at ([xshift=\tikzkvspace]locy.east) {
       %{a} \& $\txid_0$ \& {a} \& \color{gray}$\txid$ \\
       %{a} \& $\Set{\txid'}$ \& {a} \&  \color{gray} $\emptyset$\\
%};

%\tikzvalue{versiony-1-1}{versiony-2-1}{locy-v0}{$0$};
%\node[version node,draw=none,fit=(versiony-1-3) (versiony-2-3),fill=white, inner sep=0pt] (locx-v1) {\color{gray}$1$};

%\end{pgfonlayer}
%\end{tikzpicture}
%%
%\quad
%%
%\begin{tikzpicture}
%\begin{pgfonlayer}{foreground}
%%\draw[help lines] grid(5,4);

%%Location x
%\node(locx) {$\vx \mapsto$};

%\matrix(versionx) [version list]
    %at ([xshift=\tikzkvspace]locx.east) {
    %{a} \& $\txid_0$ \\
    %{a} \& $\Set{\txid}$  \\
%};
%\tikzvalue{versionx-1-1}{versionx-2-1}{locx-v0}{$0$};

%%Location y
%\path (locx.south) + (0,\tikzkeyspace) node (locy) {$\vy \mapsto$};
%\matrix(versiony) [version list]
   %at ([xshift=\tikzkvspace]locy.east) {
 %{a} \& $\txid_0$ \& {a} \& $\txid$ \\
  %{a} \& $\emptyset$ \& {a} \& $\emptyset$\\
%};

%\tikzvalue{versiony-1-1}{versiony-2-1}{locy-v0}{$0$};
%\tikzvalue{versiony-1-3}{versiony-2-3}{locy-v1}{$1$};

%\end{pgfonlayer}
%\end{tikzpicture}
%\end{center}
they should satisfy the postcondition \( \gpost \).
It is easy to see that
the fingerprint \( \Set{(\otW, \vx, 1), (\otR, \vy, 0)} \) is allowed to commit 
by \( \cass{\CB{R}}{\lrid} \) after which it returns to the region,
and \( \Set{(\otR, \vy, 1)} \) is allowed by \( \CB{U} \).
This will give us a postcondition \emph{before stabilisation}:
\[
\boxass{ \vx \pt 1 \sep \vy \pt 0 \sep \cass{\CB{L}}{\lrid} }{\lrid}{\intass} 
\lor \boxass{\vx \pt 1 \sep \vy \pt 1  \sep \cass{\CB{R}}{\lrid} \sep \cass{\CB{L}}{\lrid} }{\lrid}{\intass}
\lor \cass{\CB{L}}{\lrid} \sep \boxass{\vx \pt 0 \sep \vy \pt 1 \sep \cass{\CB{R}}{\lrid} }{\lrid}{\intass} 
\]
By stabilisation we will get the final postcondition \( \gpost_1 \) shown in \cref{fig:write-skew-si-proof}.


We can also prove the \emph{long fork} (\cref{.......}), 
which distinguish snapshot isolation (SI) from parallel snapshot isolation (PSI).
We use the similar pattern by putting back the capabilities to the region once the capabilities has been used for helping the reasoning.


\input{\RootPath/logic/transaction.tex}
\input{\RootPath/logic/program.tex}
\input{\RootPath/logic/trans_sound.tex}
\input{\RootPath/logic/prog_sound.tex}


==> appdix-property-et-example.tex <==
\section{Properties of execution tests in \cref{fig:execution.tests}}
\label{sec:property-et}

\Cref{sec:comm-et-example} presents proofs for commutativity of several execution tests shown in \cref{fig:execution-tests}.
Note that all the proofs in \Cref{sec:comm-et-example} rely on the commutativity of the \(\updateKV \) function shown in \cref{sec:updatekv-comm}.

\input{\RootPath/composition-et/updatekv-comm.tex}
\input{\RootPath/composition-et/comm-et-example.tex}
\input{\RootPath/composition-et/counter-example-si-not-cp-ua.tex}
%\input{\RootPath/composition-et/matching-view-et-example.tex}


==> composition-et/comm-et-example.tex <==
\subsection{Commutativity of execution tests}
\label{sec:comm-et-example}

To recall, an execution test is $\ET$ is \emph{commutative} if, whenever $(\cl_1, \vi_1, \fp_1)$, 
$(\cl_2, \vi_2, \fp_2)$ are non-conflicting, and $\vi_1, \vi_2 \in \Views(\mkvs_0)$,  
then for any $\mkvs_0, \mkvs', \vienv, \vienv'$ we have that 
\begin{centermultline}
(\mkvs_0, \vienv) \toET{(\cl_1, \fp_1)}
\stub \toET{(\cl_2, \fp_2)} (\mkvs', \vienv') \\
{} \implies
(\mkvs_0, \vienv) \toET{(\cl_2, \fp_2)} 
\stub \toET{(\cl_1, \fp_1)} (\mkvs', \vienv'') 
\land \vienv''(\cl_2) \viewleq \vienv'(\cl_2)
\end{centermultline}

\begin{lemma}
    \label{lem:mr-comm}
    \(\MR\) is commutative.
\end{lemma}
\begin{proof}
    Let assume:
    \[
        \mkvs_0, \vienv_0 \toET{\cl_1, \fp_1}[\MR] \mkvs_1, \vienv_1 \toET{\cl_2, \fp_2}[\MR] \mkvs_2, \vienv_2 
    \]
    where \( \cl_1 \neq \cl_2 \), \( \fora{ \key,\val } (\otW, \key, \val) \notin \fp_1 \cap \fp_2 \).
    Let \(\vi_1 = \vienv_0(\cl_1) \) and \( \vi_2 = \vienv_1(\cl_2)\).
    Assume \( \vi_1, \vi_2 \in \Views(\mkvs_0)\) and the transaction identifiers are \( \txid_1 \) and \( \txid_2 \) respectively.
    Given the specification of \(\MR\) (\cref{fig:execution-tests}), we know \( \vienv_1 = \vienv_0\rmto{\cl}{\vi'_1}\) for some \( \vi'_1 \) such that \( \vi_1 \sqsubseteq \vi'_1 \).
    Similarly \( \vienv_2 = \vienv_1\rmto{\cl'}{\vi'_2} \) for some \( \vi'_2 \) such that \(  \vi_2 \sqsubseteq \vi'_2 \). 
    We pick \( \mkvs'_1 \) and \( \vienv'_1 \) such that \( \mkvs'_1 = \updateKV[\mkvs_0,\vi_2,\fp_2,\txid_2] \) and \( \vienv'_1 = \vienv_0\rmto{\cl_2}{\vi''_2} \),
    where \( \vi''_2 = \lambda \key \ldotp \Set{ i }[ i \in \vi'_2(\key) \land i < \abs{\mkvs'_1(\key)}] \).
    Note that \( \vi''_2 \in \Views(\mkvs_1') \) and \( \vi''_2 \viewleq \vi'_2 \).
    Thus we have:
    \[
        \mkvs_0, \vienv_0 \toET{\cl_2, \fp_2}[\MR] \mkvs'_1, \vienv'_1 \toET{\cl_1,\fp_1}[\MR] \mkvs_2, \vienv'_2 
    \]
    for some \( \vienv'_2 \) such that \( \vienv'_2(\cl_2) \viewleq \vienv_2(\cl_2) \).
\end{proof}                                                                                    

\begin{lemma}
    \label{lem:mw-comm}
    \(\MW\) is commutative.
\end{lemma}
\begin{proof}
    Let assume:
    \[
        \mkvs_0, \vienv_0 \toET{\cl_1, \fp_1}[\MW] \mkvs_1, \vienv_1 \toET{\cl_2, \fp_2}[\MW] \mkvs_2, \vienv_2 
    \]
    where \( \cl_1 \neq \cl_2 \), \( \fora{ \key,\val } (\otW, \key, \val) \notin \fp_1 \cap \fp_2 \).
    Let \(\vi_1 = \vienv_0(\cl_1) \) and \( \vi_2 = \vienv_1(\cl_2)\).
    Assume \( \vi_1, \vi_2 \in \Views(\mkvs_0)\) and the transaction identifiers are \( \txid_1 \) and \( \txid_2 \) respectively.
    Since \( \vi_2  \in \Views(\mkvs_0) \), it means \( \vi_2 \) cannot observe the transaction \( \txid_1 \), \ie \( \txid_1 \notin \Tx(\mkvs_1,\vi_2) \).
    Because of \( \vi_2  \in \Views(\mkvs_0) \) and \( \allowed[\mkvs_1,\vi_2,\SO\rflx] \), it means \( \allowed[\mkvs_0,\vi_2,\SO\rflx] \).
    We pick \( \mkvs'_1 \) and \( \vienv'_1 \) such that \( \mkvs'_1 = \updateKV[\mkvs_0,\vi_2,\fp_2,\txid_2] \) and \( \vienv'_1 = \vienv_0\rmto{\cl_2}{\vienv_2(\vi''_2)} \)
    where \( \vi''_2 = \lambda \key \ldotp \Set{ n }[ n \in \vi'_2(\key) \land n < \abs{\mkvs'_1(\key)}] \).
    We now prove \( \allowed[\mkvs'_1,\vi_1,\SO\rflx] \).
    Let consider that \( \txid_2 \) has installed some new versions (i-\emph{th}) for some keys \( \key \).
    It must be the case:
    \[
        i = \abs{\mkvs'_1(\key)} - 1  = \abs{\mkvs_0(\key)}
    \]
    \begin{enumerate*}
        \item Because of \( \vi_1 \in \Views(\mkvs_0)\), it follows \( i > \max(\vi_1(\key))\);
        \item the transaction \( \txid_2 \) is the last transaction from its client \( \fora{ \txid \in \mkvs'_1} \neg \left(\txid_2 \toEDGE{\SO} \txid\right) \).
        \item the \(\allowed[\mkvs_0,\vi_1,\SO\rflx] \) predicate holds.
    \end{enumerate*}
    Combining above, we know \( \allowed[\mkvs'_1,\vi_1,\SO\rflx] \), and so:
    \[
        \mkvs_0, \vienv_0 \toET{\cl_2, \fp_2}[\MW] \mkvs'_1, \vienv'_1 \toET{\cl_1,\fp_1}[\MW] \mkvs_2, \vienv'_2 
    \]
    for some \( \vienv'_2 \) such that \( \vienv'_2(\cl_2) \viewleq \vienv_2(\cl_2) \).
\end{proof}


\begin{lemma}
    \label{lem:ryw-comm}
    \(\RYW\) is commutative.
\end{lemma}
\begin{proof}
    Let assume:
    \[
        \mkvs_0, \vienv_0 \toET{\cl_1, \fp_1}[\RYW] \mkvs_1, \vienv_1 \toET{\cl_2, \fp_2}[\RYW] \mkvs_2, \vienv_2 
    \]
    where \( \cl_1 \neq \cl_2 \), \( \fora{ \key,\val } (\otW, \key, \val) \notin \fp_1 \cap \fp_2 \).
    Let \(\vi_1 = \vienv_0(\cl_1) \) and \( \vi_2 = \vienv_1(\cl_2)\).
    Assume \( \vi_1, \vi_2 \in \Views(\mkvs_0)\) and the transaction identifiers are \( \txid_1 \) and \( \txid_2 \) respectively.
    We pick \( \mkvs'_1 \) and \( \vienv'_1 \) such that \( \mkvs'_1 = \updateKV[\mkvs_0,\vi_2,\fp_2,\txid_2] \) and \( \vienv'_1 = \vienv_0\rmto{\cl_2}{\vi''_2} \),
    where \( \vi''_2 = \lambda \key \ldotp \Set{ i }[ i \in \vi'_2(\key) \land i < \abs{\mkvs'_1(\key)}] \).
    It is trivial to see:
    \[
        \mkvs_0, \vienv_0 \toET{\cl_2, \fp_2}[\RYW] \mkvs'_1, \vienv'_1 \toET{\cl_1,\fp_1}[\RYW] \mkvs_2, \vienv'_2 
    \]
    for some \( \vienv'_2 \) such that \( \vienv'_2(\cl_2) \viewleq \vienv_2(\cl_2) \).
\end{proof}

\begin{lemma}
    \label{lem:wfr-comm}
    \(\WFR\) is commutative.
\end{lemma}
\begin{proof}
    Let assume:
    \[
        \mkvs_0, \vienv_0 \toET{\cl_1, \fp_1}[\WFR] \mkvs_1, \vienv_1 \toET{\cl_2, \fp_2}[\WFR] \mkvs_2, \vienv_2 
    \]
    where \( \cl_1 \neq \cl_2 \), \( \fora{ \key,\val } (\otW, \key, \val) \notin \fp_1 \cap \fp_2 \).
    Let \(\vi_1 = \vienv_0(\cl_1) \) and \( \vi_2 = \vienv_1(\cl_2)\).
    Assume \( \vi_1, \vi_2 \in \Views(\mkvs_0)\) and the transaction identifiers are \( \txid_1 \) and \( \txid_2 \) respectively.
    We pick \( \mkvs'_1 \) and \( \vienv'_1 \) such that \( \mkvs'_1 = \updateKV[\mkvs_0,\vi_2,\fp_2,\txid_2] \) and \( \vienv'_1 = \vienv_0\rmto{\cl_2}{\vienv_2(\vi''_2)} \)
    where \( \vi''_2 = \lambda \key \ldotp \Set{ n }[ n \in \vi'_2(\key) \land n < \abs{\mkvs'_1(\key)}] \).
    We now prove \( \allowed[\mkvs'_1,\vi_1, \WR_{\mkvs'_1} ; \SO\rflx] \).
    Let consider that \( \txid_2 \) has installed some new versions (i-\emph{th}) for some keys \( \key \).
    It must be the case:
    \[
        i = \abs{\mkvs'_1(\key)} - 1  = \abs{\mkvs_0(\key)}
    \]
    \begin{enumerate*}
        \item Because of \( \vi_1 \in \Views(\mkvs_0)\), it follows \( i > \max(\vi_1(\key))\);
        \item the transaction \( \txid_2 \) is the last transaction from its client \( \fora{ \txid \in \mkvs'_1} \neg \left(\txid_2 \toEDGE{\SO} \txid\right) \).
        \item the \(\allowed[\mkvs_0,\vi_1,\WR_{\mkvs_0} ; \SO\rflx] \) predicate holds.
    \end{enumerate*}
    Combining above, we know \( \allowed[\mkvs'_1,\vi_1,\WR_{\mkvs'_1} ; \SO\rflx] \), and so:
    \[
        \mkvs_0, \vienv_0 \toET{\cl_2, \fp_2}[\WFR] \mkvs'_1, \vienv'_1 \toET{\cl_1,\fp_1}[\WFR] \mkvs_2, \vienv'_2 
    \]
    for some \( \vienv'_2 \) such that \( \vienv'_2(\cl_2) \viewleq \vienv_2(\cl_2) \).

\end{proof}

\begin{proposition}
    \label{lem:cc-comm}
    \label{prop:cc-comm}
    \( \CC \) is commutative.
\end{proposition}
\begin{proof}
    Because \( \CC = \MR \cap \MW \cap \RYW \cap \WFR \) and all four are commutative (\cref{lem:mr-comm,lem:mw-comm,lem:ryw-comm,lem:wfr-comm}), so \( \CC \) is commutative by the \cref{prop:appendix-et-composition-2}.
\end{proof}

\begin{lemma}
    \label{lem:ua-comm}
    \(\UA\) is commutative.
\end{lemma}
\begin{proof}
    Let assume:
    \[
        \mkvs_0, \vienv_0 \toET{\cl_1, \fp_1}[\UA] \mkvs_1, \vienv_1 \toET{\cl_2, \fp_2}[\UA] \mkvs_2, \vienv_2 
    \]
    where \( \cl_1 \neq \cl_2 \), \( \fora{ \key,\val } (\otW, \key, \val) \notin \fp_1 \cap \fp_2 \).
    Let \(\vi_1 = \vienv_0(\cl_1) \) and \( \vi_2 = \vienv_1(\cl_2)\).
    Assume \(\vi_1, \vi_2 \in \Views(\mkvs_0)\) and the transaction identifiers are \( \txid_1 \) and \( \txid_2 \) respectively.
    We pick \( \mkvs'_1 \) and \( \vienv'_1 \) such that \( \mkvs'_1 = \updateKV[\mkvs_0,\vi_2,\fp_2,\txid_2] \) and \( \vienv'_1 = \vienv_0\rmto{\cl_2}{\vi''_2} \),
    where \( \vi''_2 = \lambda \key \ldotp \Set{ i }[ i \in \vi'_2(\key) \land i < \abs{\mkvs'_1(\key)}] \).
    Let consider keys \( \key \) such that \( (\otW,\key,\stub) \in \f_1 \).
    Those keys cannot be overwritten by \( \f_2 \), \ie \( \fora{\val} (\otW,\key,\val) \notin \fp_2 \),
    which means \( \abs{\mkvs_0(\key)} = \abs{\mkvs'_1(\key)} \).
    Since \( \vi_1(\key) = \Set{n}[0 \leq n < \abs{\mkvs_0(\key)}]\), so \( \vi_1(\key) = \Set{n}[0 \leq n < \abs{\mkvs'_1(\key)}]\).
    Thus we have:
    \[
        \mkvs_0, \vienv_0 \toET{\cl_2, \fp_2}[\UA] \mkvs'_1, \vienv'_1 \toET{\cl_1,\fp_1}[\UA] \mkvs_2, \vienv'_2 
    \]
    for some \( \vienv'_2 \) such that \( \vienv'_2(\cl_2) \viewleq \vienv_2(\cl_2) \).
\end{proof}

\begin{proposition}
    \( \PSI \) are commutative.
\end{proposition}
\begin{proof}
    because \( \PSI = \CC \cap \UA \) and both of them are commutative (\cref{lem:cc-comm,lem:ua-comm}), so \( \PSI \) is commutative by the \cref{prop:appendix-et-composition-2}.
\end{proof}

\begin{lemma}
    \label{lem:ser-comm}
    \( \SER \) is commutative.
\end{lemma}
\begin{proof}
    Given the specification for \( \SER \) (\cref{fig:execution-tests}), the hypothesis that \( \vi, \vi' \in \Views(\mkvs_0) \) never holds.
\end{proof}

\subsection{\( \CP \) and \( \PSI \) are not commutativity}
\label{sec:comm-counter-cp-si}

\( \CP \) and \( \PSI \) are not commutative because the view after update must be up-to-date.
We should the following counter example why \( \CP \) and \( \SI \) are not commutative.
Let consider an initial kv-store \( \mkvs \) (some writers are omitted):
\begin{centertikz}
%Location x
\node(locx) {$\key_1 \mapsto$};
\draw pic at ([xshift=\tikzkvspace]locx.east) {vlist={versionx}{%
    /$0$/$\stub$/$\emptyset$
    , /$1$/$\txid$/$\emptyset$
}};

%Location y
\path (versionx.east) + (1,0) node (locy) {$\key_2 \mapsto$};
\draw pic at ([xshift=\tikzkvspace]locy.east) {vlist={versiony}{%
    /$2$/$\stub$/$\emptyset$
    , /$3$/$\stub$/$\emptyset$
}};
\end{centertikz}
Assume two clients, \( \cl_1 \) and \( \cl_2 \), want to read the two keys \( \key_1 \) and \( \key_2 \).
Let assume the first client \( cl_1 \) initially has view 
\( \vi_1 = \Set{\key_1 \mapsto \Set{0}, \key_2 \mapsto \Set{0}} \)
With the view, we have the fingerprint for the client \( \fp_1 = \Set{(\otR, \key_1,0), (\otR, \key_2,2)} \),
which leads to the final kv-store \( \mkvs_1 \):
\begin{centertikz}
%Location x
\node(locx) {$\key_1 \mapsto$};
\draw pic at ([xshift=\tikzkvspace]locx.east) {vlist={versionx}{%
    /$0$/$\stub$/$\Set{\txid_1}$
    , /$1$/$\txid$/$\emptyset$
}};

%Location y
\path (versionx.east) + (1,0) node (locy) {$\key_2 \mapsto$};
\draw pic at ([xshift=\tikzkvspace]locy.east) {vlist={versiony}{%
    /$2$/$\stub$/$\Set{\txid_1}$
    , /$3$/$\stub$/$\emptyset$
}};
\end{centertikz}
Assume the view remains the same afterwards.
It is easy to see \( \ET_\CP \vdash (\mkvs,\vi_1) \csat \fp_1 : (\mkvs_1,\vi_1)\), and also for \( \ET_\SI \).

Now for the second client \( \cl_2 \), assume the view 
\( \vi_2 = \Set{\key_1 \mapsto \Set{0,1}, \key_2 \mapsto \Set{0}} \),
which leads to the fingerprint \( \fp_2 = \Set{(\otR, \key_1,1), (\otR, \key_2,2)} \),
and the kv-store \( \mkvs_2 \):
\begin{centertikz}
%Location x
\node(locx) {$\key_1 \mapsto$};
\draw pic at ([xshift=\tikzkvspace]locx.east) {vlist={versionx}{%
    /$0$/$\stub$/$\Set{\txid_1}$
    , /$1$/$\txid$/$\Set{\txid_2}$
}};

%Location y
\path (versionx.east) + (1,0) node (locy) {$\key_2 \mapsto$};
\draw pic at ([xshift=\tikzkvspace]locy.east) {vlist={versiony}{%
    /$2$/$\stub$/$\Set{\txid_1,\txid_2}$
    , /$3$/$\stub$/$\emptyset$
}};
\end{centertikz}
It is trivial that \( \ET_\CP \vdash (\mkvs_1,\vi_2) \csat \fp_2 : (\mkvs_2,\vi_2)\), and also for \( \ET_\SI \).

Commutative allows to swap two fingerprints from different clients and still yields the same kv-store.
It is not the case here.
If we let \( \fp_2 \) commits first we have the following kv-store \( \mkvs'_2 \):
\begin{centertikz}
%Location x
\node(locx) {$\key_1 \mapsto$};
\draw pic at ([xshift=\tikzkvspace]locx.east) {vlist={versionx}{%
    /$0$/$\stub$/$\emptyset$
    , /$1$/$\txid$/$\Set{\txid_2}$
}};

%Location y
\path (versionx.east) + (1,0) node (locy) {$\key_2 \mapsto$};
\draw pic at ([xshift=\tikzkvspace]locy.east) {vlist={versiony}{%
    /$2$/$\stub$/$\Set{\txid_2}$
    , /$3$/$\stub$/$\emptyset$
}};
\end{centertikz}
Over the \( \mkvs'_2 \), the view \( \vi_1 \) is no longer valid because in \( \ET_\CP \):
\[
0 \in \vi_1(\key_2)  
\land \wtOf(\mkvs(\key_1, 1)) \toEDGE{(((\SO \cup \WR_{\mkvs}) ; \RW_{\mkvs}^?) \cup \WW_{\mkvs})^{+}} \wtOf(\mkvs(\key_2, 0)) 
\]
but \( i \notin \vi_1(\key_1)\).
It is similar for \( \ET_\SI \).



==> composition-et/counterexamples-for-composition.tex <==
\subsection{Counter examples for compositionality}
\label{sec:counter-examples-composition}

A desirable property that one would request from execution test is compositionality:
the consistency model induced by a composite execution test can be recovered from the consistency 
models generated by each execution test: that is, 
\[ 
\fora{ \ET_1, \ET_2 } \CMs(\ET_1 \cap \ET_2) = \CMs(\ET_1) \cap \CMs(\ET_2).
\]
However, execution tests do not always satisfy this property.

\subsubsection{Commutativity}
Consider the following:
%
\[
\begin{array}{@{}l | l@{}}
    \hline
    \ET_1 & \ET_2 \\
%    
    \hline
    (\mkvs_{0}, \vi_{0}) \csat \Set{(\otW, \key, 1)} : ( \mkvs_{\key}, \vi_{0})
    &
    (\mkvs_{0}, \vi_{0}) \csat \Set{(\otW, \key', 1)} : ( \mkvs_{\key'}, \vi_{0}) 
    \vspace*{-7pt}\\\\
% %   
    (\mkvs_{\key}, \vi_{0}) \csat  \Set{(\otW, \key', 1)} : (\mkvs',\vi_{0}) 
    &
    (\mkvs_{\key'}, \vi_{0}) \csat \Set{(\otW, \key, 1)} : (\mkvs',\vi_{1}) 
    \\
\hline
\end{array}
\]%
 
\begin{align*}
    \mkvs_{\key} & = \mkvs_{0}[\key \mapsto (0, \txid_{0}, \emptyset) \lcat (1, \stub, \emptyset)] \\
    \mkvs_{\key'} & = \mkvs_{0}[\key' \mapsto (0, \txid_{0}, \emptyset) \lcat (1, \stub, \emptyset)] \\
    \mkvs' & = \mkvs[\key \mapsto (0, \txid_{0}, \emptyset) \lcat (1, \stub, \emptyset) 
                ,\key' \mapsto (0, \txid_{0}, \emptyset) \lcat (1, \stub, \emptyset)] \\
\end{align*}
%

As both $\ET_1$ and $\ET_2$ allow a version with value $1$ to be written for 
$\key, \key'$,  we have $\mkvs' \in \CMs(\ET_1) \cap \CMs(\ET_2)$. 
However, $\ET_1$ and $\ET_2$ enforce a different order in which the writes on $\key, \key'$ must happen; 
thus $\mkvs' \notin \CMs(\ET_1 \cap \ET_2)$. 

In this example, compositionality fails because execution tests 
enforced a particular order in which the updates must be committed, even though such updates 
are non-conflicting: the kv-store obtained after committing such updates is independent of the commit order. This observation is captures in the following definition: 
\begin{definition}
\label{def:conflict-commit}
Two triples $(\cl_1, \fp_1)$ and $(\cl_2, \fp_2)$ are 
conflicting if either $\cl_1 = \cl_2$, or there exists a key $\key$ such that 
$(\otW, \key, \stub) \in \fp_1, (\otW, \key, \stub) \in \fp_2$. 
\end{definition}

\begin{definition}
\label{def:app-et-comm}
An execution test is $\ET$ is \emph{commutative} if, whenever $(\cl_1, \vi_1, \fp_1)$, 
$(\cl_2, \vi_2, \fp_2)$ are non-conflicting, and $\vi_1, \vi_2 \in \Views(\mkvs_0)$,  
then for any $\mkvs_0, \mkvs', \vienv, \vienv'$ we have that 
\begin{centermultline}
(\mkvs_0, \vienv) \toET{(\cl_1, \fp_1)}
\stub \toET{(\cl_2, \fp_2)} (\mkvs', \vienv') \implies
(\mkvs_0, \vienv) \toET{(\cl_2, \fp_2)} 
\stub \toET{(\cl_1, \fp_1)} (\mkvs', \vienv'') 
\land \vienv''(\cl_2) \viewleq \vienv'(\cl_2)
\end{centermultline}
\end{definition}

\begin{proposition}
\label{prop:et-comm-matching-vi-env}
\label{lem:et-comm-matching-vi-env}
Assume an execution test is $\ET$ is \emph{commutative}.
Assume $(\cl_1, \vi_1, \fp_1)$, 
$(\cl_2, \vi_2, \fp_2)$ are non-conflicting, and $\vi_1, \vi_2 \in \Views(\mkvs_0)$,  
then for any $\mkvs_0, \mkvs', \vienv, \vienv'$ we have that:
\begin{centermultline}
(\mkvs_0, \vienv) \toET{(\cl_1, \fp_1)}
\stub \toET{(\cl_2, \fp_2)} (\mkvs', \vienv') \\
{} \implies
(\mkvs_0, \vienv) \toET{(\cl_2, \fp_2)} 
\stub \toET{(\cl_1, \fp_1)} \stub \toET{(\cl_2, \epsilon)} (\mkvs', \vienv')
\end{centermultline}
\end{proposition}

\begin{proposition}
\label{thm:appendix-et-composition-2}
\label{prop:appendix-et-composition-2}
if $\ET_1, \ET_2$ are commutative, then $\ET_1 \cap \ET_2$ is commutative.
\end{proposition}
\begin{proof}
Let \( \ET_{12} = \ET_1 \cap \ET_2 \).
Assume \(\conf_1, \conf_2, \conf_3, \cl, \cl', \vi, \vi', \fp, \fp' \) such that:
\[
    \conf_1 \toET{\cl, \fp}[\ET_{12}] \conf_2 \toET{\cl', \fp'}[\ET_{12}] \conf_3
\]
Therefore, we have:
\[
    \conf_1 \toET{\cl, \fp}[\ET_{1}] \conf_2 \toET{\cl', \fp'}[\ET_{1}] \conf_3 \land 
    \conf_1 \toET{\cl, \fp}[\ET_{2}] \conf_2 \toET{\cl', \fp'}[\ET_{2}] \conf_3
\]
Because \( \ET_1 \)  and \( \ET_2 \) are commutative, there exists a configuration \( \conf'_2 \) such that:
\[
    \conf_1 \toET{\cl', \fp'}[\ET_{1}] \conf'_2 \toET{\cl, \fp}[\ET_{1}] \conf_3 \land 
    \conf_1 \toET{\cl', \fp'}[\ET_{2}] \conf'_2 \toET{\cl, \fp}[\ET_{2}] \conf_3
\]
so we have the proof that: 
\[
    \conf_1 \toET{\cl', \fp'}[\ET_{12}] \conf'_2 \toET{\cl, \fp}[\ET_{12}] \conf_3
\]
\end{proof}

\subsubsection{Matching views}
\label{ex:noblindwrites}
\label{sec:no-blind-writes-counter}
\label{sec:matching-pre-views}
\label{sec:matching-views}
For compositionality of two execution tests, 
it is not enough that one execution test is commutative, since the views used to update kv-stores from two execution tests might not match but still yield the same final kv-store.
The following two counter examples lead us to further restrict the execution tests.

Let consider a kv-store \( \mkvs = \Set{\key \mapsto (0,\txid_0,\emptyset) \lcat (1,\txid,\emptyset) }\):
\begin{centertikz}
%Location x
\node(locx) {$\key \mapsto$};

\draw pic at ([xshift=\tikzkvspace]locx.east) {vlist={versionx}{%
    /$0$/$\txid_0$/$\emptyset$
    , /$1$/$\txid$/$\emptyset$
}};
\end{centertikz}
and the following two execution test:
\[
    \ET_1 \vdash (\mkvs, \vi_1) \csat \fp, (\mkvs',\vi') 
    \qquad 
    \ET_2 \vdash (\mkvs, \vi_2) \csat \fp, (\mkvs',\vi') 
\]
where \( \vi_1 = \Set{\key \mapsto \Set{0} }\), \( \vi' = \vi_2 = \Set{\key \mapsto \Set{0,1}} \) and \( \fp = \Set{(\otW, \key, 2)}\).
This leads to the final kv-store \( \mkvs' = \mkvs\rmto{\key}{\mkvs(\key) \lcat (2,\txid',\emptyset)} \) for some \( \txid' \):
\begin{centertikz}
%Location x
\node(locx) {$\key \mapsto$};

\draw pic at ([xshift=\tikzkvspace]locx.east) {vlist={versionx}{%
    /$0$/$\txid_0$/$\emptyset$
    , /$1$/$\txid$/$\emptyset$
    , /$2$/$\txid'$/$\emptyset$
}};
\end{centertikz}

It is easy to see \( \ET_1 \cap \ET_2  = \emptyset \) therefore \( \CMs(\ET_1 \cap \ET_2) = \emptyset \), yet \( \CMs(\ET_1) \cap \CMs(\ET_2) = \Set{\mkvs'}\).
If execution tests enforce \emph{no blind write}, \( \ET_1\) and \( \ET_2 \) cannot produce the same kv-store, thus \( \CMs(\ET_1) \cap \CMs(\ET_2) = \CMs(\ET_1 \cap \ET_2) = \emptyset\), because the initial views are different.


Let consider a kv-store \( \mkvs = \Set{\key \mapsto (0,\txid_0,\emptyset) \lcat (1,\txid,\emptyset) }\):
\begin{centertikz}
%Location x
\node(locx) {$\key_1 \mapsto$};
\draw pic at ([xshift=\tikzkvspace]locx.east) {vlist={versionx}{%
        /$0$/$\txid_0$/$\emptyset$
    , /$1$/$\txid$/$\emptyset$
}};
\end{centertikz}
and the following two execution test:
\[
    \ET_1 \vdash (\mkvs, \vi) \csat \fp, (\mkvs',\vi_1) 
    \qquad 
    \ET_2 \vdash (\mkvs, \vi) \csat \fp, (\mkvs',\vi_2) 
\]
where \( \vi = \vi_1 = \Set{\key \mapsto \Set{0} }\), \(\vi_2 = \Set{\key \mapsto \Set{0,1}} \) and \( \fp = \Set{(\otR, \key, 0)}\).
This leads to the final kv-store \( \mkvs' = \Set{\key \mapsto (0,\txid_0,\Set{\txid'}) \lcat (1,\txid,\emptyset) } \) for some \( \txid' \):
\begin{centertikz}
%Location x
\node(locx) {$\key_1 \mapsto$};
\draw pic at ([xshift=\tikzkvspace]locx.east) {vlist={versionx}{%
        /$0$/$\txid_0$/$\Set{\txid'}$
    , /$1$/$\txid$/$\emptyset$
}};

\end{centertikz}
It is easy to see \( \ET_1 \cap \ET_2  = \emptyset \) therefore \( \CMs(\ET_1 \cap \ET_2) = \emptyset \), yet \( \CMs(\ET_1) \cap \CMs(\ET_2) = \Set{\mkvs'}\).

To rule out those situations, we further constraint execution tests \( \ET_1 \) and \( \ET_2 \).
Given an execution tests, we the \(\min(\ET, \mkvs, \cl)\)  returns the minimum view for client \( \cl \) under the \( \mkvs \).

\begin{definition}[matching views]
\label{def:match-pre-view}
\label{def:match-view}
Two execution tests $\ET_1$ and $\ET_2$ have matching views if there exists a minimum client view function \( \func{minClientViews}[\ET,\mkvs,\cl] \) for \( \ET_1 \), \( \ET_2 \) and \( \ET_1 \cap \ET_2 \) such that:
\begin{itemize}
    \item for any \( \mkvs, \cl\):
    \begin{centermultline}
        \func{minClientViews}[\ET_1, \mkvs, \cl] \viewcup \func{minClientViews}[\ET_2, \mkvs, \cl] \viewleq \func{minClientViews}[\ET_1 \cap \ET_2, \mkvs, \cl]
    \end{centermultline}
    \item for any \(\mkvs, \mkvs',\fp,\vi_1,\vi_2,\vi_1',\vi_2',\cl\):
\begin{centermultline}
    (\vi_1,\vi'_1) =  \func{minFpViews}[\ET_1,\mkvs,\fp,\mkvs',\cl]
    \land (\vi_2,\vi'_2) =  \func{minFpViews}[\ET_2,\mkvs,\fp,\mkvs',\cl] \\
    \implies 
    \vi'_1 = \func{minClientView}[\ET_1, \mkvs',\cl]
    \land \vi'_2 = \func{minClientView}[\ET_2, \mkvs',\cl]  \\
    \exsts{\vi,\vi'} 
    (\vi,\vi') =  \func{minFpViews}[\ET_1 \cap \ET_2,\mkvs,\fp,\mkvs',\cl]
    \land \vi_1 \sqcup \vi_2 \viewleq \vi
    \land \vi'_1 \sqcup \vi'_2 \viewleq \vi' \\
    {} \land \vi' =  \func{minClientViews}[\ET_1 \cap \ET_2, \mkvs', \cl]
\end{centermultline}
where,
\begin{align*}
    (\vi,\vi') = \func{minFpViews}[\ET, \mkvs,\fp,\mkvs',\cl] & \defiff 
    \begin{multlined}[t]
        \func{minClientViews}[\ET, \mkvs, \cl] \viewleq \vi  \\
        {} \land \func{minClientViews}[\ET, \mkvs', \cl] \viewleq \vi' \\
        {} \land \ET \vdash (\mkvs,\vi) \csat \fp : (\mkvs',\vi') \\
        {} \land \fora{\vi'',\vi'''} \ET \vdash (\mkvs,\vi'') \csat \fp : (\mkvs',\vi''') \\
        {} \implies \vi \viewleq \vi'' \land \vi' \viewleq \vi'''
    \end{multlined} \\
    \vi \sqcup \vi' & \defeq \lambda \key \ldotp \vi(\key) \cup \vi'(\key)
\end{align*}
    \item for \( \ET_1 \) (\(\ET_2\) and \( \ET_1 \cap \ET_2\) respectively),
    if any kv-store \( \mkvs \) contains less information than \( \mkvs' \) then
    \begin{centermultline}
        \func{minClientView}[\ET_1,\mkvs,\cl] \viewleq \func{minClientView}[\ET_1, \mkvs',\cl]
    \end{centermultline}
\end{itemize}
\end{definition}

%\subsubsection{Minimum footprint}
%\sx{This condition might be useless because of the minimum in matching views condition}
 
%Let consider a kv-store \( \mkvs = \Set{\key_1 \mapsto (0,\txid_0,\emptyset) \lcat (1,\txid_1,\emptyset), \key_2 \mapsto (2,\txid_0,\emptyset) \lcat (3,\txid_2,\emptyset)}\):
%\begin{centertikz}
%%Location x
%\node(locx) {$\key_1 \mapsto$};
%\draw pic at ([xshift=\tikzkvspace]locx.east) {vlist={versionx}{%
    %/$0$/$\txid_0$/$\emptyset$
    %, /$1$/$\txid_1$/$\emptyset$
%}};

%%Location y
%\path (versionx.east) + (1,0) node (locy) {$\key_2 \mapsto$};
%\draw pic at ([xshift=\tikzkvspace]locy.east) {vlist={versiony}{%
    %/$2$/$\txid_0$/$\emptyset$
    %, /$3$/$\txid_2$/$\emptyset$
%}};
%\end{centertikz}
%and the following two execution test:
%\[
    %\ET_1 \vdash (\mkvs, \vi_1) \csat \fp, (\mkvs',\vi') 
    %\qquad 
    %\ET_2 \vdash (\mkvs, \vi_2) \csat \fp, (\mkvs',\vi') 
%\]
%where \( \vi_1 = \Set{\key_1 \mapsto \Set{0}, \key_2 \mapsto \Set{0} }\), \( \vi_2 = \Set{\key_1 \mapsto \Set{0}, \key_2 \mapsto \Set{0,1} }\) and \( \fp = \Set{(\otR, \key_1, 0)}\).
%This leads to the final kv-store \( \mkvs' = \mkvs\rmto{\key}{(0,\txid_0,\Set{\txid'}) \lcat (1,\txid_1,\emptyset)} \) for some \( \txid' \):
%\begin{centertikz}
%%Location x
%\node(locx) {$\key_1 \mapsto$};
%\draw pic at ([xshift=\tikzkvspace]locx.east) {vlist={versionx}{%
        %/$0$/$\txid_0$/$\Set{\txid'}$
    %, /$1$/$\txid_1$/$\emptyset$
%}};

%%Location y
%\path (versionx.east) + (1,0) node (locy) {$\key_2 \mapsto$};
%\draw pic at ([xshift=\tikzkvspace]locy.east) {vlist={versiony}{%
    %/$2$/$\txid_0$/$\emptyset$
    %, /$3$/$\txid_2$/$\emptyset$
%}};
%\end{centertikz}
%It is easy to see \( \ET_1 \cap \ET_2  = \emptyset \) therefore \( \CMs(\ET_1 \cap \ET_2) = \emptyset \), yet \( \CMs(\ET_1) \cap \CMs(\ET_2) = \Set{\mkvs'}\).

%\begin{definition}[Minimum footprints]
%\label{def:et-minimum-footprint}
%An execution test $\ET$ has \emph{minimum footprints} if for any key-value store \( \mkvs \)
%views \( \vi, \vi',\vi''\) and fingerprint \( \fp \),
%\[
%\begin{array}{@{}l@{}}
%\ET \vdash (\mkvs, \vi) \csat \fp : (\mkvs',\vi'')
%\land \fora{l,\key,\val} \left( (l, \key, \val) \in \fp \implies \vi(\key) = \vi'(\key) \right) 
%\implies \ET \vdash (\mkvs, \vi') \csat \fp : (\mkvs',\vi'')
%\end{array}
%\]
%\end{definition}

%\subsubsection{monotonic post-views}
%Last, the post-views are not necessary match.
%%If execution tests enforce \emph{monotonic post-views}, 
%%we have 
%%\( 
    %%\ET_1 \vdash (\mkvs, \vi) \csat \fp, (\mkvs',\vi_1) \implies 
    %%\ET_1 \vdash (\mkvs, \vi) \csat \fp, (\mkvs',\vi_2) 
%%\)
%%thus \( \CMs(\ET_1) \cap \CMs(\ET_2) = \CMs(\ET_1 \cap \ET_2) = \Set{\mkvs'}\).

%\begin{definition}
%\label{def:et-continuous-postview}
%\label{def:et-monotonic-postview}
%An execution test $\ET$ has \emph{monotonic post-views} if for any key-value store \( \mkvs \)
%views \( \vi, \vi',\vi''\) and fingerprint \( \fp \), 
%\[
%\begin{array}{@{}l@{}}
    %\ET \vdash (\mkvs, \vi) \csat \fp : (\mkvs',\vi') \land \vi' \sqsubseteq \vi'' \implies \ET \vdash (\mkvs, \vi) \csat \fp : (\mkvs',\vi'')
%\end{array}
%\]
%\end{definition}



==> composition-et/counterexamples-for-mw-ryw.tex <==
%\subsection{Example: \(\CMs[\ET_{\MW} \cap \ET_{\RYW}] \neq \CMs(\ET_{\MW+\WFR})\)}


==> composition-et/et-comm.tex <==
\subsection{Compositionality of \( \ET \)}
\label{sec:et-comm}
\label{sec:et-comp}

To make two execution tests \( \ET_1 \) \( \ET_2 \) compositional with respect to to function \( \CMs \),
they need to satisfy \cref{def:app-et-comm,def:match-view}.
%For all the definitions we have in \cref{fig:execution.tests},
%It is easy to adapt so that they satisfy \cref{def:noblidwrites,def:et-minimum-footprint,def:et-monotonic-postview},
Note that but \( \CP \) and \( \SI \) do not  satisfy \cref{def:conflict-commit}.
Now we can prove compositionality of \( \ET \) (\cref{thm:et-comm}).

\begin{theorem}                                                                            
\label{thm:et-comm}                          
Let $\ET_1, \ET_2$ be two execution tests have matching views
If $\ET_1$ is commutative, 
then $\CMs(\ET_1 \cap \ET_2) = \CMs(\ET_1) \cap \CMs(\ET_2)$. 
%Furthermore, if $\ET_1, \ET_2$ are commutative, then $\ET_1 \cap \ET_2$ 
%is commutative.
\end{theorem}
\begin{proof}
Given the definition of the \( \CMs(.) \) function (\cref{def:cm}), 
it suffices to prove that \( \CMs(\ET_{1} \cap \ET_{2}) \subseteq \CMs(\ET_1) \cap \CMs(\ET_2) \)
and \( \CMs(\ET_1) \cap \CMs(\ET_2) \subseteq \CMs(\ET_{1} \cap \ET{2}) \).
The former is proven by the \cref{lem:et12-in-et1-et2} and the later is proven by \cref{lem:et1-et2-in-et12}.
\end{proof}

\begin{lemma}
\label{lem:et12-in-et1-et2}
\( \CMs(\ET_{1} \cap \ET_{2}) \subseteq \CMs(\ET_1) \cap \CMs(\ET_2) \).
\end{lemma}
\begin{proof}
It suffices to prove a stronger result that \( \confOf[\ET_{1} \cap \ET_{2}] \subseteq \confOf[\ET_1] \cap \confOf[\ET_2] \).
By the definition of \confOf (\cref{def:cm}), it suffices to prove for configurations \( \conf_0 \) to \( \conf_n \) 
\begin{equation}
    \label{equ:et12-in-et1-et2}
    \begin{multlined}
        \conf_0 \in \Confs_0
    \land \conf_0 \toET{\stub}[\ET_1 \cap \ET_2] \cdots \toET{\stub}[\ET_1 \cap \ET_2] \conf_n \implies 
    \conf_0 \toET{\stub}[\ET_{1}] \cdots \toET{\stub}[\ET_{1}] \conf_n \land \conf_0 \toET{\stub}[\ET_{2}] \cdots \toET{\stub}[\ET_{2}] \conf_n 
    \end{multlined}
\end{equation}
We prove the \cref{equ:et12-in-et1-et2} by induction on the number \( n \).
\begin{itemize}
\item Base case: \(n = 0\). 
The \cref{equ:et12-in-et1-et2} holds when \( n = 0 \), because all initial configurations \( \conf_0 \) are included in the \( \confOf[\ET_1]\) and \( \confOf[\ET_2] \) by the definition of the \( \confOf \) function (\cref{def:cm}).

\item Inductive case: \(n = i+1\). Suppose the \cref{equ:et12-in-et1-et2} holds when \( n = i \) for some \( i \).
Let consider \( n = i + 1 \) and specifically the last step.
For any \( \conf_{i+1} = (\mkvs_{i+1}, \vienv_{i+1}) \) induced by \( \ET_{1} \cap \ET_2 \), 
there exist some client \( \cl \), views \( \vi, \vi' \) and fingerprint \( \fp \) such that:
\[
    \begin{array}{l}
    (\mkvs_i, \vienv_i) \toET{\cl, \fp}[\ET_{1} \cap \ET_{2}] (\mkvs_{i+1}, \vienv_{i+1}) 
    \land \vienv_{i+1} = \vienv_{i}\rmto{\cl}{\vi'} \land (\mkvs_i, \vi, \fp, \vi' ) \in \ET_{1} \cap \ET_{2}
    \end{array}
\]
Thus, it is easy to see that \( \conf_i \toET{\cl, \fp}[\ET_{1}] \conf_{i+1} \) and \( \conf_i \toET{\cl, \fp}[\ET_{2}] \conf_{i+1} \) by the \cref{lem:mono-et}. \qedhere
\end{itemize}
\end{proof}

\begin{lemma}
\label{lem:mono-et}
If $\conf \toET{\cl, \fp}[\ET] \conf'$ and $\ET \subseteq \ET'$, 
then $\conf \toET{\cl, \fp}[\ET'] \conf'$.
\end{lemma}
\begin{proof}
    Let \((\mkvs, \vienv)  = \conf \), \( (\mkvs', \vienv') = \conf' \) and \( \vi  =\vienv(\cl) \)
    By the definition of  $\conf \toET{\cl, \fp}[\ET] \conf'$ (\cref{def:cm}), we have \(\mkvs' \in \updateKV[\mkvs, \vi, \fp, \cl]\) and  \( \vienv' = \vienv\rmto{\cl}{\vi'} \) for some \( \vi' \) such that \( \ET \vdash (\mkvs, \vi) \csat \fp : (\mkvs',\vi') \).
    Given that \( \ET \subseteq \ET'\), we know \( \ET' \vdash (\mkvs, \vi) \csat \fp : (\mkvs',\vi') \) and so $\conf \toET{\cl, \fp}[\ET'] \conf'$.
\end{proof}

For each normal trace \( \tr \), there exists a new trace \( \func{minitrace}[\tr] \) such that each step takes minimum views:
\begin{align*}
    \func{minitrace}[\tr \toET{\cl,\vi} \stub \toEDGE{\cl,\fp} \mkvs', \vienv'] & \defeq 
    \begin{array}[t]{@{}l@{}}
        \mathtt{let} \ (\mkvs,\vienv) = \func{last}[\func{minitrace}[\tr]]  \\
        \mathtt{in} \ \tr \toET{\cl,\vi'} \stub \toEDGE{\cl,\fp} \mkvs', \vienv\rmto{\cl}{\vi''} \\
        \mathtt{where} \ \begin{array}[t]{@{}l@{}}
            (\vi',\vi'') = \func{minFpViews}[\ET,\mkvs,\fp,\mkvs',\cl] \\
            {} \land \vi'' = \func{minClientViews}[\ET,\mkvs,\cl]
        \end{array} 
    \end{array}
\end{align*}

\begin{lemma}
\label{lem:et1-et2-in-et12}
\( \CMs(\ET_1) \cap \CMs(\ET_2) \subseteq \CMs(\ET_{1} \cap \ET_{2}) \).
\end{lemma}
\begin{proof}
Assume \( \mkvs \in \CMs(\ET_{1} \cap \ET_{2}) \).
There are traces from both execution tests \( \tr_1, \dots, \tr_n \in \confOf[\ET_1] \) and \( \tr'_1, \dots, \tr'_m \in \confOf[\ET_2] \),
where the final kv-stores are the same one, \( \bigwedge_{ 1 \leq i \leq n, 1 \leq j \leq m} \lastConf[\tr_i]\projection{1} = \lastConf[\tr_j]\projection{1} = \mkvs \).
It suffices to pick specific two traces \( \tr \in \confOf[\ET_1]\) and \( \tr' \in \confOf[\ET_2] \),
and from which we construct a trace \( \tr'' \in \confOf[\ET_1 \cap \ET_2] \).
By \cref{prop:et.normalform} and \( \func{minitrace} \) function, we pick normal and minimum traces \( \tr \in \confOf[\ET_1]\) and \( \tr' \in \confOf[\ET_2] \).
Let \( \conf_1 \) to \( \conf_n \) be the configurations from trace \( \tr \), 
and \( \conf'_1 \) to \( \conf'_m \) be configurations from trace \( \tr' \):
\[
\conf_0 \toET{\stub}[\ET_{1}] \conf_1 \toET{\stub}[\ET_{1}] \cdots \toET{\stub}[\ET_{1}] \conf_n 
\land \conf_0 \toET{\stub}[\ET_{2}] \conf'_1 \toET{\stub}[\ET_{2}]  
\cdots \toET{\stub}[\ET_{2}] \conf'_m 
\land \conf_n\projection{1} = \conf'_m\projection{1} 
\]
There exists configurations from \( \conf''_1\)  to \( \conf''_k \) from trace \( \ET_1 \cap \ET_2 \):
\begin{centermultline}[equ:et1-et2-in-et12]
\conf_0 \toET{\stub}[\ET_1 \cap \ET_2] \conf''_1 \toET{\stub}[\ET_1 \cap \ET_2] \cdots \toET{\stub}[\ET_1 \cap \ET_2] \conf''_k 
\land \conf_n\projection{1} = \conf'_m\projection{1} = \conf''_k\projection{1}
\end{centermultline}
and assuming that the last fingerprint \( \fp \) committed of an arbitrary client \( cl \) is at i-\emph{th} step ( \( i \leq k\) ) in the trace \( \tr'' \), let
\begin{itemize}
\item \( \mkvs = \conf''_i\projection{1} \)
\item \( \mkvs' = \conf''_{i+1}\projection{1} \) 
\item \( \vi = \conf''_i\projection{2}(\cl) \), and
\item \( \vi' = \conf''_{i+1}\projection{2}(\cl) \), 
\end{itemize}
then the views \( \vi, \vi' \) are the one given by matching view definition (\cref{def:match-view}):
\begin{centermultline}[eq:minimum-view-for-last-fp]
    (\vi,\vi') = \func{minFpView}[\ET_1 \cap \ET_2, \mkvs,\fp,\mkvs',\cl] \land \vi' = \func{minClientViews}[\ET_1 \cap \ET_2, \mkvs, \cl]
\end{centermultline}
and since i-\emph{th} step the view for the client \( \cl \) never changes:
\begin{centermultline}[eq:minimum-view-fix-after-last]
    \conf''_k\projection{2}(\cl) = \vi'
\end{centermultline}
\Cref{eq:minimum-view-for-last-fp,eq:minimum-view-fix-after-last} mean that the view for any client will fix to be the one given by \cref{def:match-view} if there is no further fingerprint.
We prove \cref{equ:et1-et2-in-et12} by induction on the length \( m \) of the trace of \( \ET_2 \).
\begin{itemize}
    \item \caseB{\(m = 0\)}
We have the trace of \( \ET_1 \):
\begin{equation}
    \label{equ:trace-view-shift-et1}
    \conf_0 \in \Confs_0 \land \conf_0 \toET{\stub}[\ET_1] \dots \toET{\stub}[\ET_1] \conf_n
\end{equation}
for some number \( n \) and configurations from \( \conf_0 \) to \( \conf_n \) and the trace of \( \ET_2 \) with only one configuration:
\begin{equation}
    \label{equ:trace-singleton-et2}
    \conf_0
\end{equation}
By the hypothesis we have \( \conf_0\projection{1} = \conf_n\projection{1} \), which means that all the steps from the trace of \( \ET_1 \) are view shift.
We can pick the trace of \( \ET_2 \) (\cref{equ:trace-view-shift-et1}) as the trace of \( \ET_1 \cap \ET_2 \):
\begin{equation}
    \label{equ:trace-view-shift-et12}
    \conf_0 
\end{equation}
It is easy to see it satisfies \cref{eq:minimum-view-for-last-fp,eq:minimum-view-fix-after-last}, since nothing has been committed.

\item \caseI{\(m + 1\)}
Suppose that \cref{equ:et1-et2-in-et12} holds when the trace length is \( m \).
Let consider \( m + 1 \).
We have the trace for \( \ET_1 \):
\begin{equation}
    \conf_0 \toET{\stub}[\ET_{1}] \conf_1 \toET{\stub}[\ET_{1}] \cdots \toET{\stub}[\ET_{1}] \conf'_{n} 
\end{equation}
for some number \( n \) and the configurations from \(\conf_0\) to \( \conf_n \), and the trace of \(\ET_2\):
\begin{equation}
    \conf_0 \toET{\stub}[\ET_{2}] \conf'_1 \toET{\stub}[\ET_{2}] \cdots \toET{\stub}[\ET_{2}] \conf'_{m+1} 
\end{equation}
Assume a client \( \cl'_{m} \), views \( \vi'_{m}, \vi'_{m+1} \) and a fingerprint \( \fp'_{m} \) that is committed to the second last configuration \( (\mkvs'_m, \vienv'_m) = \conf'_m \) in the trace of \( \ET_2 \) which yields the final configuration \( (\mkvs'_{m+1}, \vienv'_{m+1}) = \conf_{m+1} \):
\begin{centermultline}
        (\mkvs'_i, \vienv'_i) \toET{\cl'_{m}, \fp'_{m}}[\ET_2] (\mkvs'_{m+1}, \vienv'_{m+1}) 
\end{centermultline}
There are two cases: \textbf{(i)} \( \fp'_m = \epsilon \) and \textbf{(ii)} \( \fp'_m \neq \epsilon \).
\begin{itemize}
    \item If \( \fp'_m = \epsilon \), by the \cref{lem:no-effect-for-empty-fingerprint} we know \( \conf'_{m}\projection{1} = \conf'_{m+1}\projection{1}\) from the trace of \( \ET_2 \).
Since \( \conf'_{m+1}\projection{1} = \conf_n\projection{1}\) where \( \conf_n \) is the final configuration of the trace of \( \ET_1 \), we now have \( \conf'_{m}\projection{1} = \conf_n\projection{1}\).
Applying \ih that \cref{equ:et1-et2-in-et12} holds when the length is \( m \), so there exist an trace \( \tr'' \) from configurations from \( \conf''_1 \) to \( \conf''_k \) that satisfies \cref{eq:minimum-view-for-last-fp,eq:minimum-view-fix-after-last}:
\begin{centermultline}[equ:ih-for-k-length]
    \tr'' = \conf_0 \toET{\stub}[\ET_1 \cap \ET_2] \conf''_1 \toET{\stub}[\ET_1 \cap \ET_2] \cdots \toET{\stub}[\ET_1 \cap \ET_2] \conf''_k
    \land \conf_n\projection{1} = \conf'_m\projection{1} = \conf''_k\projection{1} 
\end{centermultline}
Given the definition of the reduction (\cref{def:reduction}), when \( \fp'_m = \epsilon \) we know \( \conf'_m\projection{2}(\cl_{m+1}) \sqsubseteq  \conf'_{m+1}\projection{2}(\cl_{m+1})\).
Yet we can still pick trace \( \tr'' \) which satisfies \cref{equ:et1-et2-in-et12,eq:minimum-view-for-last-fp,eq:minimum-view-fix-after-last}.

\item If \( \fp' \neq \epsilon \), 
    the final step of trace \( \tr' \) is:
    \begin{centermultline}[equ:last-et-2]
        (\mkvs'_i, \vienv'_i) \toET{\cl'_{m}, \fp'_{m}}[\ET_2] (\mkvs'_{m+1}, \vienv'_{m+1}) \land \ET_2 \vdash (\mkvs'_m, \vi'_m) \csat \fp'_m  : (\mkvs'_{m+1},\vi'_{m+1}) \\
        \quad {} \land \vi_i' = \vienv'_m(\cl'_m) \land \vienv'_{m+1} = \vienv'_i\rmto{\cl'_i}{\vi'_{m+1}}
    \end{centermultline}
    and by \cref{lem:identical-step} there exists a step \( (\cl_j, \fp_j) \) from the trace of \( \ET_1 \) such that:
\begin{centermultline}[equ:j-th-step]
    (\mkvs_{j}, \vienv_{j}) \toET{\cl_{j}, \fp_{j}}[\ET_1] (\mkvs_{j + 1}, \vienv_{j + 1}) 
    \land \ET_1 \vdash (\mkvs_{j}, \vi_j) \csat \fp_j : (\mkvs_{j+1},\vienv_{j + 1}(\cl_{j}) ) \land \vi_j = \vienv_{j}(\cl_j)
\end{centermultline}
for some \( j, \cl_j, \vi_j\) and \( \fp_j \) such that \( 0 \leq  j < n \), \( \cl_j = \cl'_{m}\), \( \fp_j = \fp'_{m}\), and
\[ 
    \fora{\key} (\stub, \key, \stub ) \in \fp_j \implies \vi_j(\key) = \vi'_{m}(\key)
\]
We apply the commutativity of \( \ET_1 \) until the step shown in \cref{equ:j-th-step} is at the end or the second end of the trace of \( \ET_1 \).
Let consider the next two steps, (j+1)-\emph{th} and (j+2)-\emph{th} step.
Since the trace is in normal form, the (j+1)-\emph{th} step is a view shift by a client \( \cl_{j+2} \) and (j+2)-\emph{th} step is a concrete step issued by the same client \( \cl_{j+2} \) under the view \( \vi_{j+2} \):
\begin{equation}
    \label{equ:j-plus-1-th-step}
    \begin{array}{@{}l@{}}
        (\mkvs_{j+1}, \vienv_{j+1}) \toET{\cl_{j+2}, \epsilon}[\ET_1]
        (\mkvs_{j+1}, \vienv_{j+1}\rmto{\cl_{j+2}}{\vi_{j+2}}) \toET{\cl_{j+2}, \fp_{j+2}}[\ET_1] (\mkvs_{j+3}, \vienv_{j+3}) \\
        \qquad \land \ET_1 \vdash (\mkvs_{j+1},\vi_{j+2}) \csat \fp_{j+2} : (\mkvs_{j+3},\vienv_{j+3}(\cl_{j+2}) )
    \end{array}
\end{equation}
It is known that the client  \( \cl_{j+2} \) is different from \( \cl_j \) (\cref{lem:different-cl}) and \( \fp_{j+2} \) writes different keys from \( \fp_j\) (\cref{lem:different-writes}). 
Because \( \cl_j \neq \cl_{j+2} \) we can swap the view shift step shown in \cref{equ:j-plus-1-th-step} before the j-\emph{th} step shown in \cref{equ:j-th-step} which gives the following:
\begin{centermultline}[equ:swap-the-view-shift-et1]
    (\mkvs_{j}, \vienv_{j}) \toET{\cl_{j+2}, \epsilon}[\ET_1] (\mkvs_{j}, \vienv_{j}\rmto{\cl_{j+2}}{\vi_{j+2}}) \toET{\cl_{j}, \fp_{j}}[\ET_1] \\
    (\mkvs_{j + 1}, \vienv_{j + 1}\rmto{\cl_{j+2}}{\vi_{j+2}}) \toET{\cl_{j+2}, \fp_{j+2}}[\ET_1] (\mkvs_{j+3}, \vienv_{j+3})
\end{centermultline}
Now let discuss the (j+2)-\emph{th} step.
Similarly by the \cref{lem:identical-step}, there is a step \((\cl_p, \fp_p)\) from the trace of \( \ET_2 \) such that \( \cl_p = \cl_{j+2}\) and \( \fp_p = \fp_{j+2}\) and \( p < m \).
Note that the last step from \( \ET_2 \), \ie (m+1)-\emph{th} step, is not a view shift therefore the m-\emph{th} step must be a view shift so the p-\emph{th} step must be before  m-\emph{th} step.
This means the fingerprint \( \fp_p \) does not observe any change by (m+1)-\emph{th} step from the trace of \( \ET_2 \).
Therefore \( \vi_{j+2} \) does not observe any change by j-\emph{th} step from the trance of \( \ET_1\), \ie \( \vi_{j+2} \in \Views(\mkvs_j) \).
By \cref{prop:et-comm-matching-vi-env}, that allows to swap the two adjacent non-conflict steps from \cref{equ:swap-the-view-shift-et1}.
It follows a new kv-stores \( \mkvs'''_{j+2}\) and a new view environment \( \vienv'''_{j+2} \) such that:
\begin{centermultline}[equ:swap-step-et1]
    (\mkvs_{j}, \vienv_{j}) \toET{\cl_{j+2}, \epsilon}[\ET_1] (\mkvs_{j}, \vienv_{j}\rmto{\cl_{j+2}}{\vi_{j+2}}) \toET{\cl_{j+2}, \fp_{j+2}}[\ET_1] {} \\
    (\mkvs_{j + 2}''', \vienv_{j + 2}''') \toET{\cl_{j}, \fp_{j}}[\ET_1] \stub \toET{\cl_{j}, \epsilon}[\ET_1] (\mkvs_{j+3}, \vienv_{j+3})
\end{centermultline}
In the \cref{equ:swap-step-et1} the j-\emph{th} step moves to the right of (j+2)-\emph{th} step.
Note that the last view shift of \( \cl_j \) will be combined with another view shift appear later in the trace 
(more details shown in the proof of normal trace in \cref{sec:normal-form-exist}).
We keep moving the j-\emph{th} step until it is at the end or the second end of trace of \( \ET_1 \):
\[
    \begin{array}{@{}l}
        \conf_0 \toET{\stub}[\ET_{1}] \cdots \toET{\stub}[\ET_{1}] \conf_{j-1} \toET{\stub}[\ET_{1}]
        \conf'''_{j} \toET{\stub}[\ET_{1}] \dots \toET{\stub}[\ET_{1}] \conf'''_{n-1} \toET{\cl_j, \fp_j }[\ET_{1}] \conf_{n} \lor {} \\
        \conf_0 \toET{\stub}[\ET_{1}] \cdots \toET{\stub}[\ET_{1}] \conf_{j-1} \toET{\stub}[\ET_{1}] 
        \conf'''_{j} \toET{\stub}[\ET_{1}] \dots \toET{\stub}[\ET_{1}] \conf'''_{n-2} \toET{\cl_j, \fp_j }[\ET_{1}] \conf'''_{n-1} \toET{\cl_{n-1}, \epsilon }[\ET_{1}] \conf_{n}  
    \end{array}
\]
for some new configurations from \( \conf'''_{j}\) to \( \conf'''_{n-1} \).
Note that if it is the second end, the last step must be a view shift step as shown in \cref{equ:new-et-1}.
\begin{itemize}
\item If the j-\emph{th} step is at the end of the new trace of \( \ET_1 \), we have the trace:
\begin{centermultline}[equ:new-et-1]
    \conf_0 \toET{\stub}[\ET_{1}] \cdots \toET{\stub}[\ET_{1}] \conf_{j-1} \toET{\stub}[\ET_{1}] 
    \conf'''_{j} \toET{\stub}[\ET_{1}] \dots \toET{\stub}[\ET_{1}] \conf'''_{n-1} \toET{\cl_j, \fp_j }[\ET_{1}] \conf_{n}  
\end{centermultline}
Given the hypothesis that \( \conf_{n}\projection{1} = \conf'_{m+1}\projection{1} \) and the fact that the last step of the new trace of \( \ET_1 \) (\cref{equ:new-et-1}) and the last step the trace of \( \ET_2 \) (\cref{equ:last-et-2}) are the same step, the kv-stores of the second last configurations the new trace of \( \ET_1 \) (\cref{equ:new-et-1}) and the one from the trace of \( \ET_2 \) (\cref{equ:last-et-2}) are the same \(  \conf'''_{n-1}\projection{1} = \conf'_{m}\projection{1} \).
Then by applying \ih that \cref{equ:et1-et2-in-et12} holds when the length is \( m \), there exists a trace  \( \tr'' \) of \( \ET_1 \cap \ET_2 \) that satisfies \cref{eq:minimum-view-for-last-fp,eq:minimum-view-fix-after-last}:
\begin{centermultline}[equ:ih-for-merge-two-trace]
        \tr'' = \conf_0 \toET{\stub}[\ET_1 \cap \ET_2] \dots \toET{\stub}[\ET_1 \cap \ET_2] \conf''_{k-1} 
        \land \conf'''_{n-1}\projection{1} = \conf'_{m}\projection{1} = \conf''_{k-1}\projection{1}  
\end{centermultline}
for some number \( k \) and configurations from \( \conf''_1 \) to \( \conf''_{k-1} \).
Now let consider the last step.
Let relabel the subscripts of new trace of \( \ET_1 \), from \( 0 \) to \( n \).
Since the kv-stores are the same before and after the transaction from two trace,
let \( \mkvs_m = \conf'''_{n-1}\projection{1} = \conf'_{m}\projection{1} \) and 
\( \mkvs_{m+1} = \conf_{n}\projection{1} =  \conf'_{m+1}\projection{1}\).
By \cref{equ:last-et-2} and \cref{equ:new-et-1}, we have:
\begin{centermultline}[equ:et1-et2-csat]
    \ET_1 \vdash ( \mkvs_m, \conf'''_{n-1}\projection{2}(\cl_{m}) )  \csat \fp_{m} : (\mkvs_{m+1} , \conf'''_{n}\projection{2}(\cl_{m}) ) \\
        {} \land \ET_2 \vdash ( \mkvs_m, \conf'_{m}\projection{2}(\cl_{m}) )  \csat \fp_{m} : ( \mkvs_{m+1} , \conf'_{m+1}\projection{2}(\cl_{m}) ) 
\end{centermultline}
where the views have the following properties:
\begin{itemize}
    \item \( (\conf'''_{n-1}\projection{2}(\cl_{m}), \conf'''_{n}\projection{2}(\cl_{m}) )  = \func{minFpViews}[\ET_1, \mkvs_m, \fp_m,\mkvs_{m+1},\cl_m] \)
    \item \( \conf'''_{n}\projection{2}(\cl_{m}) = \func{minClientViews}[\ET_1,\mkvs_{m+1},\cl_m] \)
    \item \( (\conf'_{m}\projection{2}(\cl_{m}), \conf'_{m+1}\projection{2}(\cl_{m}) )  = \func{minFpViews}[\ET_2, \mkvs_m, \fp_m,\mkvs_{m+1},\cl_m] \)
    \item \( \conf'_{m+1}\projection{2}(\cl_{m}) = \func{minClientViews}[\ET_2,\mkvs_{m+1},\cl_m] \)
\end{itemize}
Then by the matching view definition (\cref{def:match-view})
there exists views \( \vi, \vi' \) such that:
\begin{centermultline}[equ:et12-csat]
    (\vi,\vi') = \func{minFpViews}[\ET_1 \cap \ET_2, \mkvs_m,\fp,\mkvs_{m+1},\cl_m]  \\
    {} \land \ET_1 \cap \ET_2 \vdash (\mkvs_m,\vi) \csat \fp : (\mkvs_{m+1}, \vi' ) \\
    {} \land \conf'''_{n-1}\projection{2}(\cl_{m}) \viewcup  \conf'_{m}\projection{2}(\cl_{m}) \viewleq \vi \\
    {} \land \conf'''_{n}\projection{2}(\cl_{m}) \viewcup  \conf'_{m+1}\projection{2}(\cl_{m}) \viewleq \vi' = \func{minClientViews}[\ET_1 \cap \ET_2, \mkvs_{m+1},\cl]
\end{centermultline}
By \cref{eq:minimum-view-for-last-fp,eq:minimum-view-fix-after-last}, there exists an configuration, says the p-\emph{th} where \( p \leq (k - 1) \):
\begin{centermultline}
    \conf''_{p}\projection{2}(\cl_m) = \conf''_{k-1}\projection{2}(\cl_m)
\end{centermultline}
Yet the p-\emph{th} kv-store contains less information than (k-1)-\emph{th} one:
\begin{centermultline}
    \min(\ET_1,\mkvs_p,\cl_m) \viewcup \min(\ET_2,\mkvs_p,\cl_m) \viewleq \min(\ET_1 \cap \ET_2,\mkvs_p,\cl_m)  \viewleq \min(\ET_1 \cap \ET_2,\mkvs_{k-1},\cl_m) 
\end{centermultline}
Given above and \cref{equ:et12-csat} (especially the definition of \func{minFpViews}), it is known:
\begin{centermultline}
    \conf''_{k-1}(\cl_m) \viewleq \vi
\end{centermultline}
Therefore the \cref{equ:et1-et2-in-et12} holds when length is \( m + 1\) by appending a view shift of client \( \cl_m \) and the fingerprint shown in \cref{equ:et12-csat} to the trace shown in \cref{equ:ih-for-merge-two-trace}:
\begin{centermultline}
    \conf_0 \toET{\stub}[\ET_1 \cap \ET_2] \dots \toET{\stub}[\ET_1 \cap \ET_2] (\mkvs''_{k-1}, \vienv''_{k-1}) \toET{\cl_m, \vi}[\ET_1 \cap \ET_2] \stub \toET{\cl_m, \fp_m}[\ET_1 \cap \ET_2] (\mkvs''_{k+1}, \vienv''_{k+1}) \\
    {} \land \conf'''_{n}\projection{1} = \conf'_{m+1}\projection{1} = \mkvs''_{k+1}
    \land  \vienv''_{k+1} = \vienv''_{k-1}\rmto{\cl_m}{\vi'}
\end{centermultline}

\item If the j-\emph{th} step is the second last step of the new trace of \( \ET_1 \), we have the trace:
\begin{centermultline}[equ:new-et-1-with-view-shift-tail]
\conf_0 \toET{\stub}[\ET_{1}] \cdots \toET{\stub}[\ET_{1}] \conf_{j-1} \toET{\stub}[\ET_{1}] 
\conf'''_{j} \toET{\stub}[\ET_{1}] \dots 
\toET{\stub}[\ET_{1}] \conf'''_{n-2} \toET{\cl_j, \fp_j }[\ET_{1}] 
\conf'''_{n-1} \toET{\cl_{n-1}, \epsilon }[\ET_{1}] \conf_{n}
\end{centermultline}
Since the last step is a view shift, we know \( \conf_n\projection{1} = \conf'''_{n-1}\projection{1}\), and the rest of proof is the same as the case where j-\emph{th} is the last step as shown in \cref{equ:new-et-1}. \qedhere
\end{itemize}
\end{itemize}
\end{itemize}
\end{proof}

\begin{lemma}[No effect from empty fingerprint and epsilon reduction]
    \label{lem:no-effect-for-empty-fingerprint}
    \label{lem:no-effect-for-view-shift}
    \[
    \fora{\conf, \conf', \cl,\vi} \conf \toET{\cl, \unitO}[\ET] \conf' \lor \conf \toET{\cl, \epsilon}[\ET] \conf' \implies \conf\projection{1} = \conf'\projection{1}
    \]
\end{lemma}
\begin{proof}
    Let \((\mkvs, \vienv)  = \conf \) and \( (\mkvs', \vienv') = \conf' \).
    For the case of empty fingerprint,
    by the definition of  $\conf \toET{\cl, \unitO} \conf'$ (\cref{def:reduction}), we have \(\mkvs' \in \updateKV[\mkvs, \vi, \unitO, \cl]\), and therefore \( \mkvs' = \mkvs \).
    For the case of view shift, by the definition of  $\conf \toET{\cl, \epsilon} \conf'$ (\cref{def:reduction}) it is easy to see \( \mkvs' = \mkvs \).
\end{proof}

We define a \(  \mkvs(\txid) \) function that returns the fingerprint associate with the transaction identifier \( \txid \):
\begin{align*}
    \mkvs(\txid) & \defeq \Set{(\otW, \key, \val)}[\exsts{i} \mkvs(\key)(i) = (\val, \txid, \stub)] \cup  \Set{(\otR, \key, \val)}[\exsts{i,\txidset} \mkvs(\key)(i) = (\val, \stub, \txidset) \land \txid \in \txidset]
\end{align*}

\begin{lemma}[Transactions persistence]
    \label{lem:mono-fingerprint}
    \[
        \fora{\ET,\conf,\conf',\txid,\fp} \conf\projection{1}(\txid) = \fp \land \conf \toET{\stub}[\ET] \conf' \implies \conf'\projection{1}(\txid) = \fp
    \]
\end{lemma}
\begin{proof}
    It is easy to prove this by case analysis on the reduction relation.
\end{proof}

\begin{lemma}[Same steps]
\label{lem:identical-step}
Given a trace of \( \ET_1 \) and a trace of \( \ET_2 \),
if the have the same final kv-store,
the trace contains the same concrete steps (free variables are globally quantified):
\begin{multline*}
    \conf_0 \toET{\cl_1, \fp_1}[\ET_{1}] \cdots \toET{\cl_n, \fp_n}[\ET_{1}] \conf_n \land
    \conf_0 \toET{\cl'_1, \fp'_1}[\ET_{2}] \cdots \toET{\cl'_m, \fp'_m}[\ET_{2}] \conf'_m 
    \land \conf_n\projection{1} = \conf'_m\projection{1} \\
    \quad \implies \fora{i: 0 < i \leq n} 
    \fp_i = \epsilon 
    \lor \exsts{j: 0 < j \leq m}  \\
    \cl_i = \cl'_j \land \fp_i = \fp'_j \land ( \fora{\key} (\otR, \key, \stub) \in \fp_i \implies \max(\vi_i(\key)) = \max(\vi'_j(\key)) )
\end{multline*}
\end{lemma} 
\begin{proof}
    We prove by contradiction.
    First because \( \mkvs_n = \mkvs'_m \), we know that:
    \begin{equation}
        \label{equ:same-kv-store}
        \fora{\txid, \fp} \mkvs_n(\txid) = \fp \iff \mkvs'_m(\txid) = \fp
    \end{equation}
    Let \(\conf_n = (\mkvs_n,\vienv_n) \) and \(\conf'_m = (\mkvs'_m,\vienv'_m) \).
    Assume a step \( \conf_i \toET{\cl, \fp }[\ET_1] \conf_{i+1} \)  from the trace of \( \ET_1 \) where the transaction identifier is \( \txid \) and \( \fp \neq \unitO \).
    It must have a step from the trace of \( \ET_2 \), which commits some fingerprint via the same transaction identifier  \( \txid \).
    We know \( \mkvs_n(\txid) = \fp \) by \cref{lem:mono-fingerprint}, thus \( \mkvs'_m(\txid) = \fp \) by \cref{equ:same-kv-store}.
    Let assume a key \( \key \) that \( (\otR, \key, \stub) \in \fp\).
    %where \( \vi_i\) and \( \vi'_j\) are the views immediate before the commit of the fingerprint \( \fp \) in traces of \( \ET_1\) and \( \ET_2 \) respectively.
    Since that the final kv-stores are the same, that means the new transaction added itself to the reader set of the same version.
    Thus, \( \max(\vi(\key)) = \max(\vi'(\key)) \).
\end{proof}

We define \( \max_\cl(\conf) \) function that returns the most recent transaction identifier for client \( \cl \) in the configuration \( \conf \) 
\begin{align*}
    \max_\cl((\mkvs, \vienv)) & \defeq \max\Set{\txid^{n}_\cl}[\txid^{n}_\cl \text{ appear in } \mkvs] \\
\end{align*}

\begin{lemma}[Transactions from different clients]
\label{lem:different-cl}
Given a trace of \( \ET_1 \) and a trace of \( \ET_2 \),
if the i-\emph{th} step from \( \ET_1 \) issued by the client \( \cl_i \) 
is the same as the last step from \( \ET_2 \),
then in the trace of \( \ET_1 \) 
there is no concrete step issued by the client \(\cl_i \) after the i-\emph{th} step (free variables are globally quantified):
\[
\begin{array}{@{}l}
    \conf_0 \toET{\cl_1, \fp_1}[\ET_{1}] \cdots \toET{\cl_n, \fp_n}[\ET_{1}] \conf_n 
    \land \conf_0 \toET{\cl'_1, \fp'_1}[\ET_{2}] \cdots \toET{\cl'_m, \fp'_m}[\ET_{2}] \conf'_m 
    \land \conf_n\projection{1} = \conf'_m\projection{1} 
    \land \fp'_m \neq \unitO \\
    \quad {} \land \exsts{i}  
    \cl_i = \cl'_m
    \land \fp_i = \fp'_m 
    \implies \fora{j > i} 
    \fp_j = \epsilon \lor \fp_j = \unitO \lor \cl_i \neq \cl_j
\end{array}
\]
\end{lemma}
\begin{proof}
    We prove by deriving contradiction.
    Assume the last step of the trace of \( \ET_2 \) is:
    \begin{equation}
        \label{equ:last-step-for-cl-et2}
        \conf'_{m-1} \toET{\cl'_m, \fp'_m}[\ET_{2}] \conf'_m
    \end{equation}
    Assume a step of the trace of \( \ET_1 \):
    \begin{equation}
        \label{equ:identical-step-for-cl-et1}
        \conf_{i-1} \toET{\cl_i, \fp_i}[\ET_{1}] \conf_i
    \end{equation}
    where \( \cl_i = \cl'_m \) and \( \fp_i = \fp'_m \).
    Because these two steps (\cref{equ:last-step-for-cl-et2} and \cref{equ:identical-step-for-cl-et1}) are issued by the same transaction identifier,
    we know \( \max{}_{\cl_m}(\conf'_m) = \max{}_{\cl_m}(\conf_i) \).
    Assume that there exists a step from the trace of \( \ET_1 \), says j-\emph{th} step, such that:
    \[
        \conf_{j-1} \toET{\cl_j, \fp_h}[\ET_{1}] \conf_j \land j > i \land \fp_j \neq \unitO \land \cl_i = \cl_j 
    \]
    Therefore we have \( \max{}_{\cl_m}(\conf_j) > \max{}_{\cl_m}(\conf_i) \) by \cref{lem:kv-max-cl}.
    That means \( \max{}_{\cl_m}(\conf_n) > \max{}_{\cl_m}(\conf_j) > \max{}_{\cl_m}(\conf_i) = \max{}_{\cl_m}(\conf'_m) \), which contradicts to \( \conf_n\projection{1} = \conf'_m\projection{1}\).
\end{proof}

\begin{lemma}[Reduction following session order]
\label{lem:kv-max-cl}
\begin{centermultline}
    \fora{\conf, \conf' ,\cl, \fp, \ET}
    \conf \toET{\cl, \fp}  \conf'  \\
    {} \land 
    \left( 
        \fp \neq \unitO \implies \max{}_\cl(\conf) < \max{}_\cl(\conf') )
        \lor ( \fp = \unitO \implies \max{}_\cl(\conf) = \max{}_\cl(\conf')
    \right)
\end{centermultline}
\end{lemma}
\begin{proof}
    Assume a step \( (\mkvs, \vienv) \toET{\cl, \fp} (\mkvs', \vienv') \).
    By the definition of \( \toET{\stub}[\ET]\) (\cref{def:reduction}), we know \( \mkvs' \in \updateKV[\mkvs, \vi, \fp, \cl] \).
    The \( \updateKV[\mkvs, \vi, \fp, \cl] \) picks a fresh transaction identifier \( \txid_\cl^{m} \) that is greater than any transaction identifiers \( \txid_\cl^{n} \) in \( \mkvs \) via \( \nextTxid \) function, \ie \( m > n \).
    If the fingerprint \( \fp \) is not empty, the new identifier appears in \( \mkvs' \), so \( \max{}_\cl(\conf) < \max{}_\cl(\conf') \).
    Otherwise  the fingerprint is empty, the new identifier will not appear anywhere in \( \mkvs' \), so \( \max{}_\cl(\conf) = \max{}_\cl(\conf') \). 
\end{proof}

\begin{lemma}[Writing different keys]
\label{lem:different-writes}
Given a trace of \( \ET_1 \) and a trace of \( \ET_2 \),
if the i-\emph{th} step from \( \ET_1 \) that writes to key \( \key \) 
is the same as the last step from \( \ET_2 \),
then in the trace of \( \ET_1 \) 
there is no concrete step writing to the key \(\key\) after the i-\emph{th} step (free variables are globally quantified):
\[
\begin{array}{@{}l}
    \conf_0 \toET{\cl_1, \fp_1}[\ET_{1}] \cdots \toET{\cl_n, \fp_n}[\ET_{1}] \conf_n \land \conf_0 \toET{\cl'_1, \fp'_1}[\ET_{2}] \cdots \toET{\cl'_m, \fp'_m}[\ET_{2}] \conf'_m 
    \land \conf_n\projection{1} = \conf'_m\projection{1} 
    \land \fp'_m \neq \unitO \\
    \quad {} \land \exsts{i} 
    \cl_i = \cl'_m
    \land \fp_i = \fp'_m
    \implies \fora{j > i} \nexists{\key} \ldotp (\otW, \key, \stub) \in \fp_j \cap \fp_i
\end{array}
\]
\end{lemma}
\begin{proof}
    We prove this by deriving contradiction.
    Assume the last step from the trace of \( \ET_2 \):
    \begin{equation}
        \label{equ:last-step-for-write-et2}
        \conf'_{m-1} \toET{\cl'_m, \fp'_m}[\ET_{2}] (\mkvs'_m, \vienv'_m )
    \end{equation}
    Assume the transaction identifier for the \cref{equ:last-step-for-write-et2} is \( \txid \), and by the definition of \( \toET{}[\ET]\) (\cref{def:reduction}) we know:
    \begin{equation}
        \label{equ:write-fingerprint}
        \fora{\key} (\otW, \key, \stub) \in \fp'_m \implies \mkvs'_m(\key)(\lvert\mkvs'_m(\key)\rvert - 1) = (\stub, \txid, \stub)
    \end{equation}
    Assume a step of the trace of \( \ET_1 \) that is issued by the same transaction identifier with the same fingerprint:
    \begin{equation}
        \label{equ:identical-step-for-write-et1}
        \conf_{i-1} \toET{\cl_i, \fp_i}[\ET_{1}] (\mkvs_i, \vienv_i)
    \end{equation}
    where \( \cl_i = \cl'_m \) and \( \fp_i = \fp'_m \).
    Given \cref{equ:write-fingerprint} and \cref{equ:identical-step-for-write-et1}, it follows:
    \[
        \fora{\key} (\otW, \key, \stub) \in \fp_i \implies \mkvs_i(\key)(\lvert\mkvs_i(\key)\rvert - 1) = (\stub, \txid, \stub)
    \]
    Assume a step, says j-\emph{th}, after i-\emph{th} step that writes to the same key:
    \[
        \conf_{j-1} \toET{\cl_j, \fp_j}[\ET_{1}] (\mkvs_j, \vienv_j) 
        \land j > i
        \land \exsts{\key} (\otW, \key, \stub) \in \fp_i \cap \fp_j
    \]
    Therefore, by \cref{lem:unique-writer} we have:
    \[
        \exsts{\key,i} (\otW, \key, \stub) \in \fp_i \cap \fp_j \land \mkvs_j(\key)(i) = \txid \land \mkvs_j(\key)(\lvert \mkvs_j(\key) \rvert - 1) \neq \txid
    \]
    Note that \( \fp_i = \fp'_m\).
    Since the writer of a version cannot be overwritten, for the final configuration of the trace of \( \ET_1 \) \((\mkvs_n, \vienv_n)\), we know:
    \[
        \exsts{\key,i} (\otW, \key, \stub) \in \fp_i \cap \fp_j \land \mkvs_n(\key)(i) = \txid \land \mkvs_n(\key)(\lvert \mkvs_n(\key) \rvert - 1) \neq \txid
    \]
    Last, by \cref{equ:write-fingerprint} and \( \fp_i = \fp'_m\), it follows:
    \[
        \exsts{\key} (\otW, \key, \stub) \in \fp'_m \land \mkvs_n(\key)(\mkvs_n(\key) - 1) \neq \txid \land \mkvs'_m(\key)(\lvert\mkvs'_m(\key)\rvert - 1)\projection{2} = \txid
    \]
    which contradicts with \( \mkvs'_m = \mkvs_n\).
\end{proof}

\begin{lemma}[Version persistence]
    \label{lem:unique-writer}
    \[
    \begin{array}{@{}l}
        \fora{\mkvs, \mkvs',\vienv,\vienv', \cl, \vi, \fp, i} 
        (\mkvs, \vienv) \toET{\cl, \fp}[\ET] (\mkvs', \vienv')
        \land (\otW, \key, \stub) \in \fp  
        \land 0 \leq i < \lvert \mkvs'(\key) \rvert - 1 \\
        \quad {} \implies \mkvs'(\key)(i)\projection{2} \neq \mkvs'(\key)(\lvert \mkvs'(\key) \rvert - 1)\projection{2}
    \end{array}
    \]
\end{lemma}
\begin{proof}
    By the definition of \( \toET{\stub}[\ET] \) (\cref{def:reduction}), the \( \mkvs' \in \updateKV[\mkvs, \vi, \fp, \cl] \).
    Given the definition of \( \updateKV[\mkvs, \vi, \fp, \cl]\), it the picks a fresh transaction identifier \( \txid \) such that does not appear in \( \mkvs \).
    For any write fingerprint \( (\otW, \key, \stub) \in \fp \), a new version is appended to the end of the key \( \key \) and the writer (the second projection) is assigned to be the fresh identifier \( \txid \).
    Thus we have the proof.
\end{proof}


==> composition-et/et-mono-new.tex <==
\subsection{Extra Monotonic \( \ET \)}
The relation \( \ET_1(\txidset_1,\rel_1) \etleq \ET_2(\txidset_2,\rel_2) \) is defined as the following:
\begin{align*}
    \ET_1(\txidset_1,\rel_1) \etleq \ET_2(\txidset_2,\rel_2) 
    & \defiff \fora{\mkvs,\vi,\cl,\fp} \txidset_2(\mkvs,\vi,\cl,\fp) \subseteq \txidset_1(\mkvs,\vi,\cl,\fp) \land \rel_2(\mkvs,\vi,\cl,\fp) \subseteq \rel_1(\mkvs,\vi,\cl,\fp)
\end{align*}
%For brevity, we write \(\txidset\) and \(\rel\) which are implicitly parametrised by \( \mkvs,\vi,\cl,\fp \).
%\begin{proposition}
%if $\ET_1(\txidset_1, \rel_1) \etleq \ET_2(\txidset_2,\rel_2)$ then $\ET_1 \subseteq \ET_2$.
%\end{proposition}
%\begin{proof}
%Assume \( (\mkvs,\vi,\cl,\fp) \in \ET_2 \).
%By definition
%\begin{centermultline}
    %\vi = \getView[\mkvs,\mu X \ldotp \txidset_2 \cup \rel^{-1}_2(X)]
%\end{centermultline}
%By \( \ET_1(\txidset_1, \rel_1) \etleq \ET_2(\txidset_2,\rel_2) \), 
%it follows \( \mu X \ldotp \txidset_2 \cup \rel^{-1}_2(X) \subseteq \mu X \ldotp \txidset_1 \cup \rel^{-1}_1(X)\),
%which means
%\begin{centermultline}
    %\vi = \getView[\mkvs,\mu X \ldotp \txidset_2 \cup \rel^{-1}_2(X)]
%\end{centermultline}
%Thus, \( (\mkvs,\vi,\cl,\fp) \in \ET_2 \).
%\end{proof}


==> composition-et/et-mono.tex <==
\subsection{Monotonic \( \ET \)}
\label{sec:mono-et}
\begin{proposition}
\label{prop:mono-et}
if $\ET_1 \subseteq \ET_2$ then $\CMs(\ET_1) \subseteq \CMs(\ET_2)$.
\end{proposition}
\begin{proof}
It is sufficient to prove that \(\ET_1 \subseteq \ET_2 \implies \confOf[\ET_1] \subseteq \confOf[\ET_2] \).
We prove it by induction on the length of the traces, \( i \).

\caseB{i = 0}
We have \( \conf_0 \in \confOf[\ET_1] \) and \( \conf_0 \in \confOf[\ET_2]\).
\caseI{i + 1}
Suppose identical traces of \( \ET_1 \) and \( \ET_2 \) respectively with length \( i \).
Let the final configuration be \( \conf_i = ( \mkvs_i, \vienv_i ) \).
If the next step is a view shift or a step with empty fingerprint, it trivially holds.
If the next step is a step by a client \( \cl \) with fingerprint \( \fp \),
we have \( \ET_1 \vdash (\mkvs_i, \vienv_i(\cl)) \csat \fp : (\mkvs_{i+1}, \vi') \),
where \( \mkvs_{i+1} \in \updateKV[ \mkvs_i, \vienv_i(\cl), \fp, \cl] \)
The next configuration from \( \ET_1 \) is \( \conf_{i+1} =  (\mkvs, \vienv_i\rmto{\cl}{\vi'})\).
Since \( \ET_1 \subseteq \ET_2 \), so \( \ET_2 \vdash (\mkvs_i, \vienv_i(\cl)) \csat \fp : (\mkvs_{i+1}, \vi') \) holds.
It is possible for \( \ET_2 \) to have the exactly same next configuration \( \conf_{n+1}\).
\end{proof}


==> composition-et/matching-view-et-example.tex <==
\subsection{\( \ET \)s matching views}
\label{sec:et-match-view}

To recall, 
two execution tests $\ET_1$ and $\ET_2$ have matching views if there exists a minimum client view function \( \func{minClientViews}[\ET,\mkvs,\cl] \) for \( \ET_1 \), \( \ET_2 \) and \( \ET_1 \cap \ET_2 \) such that:
\begin{itemize}
    \item for any \( \mkvs, \cl\):
    \begin{centermultline}
        \func{minClientViews}[\ET_1, \mkvs, \cl] \viewcup \func{minClientViews}[\ET_2, \mkvs, \cl] \viewleq \func{minClientViews}[\ET_1 \cap \ET_2, \mkvs, \cl]
    \end{centermultline}
    \item for any \(\mkvs, \mkvs',\fp,\vi_1,\vi_2,\vi_1',\vi_2',\cl\):
\begin{centermultline}
    (\vi_1,\vi'_1) =  \func{minFpViews}[\ET_1,\mkvs,\fp,\mkvs',\cl]
    \land (\vi_2,\vi'_2) =  \func{minFpViews}[\ET_2,\mkvs,\fp,\mkvs',\cl] \\
    \implies 
    \vi'_1 = \func{minClientView}[\ET_1, \mkvs',\cl]
    \land \vi'_2 = \func{minClientView}[\ET_2, \mkvs',\cl]  \\
    \exsts{\vi,\vi'} 
    (\vi,\vi') =  \func{minFpViews}[\ET_1 \cap \ET_2,\mkvs,\fp,\mkvs',\cl]
    \land \vi_1 \sqcup \vi_2 \viewleq \vi
    \land \vi'_1 \sqcup \vi'_2 \viewleq \vi' \\
    {} \land \vi' =  \func{minClientViews}[\ET_1 \cap \ET_2, \mkvs', \cl]
\end{centermultline}
where,
\begin{align*}
    (\vi,\vi') = \func{minFpViews}[\ET, \mkvs,\fp,\mkvs',\cl] & \defiff 
    \begin{multlined}[t]
        \func{minClientViews}[\ET, \mkvs, \cl] \viewleq \vi 
        \land \func{minClientViews}[\ET, \mkvs', \cl] \viewleq \vi' \\
        {} \land \ET \vdash (\mkvs,\vi) \csat \fp : (\mkvs',\vi') \\
        {} \land \fora{\vi'',\vi'''} \ET \vdash (\mkvs,\vi'') \csat \fp : (\mkvs',\vi''')
        \implies \vi \viewleq \vi'' \land \vi' \viewleq \vi'''
    \end{multlined} \\
    \vi \sqcup \vi' & \defeq \lambda \key \ldotp \vi(\key) \cup \vi'(\key)
\end{align*}
    \item for \( \ET_1 \) (\(\ET_2\) and \( \ET_1 \cap \ET_2\) respectively),
    if any kv-store \( \mkvs \) contains less information than \( \mkvs' \) then
    \begin{centermultline}
        \func{minClientView}[\ET_1,\mkvs,\cl] \viewleq \func{minClientView}[\ET_1, \mkvs',\cl]
    \end{centermultline}
\end{itemize}

\Cref{tab:et-minimum-view} presents the minimum client views for execution tests.
\begin{table}[h!]
    \centering
    \caption{Minimum view for clients}
    \label{tab:et-minimum-view}
\begin{tabular}{ @{} l r  @{} }
\hline
Model & \(\func{minClientViews}(\ET, \mkvs, \cl)\)
\\
\hline
\MR & $\getView[\mkvs,\Set{\txid }[\exsts{\txid_{\cl}} \txid \toEDGE{\WR_\mkvs} \txid_{\cl}] \cup \Set{\txid_0} ]$
\\
\MW & \(\vi_0\) \\
\RYW & $\getView[\mkvs,\Set{\txid_{\cl} \in \mkvs }\cup \Set{\txid_0} ]$  \\
\WFR & \(\vi_0\) \\
\(\MR \cap \MW \cap \RYW \cap \WFR\) & 
\(
\getView[\mkvs,\func{lfxTx}[%
        \mkvs,\Set{\txid }[\exsts{\txid_{\cl}} \txid \toEDGE{\WR_\mkvs} \txid_{\cl}] 
        \cup \Set{\txid_{\cl} \in \mkvs }  \cup \Set{\txid_0}, \SO\rflx \cup (\WR_\mkvs ; \SO\rflx)
    ] ]
\) \\
\hline
\end{tabular}%
\end{table}
\begin{align*}
    \func{lfpTx}[\mkvs,\txidset, R] 
    & \defeq 
    \mu X . 
    \begin{bracketarray}
        \txidset \subseteq X  
        \land \fora{ \txid \in X, \txid' \in \mkvs} \txid' \toEDGE{R} \txid \implies \txid' \in X 
    \end{bracketarray} 
\end{align*}


\begin{theorem}
    \( \MR \), \( \MW \), \( \RYW \) and \( \WFR \) have matching views.
\end{theorem}
\begin{proof}
Given \cref{tab:et-minimum-view}, it is easy to see for any \( \mkvs, \cl \):
\begin{centermultline}
    \begin{bracketarray}
    \func{minClientViews}[\ET_{\MR},\mkvs,\cl]
    \viewcup \func{minClientViews}[\ET_{\MW},\mkvs,\cl] \\
    \quad {} \viewcup \func{minClientViews}[\ET_{\RYW},\mkvs,\cl]
    \viewcup \func{minClientViews}[\ET_{\WFR},\mkvs,\cl] 
    \end{bracketarray} \\
    \viewleq \func{minClientViews}[\ET_{\MR} \cap \ET_{\MW} \cap \ET_{\RYW} \cap \ET_{\WFR},\mkvs,\cl]
\end{centermultline}
Also for any \( \ET \in \Set{\ET_{\MR}, \ET_{\MW}, \ET_{\RYW}, \ET_{\WFR}, \ET_{\MR} \cap \ET_{\MW} \cap \ET_{\RYW} \cap \ET_{\WFR}} \),
kv-stores \( \mkvs, \mkvs'\) where \( \mkvs \) contains less information than \( \mkvs' \), given \cref{tab:et-minimum-view} it follows:
\begin{centermultline}
    \func{minClientViews}[\ET,\mkvs,\cl] \viewleq \func{minClientViews}[\ET,\mkvs',\cl] 
\end{centermultline}
Now take arbitrary kv-stores \(\mkvs,\mkvs'\), fingerprint \( \fp \) and client \( \cl \), the \cref{tab:et-minimum-fingerprint}
shows the views given by the \( (\vi,\vi') = \func{minFpviews}[\ET,\mkvs,\fp,\mkvs',\cl] \) functions.
\begin{table}[h!]
    \centering
    \caption{Minimum views for fingerprints}
    \label{tab:et-minimum-fingerprint}
\begin{tabular}{ @{} l r r @{} }
\hline
Model & \(\vi\) & \(\vi'\)
\\
\hline
\MR 
& $\getView[\mkvs,\Set{\txid}[\exsts{\txid_{\cl}} \txid \toEDGE{\WR_{\mkvs}} \txid_{\cl}] \cup \Set{\txid_0} \cup \dagger ]$ 
& $\getView[\mkvs',\Set{\txid}[\exsts{\txid_{\cl}} \txid \toEDGE{\WR_{\mkvs'}} \txid_{\cl}] \cup \Set{\txid_0} ]$ \\
\MW 
& \(\getView[\mkvs,\func{lfpTx}[\mkvs,\dagger,\SO\rflx] ]\)
& \(\vi_0\) \\
\RYW 
& $\getView[\mkvs,\Set{\txid_{\cl} \in \mkvs} \cup \Set{\txid_0} \cup \dagger ]$
& $\getView[\mkvs',\Set{\txid_{\cl} \in \mkvs'} \cup \Set{\txid_0} ]$ \\
\WFR 
& \(\getView[\mkvs,\func{lfpTx}[\mkvs,\dagger,\WR_\mkvs ; \SO\rflx] ]\)
& \(\vi_0\) \\
\hline
\end{tabular}%
\end{table}

The \( \dagger \) is the versions read by the new transaction (\(\txid'\)) from client \( \cl \):
\begin{align*}
    \dagger & \equiv \Set{\txid}[\exsts{\txid'} \txid \in \mkvs' \land \txid' \notin \mkvs \land \txid \toEDGE{\WR_{\mkvs'}} \txid]
\end{align*}
Note that the \( \vi' \) in \cref{tab:et-minimum-fingerprint} already satisfies \( \vi' = \func{minClientViews}[\ET,\mkvs',\cl]\).
Assume the following where \( \vi_i, \vi'_i \) are taken the ones from \cref{tab:et-minimum-fingerprint}:
\begin{centermultline}
    \ET_{\MR} \vdash (\mkvs,\vi_1) \csat \fp : (\mkvs', \vi_1' ) 
    \land \ET_{\MW} \vdash (\mkvs,\vi_2) \csat \fp : (\mkvs', \vi_2' ) \\
    {} \land \ET_{\RYW} \vdash (\mkvs,\vi_3) \csat \fp : (\mkvs', \vi_3' )
    \land \ET_{\WFR} \vdash (\mkvs,\vi_4) \csat \fp : (\mkvs', \vi_4' ) 
\end{centermultline}
Let \( \vi \)
\begin{centermultline}
    \vi = \getView[\mkvs,\func{lfxTx}[%
        \mkvs,\Set{\txid }[\exsts{\txid_{\cl}} \txid \toEDGE{\WR_\mkvs} \txid_{\cl}] 
        \cup \Set{\txid_{\cl} \in \mkvs }  \cup \dagger \cup \Set{\txid_0}, \SO\rflx \cup (\WR_\mkvs ; \SO\rflx)
    ] ]
\end{centermultline}
and \( \vi' \)
\begin{centermultline}
    \vi' = \getView[\mkvs',\func{lfxTx}[%
        \mkvs,\Set{\txid }[\exsts{\txid_{\cl}} \txid \toEDGE{\WR_{\mkvs'}} \txid_{\cl}] 
        \cup \Set{\txid_{\cl} \in \mkvs' } \cup \Set{\txid_0}, \SO\rflx \cup (\WR_{\mkvs'} ; \SO\rflx)
    ] ]
\end{centermultline}
It is easy to see \( \vi_1 \viewcup \vi_2 \viewcup \vi_3 \viewcup \vi_4 \viewleq \vi \) 
and  \( \vi'_1 \viewcup \vi'_2 \viewcup \vi'_3 \viewcup \vi'_4 \viewleq \vi = \func{minClientViews}[\MR \cap \MW \cap \RYW \cap \WFR, \mkvs',\cl] \).
We now prove that \( \ET_\MR \cap \ET_\MW \cap \ET_\RYW \cap \ET_\WFR \vdash (\mkvs,\vi) \csat \fp : (\mkvs',\vi')\), which can implied by proving \( \bigwedge_{1 \leq i \leq 4} \max(\vi)(\key) = \max(\vi_i)(\key) \) for any key \( \key \) being read.
\end{proof}




\begin{lemma}
\( \MR \) and \( \MW \) have matching views.
\end{lemma}
\begin{proof}
Assume kv-stores \( \mkvs, \mkvs' \), a fingerprints \( \fp \) and views \( \vi_1, \vi'_1, \vi_2, \vi'_2 \):
\begin{centermultline}
    \ET_{\MR} \vdash (\mkvs,\vi_1) \csat \fp : (\mkvs', \vi_1' ) \land
    \ET_{\MW} \vdash (\mkvs,\vi_2) \csat \fp : (\mkvs', \vi_2' )
    \land \begin{bracketarray}\fora{l, \key, \val} (l, \key, \val) \in \fp \implies \max(\vi_1(\key)) = \max(\vi_2(\key))\end{bracketarray} 
\end{centermultline}
We pick \(\vi, \vi' \) such that:
\begin{centermultline}
    \fora{\key} 
    \begin{bracketarray}\exsts{l,\val} (l,\key,\val) \in \fp \implies \vi_1(\key) \cup \vi_2(\key) = \vi(\key)\end{bracketarray} \\
    {} \land \begin{bracketarray}
        \nexists l,\val \ldotp \; (l,\key,\val) \in \fp 
        \implies \vi_1(\key) \cup \vi_2(\key) \cup \vi'_1(\key) \cup \vi'_2(\key) = \vi(\key)
\end{bracketarray}
    \land \vi'(\key) = \vi'_1(\key) \cup \vi'_2(\key)
\end{centermultline}
Given \( \vi_1 \viewleq \vi'_1 \) it is easy to see that \( \vi \viewleq \vi' \) and then \( \ET_\MR \vdash (\mkvs,\vi) \csat \fp : (\mkvs',\vi') \).
Given that \( \fora{\key} \exsts{l,\val}  (l,\key,\val) \in \fp \implies \vi_1(\key) \cup \vi_2(\key) = \vi(\key) \), it means \( \allowed[\mkvs,\vi,\fp,\SO\rflx]\),
and thus \( \ET_\MW \vdash (\mkvs,\vi) \csat \fp : (\mkvs',\vi') \).
\end{proof}

\begin{lemma}
    \( \MR \) and \( \RYW \) have matching views.
\end{lemma}
\begin{proof}
Assume kv-stores \( \mkvs, \mkvs' \), a fingerprints \( \fp \) and views \( \vi_1, \vi'_1, \vi_2, \vi'_2 \):
\begin{centermultline}
    \ET_{\MR} \vdash (\mkvs,\vi_1) \csat \fp : (\mkvs', \vi_1' ) \land
    \ET_{\RYW} \vdash (\mkvs,\vi_2) \csat \fp : (\mkvs', \vi_2' )
    \land \begin{bracketarray}\fora{l, \key, \val} (l, \key, \val) \in \fp \implies \max(\vi_1(\key)) = \max(\vi_2(\key))\end{bracketarray} 
\end{centermultline}
We pick \(\vi, \vi' \) such that:
\begin{centermultline}
    \fora{\key} 
    \begin{bracketarray}\exsts{l,\val} (l,\key,\val) \in \fp \implies \vi_1(\key) \cup \vi_2(\key) = \vi(\key)\end{bracketarray} \\
    {} \land \begin{bracketarray}
        \nexists l,\val \ldotp \; (l,\key,\val) \in \fp 
        \implies \vi_1(\key) \cup \vi_2(\key) \cup \vi'_1(\key) \cup \vi'_2(\key) = \vi(\key)
\end{bracketarray}
    \land \vi'(\key) = \vi'_1(\key) \cup \vi'_2(\key)
\end{centermultline}
Given \( \vi_1 \viewleq \vi'_1 \) it is easy to see that \( \vi \viewleq \vi' \) and then \( \ET_\MR \vdash (\mkvs,\vi) \csat \fp : (\mkvs',\vi') \).
Since that \( \vi'(\key) = \vi'_1(\key) \cup \vi'_2(\key) \) for any key \(\key\), 
it follows that \( \vi' \) contains all the version written by the client of the new transaction \( txid \):
\[
    \fora{key,i} \txid \in \mkvs' \land \txid \notin \mkvs \wtOf[\mkvs'(\key,i)] \toEDGE{\SO\rflx} \txid \implies i \in \vi'(\key)
\]
That is, \( \ET_\RYW \vdash (\mkvs,\vi) \csat \fp : (\mkvs',\vi') \).
\end{proof}



==> composition-et/normal-trace.tex <==
%\subsection{Normal \( \ET \) Traces}
\label{sec:normal-form-exist}
Given a program $\prog$ and an execution test $\ET$, we say that an \emph{execution fragment} of 
$\prog$ under $\ET$ is a sequence of transitions 
$(\mkvs_{0}, \vienv_{0}, \thdenv_{0} ), \prog \toCMD{\_}_{\ET}^{\ast} ( \mkvs, \vienv, \thdenv ) , \prog' )$, 
where $(\mkvs_{0}, \vienv_{0})$ is an initial configuration and $\thdenv_{0}$ is a partial function mapping 
clients in $\lambda x. 0$. If $\prog'(\cl) = \pskip$ whenever $\prog'(\cl)$ is defined, then 
we refer to the sequence of execution above as an \emph{execution} of $\prog$ under $\ET$, and 
we say that $\mkvs$ is \emph{reachable} by executing $\prog$ under $\ET$.

Throughout this Section, we assume that the execution test $\ET$ is fixed. 
Our aim is that of relating  executions of programs under the execution test $\ET$, and $\ET$-traces. 
In particular, we prove  \cref{thm:ettraces2sem}. To this end, we show the following: 

\begin{proposition}
\label{prop:sem2ettraces}
$\bigcup_{\prog} \interpr{\prog}_{\ET} \subseteq \CMs(\ET)$.
\end{proposition}

\begin{proposition}
\label{prop:ettraces2sem}
$\CMs(\ET) \subseteq \bigcup_{\prog} \interpr{\prog}_{\ET}$
\end{proposition}

Let us focus first on the proof of \cref{prop:sem2ettraces}. First, given a program $\prog$, 
we encode the execution of some transactional code $\ptrans{\trans}$ in a program, 
terminating in a configuration $\conf$, into a sequence of $\ET$-reductions also terminating 
in $\conf$. Then we lift this result to execution fragments generated by the program $\prog$ by using 
a simple inductive argument. Because an execution of $\prog$ under $\ET$ is also an execution fragment, 
each execution of $\prog$ terminating in a configuration $\conf$ induces a $\ET$-trace terminating in 
the same configuration, thus showing that $\conf \in \CMs(\ET)$.

\begin{lemma}
\label{lem:sem2ettrace}
For all programs $\prog$ and transitions of the form 
form $\vdash (\mkvs, \vienv, \thdenv ), \prog \toCMD{(\cl, \vi, \fp)}_{\ET}^{\ast} ( \mkvs', \vienv', \thdenv' ) , \prog' )$,  
we have that  
\[
(\mkvs, \vienv) \toET{(\cl, \varepsilon)} (\mkvs, \vienv\rmto{\cl}{\vi}) \toET{(\cl, \fp)} (\mkvs', \vienv').
\]
\end{lemma}

\ac{The semantics of programs for clients has some degree of redundancy that 
should be eliminated. In particular in the transition 
$\cl \vdash 
        ( \mkvs, \vi, \stk ), \ptrans{\trans} 
        \toCMD{(\cl, \vi'', \fp)}_{\ET}
        (\mkvs',\vi', \stk' ) , \pskip$, the parameter $\cl$ is used twice. 
Choose which of the two occurrences you want to keep, and remove the other. 
In the rest of the proof I will assume that the parameter $\cl$ has been removed from the 
action of the transition, and that Rule PProg has been modified to reintroduce the parameter 
$\cl$ into the action. Note that keeping the parameter $\cl$ in both places in the transition above 
complicates the proof of \cref{lem:sem2ettrace}, as it requires proving the following (trivial) lemma: 
if $\cl \vdash (\mkvs, \vi, \stk, \cmd) \toCMD(\cl', \mu) (\mkvs', \vi', \stk', \cmd')$, then $\cl = \cl'$.}

\begin{proof}
Suppose that $ \vdash (\mkvs, \vienv, \thdenv ), \prog \toCMD{(\cl, \vi, \varepsilon)}_{\ET} 
( \mkvs', \vienv', \thdenv') , \prog' )$. This transition could have been derived only by 
applying Rule $\rl{PProg}$, from which it follows that $\cl \vdash (\mkvs, \vi'', \stk), \cmd \toCMD{(\vi, \fp)} 
(\mkvs', \vi', \stk'), \cmd'$, where $\vi'' = \vienv(\cl)$, $\vienv' = \vienv\rmto{\cl}{\vi'}$, $\stk = \thdenv(\cl)$, $\thdenv' = \thdenv\rmto{\cl}{\stk'}$, $\cmd = \prog(\cl)$ 
and $\prog' = \prog\rmto{\cl}{\cmd'}$. The rest of the proof is performed by Rule induction on the 
derivation of the transition $\cl \vdash (\mkvs, \vi'', \stk), \cmd \toCMD{(\vi, \fp)} 
(\mkvs', \vi', \stk')$. 
\begin{itemize}
\item The only base case corresponds to such a transition being derived via an 
application of  Rule $\rl{CAtomicTrans}$. In this case we have that 
$\vi'' \sqsubseteq \vi$, $(\stk, \sn, \emptyset) \toTRANS^{\ast} (\stk', \_, \fp)$ for $\sn = \snapshot[\mkvs, \vi]$, 
$\mkvs' = \updateKV[\mkvs, \vi, \fp \txid]$ for some $\txid \in \nextTxid[\cl, \mkvs]$ and 
$\ET \vdash (\mkvs,\vi) \csat \fp: (\mkvs', \vi')$. Because $\vi'' \sqsubseteq \vi'$ and $\vienv(\cl) = \vi''$, 
we have that $(\mkvs, \vienv) \toET(\cl, \varepsilon) \mkvs, \vienv\rmto{\cl}{\vi}$. Also, because 
$\mkvs' = \updateKV[\mkvs, \vi, \fp, \txid]$, $\txid \in \nextTxid[\cl, \mkvs]$, and $\ET \vdash (\mkvs, \vi) 
\csat \fp: (\mkvs', \vi')$, we have that 
$(\mkvs, \vienv\rmto{\cl}{\vi}) \toET{(\cl, \fp)} (\mkvs', \vienv\rmto{\cl}{\vi'}) = (\mkvs', \vienv')$, as we wanted 
to prove.
\item For the inductive case, the only rule that can have been applied to infer the transition 
$\cl \vdash (\mkvs, \vi'', \stk), \cmd \toCMD{(\vi, \fp)} (\mkvs', \vi', \stk'), \cmd'$ is Rule $\rl{CSeq}$. 
In this case we have that $\cmd = \cmd_1 ; \cmd_2$, $\cmd' = \cmd_1' ; \cmd_2$ for some $\cmd_1, \cmd_1', \cmd_2$, 
$\cl \vdash (\mkvs, \vi'', \stk), \cmd_1 \toCMD{(\vi, \fp)} (\mkvs', \vi', \stk'), \cmd_1'$. By the inductive hypothesis, 
we obtain that 
$(\mkvs, \vienv) \toET{(\cl, \varepsilon)} (\mkvs, \vienv\rmto{\cl}{\vi}) \toET{(\cl, \fp)} (\mkvs', \vienv')$.
\end{itemize}
\end{proof}

\paragraph{Proof of \cref{prop:sem2ettraces}.} 
Recall that we let $\mkvs_{0}$ be the initial kv-store that maps 
each key in the list of locations containing the single version $(0, \txid_{0}, \emptyset)$, 
and we use $\vienv_{0}$ to denote an arbitrary partial mapping of clients into the only valid view 
of $\mkvs_{0}$.

Fix an arbitrary program $\prog$. We prove a more general result: 
whenever $(\mkvs_{0}, \vienv_{0}, \thdenv_{0}) \prog \toCMD{\stub}^{\ast} (\mkvs', \vienv', \thdenv'), prog'$, 
then there exists an $\ET$-trace $\tau$ terminating in the configuration $(\mkvs', \vienv')$, 
and therefore $\mkvs' \in \CMs(\ET)$.
Then \cref{prop:sem2ettraces} follows immediately by considering the 
special case when $\prog'$ is such that $\forall \cl \in \dom(\prog').\; \prog'(\cl) = \pskip$.

Suppose that $(\mkvs,_{0} \vienv_{0}, \thdenv_{0}) \prog \toCMD{\stub}^{\ast} (\mkvs', \vienv', \thdenv'), \prog'$. 
By definition, then $(\mkvs, \vienv, \thdenv_{0}) \prog \toCMD{\stub}^{n} (\mkvs', \vienv', \thdenv'), \prog'$ 
for some $n \geq 0$. We prove that there exists a $\ET$-trace $\tau$ terminating in $(\mkvs\, \vienv')$ 
by induction on $n$. 
\begin{itemize}
\item Base case: $n = 0$. In this case $(\mkvs', \vienv') = (\mkvs_{0}, \vienv_{0})$, and the latter 
is also an $\ET$-trace with no $\ET$-reductions. This case is trivial. 
\item Inductive step: $n > 0$. In this case we have that $(\mkvs_{0}, \vienv_{0}, \thdenv_{0}), \prog \toCMD{\stub}^{n-1} (\mkvs'', \vienv'', \thdenv''), \prog''
\toCMD{\lambda} (\mkvs', \vienv', \thdenv'), \prog'$ for some $\mkvs'', \vienv'', \thdenv'',\prog''$. By inductive hypothesis, 
there exists an $\ET$-trace $\tau_{n-1}$ terminating in the configutration $(\mkvs'', \vienv'')$. 
We distinguish between two cases, according to action $\lambda$: 
\begin{itemize}
\item $\lambda = (\cl, \iota)$ for some client $\cl$. A simple rule induction on the rules of \cref{fig:full-semantics} 
reveals that in this case we have that $(\mkvs', \vienv') = (\mkvs'', \vienv'')$, and therefore we let $\tau := \tau_{n-1}$; 
\item of $\lambda = (\cl, \vi, \fp)$ for some $\cl, \vi, \fp$. By \cref{lem:sem2ettrace}, there exists a sequence 
of $\ET$-reductions $(\mkvs'', \vienv'') \toET{(\cl, \varepsilon)} (\mkvs'', \vienv''\rmto{\cl}{\vi}) \toET{(\cl, \fp)} (\mkvs', \vienv')$. 
Because the $\ET$-trace $\tau_{n-1}$ terminates in the configuration $(\mkvs'', \vienv'')$, then
\[
\tau := \tau_{n-1} \toET{(\cl, \varepsilon)} (\mkvs'', \vienv''\rmto{\cl}{\vi}) \toET{(\cl, \fp)} (\mkvs', \vienv')
\]
is a well-defined $\ET$-trace that terminates in the configuration $(\mkvs', \vienv')$, which concludes the proof.\hfil\qed
\end{itemize}
\end{itemize}

Let us turn our attention to the proof of \cref{prop:ettraces2sem}. The proof of this result is more involved 
technically than the previous proof, because of two reasons. The first reason is that  
executions of programs under the execution test $\ET$ and $\ET$-traces. Whereas in executions of 
programs under the execution test $\ET$
a client can only shift its view immediately before executing a transaction, in $\ET$-traces a client 
can perform a view shift arbitrarily. It would seem then that $\ET$-traces are more expressive than 
executions of programs. However, this difference in expressive power is only apparent: for any 
$\ET$-trace $\tau$ ending in a configuration $(\mkvs, \_)$, we can always construct another 
$\ET$-trace $\tau'$ that ends in the same configuration and that is in \emph{normal form}: 
all view shifts performed by a client immediately precede a transaction commit performed by 
the same client.

%
%First, we show how to convert an $\ET$-trace $\tau$, ending in a configuration of the form $(\mkvs, \_)$, 
%into a \emph{normal} trace $\tau'$, also ending in $(\mkvs, \_)$ 
%and with the additional property that in view shifts of clients, i.e. actions of the form $(\cl, \varepsilon)$, 
%immediately precede a transaction commit performed by the same client, i.e. an action of the form $(\cl, \fp)$. 
\begin{definition}
Let $\ET$ be an execution test. The $\ET$-trace
\[
\conf_0 \toET{(\cl_{0}, \alpha_0)} \conf_1 \toET{(\cl_1, \alpha_1)} \cdots \toET{(\cl_{(2\cdot n) - 1}, \alpha_{2\ cdot n - 1})} \conf_{2 \cdot n}
\]
is in \emph{normal form} if \textbf{(i)} $\conf_0$ is initial, and 
\textbf{(ii)} $\forall  i.\; 0 \leq i < n$ 
\ac{Throughout the text sometimes we use $\forall i. P$, other times we use $\forall i: P$. The style should be 
made consistent. Also, I know you really like to use define macros for everything, but sometimes you define too 
many of them. I still don't see the point of the \textbf{fora} command.}

there exists a client $\cl_i$ and set of operations $\fp_{i}$ such that 
$\alpha_{2 \cdot i} = \varepsilon$, $\cl_{2 \cdot i + 1} = \cl_{2 \cdot i}$ and $\alpha_{2 \cdot i + 1} = \fp_{i}$ for some $\fp_{i} \subseteq \opset$.
\end{definition}


%Note that the structure of $\ET$-reductions in normal $\ET$-traces matches closely the structure of 
%transitions in executions of  programs under $\ET$. 
%In fact, in the latter a transition of the form $(\mkvs, \vienv, \thdenv ), \prog \toCMD{(\cl, \vi, \fp)}_{\ET} ( \mkvs', \vienv', \thdenv' ) , \prog' )$ 
%corresponds to client $\cl$ shifting its view to $\vi$, and then committing a transaction with 
%fingerprint $\fp$. 
%Converting a $\ET$-trace in normal form is a necessary step towards proving \cref{thm:ettraces2sem}. 
\begin{proposition}[Normal \( \ET \) Traces]
\label{prop:et.normalform}
Let $\ET$ be an execution test, and suppose that $\mkvs \in \CMs(\ET)$. Then there exists a $\ET$-trace  
\[
(\mkvs_0, \vienv_0) \toET{\stub} \cdots \toET{\stub} (\mkvs_n, \vienv_{n})
\]
that is in normal form, and such that $\mkvs_{n} = \mkvs$.
\end{proposition}
%
%The proof \cref{prop:et.normalform}, which we will illustrate shortly, relies on constructing
%repeatedly re-arranging the view-shifts appearing in a $\ET$-trace $\tau$, while preserving 
%the order in which fingerprints are committed in $\tau$, as well as the view that clients use 
%to commit such fingerprints. To achieve this, we identify two particular transformations over 
%$\ET$-traces: view-shift absorptions and view-shift  right-moves. 
%
%\begin{lemma}[View-shift Absorption]
%\label{lem:et.absorb}
%If $\conf \toET{(\cl, \varepsilon)} \conf' \toET{(\cl, \varepsilon)} \conf''$, then 
%$\conf \toET{(\cl, \varepsilon)} \conf''$.
%\end{lemma}
%
%\begin{proof}
%Let $\conf = (\mkvs, \vienv)$, $\conf' = (\mkvs', \vienv')$, $\conf'' = (\mkvs', \vienv'')$. 
%By the reduction it must be the case that $\mkvs = \mkvs'$, and $\vienv' = \vienv\rmto{\cl}{\vi'}$ 
%for some $\vi' : \vi \sqsubseteq \vi'$. It must also be the case that $\mkvs' = \mkvs''$, and $\vienv'' = \vienv'\rmto{\cl}{\vi''}$ 
%for some $\vi'': \vi' \sqsubseteq \vi''$. Therefore we have that $\mkvs'' = \mkvs' = \mkvs$, and 
%$\vienv'' = \vienv'\rmto{\cl}{\vi''} = (\vienv\rmto{\cl}{\vi'})\rmto{\cl}{\vi''} = \vienv\rmto{\cl}{\vi''}$, 
%and $\vi \sqsubseteq \vi''$. 
%It follows that $\conf = (\mkvs, \vienv) \toET{(\cl, \varepsilon)} (\mkvs'', \vienv'') = \conf''$.
%\end{proof}
%
%\begin{lemma}[View-shift Swap]
%\label{lem:viewshift.rightmover}
%Let $\conf \toET{(\cl, \varepsilon)} \conf_1 \toET{(\cl', \alpha)} \conf'$ 
%for some $\conf, \conf_1, \conf''$ and $\cl, \cl'$ such that $\cl' \neq \cl$. 
%Then $\conf \toET{(\cl', \alpha)} \conf_2 \toET{(\cl, \varepsilon)} \conf'$ 
%\end{lemma}
%
%\begin{proof}
%We only consider the case where $\alpha = \fp$ for some fingerprint $\fp$. The case where 
%$\alpha = \varepsilon$ is simpler to prove.
%Let $\conf = (\mkvs, \vienv)$, $\conf_1 = (\mkvs_1, \vienv_1)$, $\conf' = (\mkvs', \vienv')$. 
%Let also $\vi = \vienv(\cl)$.
%By the reduction rule we have that $\mkvs_1 = \mkvs, \vienv_1 = \vienv\rmto{\cl}{\vi_1}$ for 
%some $\vi_1: \vi_1 \sqsubseteq \vi_1$. Let $\vi' = \vienv(\cl')$: then we have that $\vienv_1(\cl') = 
%\vi'$. Because $(\mkvs_1, \vienv_1) \toET{(\cl', \fp)} (\mkvs', \vienv')$, we have that 
%$\ET \vdash (\mkvs_1, \vi') \csat \fp : (\mkvs',\vi'') $, where $\vi'' = \vienv'(\cl')$. Because $\mkvs_1 = \mkvs$, 
%that means that $\ET \vdash (\mkvs, \vi') \csat \fp: (\mkvs', \vi'')$, then it follows that 
%$(\mkvs, \vienv) \toET{(\cl', \fp)} (\mkvs', \vienv\rmto{\cl'}{\vi''}) 
%\toET{(\cl, \varepsilon)} (\mkvs', \vienv\rmto{\cl'}{\vi''}\rmto{\cl}{\vi_1}) = 
%(\mkvs', \vienv\rmto{\cl}{\vi_1}\rmto{\cl'}{\vi''}) = (\mkvs', \vienv_1\rmto{\cl'}{\vi''}) = 
%(\mkvs', \vienv')$, as we wanted to prove.
%\end{proof}

\begin{proof}
Let $\mkvs \in \CMs(\ET)$. By definition, there exists a $\ET$-trace  
\begin{equation}
\label{eq:normalform.sequence}
\tau = (\mkvs_{0}, \vienv_{0}) \toET{(\cl_0, \alpha_0)} \cdots \toET{(\cl_{n-1}, \alpha_{n-1})} (\mkvs_n, \vienv_{n})
\end{equation}
such that $\mkvs_{n} = \mkvs$. 
We show that there exists a $\ET$-trace 
\[
\tau' = (\mkvs'_{0} \vienv'_{0}) \toET{(\cl'_{0}, \alpha'_{0})} \cdots \toET{(\cl'_{m-1}, \alpha'_{m-1})} (\mkvs'_{m}, \vienv'_{m})
\]
that is in normal form, such that $\mkvs'_{m} = \mkvs$ and for any client $\cl \in \dom(\vienv_{n})$, $\vienv'_{m}(\cl) \sqsubseteq 
\vienv_{n}(\cl)$. The proof is done by induction on the length $n$ of $\tau$. 
\begin{itemize}
\item Base case: $n = 0$. In this case $\tau = (\mkvs, \vienv_{0})$, which by definition is in normal form. Then it 
suffices to choose $\tau' = \tau$; also, for any client $\cl \in \dom(\vienv_{0})$, the inequality $\vienv_{0}(\cl) \sqsubseteq 
\vienv_{0}(\cl)$ trivially holds, 
\item Inductive case: let $n > 0$, and consider the fragment of $\tau$ given by 
\[
\tau'' = (\mkvs_{0}, \vienv_{0}) \toET{(\cl_0, \alpha_0)} \cdots \toET{(\cl_{n-2}, \alpha_{n-2})} (\mkvs_{n-1}, \vienv_{n-1}).
\]
By inductive hypothesis, there exists a trace $\tau'''$ of the form 
\[
\tau''' = (\mkvs'_{0} \vienv'_{0}) \toET{(\cl'_{0}, \alpha'_{0})} \cdots \toET{(\cl'_{m-1}, \alpha'_{j-1})} (\mkvs'_{j}, \vienv'_{j})
\]
that is in normal form, and such that $\mkvs'_{j} = \mkvs_{n-1}$, for any $\cl \in \dom(\vienv_{n-1})$, $\vienv'_{j}(\cl) \sqsubseteq 
\vienv_{n-1}(\cl)$. Next, consider the transition $(\mkvs_{n-1}, \vienv_{n-1}) \toET{(\cl_{n-1}, \alpha_{n-1})} (\mkvs_{n}, \alpha_{n})$. 
There are two different cases, according to the structure of the action $\alpha_{n-1}$: 
\begin{itemize}
\item $\alpha_{n-1} = \varepsilon$, or $\alpha_{n-1} = \emptyset$. In this case, $\mkvs_{n} = \mkvs_{n-1}$, and $\vienv_{n} = \vienv_{n-1}\rmto{\cl_{n-1}}{\vi}$, 
for some $\vi : \vienv_{n-1}(\cl_{n-1}) \sqsubseteq \vi$. In particular, we have that $\dom(\vienv_{n-1}) = \dom(\vienv_{n})$, 
and for any $\cl \in \dom(\vienv_{n-1})$, then $\vienv_{n-1}(\cl) \sqsubseteq \vienv_{n}(\cl)$. In this case, we let $\tau' := \tau'''$. 
By the inductive hypothesis, we have that $\mkvs'_{j} = \mkvs_{n-1} = \mkvs$, and for any $\cl \in \dom(vienv_{n})$, 
$\vienv'_{j}(\cl) \sqsubseteq \vienv_{n-1}(\cl) \sqsubseteq \vienv_{n}(\cl)$, 
\item $\alpha_{n-1} = \fp$ for some $\fp \neq \emptyset$. 
Let $\vi_{n-1} = \vienv_{n-1}(\cl_{n-1})$, $\vi_{n} = \vienv_{n}(\cl_{n-1})$. Then \textbf{(a)} there exists $\txid \in \nextTxid(\cl, \mkvs)$ 
such that $\mkvs_{n} = \updateKV(\mkvs_{n-1}, \vi_{n-1}, \fp, \txid)$, $\ET \vdash (\mkvs_{n-1}, \vi_{n-1}) \triangleright \fp: (\mkvs_{n}, \vi_{n})$ 
and $\vienv_{n} = \vienv_{n-1}\rmto{\cl_{n-1}}{\vi_{n}}$. 
We also have that \textbf{(b)} $\vienv_{n-1}(\cl)$ is defined and equal to $\cl$, which means that $\vienv'_{j}(\cl) \sqsubseteq \vienv_{n-1}$. 
Using \textbf{(a)} and \textbf{(b)} above, and knowing that $\mkvs'_{j} = \mkvs_{n-1}$ by induction,   we can extend 
$\tau'''$ with the sequence of $\ET$-reduction 
\[ (\mkvs'_{j}, \vienv'_{j}) = (\mkvs_{n-1}, \vienv'_{j}) 
 \toET{(\cl_{n-1}, \varepsilon)} (\mkvs_{n}, \vienv'_{j}\rmto{\cl_{n-1}}{\vi_{n-1}}) \toET{(\cl_{n-1}, \fp)} (\mkvs_{n}, \vienv'_{j}\rmto{\cl_{n-1}}{\vi_{n}}.
 \]
Let $\tau''$ be the resulting trace, and let $(\mkvs'', \vienv'')$ be the last configuration of $\tau''$. 
Obviously, $\mkvs'' = \mkvs_{n}$. Furthermore, let $\cl \in \dom(\vienv_{n})$. Then either $\cl = \cl_{n-1}$, 
in which case $\vienv_{n}(\cl_{n-1}) = \vi_{n} = \vienv''(\cl_{n-1})$, or 
$\vienv_{n}(\cl) = \vienv_{n-1}(\cl) \sqsubseteq \vienv'_{j}(\cl) = \vienv''(\cl)$. That is, for any $\cl \in \dom(\vienv_{n})$, 
$\vienv''(\cl) \sqsubseteq \vienv_{n}(\cl)$, and there is nothing left to prove.
\end{itemize}

\end{itemize}

\end{proof}

The second problem that we face, when proving \cref{prop:ettraces2sem}, 
is that for any $\ET$-trace $\tau$ that is in normal form and 
that terminates in the configuration $(\mkvs, \_)$, we need to define a program 
$\prog_{\tau}$ which has an execution terminating in the same configuration. 
To this end, we first map fingerprints into transactional code, and then we lift 
this mapping to $\ET$-traces and programs. 

\begin{definition}
\label{def:fp2prog}
\ac{This mapping assumes that fingerprints are finite. This assumption was lifted when we 
decided to admit the initial transaction into abstract executions, which leads to such a transaction 
having an infinite fingerprint. It may be useful to state that $\txid_{0}$ is the only transaction that is 
allowed to have an infinite fingerprint.}

Note that any fingerprint set 
$\fp$ is either the empty set $\fp$; or it has the form $\{(\otR, \key, \val)\} \uplus \fp'$ for 
some $\fp'$ such that $(\otR, \key, \val') \notin \fp'$ for any $\val' \in \Val$; 
or it has the form $\{(\otW, \key, \val)\} \uplus \fp'$ for some $\key, \val$ such that 
$(\otW, \key', \val') \notin \fp'$ for any $\key' \in \Keys, \val' \in \Val$, and 
$(\otR, \key, \val') \notin \fp'$, for any $\val' \in \Val$.  

Given a (finite) fingerprint $\fp$, we define the transactional code $\trans_{\fp}$ by induction 
on $\fp$, via an induction schema based on the characterisation of finite fingerprints given above.
\begin{itemize}
\item if $\fp = \emptyset$, then $\trans_{\fp} = \pskip$, 
\item if $\fp = \{(\otR, \key, \val)\} \uplus \fp'$ for some $\key, \val, \fp'$, and $(\otR,\key,\val') \notin \fp'$ for any 
$\val' \in \Val$, then $\trans_{\fp'} = \plookup{\_}{\key} ; \trans_{\fp'}$, 
\item if $\fp = \{(\otW, \key, \val)\} \uplus \fp'$ for some $\key, \val, \fp'$, $(\otR,\key', \val') \notin \fp'$ for all 
$\val' \in \Val$ and $\key \in \Keys$, $(\otW, \key, \val') \notin \fp'$ for all $\val' \in \Val$, 
then $\trans_{\fp} = \pmutate{\key}{\val} ; \trans_{\fp'}$.
\end{itemize}
\ac{To be pedantic, the definition above is ill-formed, as the same fingerprint can lead to multiple 
definitions of $\fp$. This should be fixed by defining a set of transactional commands for 
fingerprints, and prove the necessary properties for all the transactional commands induced 
by a fingerprint.}

Consider an $\ET$-trace $\tau$ that is in normal form and that terminates in the configuration $(\mkvs, \vienv)$. Let $C = \dom(\vienv)$. 
We define the program $\prog_{\tau}$ by induction on the structure of $\tau$. 
\begin{itemize}
\item if $\tau = (\mkvs_{0}, \vienv_{0})$, i.e. it has no transitions, then $\prog_{\tau} = \lambda \cl \in C. \pskip$, 
\item if $\tau = \tau' \toET{(\cl, \varepsilon)} (\mkvs', \vienv') \toET{(\cl, \fp)} (\mkvs, \vienv)$, then 
$\prog_{\tau} = \prog_{\tau'}\rmto{\cl}{\prog_{\tau'}(\cl)}; \ptrans{\trans_{\fp}}$.
\end{itemize}
\end{definition}

Clearly, the command $\trans_{\fp}$  is defined in a way that its 
execution from a client whose local state agrees with the read operations 
of $\fp$,  leads to the fingerprint $\fp$ itself. More formally, we have the 
following result: 
\begin{lemma}
\label{lem:fp2trans}
Let $\fp$ be an arbitrary, finite fingerprint, and let $\sn$ be such that, whenever 
$(\otR, \key, \val) \in \fp$, then $\sn(\key) = \val$. Then, for any $\stk \in \Vars \rightarrow \Val$,
\[
(\stk, \sn, \emptyset), \trans_{\fp} \trans_{\fp} \toTRANS^{\ast} (\stub, \stub, \fp), \pskip
\]
\end{lemma}

\begin{proof}
The proof of \cref{lem:fp2trans} is by induction on the structure $\fp$, via an 
induction schema that follows the characterisation of fingerprints from \cref{def:fp2prog}.

If $\fp = \emptyset$ then $\trans_{\fp} = \pskip$, and $(\stk, \sn, \emptyset), 
\pskip \toTRANS^{\ast} (\stk, \sn, \emptyset)$. 
Suppose then that $\fp = \{(\otR, \key, \val)\} \uplus \fp'$, and that 
$(\otR, \key, \val') \notin \fp'$ for any $\val' \in \Val$. 
Suppose also that $\sn$ is such that whenever $(\otR, \key', \val') \in \fp$ then $\sn(\key') = \val'$. 
In particular, because $(\otR,\ ke, \val) \in \fp$, then $\sn(\key) = \val$; and for any $(\otR,\ ke', \val') \in \fp'$, 
then $\sn(\key') = \val'$. 
By definition, $\trans_{\fp} = \plookup{\_}{\key} ; \trans_{\fp'}$. By applying Rule \rl{Tprimitive} 
we obtain the derivation 
\[
(\_, \sn, \emptyset), \plookup{\_}{\key} ; \trans_{\fp'} \toTRANS (\_, \sn, \{(\otR, \key, \val)\}) \trans_{\fp'}
\]
Also,because whenever $(\otR,\ ke', \val') \in \fp'$, 
then $\sn(\key') = \val'$,  we can apply the inductive hypothesis and infer that $(\_, \sn, \emptyset), \trans_{\fp'} \toTRANS^{\ast} (\stub, \stub, \fp'), \pskip$. 
\ac{To be pedantic the result below should be proved: it requires first a rule induction on 
transitions of the form $(\stk, \sn, \fp), \trans \toTRANS (\stk', \sn', \fp'), \trans'$, followed by an induction on the 
number of transitions in a judgement of the form $(\_, \sn, \fp), \trans^{\ast} \toTRANS (\_, \_, \fp'), \trans' $.}
An immediate consequence of this fact is that 
$(\_, \sn, \{(\otR,\key, \val)\}) \trans_{\fp'} \toTRANS^{\ast} (\stub \stub, \{(\otR,\ ke, \val)\} \uplus \fp'), \pskip$. 
That is, we have that 
\[
(\_, \sn, \emptyset), \plookup{\_}{\key} ; \trans_{\fp'} \toTRANS (\_, \_, \{(\otR, \key, \val)\}) \trans_{\fp'} \toTRANS^{\ast} (\_, \_, \fp'), \pskip.
\]

Finally, suppose that $\fp = \{(\otW, \key, \val)\} \uplus \fp'$, and 
for no  $\key', \val'$ $(\otR,\key', \val') \in \fp'$, and for no $\val'$ 
$(\otW, \key, \val') \in \fp'$. In this case we have that $\trans_{\fp} = 
\pmutate{\key}{\val} \uplus \fp'$. Let $\sn$ be an arbitrary snapshot. 
By applying Rule \rl{Tprimitive} we obtain that $(\_, \sn, \emptyset) \pmutate{\key}{\val} ; \trans_{\fp'} 
\toTRANS (\_, \sn\rmto{\key}{\val}, \{(\otW, \key, \val)\}), \trans_{\fp'}$. Because $\fp'$ does not contain 
any operation of the form $(\otR, \key', \val')$, the statement \emph{if $(\otR,\key',\val') \in \fp'$ then 
$\sn\rmto{\key}{\val}(\key') = \val'$} is trivially satisfied. By the inductive hypothesis, we have that 
$(\_, \sn\rmto{\key}{\val}, \emptyset), \trans_{\fp'} \toTRANS^{\ast} (\_, \_, \fp'), \pskip$, 
from which it is immediate to infer that 
\[
(\_, \sn\rmto{\key}{\val}, \{(\otW, \key, \val)\}), \trans_{\fp'} \toTRANS^{\ast} (\_, \_, \{(\otW, \key, \val)\} \uplus \fp'), \pskip. 
\]
Finally, we have that 
\[
(\_, \sn, \emptyset), \pmutate{\key}{\val} ; \trans_{\fp'} \toTRANS (\_, \_, \{(\otW, \key, \val)\}), \trans_{\fp'} \toTRANS^{\ast} (\_, \_, \fp), \pskip
\]
as we wanted to prove.
\end{proof}

We now have everything we need to prove \cref{prop:ettraces2sem}.
\paragraph{Proof of \cref{prop:ettraces2sem}.}
Let $\mkvs \in \CMs(\ET)$. By definition there exists a $\ET$-trace $\tau$ that 
terminates in a configuration of the form $(\mkvs, \_)$. By \cref{prop:et.normalform}, we 
can assume that $\tau$ is in normal form, hence the program $\prog_{\tau}$ is well-defined. 
In particular, let 
\[
\tau = (\mkvs_{0}, \vienv_{0}), \toET{(\cl_{0}, \varepsilon_{0})} (\mkvs_{0}', \vienv_{0}') \toET{(\cl_{0}, \fp_{0})} (\mkvs_{1}, \vienv_{1}) 
\toET{(\cl_{2}, \varepsilon_{2})} \cdots \toET{(\cl_{n-1}, \fp_{n-1})} (\mkvs_{n}, \vienv_{n}),
\]
where $\mkvs_{n} = \mkvs$. Then for any $i =0,\cdots, n-1$, we have that $\mkvs_{i} = \mkvs'_{i}$, 
and $\vienv'_{i} = \vienv_{i}\rmto{\cl_{i}}{\vi_{i}}$ for some $\vi_{i}. \vienv_{i}(\cl_{i}) \sqsubseteq \vi_{i}$.
Let $\mathsf{Cl}_{\tau} = \dom(\vienv_{0})$, and $\thdenv_{0} = \lambda \cl \in \mathsf{Cl}_{\tau}. \lambda x \in \Vars. \val_{0}$. 
For $i=0,\cdots, n$, let $\tau_{i}$ be the prefix of $\tau$ terminating in the configuration $(\mkvs_{i}, \vienv_{i})$.
We prove that, for any $i=0,\cdots, n-1$, 
then $(\mkvs_{0}, \vienv_{0}), \thdenv_{0}), \prog_{\tau_{i}} \toCMD{\stub}^{\ast}_{\ET} (\mkvs_{i}, \vienv_{i}, \thdenv_{i}), (\lambda \cl \in \mathsf{Cl}_{\tau}.\pskip)$, 
for some $\thdenv_{i}$. By definition $\mkvs = \mkvs_{n} \in \interpr{\prog_{\tau}}_{\ET}$. 
The proof of this claim is by induction on $n$.

\begin{itemize}
\item The base case where  $n = 0$, as $\tau_{0}$ consists of the initial configuration $(\mkvs_{0}, \_)$. 
By definition $\prog_{\tau_{0}}(\cl) = \lambda \cl \in \mathsf{Cl}_{\tau}.\pskip$, and there is nothing to prove.

\item Next let $i: 0 < i < n$, and suppose that the claim holds for $\tau_{i-1}$: specifically, there exists 
$\thdenv_{i}$ such that $(\mkvs_{0}, \vienv_{0}, \thdenv_{0}), \prog_{\tau_{i-1}} \toCMD{-}^{\ast}_{\ET} 
(\mkvs_{i}, \vienv_{i}, \thdenv_{i}), \lambda \cl \in \dom(\mathsf{Cl}_{\tau}).\pskip$. Note that 
$\prog_{\tau_{i}} = \prog_{\tau_{i-1}}\rmto{\cl_{i-1}}{\prog_{\tau_{i-1}}(\cl_{i-1}) ; \ptrans{\trans_{\fp_{i-1}}}}$, 
from which it follows that 
\[
(\mkvs_{0}, \vienv_{0}, \thdenv_{0}), \prog_{\tau_{i}} \toCMD{-}^{\ast}_{\ET} 
(\mkvs_{i}, \vienv_{i}, \thdenv_{i}), (\lambda \cl \in \dom(\mathsf{Cl}_{\tau}).\pskip)\rmto{\cl_{i-1}}{\ptrans{\trans_{\fp_{i-1}}}}.
\]
Next, we prove that $\cl_{i} \vdash (\mkvs_i, \vienv_{i}(\cl_{i}), \thdenv_{i}(\cl_{i}), \ptrans{\fp_{i}} 
\toCMD{(\cl_{i-1}, \_, \fp_{i-1})} (\mkvs_{i}, \vienv_{i}(\cl_{i-1}), \_), \pskip$, 
from which we can infer 
\[
(\mkvs_{i}, \vienv_{i}, \thdenv_{i}), (\lambda \cl \in \dom(\mathsf{Cl}_{\tau}).\pskip)\rmto{\cl_{i}}{\ptrans{\trans_{\fp_{i}}}} 
\toPROG{(\cl_{i-1}, \_, \fp_{i-1})} (\mkvs_{i+1}, \vienv_{i+1}, \_), \lambda \cl \in \dom(\mathsf{Cl}_{\tau}.\pskip),
\]
which is what we want to prove. 

To prove that $\cl_{i} \vdash (\mkvs_i, \vienv_{i}(\cl_{i}), \thdenv_{i}(\cl_{i}), \ptrans{\fp_{i}} 
\toCMD{(\cl_{i-1}, \_, \fp_{i-1})} (\mkvs_{i}, \vienv_{i}(\cl_{i-1}), \_), \pskip$, 
we consider the sequence of $\ET$-reductions $(\mkvs_{i-1}, \vienv_{i-1}) \toET{(\cl_{i-1}, \varepsilon} (\mkvs_{i-1}', \vienv_{i-1}') 
\toET{(\cl_{i-1}, \fp_{i-1})} (\mkvs_{i}, \fp_{i})$. The $\ET$-reduction ensures the following: 
\begin{itemize}
\item let $\vi_{i-1} = \vienv_{i-1}(\cl_{i-1})$. Then there exists $\vi_{i-1}'$ such that $\vi_{i-1} \sqsubseteq \vi_{i-1}'$ and
$\vienv_{i-1}'('cl_{i-1}) = \vienv_{i-1}\rmto{\cl_{i-1}}(\vi_{i-1}')$, 
\item $\mkvs_{i-1}' = \mkvs_{i-1}$.
\end{itemize}
The $\ET$-reduction $(\mkvs_{i-1}', \vienv_{i-1}') 
\toET{(\cl_{i-1}, \fp_{i-1})} (\mkvs_{i}, \fp_{i})$ ensures the following: 
\begin{itemize}
\item $\mkvs_i = \updateKV(\mkvs_{i-1}, \vi_{i-1}', \fp_{i-1}, \txid)$ for some $\txid \in \nextTxid(\cl_{i-1}, \mkvs_{i-1}$, 
\item $\ET \vdash (\mkvs_{i-1}, \vi_{i-1}') \triangleright \fp_{i-1} (\mkvs_{i}, \vi_{i}$, where $\vi_{i} = \vienv_{i}(\cl_{i-1})$; 
by the definition of execution test, this also ensures that 
\item whenever $(\otR, \key, \val) \in \fp_{i-1}$, then $\snapshot(\mkvs_{i-1}, \vi_{i-1}')(\key) = \val$.
\end{itemize}
The latter statement, together with \cref{lem:fp2trans}, leads to the following: let $\stk_{i-1} = \thdenv_{i-1}(\cl_{i-1}$, 
$\sn_{i-1} = \snapshot(\mkvs_{i-1}, \vi_{i-1}')$; then 
$(\stk_{i-1}, \sn_{i-1}, \emptyset), \trans_{\fp_{i-1}} \toTRANS^{\ast} (\_, \_, \fp_{i-1}) \pskip$. 
By putting all the statements together, we infer the transition 
\[\cl_{i} \vdash (\mkvs_i, \vienv_{i}(\cl_{i}), \thdenv_{i}(\cl_{i}), \ptrans{\fp_{i}} 
\toCMD{(\cl_{i-1}, \_, \fp_{i-1})} (\mkvs_{i}, \vienv_{i}(\cl_{i-1}), \_), \pskip,\]
which is exactly 
what we wanted to prove.
\end{itemize}
%
%\ac{Old Appendix starts here}
%
%\[
%\conf_0 \toET{(\cl_{0}, \alpha_{0})} \conf_{1} \toET{(\cl_{1}, \alpha_1)} \cdots \toET{(\cl_{n-1}, \alpha_{n-1})} \conf_{n},
%\] 
%where for any $i=0,\cdots, n$, $\conf_{i} = (\mkvs_{i}, \vienv_{i})$ for some $\mkvs_{i},\vienv_{i}$, 
%can be converted into a \emph{normal trace}, where a view shift from
%
%\ac{Context is missing. What's the purpose of this appendix? 
%Normal $\ET$-traces is not enough. There should be an introductory 
%paragraph. Try to point to the main text. E.g. \emph{In \cref{sec:?} we 
%stated that $\cdots$. Here we give a formal proof of the result.} 
%Then you give an high level outline of the proof. E.g. \emph{First, we prove 
%that $\ET$-traces can be converted into a normal form. Then we show how to convert 
%$\ET$-traces in normal form into a trace of a program $\prog$ in the operational semantics.}}
%
%\ac{I believe that the aim of this Section is that of proving Theorem 4.4. This proof is not in the appendix 
%as of now, but it follows immediately from the results that we already have. I will put the structure of the 
%proof at the end of this section.}
%
%For technical reasons, it will be convenient to adopt a reduction strategy for inferring kv-stores induced by an 
%execution test: such an execution strategy require that clients only commit transactions with non-empty fingerprints, 
%and a client updates its view only immediately before committing a transaction. 
%The next proposition states that all kv-stores induced by an execution test $\ET$ can be 
%obtained via a sequence of reductions that adhere to the reduction strategy outlined above. 
%Throughout this section, we assume that the execution test $\ET$ is fixed.
%
%\begin{definition}
%Let $\ET$ be an execution test. The $\ET$-trace
%\[
%\conf_0 \toET{\alpha_0} \conf_1 \toET{\alpha_1} \cdots \toET{\alpha_{2n}} \conf_{2n + 1}
%\]
%is in \emph{normal form} if \textbf{(i)} $\conf_0$ is initial, and 
%\textbf{(ii)} $\fora{ i : 0 \leq i \leq n}$ there exists a client $\cl_i$ and set of operations $\fp_{i}$ such that 
%$\alpha_{2 \cdot i} = (\cl_{i}, \varepsilon)$, and $\alpha_{2 \cdot i + 1}$ is defined and equal to $(\cl_{i}, \fp_{i})$ where \( \fp_i \neq \emptyset \).
%\end{definition}
%\ac{In the main text $\alpha$ ranges over $\{\varepsilon\} \cup \{\fp_{i}\}$, but here it ranges over pairs 
%of the form $\{(\cl, \varepsilon)\} \cup \{(\cl, \fp_{i})\}$, while $\mu$ ranges over $\{\varepsilon\} \cup \{\fp_{i}\}$. 
%Fix.}
%\ac{In the explicit sequence of reductions above, the last index on $\alpha$ is $2 \cdot n$, but the definition 
%mandates that the last index on $\alpha$ must have the form $2\ cdot i + 1$ for some $i$. Fix.
%}
%
%For any trace satisfying \( \CMs(\ET) \), 
%there exists a equivalent normal trace ends up with the same state (\cref{prop:et.normalform}).
%
%\ac{The proposition below uses several side results (see items (1) and (2) below, and the notion of 
%transitions in place. The best way to present the result clearly is to \textbf{(a)} state the main result 
%that you want to prove, i.e. \cref{prop:et.normalform}. \textbf{(b)} Give an intuition about how the 
%proof is performed (i.e. you transform the original $\ET$-reduction by merging view-shifts and pushing client commits to the left of view-shifts from 
%different clients, see lemmas \ref{lem:et.absorb} and \ref{lem:viewshift.rightmover}). 
%\textbf{(c)} Once you have introduced these two lemmas, give their proof straight away.
%\textbf{(d)} Having a high-level overview of what you are doing you can introduce  
%in-place and out of place reductions. At this point it should be clear that a reduction in-place is one that does 
%not need to be  moved around anymore, when constructing a normal $\ET$-trace. 
%\textbf{(e)} Give the proof of \cref{prop:et.normalform}} 
%\begin{proposition}[Normal \( \ET \) Traces]
%\label{prop:et.normalform}
%Let $\ET$ be an execution test, and suppose that $\mkvs \in \CMs(\ET)$. Then there exists a $\ET$-trace  
%\[
%(\mkvs_0, \vienv_0) \toET{\stub} \cdots \toET{\stub} (\mkvs_n, \vienv_{n})
%\]
%that is in normal form, and such that $\mkvs_{n} = \mkvs$.
%\end{proposition}
%\begin{proof}
%Let $\mkvs \in \CMs(\ET)$. By definition, there exists a sequence of reductions 
%\begin{equation}
%\label{eq:normalform.sequence}
%(\mkvs_{0}, \vienv_{0}) \toET{(\cl_0, \mu_0)} \cdots \toET{(\cl_{n-1}, \mu_{n-1})} (\mkvs_n, \vienv_{n})
%\end{equation}
%such that $\mkvs_{n} = \mkvs$. Given an index $i = 1,\cdots, n-1$, we say that the action $(\cl_{i}, \mu_{i})$ is \emph{in place} 
%if, $\mu_{i} = \fp_{i}$ for some $\fp_{i}$, $\cl_{i-1} = \cl_{i}$, $\mu_{i-1} = \varepsilon$, and if $(\cl_{j}, \mu_{j}) = (\cl_{i}, \varepsilon)$, 
%for some  $j = 0,\cdots, i-2$, then there exists $j': j < j' < i$ such that $(\cl_{j'}, \mu_{j'}) = (\cl_i, \fp_{j'})$. An action of the 
%form $(\cl_{i}, \mu_{i})$ is \emph{out of place} if it is not in place. 
%
%Given the sequence of reductions in \cref{eq:normalform.sequence}, we show the following: 
%\begin{enumerate}
%\item if the sequence has no action out of place, then there exists a sequence 
%\[
%(\mkvs'_{0}, \vienv'_{0}) \toET{(\cl'_{0}, \mu'_{0})} \cdots \toET{(\cl'_{m-1}, \mu'_{m-1})} (\mkvs'_{m}, \vienv'_{m})
%\]
%that is in normal form, and such that $\mkvs'_{m} = \mkvs_{n}$, and 
%\item if the sequence has $h$ actions out of place, for some $h > 0$, then there exists a sequence 
%\[
%(\mkvs'_{0}, \vienv'_{0}) \toET{(\cl'_{0}, \mu'_{0})} \cdots \toET{(\cl'_{m-1}, \mu'_{m-1})} (\mkvs'_{m}, \vienv'_{m})
%\]
%that has $h-1$ actions out of place, and such that $\mkvs'_{m} = \mkvs_{n}$.
%\end{enumerate}
%Combining the two facts above, we obtain that if $\mkvs \in \CMs(\ET)$, then there exists a sequence of reductions in formal form whose final 
%configuration is $(\mkvs, \_)$, as we wanted to prove.
%
%\begin{enumerate}
%\item 
%Suppose that the sequence of reductions from \cref{eq:normalform.sequence} has no action out of place. 
%Let $i=0,\cdots, n-1$, and consider the greatest index $i=0,\cdots, n-1$ such that  
%$\mu_{i} = \varepsilon$, and either $i = n-1$, or 
%$\fora{ \fp } (\cl_{i+1}, \mu_{i+1}) \neq (\cl_{i}, \fp)$. 
%If such an index does not exist, then the sequence of transitions from \cref{eq:normalform.sequence} is in 
%normal form, and there is nothing to prove. Otherwise, note that for any $j = i+1,\cdots, n-1$, 
%$\fora{ \fp } (\cl_{j}, \mu_{j}) \neq (\cl_{i}, \fp)$. 
%
%Suppose in fact that there existed 
%an index $j = i+1,\cdots, n-1$ such that $(\cl_{j}, \mu_{j}) = (\cl_{i}, \fp_{j})$ for some 
%$\fp_{j}$, and without loss of generality assume that $j$ is the smallest such index. This implies that 
%there exists no index $j': i < j' < j$ such that $(\cl_{j'}, \mu_{j'}) = (\cl_{i}, \fp_{j'})$ for some 
%$\fp_{j'}$. Also, it cannot be $j = i+1$, because we are assuming that $\fora{ \fp } (\cl_{i+1}, \mu_{i+1}) \neq 
%(\cl_{i}, \fp)$.  We have that $j \geq i+2$; we also have that  $(\cl_{j}, \mu_{j}) = (\cl_{i}, \fp_{j})$, 
%$(\cl_{i}, \mu_{i}) = (\cl_{i}, \varepsilon)$, $\fora{ j': i < j < j', \fp } (\cl_{j'}, \mu_{j'}) \neq (\cl_{i}, \fp)$. 
%By definition, the action $(\cl_{j}, \mu_{j})$ is out of place, contradicting the assumption that the sequence of 
%reduction of \cref{eq:normalform.sequence} has no actions out of place.
%
%We have proved that $\fora{ j : i+1 \leq j \leq n-1, \fp } (\cl_{j}, \mu_{j}) \neq (\cl_{i}, \fp)$. 
%Also, because we are assuming that $\mu_{i}$ is the greatest index such that $\mu_{i} = \varepsilon$, 
%and either $i= n-1$ or $\fora{ \fp } (\cl_{i+1},\mu_{i+1}) \neq (\cl_{i}, \fp)$, 
%then $\fora{ j : i+1 \leq j \leq n-1, \mu } (\cl_{j}, \mu_{j}) \neq (\cl_{i}, \mu)$. 
%Consider the transition 
%\[
%(\mkvs_{i}, \vienv_{i}) \toET{(\cl_{i}, \mu_{i})} (\mkvs_{i+1}, \vienv_{i+1}).
%\]
%Let $\vi = \vienv_{i}(\cl)$. Because $\mu_{i} = \varepsilon$, then it must be the case that 
%$\mkvs_{i} = \mkvs_{i+1}$, $\vienv_{i+1} = \vienv_{i}\rmto{\cl}{\vi'}$ for some $\vi' : \vi \sqsubseteq \vi'$. 
%For any $j \geq i$, we have that $\cl_{j} \neq \cl_{i}$. We can replace the transition 
%\[
%(\mkvs_{j}, \vienv_{j}) \toET{(\cl_{j}, \mu_{j})} (\mkvs_{j+1}, \vienv_{j+1})
%\]
%with 
%\[
%(\mkvs_{j}, \vienv_{j}\rmto{\cl_{i}}{\vi}) \toET{(\cl_{j}, \mu_{j})} (\mkvs_{j+1}, \vienv_{j+1}\rmto{\cl_{i}}{\vi}.
%\]
%It follows that the sequence of transitions 
%\[ 
%\begin{array}{@{}l@{}}
%(\mkvs_{0}, \vienv_{0}) \toET{(\cl_{0}, \mu_{0})} \cdots \toET{(\cl_{i-1},\mu_{i-1})} 
%(\mkvs_{i}, \vienv_{i}) = (\mkvs_{i+1}, \vienv_{i+1}\rmto{\cl_{i}}{\vi})  \\
%\quad \toET{(\cl_{i+1}, \mu_{i+1})} \cdots 
%\toET{(\cl_{n-1}, \mu_{n-1})} (\cl_{n}, \vienv_{n}\rmto{\cl_{i}, \vi})
%\end{array}
%\]
%Note that this sequence has one reduction less than the original sequence from \eqref{eq:normalform.sequence} (specifically, 
%the reduction $(\mkvs_{i}, \vienv_{i}) \toET{(\cl_{i}, \mu_{i})} (\mkvs_{i+1}, \vienv_{i+1})$ has 
%been removed). We can repeat this procedure until the resulting sequence of reductions has no index $i=0,\cdots, n-1$ such that  
%$\mu_{i} = \varepsilon$, and either $i = n-1$, or 
%$\fora{ \fp } (\cl_{i+1}, \mu_{i+1}) \neq (\cl_{i}, \fp)$. That is, the resulting sequence of reductions is in normal form, 
%and its final configuration is $(\mkvs_{n}, \_)$.
%
%\item Suppose that the sequence from \cref{eq:normalform.sequence} has $h$ actions out of place, 
%where $h > 0$. Let $i$ be the smallest index such that $(\cl_{i}, \mu_{i})$ is out of place. 
%This means that either $i = 0$, or $(\cl_{i-1}, \mu_{i-1}) \neq (\cl_{i}, \varepsilon)$, 
%or there exists an index $j < i -1 $ such that $(\cl_{j}, \mu_{j}) = (\cl_{i}, \varepsilon)$ 
%and, $\fora{ j': j < j' < i, \fp } (\cl_{j'}, \mu_{j'}) \neq (\cl_{i}, \fp)$. 
%Without loss of generality, we can assume that $i \neq 0$ and $(\cl_{i-1}, \mu_{i-} = (\cl_{i}, \varepsilon)$. 
%This is because we can always transform the sequence of reductions of \cref{eq:normalform.sequence} by 
%introducing a transition of the form $(\mkvs_{i}, \vienv_{i}) \toET{(\cl_{i}, \varepsilon)}
%(\mkvs_{i}, \vienv_{i})$, leading to the sequence of reductions
%\[
%\begin{array}{@{}l@{}}
%(\mkvs_{0}, \vienv_{0}) \toET{(\cl_{0}, \mu_{0})} \cdots \toET{(\cl_{i-1}, \mu_{i-1})}
%(\mkvs_{i}, \vienv_{i}) \\
%\quad \toET{(\cl_{i}, \varepsilon)} (\mkvs_{i}, \vienv_{i}) \toET{(\cl_{i+1}, \mu_{i+1})}
%\cdots \toET{(\cl_{n-1}, \mu_{n-1})} (\mkvs_{n}, \vienv_{n})
%\end{array}
%\]
%
%Therefore, it must be the case that there exists an index $j < i-1$ such that $(\cl_{j}, \mu_{j}) = (\cl_{i}, \varepsilon)$, 
%and $\fora{ j': j< j' < i, \fp } (\cl_{j'}, \mu_{j'}) \neq (\cl_{i}, \fp)$. Let then $j$ be the smallest such index. 
%Let $d = (i-1)-j$ be the number of reductions that separate the configuration $(\mkvs_{j}, \mu_{j})$ from 
%$(\mkvs_{i-1}, \mu_{i-1})$ in \cref{eq:normalform.sequence}. Note that it must be the case that $d > 0$. We show that we can 
%construct a sequence of reductions where the distance between these two configurations is reduced to $0$: 
%a consequence of this fact is such a sequence of reductions would have exactly $h-1$ actions out of place.
%Consider the following fragment in the sequence of reductions from \cref{eq:normalform.sequence}:
%\[
%(\mkvs_{j}, \vienv_{j}) \toET{(\cl_{j}, \mu_{j})} (\mkvs_{j+1}, \vienv_{j+1}) 
%\toET{(\cl_{j+1}, \mu_{j+1})} (\mkvs_{j+2}, \vienv_{j+2})
%\]
%We have two possible cases: 
%\begin{itemize}
%\item $\cl_{j+1} \neq \cl_{j}$. In this case we can apply \cref{lem:viewshift.rightmover} and infer the sequence of 
%reductions 
%\[
%(\mkvs_{j}, \vienv_{j}) \toET{(\cl_{j+1}, \mu_{j+1})} (\mkvs_{j+1}', \vienv_{j+1}') 
%\toET{(\cl_{j}, \mu_{j})} (\mkvs_{j+1}, \vienv_{j+1})
%\]
%which leads to the whole sequence of reductions 
%\[
%\begin{array}{@{}l@{}}
%(\mkvs_{0}, \vienv_{0}) \toET{(\cl_{0}, \mu_{0})} \cdots 
%\toET{(\cl_{j-1}, \mu_{j-1})} (\cl_{j}, \mu_{j}) 
%\toET{(\cl_{j+1}, \mu_{j+1})} (\mkvs'_{j+1}, \vienv'_{j+1})  \\
%\quad \toET{(\cl_{j}, \mu_{j})} (\mkvs_{j+1}, \vienv_{j+1})  
%\toET{(\cl_{j+2}, \mu_{j+2})} \cdots \toET{(\cl_{n-1}, \mu_{n-1})} \mkvs_{n}, \vienv_{n}
%\end{array}
%\]
%\item $\cl_{j+1} = \cl_{j}$. In this case we can apply \cref{lem:et.absorb} and infer the reduction 
%\[
%(\mkvs_{j}, \vienv_{j}) \toET{(\cl_{j}, \varepsilon)} (\mkvs_{j+2}, \vienv_{j+2})
%\]
%which leads to the sequence of reductions 
%\[
%\begin{array}{@{}l@{}}
%(\mkvs_{0}, \vienv_{0}) \toEDGE{(\cl_{0}, \mu_{0})}_{\ET} \cdots 
%\toET{(\cl_{j-1}, \mu_{j-1})}[\ET] (\mkvs_{j}, \vienv_{j}) \toET{(\cl_{j}, \varepsilon)}  \\
%\quad (\mkvs_{j+2}, \vienv_{j+2}) \toET{(\cl_{j+2}, \mu_{j+2})} \cdots 
%\toET{(\cl_{n-1}, \mu_{n-1})} (\mkvs_{n}, \vienv_{n})
%\end{array}
%\]
%\end{itemize}
%In both cases, in the resulting sequence of reductions the number of reductions that separate 
%the configuration $(\mkvs_{j}, \vienv_{j})$ from $(\mkvs_{i-1}, \vienv_{i-1})$ is strictly 
%less than $d$. We can repeating applying the procedure outlined above until there are 
%no reductions that separate the configuration $(\mkvs_{j}, \vienv_{j})$ from 
%$(\mkvs_{i}, \vienv_{i})$.
%\end{enumerate}
%\end{proof}
%\ac{This was more of a proof sketch, rather than a real proof. For the moment it will suffice, though 
%I will need to go back at it when all the other results are sorted.}
%
%
%\begin{lemma}[Absorption]
%\label{lem:et.absorb}
%If $\conf \toET{(\cl, \varepsilon)} \conf' \toET{(\cl, \varepsilon)} \conf''$, then 
%$\conf \toET{(\cl, \varepsilon)} \conf''$.
%\end{lemma}
%
%\begin{proof}
%Let $\conf = (\mkvs, \vienv)$, $\conf' = (\mkvs', \vienv')$, $\conf'' = (\mkvs', \vienv'')$. 
%By the reduction it must be the case that $\mkvs = \mkvs'$, and $\vienv' = \vienv\rmto{\cl}{\vi'}$ 
%for some $\vi' : \vi \sqsubseteq \vi'$. It must also be the case that $\mkvs' = \mkvs''$, and $\vienv'' = \vienv'\rmto{\cl}{\vi''}$ 
%for some $\vi'': \vi' \sqsubseteq \vi''$. Therefore we have that $\mkvs'' = \mkvs' = \mkvs$, and 
%$\vienv'' = \vienv'\rmto{\cl}{\vi''} = (\vienv\rmto{\cl}{\vi'})\rmto{\cl}{\vi''} = \vienv\rmto{\cl}{\vi''}$, 
%and $\vi \sqsubseteq \vi''$. 
%It follows that $\conf = (\mkvs, \vienv) \toET{(\cl, \varepsilon)} (\mkvs'', \vienv'') = \conf''$.
%\end{proof}
%
%\begin{lemma}[Independence of commit]
%\label{lem:viewshift.rightmover}
%Let $\conf \toET{(\cl, \varepsilon)} \conf_1 \toET{(\cl', \mu)} \conf'$ 
%for some $\conf, \conf_1, \conf''$ and $\cl, \cl'$ such that $\cl' \neq \cl$. 
%Then $\conf \toET{(\cl', \mu)} \conf_2 \toET{(\cl, \varepsilon)} \conf'$ 
%\end{lemma}
%
%\begin{proof}
%We only consider the case where $\mu = \fp$ for some fingerprint $\fp$. The case where 
%$\mu = \varepsilon$ is simpler to prove.
%Let $\conf = (\mkvs, \vienv)$, $\conf_1 = (\mkvs_1, \vienv_1)$, $\conf' = (\mkvs', \vienv')$. 
%Let also $\vi = \vienv(\cl)$.
%By the reduction rule we have that $\mkvs_1 = \mkvs, \vienv_1 = \vienv\rmto{\cl}{\vi_1}$ for 
%some $\vi_1: \vi_1 \sqsubseteq \vi_1$. Let $\vi' = \vienv(\cl')$: then we have that $\vienv_1(\cl') = 
%\vi'$. Because $(\mkvs_1, \vienv_1) \toET{(\cl', \fp)} (\mkvs', \vienv')$, we have that 
%$\ET \vdash (\mkvs_1, \vi') \csat \fp : (\mkvs',\vi'') $, where $\vi'' = \vienv'(\cl')$. Because $\mkvs_1 = \mkvs$, 
%that means that $\ET \vdash (\mkvs, \vi') \csat \fp: (\mkvs', \vi'')$, then it follows that 
%$(\mkvs, \vienv) \toET{(\cl', \fp)} (\mkvs', \vienv\rmto{\cl'}{\vi''}) 
%\toET{(\cl, \varepsilon)} (\mkvs', \vienv\rmto{\cl'}{\vi''}\rmto{\cl}{\vi_1}) = 
%(\mkvs', \vienv\rmto{\cl}{\vi_1}\rmto{\cl'}{\vi''}) = (\mkvs', \vienv_1\rmto{\cl'}{\vi''}) = 
%(\mkvs', \vienv')$, as we wanted to prove.
%\end{proof}


==> composition-et/updatekv-comm.tex <==
\subsection{Commutativity \( \updateKV \)}
\label{sec:updatekv-comm}

By \cref{cor:updatekv.singlecell}, then \cref{prop:updatekv.comm} holds, that is,
given two non-conflict commits, it is possible to swap the commit order as shown in \cref{prop:updatekv.comm}.


\begin{proposition}
\label{prop:updatekv.comm}
\label{prop:swap-update}
Let $\mkvs \in \MKVSs$, $\vi_1, \vi_2 \in \Views(\mkvs)$ and let $\cl_1, \cl_2 \in \Clients$ 
be such that $\cl_1 \neq \cl_2$. 
Let also $\fp_1, \fp_2 \in \pset{\Ops}$ be such that 
whenever $(\otW, \key, \stub) \in \fp_1$ for some key $\key$, then 
$(\otW, \key, \val) \notin \fp_2$ for all $\val \in \Val$. Then 
\begin{centermultline}
\Set{ \updateKV[\mkvs_1, \vi_2, \fp_2, \cl_2]}[\mkvs_1 \in \updateKV[\mkvs, \vi_1, \fp_1, \cl_1]] =  \\
\Set{ \updateKV[\mkvs_2, \vi_1, \fp_1, \cl_1]}[\mkvs_2 \in \updateKV[\mkvs, \vi_2, \fp_2, \cl_2]]
\end{centermultline}
\end{proposition}

\begin{proof}
Assume $\mkvs_1 = \updateKV[\mkvs, \vi_1, \fp_1, \txid_1]$, $\mkvs_2 = \updateKV[\mkvs, \vi_2, \fp_2, \txid_2]$. 
It suffices to show that for any key $\key$:
\[\lvert \updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key) \rvert = \lvert 
\updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key) \rvert
\]
and for any index $i$ such that \( 0 \leq i < \lvert \updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key) \rvert \):
\[
\updateKV[\mkvs_1, \vi_2,\fp_2, \txid_2](\key, i) = \updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key_1)
\]

First, fix a key $\key \in \Keys$. Note that if $(\otW, \key, \stub) \in \fp_1$, then 
by Corollary \ref{cor:updatekv.singlecell} we have that $\lvert \updateKV[\mkvs, \vi_1, \fp_1, \txid_1](\key) \rvert = 
\lvert \mkvs(\key) \rvert$. Because $\fp_1$ is not conflicting with $\fp_2$, it must be the case 
that $\fora{ \val } (\otW,\key,\val) \notin \fp_2$, and therefore by \cref{cor:updatekv.singlecell} 
we have that 
\[
\lvert \updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key) \rvert = \lvert \mkvs_1(\key) \rvert = \lvert \mkvs(\key) \rvert + 1.
\] 
Similarly, because $\fora{ \val } (\otW,\key,\val)\notin \fp_2$ 
and $(\otW,\key,\stub) \in \fp_1$, then 
\[
\lvert \updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key) \rvert = \lvert \mkvs_2(\key) \rvert + 1 
= \lvert \updateKV[\mkvs, \vi_2, \fp_2, \txid_2](\key) \rvert = \lvert \mkvs(\key) \rvert + 1
\]
Therefore, if $(\otW, \key, \stub) \in \fp_1$, we have that 
\[ 
\lvert \updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key) \rvert = 
\lvert \updateKV[\mkvs_1(\key), \vi_2, \fp_2, \txid_2](\key) \rvert
\]

Analogously, we can prove that this claim holds also when $(\otW, \key, \stub) \in \fp_2$. 
Finally, if $(\fora{ \val } (\otW,\key,\stub) \notin \fp_1) \land (\fora{ \val } (\otW,\key,\val) \notin \fp_2)$, 
then by \cref{cor:updatekv.singlecell} we have that 
\[
\lvert \updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key) \rvert = 
\lvert \mkvs_1(\key) \rvert = \lvert \updateKV[\mkvs, \vi_1, \fp_1, \txid_1](\key) \rvert = \lvert \mkvs(\key) \rvert
\]
and
\[
\lvert \updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key) \rvert = 
\lvert \mkvs_2(\key) \rvert = \lvert \updateKV[\mkvs, \vi_2, \fp_2, \txid_2](\key) \rvert = \lvert \mkvs(\key) \rvert
\]
This concludes the proof that, for any key $\key \in \Keys$,
\[ \lvert \updateKV[\mkvs_1,\vi_2,\fp_2,\txid_2] \rvert = 
\lvert \updateKV[\mkvs_2,\vi_1,\fp_1,\txid_1] \rvert
\]

Next, fix a key $\key$ and a index $i$ such that $0 \leq i < \abs{ \mkvs(\key) } - 1$. 
We show that:
\[ 
    \updateKV[\mkvs_1,\vi_2,\fp_2,\txid_2](\key, i) = \updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key, i)
\]
by performing a case analysis on $\vi_1$: 
\begin{enumerate}
    \item $i \neq \max_{<}(\vi_1(\key))$. 
In this case, by \cref{cor:updatekv.singlecell}\cref{item:updatekv.singlecell.noview}, 
we have that 
\begin{equation}
\mkvs_1(\key, i) = \updateKV[\mkvs, \vi_1, \fp_1, \txid_1](\key, i) = \mkvs(\key, i)
\label{eq:v1.nord.hh1}
\end{equation}
and 
\begin{equation}
\updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key, i) = \mkvs_2(\key, i)
\label{eq:v1.nord.uhh2}
\end{equation}
Then, we have three possible sub-cases: 
\begin{enumerate}
    \item $i \neq \max_{<}(\vi_2(\key))$: in this case, by \cref{cor:updatekv.singlecell}\cref{item:updatekv.singlecell.noview} we have that 
\[
\updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key, i) = 
\mkvs_1(\key, i) \stackrel{\cref{eq:v1.nord.hh1}}{=} \mkvs(\key, i)
\]
and
\[
\updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1] \stackrel{\cref{eq:v1.nord.uhh2}}{=} \mkvs_2(\key,i) = 
\updateKV[\mkvs, \vi_2, \fp_2, \txid_2](\key, i) = \mkvs(\key, i)
\]
\item $i = \max_{<}(\vi_2(\key))$, and $(\otR, \key, \stub) \notin \fp_2$. In this case the proof is analogous to the previous case, 
only \cref{cor:updatekv.singlecell}\cref{item:updatekv.singlecell.nord} needs to be applied in place 
of \cref{cor:updatekv.singlecell}\cref{item:updatekv.singlecell.noview}.
\item $i = \max_{<}(\vi_2(\key))$, and $(\otR, \key, \stub) \in \fp_2$. In this case we can apply \cref{cor:updatekv.singlecell}\cref{item:updatekv.singlecell.rd}, 
and deduce that 
\begin{equation}
\updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key, i) = \mkvs_1(\key, i) \oplus \Set{\txid_2}
\label{eq:v1.nord.v2.rd.uhh1}
\end{equation}
\begin{equation}
\mkvs_2(\key, i) = \updateKV[\mkvs, \vi_2, \fp_2, \txid_2](\key, i) = \mkvs(\key,i) \oplus \Set{\txid_2}
\label{eq:v1.nord.v2.rd.hh2}
\end{equation}
It follows that 
\[
\begin{array}{l}
\updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key, i) \stackrel{\cref{eq:v1.nord.v2.rd.uhh1}}{=} \mkvs_1(\key, i) \oplus \Set{\txid_2} \stackrel{\cref{eq:v1.nord.hh1}}{=} \mkvs(\key, i) \oplus \Set{\txid_2}\\
\updateKV[\mkvs_2,\vi_1,\fp_1, \txid_1](\key, i) \stackrel{\cref{eq:v1.nord.uhh2}}{=} \mkvs_2(\key, i) \stackrel{\cref{eq:v1.nord.v2.rd.hh2}}{=} \mkvs(\key, i) \oplus \Set{\txid_2}
\end{array}
\]
\end{enumerate}
\item $i = \max_{<}(\vi_1(\key))$, $(\otR, \key, \stub) \notin \fp_1$. This case is similar to the previous one: we can infer 
that Equations \cref{eq:v1.nord.hh1} and \cref{eq:v1.nord.uhh2} are valid in this case using \cref{cor:updatekv.singlecell}
\cref{item:updatekv.singlecell.nord}, then we can proceed by performing a case analysis on $\vi_2$ and $\fp_2$ as in the previous case.
\item $i = \max_{<}(\vi_1(\key))$, $\otR,\ ke, \stub) \in \fp_1$. We can apply \cref{cor:updatekv.singlecell}\cref{item:updatekv.singlecell.rd} 
to deduce the following: 
\begin{equation}
\mkvs_1(\key, i) = \updateKV[\mkvs, \vi_1, \fp_1, \txid_1](\key, i) = \mkvs(\key, i) \oplus \Set{\txid_1}
\label{eq:v1.rd.hh1}
\end{equation}
and
\begin{equation}
\updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key, i) = \mkvs_2(\key, i) \oplus \Set{\txid_1}
\label{eq:v1.rd.uhh2}
\end{equation}
We have two different sub-cases to consider: 
\begin{enumerate}
\item $i \neq \max_{<}(\vi_2(\key))$, or $i = \max_{<}(\vi_2(\key))$ with $(\otR,\key,\stub) \notin \fp_2$. In this case, we can apply either 
\cref{cor:updatekv.singlecell}\cref{item:updatekv.singlecell.noview} (if $i \neq \max_{<}(\vi_2(\key))$ ), or 
\cref{cor:updatekv.singlecell} \cref{item:updatekv.singlecell.nord} (if $i = \max_{<}(\vi_2(\key))$ and $(\otR, \key, \stub) \notin \fp_2$), 
to obtain 
\[
\updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key, i) = \mkvs_1(\key, i) \stackrel{\cref{eq:v1.rd.hh1}}{=} \mkvs(\key, i) \oplus \Set{\txid_1}
\]
and
\[
\updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key, i) \stackrel{\cref{eq:v1.rd.uhh2}}{=} \mkvs_2(\key, i) \oplus \Set{ \txid_1 } = 
\mkvs(\key, i) \oplus \Set{ \txid_1 }
\]
\item if $i = \max_{<}(\vi_2(\key))$ and $(\otR, \key, \stub) \in \fp_2$, then by \cref{cor:updatekv.singlecell}\cref{item:updatekv.singlecell.rd} 
we obtain that 
\begin{equation}
\mkvs_2(\key, i) = \updateKV[\mkvs, \vi_2, \fp_2, \txid_2](\key, i) = \mkvs(\key, i) \oplus \Set{\txid_2}
\label{eq:v1.rd.v2.rd.hh2}
\end{equation}
\begin{equation}
\updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key, i) = \mkvs_1(\key, i) \oplus \Set{ \txid_2}
\label{eq:v1.rd.v2.rd.uhh1}
\end{equation}
From these facts it follows that
\[
\begin{array}{l}
\updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key, i) \stackrel{\cref{eq:v1.rd.v2.rd.uhh1}}{=} 
\mkvs_1(\key, i) \oplus \Set{\txid_2} \stackrel{\cref{eq:v1.rd.hh1}}{=} 
(\mkvs(\key, i) \oplus \Set{\txid_1}) \oplus \Set{\txid_2 } = \mkvs(\key, i) \oplus \Set{\txid_1, \txid_2}\\
\updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key, i) \stackrel{\cref{eq:v1.rd.uhh2}}{=} 
\mkvs_2(\key, i) \oplus \Set{\txid_1} 
\stackrel{\cref{eq:v1.rd.v2.rd.hh2}}{=} (\mkvs(\key, i) \oplus \Set{\txid_2}) \oplus \Set{\txid_1} = \mkvs(\key, i) \oplus \Set{\txid_1, \txid_2}
\end{array}
\]
\end{enumerate}
\end{enumerate}

Next, note that if $\fora{ \val \in \Val } (\otW,\key,\val) \notin \fp_1 \land (\otW, \key, \val) \notin 
\fp_2$, then 
\[
\lvert \updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key) \rvert = \lvert \mkvs(\key) \rvert = 
\lvert \updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key) \rvert
\]
Because we have already proved that 
\[
    \fora{ i = 0,\cdots, \lvert \mkvs(\key) \rvert } \updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key, i) = \updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key, i)
\]
It follows that
\[ 
    \updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key) = \updateKV[\mkvs_2,\vi_1,\fp_1,\txid_1](\key)
\]
and there is nothing left to prove.

Suppose then that  either $(\otW, \key, \val) \in \fp_1$ or $(\otW,\key, \val) \in \fp_2$ 
for some $\val$. Without loss of generality, let $(\otW,\key,\val) \in \fp_1$ for some $\val \in \Val$; 
because we are assuming that $\fp_1$ does not conflict with $\fp_2$, then 
it must be the case that $\fora{ \val' \in \Val } (\otW,\key,\val') \notin \fp_2$. 
Using \cref{cor:updatekv.singlecell}\cref{item:updatekv.singlecell.nowr} and 
\cref{cor:updatekv.singlecell}\cref{item:updatekv.singlecell.wr}, 
\[
\begin{array}{l}
\updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2](\key, \lvert \mkvs(\key) \rvert) = 
\mkvs_1(\key, \lvert \mkvs(\key) \rvert) = \updateKV[\mkvs, \vi_1, \fp_1, \txid_1](\lvert \mkvs(\key) \rvert) = (\val, \txid_1, \emptyset)\\
{} \land \updateKV[\mkvs_2, \vi_1,\fp_1, \txid_1](\key, \lvert, \mkvs(\key) \rvert) = (\val, \txid_1, \emptyset)
\end{array}
\]
We have now proved that if $(\otW,\key,\val) \in \fp_1$, then $\lvert \updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2] \rvert = 
\lvert \updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1] \rvert$, and for all 
$i=0,\cdots, \lvert \updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2] \rvert - 1$, 
$\updateKV[\mkvs_1,\vi_2, \fp_2, \txid_2](\key, i) = \updateKV[\mkvs_2, \vi_1, \fp_1, \txid_1](\key, i)$. 
This concludes the proof that for any key \( \key \), $\updateKV[\mkvs_1,\vi_2,\fp_2,\txid_2](\key) = 
\updateKV[\mkvs_2,\vi_1,\fp_1,\txid_1](\key)$, and therefore 
$\updateKV[\mkvs_1, \vi_2, \fp_2, \txid_2] = \updateKV[\mkvs_2, \vi_1,\fp_1,\txid_1]$.
\end{proof}


==> composition-et/updatekv-well-defined.tex <==
\subsection{Well-defined \( \updateKV \)}
\label{sec:updatekv-well-defined}
The \cref{lem:updatekv.explicit} and then \cref{cor:updatekv.singlecell} shows that
swapping the operations of one key yields the same result.

\begin{lemma}[Swapping Operation]
\label{lem:updatekv.explicit}
Let $\mkvs$ be a kv-store, $\vi \in \Views(\mkvs)$, $\txid \in \TxID$ and $\fp \in \pset{\Ops}$. 
Let also $\key \in \Keys$. Then
\begin{enumerate}
    \item\label{item:updatekv.explicit.none} 
        $\fora{\val} (\otR, \key, \val) \notin \fp \land (\otW, \key, \val) \notin \fp \implies \updateKV[\mkvs, \vi, \fp, \txid](\key) = \mkvs(\key)$
\item\label{item:updatekv.explicit.rd} 
    $\fora{\val} (\otR, \key, \stub) \in \fp \land (\otW, \key, \val) \notin \fp 
    \implies 
    \begin{array}[t]{@{}l@{}}
    \updateKV[\mkvs, \vi, \fp, \txid](\key) = \\
    \qquad \text{let} \ (\val', \txid', \txidset') = \mkvs(\key, \max<(\vi(\key))) \\
    \qquad \text{in} \ \mkvs(\key)\rmto{\max<(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})}
    \end{array}
    $
\item\label{item:updatekv.explicit.wr} 
    $
    \begin{array}[t]{@{}l@{}}
    \fora{ \val, \val'}(\otR, \key, \val) \notin \fp \land (\otW, \key, \val) \in \fp 
    \implies \updateKV[\mkvs, \vi, \fp, \txid](\key) = \mkvs(\key) \lcat (\val, \txid, \emptyset)
    \end{array}
    $
\item\label{item:updatekv.explicit.rdwr}
    $
    \fora{\val} (\otR, \key, \stub) \in \fp \land (\otW, \key, \val) \in \fp 
    \implies 
    \begin{array}[t]{@{}l@{}}
    \updateKV[\mkvs,\vi,\fp,\txid](\key) =  \\
    \qquad \text{let} \ (\val', \txid', \txidset') = \mkvs(\key, \max(\vi(\key)))  \\
    \qquad \text{in} \ \mkvs(\key)\rmto{\max(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid}) } \lcat (\val, \txid, \emptyset)
    \end{array}
    $
\end{enumerate}
\end{lemma}

\begin{proof}
All the four statements are proved by induction on $\fp$, by keeping the variable $\mkvs$ universally quantified in the inductive hypothesis. 
Statement \cref{item:updatekv.explicit.rd} and \cref{item:updatekv.explicit.wr} requires 
proving \cref{item:updatekv.explicit.none} first, while Statement \cref{item:updatekv.explicit.rdwr} requires proving all the other statements. 
Fix then an arbitrary $\key \in \Keys$.
\begin{enumerate}
	\item 
	Suppose that for any $\val$, $(\otR, \key, \val) \notin \fp$ and $(\otW, \key, \val)) \notin \fp$. We prove that $\updateKV[\mkvs, \vi, \fp, \txid](\key) = 
	\mkvs(\key)$.
	\begin{itemize}
        \item \caseB{$\fp = \emptyset$} in this case we have that 
		\[
		\updateKV[\mkvs, \vi, \emptyset, \txid](\key) \stackrel{\cref{eq:updatekv}}{=} \mkvs(\key).
		\]
    \item  
        Suppose that $\fp = \fp' \uplus \Set{(\otR, \key', \val')}$ for some $\key', \val'$. Because we are assuming that 
		$(\otR, \key, \val) \notin \fp$ for any $\val \in \Val$, then it must be the case that 
		\begin{equation}
		\label{eq:updatekv.explicit.none.keneqkepRD}
		\key \neq \key'.
		\end{equation}
		Also, we have that $(\otR,\key, \val) \notin \fp'$ and $(\otW, \key, \val) \notin \fp$ for any $\val \in \Val$. 
		By inductive hypothesis we can assume 
		\begin{equation}
            \fora{ \mkvs' }\updateKV[\mkvs', \vi, \fp', \txid](\key) = \mkvs'(\key)
		\label{eq:updatekv.explicit.none.IHrd}
		\end{equation} 
		Therefore we have 
		\begin{align*}
        \updateKV[\mkvs, \vi, \fp, \txid](\key) 
            & =  
            \updateKV[\mkvs, \vi, \fp' \uplus \Set{(\otR, \key', \val')}, \txid](\key) \\
            & \stackrel{\cref{eq:updatekv}}{=}
            \begin{multlined}[t]
                \text{let} \ (\val', \txid', \txidset') = \mkvs(\key', \max_{<}(\vi(\key))) \\
                \text{in} \ \updateKV[\mkvs\rmto{\key'}{\mkvs(\key')\rmto{\max_{<}(\vi(\key'))}{\left(\val', \txid', \txidset' \cup \Set{\txid}\right)}}, \vi, \fp', \txid](\key) 
            \end{multlined} \\
            & \stackrel{\cref{eq:updatekv.explicit.none.IHrd}}{=}
            \begin{multlined}[t]
		    \text{let} \ (\val', \txid', \txidset') = \mkvs(\key', \max_{<}(\vi(\key'))) \\
            \text{in} \ \mkvs\rmto{\key'}{\mkvs(\key')\rmto{\max_{<}(\vi(\key'))}{\left(\val', \txid', \txidset' \Set{\txid}\right)}}(\key) 
            \end{multlined} \\
            &\stackrel{\cref{eq:updatekv.explicit.none.keneqkepRD}}{=} 
		    \text{let} \ (\val', \txid', \txidset') = \mkvs(\key', \max_{<}(\vi(\key'))) \text{ in } \mkvs(\key) \big) \\
            & = \mkvs(\key)
		\end{align*}

		\item Suppose that $\fp = \fp' \uplus \Set{(\otW, \key', \val')}$ for some $\val' \in \Val$. Then it must be the 
		case that 
		\begin{equation}
		\label{eq:updatekv.explicit.none.keneqkepWR}
		\key \neq \key'
		\end{equation}
		Also, we have that $(\otR,\key, \val) \notin \fp'$ and $(\otW, \key, \val) \notin \fp$ for any $\val \in \Val$. 
		By inductive hypothesis we can assume 
		\begin{equation}
            \fora{ \mkvs'}\updateKV[\mkvs', \vi, \fp', \txid](\key) = \mkvs'(\key)
		\label{eq:updatekv.explicit.none.IHwr}
		\end{equation}
		Therefore we have 
        \begin{align*}
            \updateKV[\mkvs, \key, \fp, \txid](\key)
            & =
            \updateKV[\mkvs, \key, \fp \uplus \Set{(\otW, \key', \val')}, \txid](\key) \\
            & \stackrel{\cref{eq:updatekv}}{=} 
            \updateKV[\mkvs\rmto{\key'}{\mkvs(\key')\lcat (\val', \txid, \emptyset)}, \vi, \fp, \txid ](\key)  \\
            &\stackrel{\cref{eq:updatekv.explicit.none.IHwr}}{=}
            \mkvs\rmto{\key'}{\mkvs(\key') \lcat (\val', \txid, \emptyset)}(\key) \\
            & \stackrel{\cref{eq:updatekv.explicit.none.keneqkepWR}}{=} \mkvs(\key)
		\end{align*}
	\end{itemize}

	\item Suppose $(\otR, \key, \stub) \in \fp$, and $(\otW, \key, \val) \notin \fp$ for all $\val \in \Val$. 
        Let $(\val, \txid', \txidset) = \mkvs(\key, \max_{<}(\vi(\key)))$. We prove that 
    \[
        \updateKV[\mkvs, \vi, \fp, \txid](\key) = \mkvs(\key)\rmto{\vi(\key)}{(\val, \txid', \txidset \cup \Set{\txid})}
    \]
		\begin{itemize}
        \item \caseB{$\fp = \emptyset$} this case is vacuous, as $(\otR, \key, \val) \notin \fp$ for all $\val \in \Val$, 
		against the assumption that $(\otR, \key, \stub) \in \fp$. 

		\item Suppose that $\fp = \fp' \cup \Set{(\otR, \key', \stub)}$ for some $\key'$. 
            We have two possible cases: 
			\begin{enumerate}
			\item $\key = \key'$, in which case we know that $(\otR, \key, \val') \notin \fp'$ for all $\val' \in \Val$ because of 
			the assumptions that we make on the structure of $\fp$. 
            By \cref{lem:updatekv.explicit}\cref{item:updatekv.explicit.none} we have that
			\begin{equation}
            \fora{ \mkvs' } \updateKV[\mkvs', \vi, \fp', \txid](\key) = \mkvs'(\key).
			\label{eq:updatekv.explicit.rd.applynone}
			\end{equation}
			In this case we have that 
            \begin{align*}
                \updateKV[\mkvs, \vi, \fp, \txid](\key) 
                & =
                \updateKV[\mkvs,\vi, \fp' \uplus \Set{(\otR, \key, \val')}, \txid](\key) \\
                & \stackrel{\cref{eq:updatekv}}{=} 
                \updateKV[\mkvs\rmto{\key}{\mkvs(\key)\rmto{\max_{<}(\vi(\key))}{(\val, \txid', \txidset \cup \Set{\txid})}}, \vi, \fp', \txid](\key) \\
                & \stackrel{\cref{eq:updatekv.explicit.rd.applynone}}{=}
                \mkvs\rmto{\key}{\mkvs(\key)\rmto{\max_{<}(\vi(\key))}{(\val, \txid', \txidset \cup \Set{\txid})}}(\key) \\
                & = \mkvs(\key)\rmto{\max(\vi(\key))}{(\val, \txid', \txidset \cup \Set{\txid})}
            \end{align*}
            \item \( \key \neq \key' \).
			In this case we know that because $(\otR, \key, \stub) \in \fp$, then 
            it must be $(\otR, \key, \stub) \in \fp'$. We also know that $\fora{ \val } (\otW, \key, \val) \notin \fp$. 
			By the inductive hypothesis, we have that 
			\begin{equation}
			\label{eq:updatekv.explicit.rd.IHrd}
            \begin{array}{l}
			\fora{ \mkvs' } \updateKV[\mkvs', \vi, \fp', \txid](\key) 
            = \mkvs'(\key)\rmto{\max_{<}(\vi(\key))}{(\val, \txid', \txidset \cup \Set{\txid})}
            \end{array}
			\end{equation}
			In this case we have 
			\begin{align*}
                \updateKV[\mkvs, \vi, \fp, \txid](\key) 
                & =
                \updateKV[\mkvs, \vi, \fp' \uplus \Set{(\otR, \key', \stub)}, \txid](\key) \\
                & \stackrel{\cref{eq:updatekv}}{=}
			    \updateKV[\mkvs\rmto{\key'}{\stub}, \vi, \fp, \txid](\key) \\
                & \stackrel{\cref{eq:updatekv.explicit.rd.IHrd}}{=} 
                \mkvs\rmto{\key'}{\stub}(\key)\rmto{\max_{<}(\vi(\key))}{(\val, \txid', \txidset' \cup \Set{\txid})} \\
                &\stackrel{\key \neq \key'}{=}
                \mkvs(\key)\rmto{\max_{<}(\vi(\key))}{(\val, \txid', \txidset' \cup \Set{\txid})}
			\end{align*}
		\end{enumerate}

		\item $\fp = \fp' \uplus \Set{(\otW, \key', \val')}$ for some $\val' \in \Val$. Because $(\otW, \key, \val) \notin \fp$ 
		for any $\val \in \Val$, it must be the case that 
		\begin{equation}
		\key \neq \key'
		\label{eq:updatekv.explicit.rd.keneqkepWR}
		\end{equation}
		Because $(\otR, \key, \stub) \in \fp$, it must also be the case that $(\otR, \key, \stub) \in \fp'$. By the inductive hypothesis, 
		we have that 
		\begin{equation}
		\label{eq:updatekv.explicit.rd.IHwr}
        \begin{array}{l}
        \fora{ \mkvs' }\updateKV[\mkvs', \vi, \fp', \txid](\key) 
        {} = \mkvs(\key)\rmto{\max_{<}(\vi(\key))}{(\val, \txid', \txidset \cup \Set{\txid})}
        \end{array}
		\end{equation}
		It follows that 
        \begin{align*}
		    \updateKV[\mkvs, \vi, \fp, \txid](\key) 
            & =
            \updateKV[\mkvs, \vi, \fp' \uplus \Set{(\otW, \key', \val')}, \txid](\key) \\
            & \stackrel{\cref{eq:updatekv}}{=}
		    \updateKV[\mkvs\rmto{\key'}{\stub}, \vi, \fp', \txid](\key) \\
            & \stackrel{\cref{eq:updatekv.explicit.rd.IHwr}}{=} 
            \mkvs(\rmto{\key'}{\stub}(\key)\rmto{\max_{<}(\vi(\key))}{(\val, \txid', \txidset \cup \Set{\txid})} \\
            & \stackrel{\cref{eq:updatekv.explicit.rd.keneqkepWR}}{=} 
            \mkvs(\key)\rmto{\max_{<}(\vi(\key))}{(\val, \txid', \txidset \cup \Set{\txid})}
        \end{align*}
	\end{itemize}
	
	\item Suppose that $(\otW, \key, \val) \in \fp$ for some $\val \in \Val$, and 
	$(\otR, \key, \val') \notin \fp$ for any $\val' \in \Val$. We prove that 
	$\updateKV[\mkvs, \vi, \fp, \txid](\key) = \mkvs(\key) \lcat (\val, \txid, \emptyset)$. 
		\begin{itemize}
        \item \caseB{$\fp = \emptyset$} This case is vacuous, as $(\otW, \key, \val) \in \fp$.
		\item Suppose that $\fp = \fp' \uplus \Set{(\otR, \key', \stub)}$ for some 
		$\key'$. Note that, because we are assuming that $\Set{(\otR, \key, \val')} \notin \fp$ 
		for all $\val' \in \Val$, then it must be the case that 
		\begin{equation}
		\key \neq \key'
		\label{eq:updatekv.explicit.wr.kenqkepRD}
		\end{equation}	
		We also have that $\Set{(\otR, \key, \val')} \notin \fp'$ for all $\val' \in \Val$, and 
		$(\otW, \key, \val) \in \fp'$. By the inductive hypothesis we have that 
		\begin{equation}
        \fora{\mkvs'} \updateKV[\mkvs', \vi, \fp', \txid](\key) = \mkvs'(\key) \lcat (\val, \txid, \emptyset)
		\label{eq:updatekv.explicit.wr.IHrd}
		\end{equation}
		Therefore, we have that 
        \begin{align*}
		    \updateKV[\mkvs, \vi, \fp, \txid]]\key) 
            & = 
            \updateKV[\mkvs, \vi, \fp' \uplus \Set{(\otR, \key', \stub)}, \txid](\key) \\
            & \stackrel{\cref{eq:updatekv}}{=}
		    \updateKV[\mkvs\rmto{\key'}{\stub}, \vi, \fp',\txid ](\key) \\
            & \stackrel{\cref{eq:updatekv.explicit.wr.IHrd}}{=} 
            \mkvs\rmto{\key'}{\stub}(\key) \lcat (\val, \txid, \emptyset) \\
            & \stackrel{\cref{eq:updatekv.explicit.wr.kenqkepRD}}{=} 
		    \mkvs(\key) \lcat (\val, \txid, \emptyset)
		\end{align*}
		
		\item Suppose that $\fp = \fp' \uplus \Set{(\otW, \key', \val')}$ 
		for some $\key'$. We distinguish two possible cases:
			\begin{enumerate}
			\item $\key = \key'$. In this case the structure of $\fp$ also imposes that $\val = \val'$, 
			and $(\otW, \key, \val'') \notin \fp'$ for any $\val'' \in \Val$. Furthermore, we have 
			that $(\otR, \key, \val'') \notin \fp'$ for any $\val'' \in \Val$. 
			By \cref{lem:updatekv.explicit}\cref{item:updatekv.explicit.none}, we have that 
			\begin{equation}
            \fora{\mkvs'} \updateKV[\mkvs', \vi, \fp', \txid](\key) = \mkvs(\key)
			\label{eq:updatekv.explicit.wr.applynone}
			\end{equation}
			from which it follows 
            \begin{align*}
			    \updateKV[\mkvs, \vi, \fp, \txid](\key) 
                & =
			    \updateKV[\mkvs, \vi, \fp' \uplus \Set{(\otW, \key', \val')}, \txid](\key) \\
                & = 
                \updateKV[\mkvs, \vi, \fp' \uplus \Set{(\otW, \key, \val)}, \txid](\key) \\
                & \stackrel{\cref{eq:updatekv}}{=} 
                \updateKV[\mkvs\rmto{\key}{\mkvs(\key) \lcat (\val, \txid, \emptyset)}, \vi, \fp', \txid](\key) \\
                & \stackrel{\cref{eq:updatekv.explicit.wr.applynone}}{=} 
                \mkvs\rmto{\key}{\mkvs(\key) \lcat (\val, \txid, \emptyset)}(\key) \\
                & = \mkvs(\key) \lcat (\val, \txid, \emptyset)
			\end{align*}
			
            \item \( \key \neq \key'\).
			In this case we have that, because $(\otW, \key, \val) \in \fp$, then it must 
			be $(\otW, \key, \val) \in \fp'$. Furthermore, we also have that $(\otR, \key, \val'') \notin \fp'$ 
			for any $\val'' \in \Val$. By the inductive hypothesis, we have that 
			\begin{equation}
            \fora{\mkvs'}\updateKV[\mkvs', \vi, \fp', \txid](\key) = \mkvs(\key) \lcat (\val, \txid, \emptyset)
			\label{eq:updatekv.explicit.wr.IHwr}
			\end{equation}
			from which it follows 
            \begin{align*}
			    \updateKV[\mkvs, \vi, \fp, \txid](\key) 
                & =
                \updateKV[\mkvs, \vi, \fp' \uplus \Set{(\otW,\key', \val')}, \txid](\key) \\
                & \stackrel{\cref{eq:updatekv}}{=}
			    \updateKV[\mkvs\rmto{\key'}{\stub}, \vi, \fp, \txid](\key) \\
                & \stackrel{\cref{eq:updatekv.explicit.wr.IHwr}}{=} 
                \mkvs\rmto{\key'}{\stub}(\key) \lcat (\val, \txid, \emptyset) \\
                & \stackrel{\key \neq \key'}{=} 
                \mkvs(\key) \lcat (\val, \txid, \emptyset)
			\end{align*}
			\end{enumerate}
		\end{itemize}
		
		\item Suppose that $(\otW, \key, \val) \in \fp$ for some $\val \in \Val$, and $(\otR, \key, \stub) \in \fp$. 
		Let $\mkvs(\key, \vi) = (\val', \txid', \txidset')$. We prove that 
        \[ 
            \updateKV[\mkvs, \vi, \fp, \txid](\key) = 
            \mkvs(\key)\rmto{\vi(\key)}{(\val', \txid', \txidset' \cup \Set{\txid})} \lcat (\val, \txid, \emptyset)
        \]
		by induction on $\fp$:
			\begin{itemize}
			\item $\fp = \emptyset$; this case is vacuous.
			\item $\fp = \fp' \uplus \Set{(\otR, \key', \stub)}$. We distinguish two cases, according to 
			whether $\key = \key'$ or $\key \neq \key'$. If $\key = \key'$, then we know that 
			$(\otW, \key, \val) \in \fp'$ and $(\otR, \key, \val'') \notin \fp$ for any $\val'' \in \Val$. 
			By Lemma \cref{lem:updatekv.explicit}\cref{item:updatekv.explicit.wr} we have that 
			\begin{equation}
            \fora{\mkvs'}\updateKV[\mkvs,\vi,\fp',\txid](\key) = \mkvs(\key) \lcat (\val, \txid, \emptyset)
			\label{eq:updateKV.explicit.rdwr.applyWR}
			\end{equation}
			from which it follows that 
			\begin{align*}
			    \updateKV[\mkvs, \vi, \fp, \txid](\key)
                & =
                \updateKV[\mkvs, \vi, \fp' \uplus \Set{(\otR, \key', \stub)}, \txid](\key) \\
                & = 
			    \updateKV[\mkvs, \vi, \fp' \uplus \Set{(\otR, \key, \stub)}, \txid](\key) \\
                & \stackrel{\cref{eq:updatekv}}{=}
                \updateKV[\mkvs\rmto{\key}{\mkvs(\key)\rmto{\max_{<}(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})}}, \vi, \fp', \txid](\key) \\
                & \stackrel{\cref{eq:updateKV.explicit.rdwr.applyWR}}{=} 
                \mkvs\rmto{\key}{\mkvs(\key)\rmto{\max_{<}(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})}}(\key) \lcat (\val, \txid, \emptyset) \\
                & = 
			    \mkvs(\key)\rmto{\max_{<}(\vi(\key))}{(\val' \txid', \txidset' \cup \Set{\txid}} \lcat (\val, \txid, \emptyset)
            \end{align*}
			If $\key \neq \key'$, then we have that both $(\otR, \key, \stub) \in \fp'$ and 
			$(\otW, \key, \val) \in \fp'$. In this case, by the inductive hypothesis we have that 
			\begin{equation}
			\label{eq:updatekv.explicit.rdwr.IHrd}
            \begin{array}{l}
            \fora{\mkvs'}\updateKV[\mkvs,\vi,\fp',\txid](\key) = 
            \mkvs'(\key)\rmto{\max_{<}(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})} \lcat (\val, \txid, \emptyset)
            \end{array}
			\end{equation}
			from which it follows that 
            \begin{align*}
			    \updateKV[\mkvs, \vi, \fp,\txid](\key)
                & = 
                \updateKV[\mkvs, \vi, \fp' \uplus \Set{(\otR, \key', \stub)}, \txid](\key) \\
                & \stackrel{\cref{eq:updatekv}}{=}
			    \updateKV[\mkvs\rmto{\key'}{\stub}, \vi, \fp', \txid](\key) \\
                & \stackrel{\cref{eq:updatekv.explicit.rdwr.IHrd}}{=} 
                \mkvs\rmto{\key'}{\stub}(\key)\rmto{\max_{<}(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})} \lcat (\val, \txid, \emptyset) \\
                & = 
                \mkvs(\key)\rmto{\max_{<}(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})} \lcat (\val, \txid, \emptyset)
            \end{align*}
			
			\item $\fp = \fp' \uplus \Set{(\otW, \key'', \val'')}$ for some $\key'', \val''$. Again, 
			there are two possible cases to consider. If $\key = \key''$, then $\val = \val''$ because of the structure imposed on $\fp$.
			Furthermore, we have that 
			$(\otR, \key, \stub) \in \fp'$ and $(\otW, \key, \val''') \notin \fp$ for all $\val''' \in \Val$.
			By \cref{lem:updatekv.explicit}\cref{item:updatekv.explicit.rd} we have that 
			\begin{equation}
			\label{eq:updatekv.explicit.rdwr.applyRD}
            \begin{array}{l}
            \fora{\mkvs'}\updateKV[\mkvs', \vi, \fp', \txid](\key) =
            \mkvs'(\key)\rmto{\max_{<}(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})} 
            \end{array}
			\end{equation}
			We have that 
            \begin{align*}
			    \updateKV[\mkvs,\vi,\txid, \fp](\key)
                & =
                \updateKV[\mkvs, \vi, \fp' \cup \Set{(\otW, \key'', \val'')}, \txid](\key) \\
                & =
			    \updateKV[\mkvs,\vi, \fp' \cup \Set{(\otW, \key, \val)}, \txid](\key) \\
                & \stackrel{\cref{eq:updatekv}}{=}
			    \updateKV[\mkvs\rmto{\key}{\mkvs(\key) \lcat (\val, \txid, \emptyset)}, \vi, \fp', \txid](\key) \\
                & \stackrel{\cref{eq:updatekv.explicit.rdwr.applyRD}}{=}
			    \mkvs\rmto{\key}{\mkvs(\key) \lcat (\val, \txid, \emptyset)}(\key)\rmto{\max_{<}(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})} \\
                & =
			    \left(\mkvs(\key) \lcat (\val, \txid, \emptyset)\right)\rmto{\max_{<}(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})} \\
                & = 
			    \mkvs(\key)\rmto{\max_{<}(\vi(\key))}{(\val',\txid', \txidset' \cup \Set{\txid})} \lcat (\val, \txid, \emptyset)
            \end{align*}
			Finally, if $\key \neq \key'$, then we have that $(\otR, \key, \stub) \in \fp'$ and $(\otW, \key, \val) \in \fp'$. 
			By the inductive hypothesis, we obtain 
			\begin{equation}
			\label{eq:updatekv.explicit.rdwr.IHwr}
            \begin{array}{l}
            \fora{\mkvs'}\updateKV[\mkvs', \vi, \fp', \txid](\key) = 
            \mkvs'(\key)\rmto{\max_{<}(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})} \lcat (\val, \txid, \emptyset)
            \end{array}
			\end{equation}
			It follows that 
            \begin{align*}
			    \updateKV[\mkvs, \vi, \fp, \txid](\key)
                & =
                \updateKV[\mkvs, \vi, \fp' \uplus \Set{(\otW, \key', \stub)}, \txid](\key) \\
                & \stackrel{\cref{eq:updatekv}}{=} 
			    \updateKV[\mkvs\rmto{\key'}{\stub}, \vi, \txid, \fp'](\key) \\
                & \stackrel{\cref{eq:updatekv.explicit.rdwr.IHwr}}{=}
                \mkvs\rmto{\key'}{\stub}(\key)\rmto{\max_{<}(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})} \lcat (\val, \txid, \emptyset) \\
                & =
                \mkvs\rmto{\max_{<}(\vi(\key))}{(\val', \txid', \txidset' \cup \Set{\txid})} \lcat (\val, \txid, \emptyset)
            \end{align*}
			\end{itemize}
\end{enumerate}
\end{proof}

In the following, given a version $\ver = (\val, \txid', \txidset)$ and a set of 
transaction identifiers $\txidset'$, we let $\ver \oplus \txidset' = (\val, \txid', \txidset \cup \txidset')$. 
Clearly the operator $\oplus$ is commutative over sets of transactions: 
$\fora{ \ver, \txidset, \txidset' } (\ver \oplus \txidset) \oplus \txidset' = (\ver \oplus \txidset') \oplus \txidset = 
\ver \oplus (\txidset \cup \txidset')$.

\begin{corollary}
\label{cor:updatekv.singlecell}
Let $\mkvs$ be a kv-store, $\vi \in \Views(\mkvs)$, $\txid \in \TxID$ and $\fp \in \pset{\Ops}$. 
Let also $\key \in \Keys$. Then 
\begin{enumerate}
\item\label{item:updatekv.singlecell.noview} 
    $ 
    \begin{array}[t]{l}
        \fora{ i } 0 \leq i < \abs{\mkvs(\key) } - 1 \land i \neq \max_{<}(\vi(\key)) 
        \implies \updateKV[\mkvs, \vi, \fp, \txid](\key, i) = \mkvs(\key, i)
    \end{array}
    $
\item\label{item:updatekv.singlecell.rd} $\fora{ \val } (\otR, \key, \stub) \in \fp \implies \updateKV[\mkvs,\vi, \fp,\txid](\key, \vi) = \mkvs(\key, \max_{<}(\vi(\key))) \oplus \Set{\txid}$
\item\label{item:updatekv.singlecell.nord} $\fora{ \val } (\otR,\key, \val) \notin \fp \implies \updateKV[\mkvs,\vi, \fp,\txid](\key,\vi) = \mkvs(\key, \max_{<}(\vi(\key)))$
\item\label{item:updatekv.singlecell.wr} 
    $\begin{array}[t]{@{}l@{}}
        \fora{\val} (\otW, \key, \val) \in \fp \\
        \quad {} \implies
        \lvert \updateKV[\mkvs,\vi,\fp,\txid](\key) \rvert = 
        \lvert \mkvs(\key) \rvert + 1 \wedge
        \updateKV[\mkvs,\vi,\fp,\txid](\key, \lvert \mkvs(\key) \rvert) = (\val, \txid, \emptyset)
    \end{array}$
\item\label{item:updatekv.singlecell.nowr} $\fora{ \val } (\otW, \key, \val) \notin \fp \implies \lvert \updateKV[\mkvs,\vi,\fp,\txid](\key) \rvert = \lvert \mkvs(\key) \rvert$
\end{enumerate}
\end{corollary}

\begin{proof}
A simple consequence of \cref{lem:updatekv.explicit}.
\end{proof}


==> cops/pseudocode <==
COPS-GT SYSTEM PSEUDO_CODE

// local time and ID are totally ordered separately
VersionNo :: LocalTime + ID

// replica has a unique identifier,
// a local store and local time
Replica :: ID -> (KV,LocalTime)

// each key in the local store has a list of tuples 
// consisting of value, version and the dependency.
KV :: Key -> List(Val,VersionNo,Dep)

// Dependency is a set of versions.
// Each individual write operation corresponds to a version.
Dep :: Set(Key,VersionNo)

// A queue for sending put_after message.
// Messages have key, value, version number, the dependency.
ReplQueue :: List(Key,Val,VersionNo,Deps)
Ctx :: {
    readers : List(Key,VersionNo,Dep)
    writers : List(Key,VersionNo,Dep)
}


//  ******* replica API ********** //

// write to a key local

// Deps set come from read operations and 
// vers set come write operations
// nearest set is nearest of deps.
// For local call, all the nearest should already exist,
// since those has been checked the moment reading them
VersionNo put_after(k,v,deps,nearest,vers){
    for (k,ver) in nearest
        wait until (_,ver,_) (*$\in$*) kv(k);

    time = inc(local_time);

    // appending local kv with a new version.
    list_isnert(kv[k], (v, (time ++ id), deps) );

    asyn_brordcase(k, v, (time ++ id), deps);
    return (local_time + id);
}

// receive a write message from other replica
on_receive(k,v,ver,deps) {
    // for a single machine
    // the following check immediately holds
    for (k',ver') in deps {
        wait until (_,ver',_) (*$\in$*) kv(k');
    }

    list_isnert(kv[k],(v,ver,deps));
    (remote_local_time + id) = ver;
    local_time = max(remote_local_time, local_time);
}

// Read by version number
(Val,Version,Dep) get_by_version(k,ver) {

    if (ver  = LATEST){
        ver := max(kv[k].vers);
    }

    wait until (_,ver,_) (*$\in$*) kv(k);
    
    let (val,ver,deps) from kv[k];
    return (val,ver,deps);
}

Dep ctx_to_dep(ctx) {
    return { (k,ver) | (k,ver,_) (*$\in$*) ctx.readers (*$\lor$*)
                (k,ver,_) (*$\in$*) ctx.writers }
}

Dep dep_to_nearest(deps) {
    return { (k,ver) | (*$\forall$*)k',ver',deps'.
            (k',ver',deps') (*$\in$*) deps (*$\implies$*) (k,ver) (*$\notin$*) deps' };
}

//  ******* client API ********** //

// write a key
Ctx put(k,v,ctx) {

    // add up all the read and write dependency
    deps = ctx_to_dep(ctx);

    ver = put_after(k,v, deps,dep_to_nearest(deps));

    ctx.writers += (k,ver,deps);

    return ctx;
}

// read
List(Val) get_trans(ks,ctx) {
    for k in ks {
        // only guarantee to read up-to-date value 
        // the moment reading the individual key
        rst[k] = get_by_version(k,LATEST);
    }

    for k in ks {
        ccv[k] = max (ccv[k],rst[k].ver);
        for dep in rst[k].deps
            if ( dep.key (*$\in$*) ks )
                ccv[k] = max (ccv[dep.key],dep.vers);
    }

    for k in ks 
        if ccv[k] > rst[k].vers
            rst[k] = get_by_version(k,ccv[k]);

    // update the ctx
    for (k,ver,deps) in rst
        ctx.readers += (k,ver,deps);

    return to_vals(rst);
}                                   


==> kv2aexec/et-top-equiv.tex <==
\subsection{\( \ET_{\top}\)}
The \( \ET_{\top} \) is the most permissive execution test.
\begin{align*}
    \ET_{\top} & \defeq \Set{(\mkvs,\vi,\cl,\fp)}[%
        \vi \in \Views(\mkvs) 
        \land \fora{\key,\val} (\otR,\key,\val) \in \fp 
        \implies 
        \val = \valueOf[\mkvs(\key,\max(\vi(\key)))]
    ]
\end{align*}

\begin{lemma}
    \CMs[\ET(\emptyset, \emptyset)] = \CMs[\ET_{\top}]
\end{lemma}
\begin{proof}
    It is easy to see \( \ET(\emptyset, \emptyset) \subseteq \ET_{\top}\) and then \( \CMs[\ET(\emptyset, \emptyset)] \subseteq \CMs[\ET_{\top}] \).
    Let consider \( \CMs[\ET_{\top}] \subseteq \CMs[\ET(\emptyset, \emptyset)] \).
    Assume \( \mkvs \in  \CMs[\ET_{\top}] \), which means there is a trace \( \tr \):
    \begin{centermultline}
        \tr = \conf_0 \toET{\alpha_0}[\ET_{\top}] \conf_1 \toET{\alpha_1}[\ET_{\top}] \dots \toET{\alpha_{n-1}}[\ET_{\top}] \conf_n
    \end{centermultline}
    By \cref{prop:et.normalform}, we can assume \( \tr \) is a normal trace.
    We prove that there exists a trace \( \tr' \) with the same length \( n \)
    \begin{centermultline}[equ:et-top-et-empty-sets]
        \tr' = \conf_0 \toET{\alpha_0}[\ET(\emptyset, \emptyset)] \conf'_1 \toET{\alpha_1}[\ET(\emptyset, \emptyset)] \dots \toET{\alpha_{n-1}}[\ET(\emptyset, \emptyset)] \conf'_n \\
        \land \fora{\cl} \conf'_n\projection{2}(\cl) = \vi_0
        \land \conf'_n\projection{1} = \conf_n\projection{1}
    \end{centermultline}
    We prove \cref{equ:et-top-et-empty-sets} by induction on the length \( n \).
    \begin{itemize}
        \item \( n = 0 \). In this case \( \tr = \conf_0 \) and we pick \( \tr'  = \conf_0 \).
        \item \( n + 1 \).
        Suppose \cref{equ:et-top-et-empty-sets} when the length is \( n \), let consider the \( n + 1 \).
        There are two possible cases for the trace \( \tr \): the last step ((n+1)-\emph{th} step) is a view shift or a fingerprint step.
        \begin{itemize}
            \item The last step of \( \tr \) is a view shift, \ie
            \begin{centermultline}
                \tr = \conf_0 \toET{\alpha_0}[\ET_{\top}] \conf_1 \toET{\stub}[\ET_{\top}] \dots \toET{\alpha_1}[\ET_{\top}] \conf_n \toET{\cl_n,\epsilon}[\ET_{\top}] \conf_{n + 1}
            \end{centermultline}
            By \ih there exists a trace \( \tr'' \) with \( n \) steps that satisfies \cref{equ:et-top-et-empty-sets}:
            \begin{centermultline}
                \tr'' = \conf_0 \toET{\alpha_0}[\ET(\emptyset, \emptyset)] \conf'_1 \toET{\alpha_1}[\ET(\emptyset, \emptyset)] \dots \toET{\alpha_{n-1}}[\ET(\emptyset, \emptyset)] \conf'_n \\
                \land \fora{\cl} \conf'_n\projection{2}(\cl) = \vi_0
                \land \conf'_n\projection{1} = \conf_n\projection{1}
            \end{centermultline}
            We can pick the trace \( \tr' = \tr'' \toET{\cl_n,\epsilon} \conf'_{n+1} \), which means appending a view shift step without changing the view of \( \cl_n \).
            Note that \( \fora{\cl} \conf'_{n}(\cl) = \vi_0 \) and then \( \fora{\cl} \conf'_{n+1}(\cl) = \vi_0 \).
            Also we know \( \conf_n\projection{1} = \conf_{n+1}\projection{1} = \conf'_n\projection{1} = \conf'_{n+1}\projection{1} \).
            Thus \( \tr' \) satisfies \cref{equ:et-top-et-empty-sets}.
            \item The last step of \( \tr \) is a fingerprint step, \ie
            \begin{centermultline}
                \tr = \conf_0 \toET{\alpha_0}[\ET_{\top}] \conf_1 \toET{\stub}[\ET_{\top}] \dots \toET{\alpha_1}[\ET_{\top}] \conf_n \toET{\cl_n,\fp_n}[\ET_{\top}] \conf_{n + 1}
            \end{centermultline}
            By \ih there exists a trace \( \tr'' \) with \( n \) steps that satisfies \cref{equ:et-top-et-empty-sets}:
            \begin{centermultline}
                \tr'' = \conf_0 \toET{\alpha_0}[\ET(\emptyset, \emptyset)] \conf'_1 \toET{\alpha_1}[\ET(\emptyset, \emptyset)] \dots \toET{\alpha_{n-1}}[\ET(\emptyset, \emptyset)] \conf'_n \\
                \land \fora{\cl} \conf'_n\projection{2}(\cl) = \vi_0
                \land \conf'_n\projection{1} = \conf_n\projection{1}
            \end{centermultline}
            Let \(\mkvs_n = \conf_n\projection{1} = \conf'_n\projection{1} \), and the views \( \vi_n = \conf_n\projection{2}(\cl_n) \) 
            and \[ \vi'_n = \getView[\mkvs,\lfpTx[\mkvs,\extRead[\mkvs_n,\fp_n,\vi_n], \emptyset] ] \]
            That is, \( (\mkvs_n,\vi'_n,\cl_n,\fp_n) \in \ET(\emptyset,\emptyset) \) and \( \updateKV[\mkvs_n,\vi_n,\fp_n,\cl_n] = \updateKV[\mkvs_n,\vi'_n,\fp_n,\cl_n] \).
            The new trace \( \tr''' \) can be constructed by appending a view shift for client \( \cl_n \) and the fingerprint step to \( \tr'' \):
            \begin{centermultline}
                \exsts{\conf'_{n+1}}
                \tr''' = \tr'' \toET{\cl_n,\epsilon}[\ET(\emptyset,\emptyset)] (\mkvs_n,\conf'_{n}\projection{2}\rmto{\cl_n}{\vi'_n}) 
                \toET{\cl_n,\fp_n}[\ET(\emptyset,\emptyset)] \conf'_{n+1} \\
                {} \land \fora{\cl} \conf'_{n+1}\projection{2}(\cl) = \vi_0
                \land \conf'_{n+1}\projection{1} = \conf_{n+1}\projection{1}
            \end{centermultline}
            Note that the last step of \( \tr'' \) is also a view shift.
            By \cref{lem:et.absorb}, 
            the new view shift in \( \tr''' \) can be absorbed with previous view shift which yields \( \tr' \) that has length \( n + 1 \) and satisfies \cref{equ:et-top-et-empty-sets}. \qedhere
        \end{itemize}
    \end{itemize}
\end{proof}


==> kv2aexec/galois-aexec-kv.tex <==
\subsection{Galois connection}
\label{sec:galois-kv-aexec}
Now we can prove \cref{thm:kvtrace2aexec}, which we rephrase in \cref{thm:kvtrace2aexec.app}.
The last statement in \cref{thm:kvtrace2aexec} implies that there is a \emph{Galois connection}
between the set of $\ET_{\top}$-traces, and the set of abstract executions that satisfy the 
last write wins policy. The lower and upper adjoints of this connection are the 
lifting of the functions $\aeset(\cdot)$ and $\KVtrace(\cdot)$ to sets of $\ET_{\top}$-traces 
and abstract executions, respectively. However, these two sets are not isomorphic: 
when converting a set of abstract executions into kv-traces, we abstract away the 
pairs $\txid \toEDGE{\VIS} \txid'$ in the visibility relation where $\txid$ is a read-only transaction.
When converting a $\ET_{\top}$-trace into a set of abstract executions, 
we (partially) lose the information about the views of clients immediately after it executed a transaction.

\begin{theorem}[Galois connection between kv-store trace and abstract execution]
\label{thm:kvtrace2aexec.app}
Given a $\ET_{\top}$-trace $\tr$, there exists a set of abstract executions $\aeset({\tr})$ 
such that $\lastConf(\tr) = (\mkvs, \_)$ for any $\mkvs \in \aeset(\tr)$.
Given an abstract execution $\aexec$ satisfying the last write wins resolution policy,
there exists a set of $\ET_{\top}$-traces $\KVtrace({\aexec})$ in normal form
such that $\lastConf(\tr) = (\mkvs_{\aexec}, \_)$ for any $\tr \in \KVtrace({\aexec})$.
\end{theorem}
\begin{proof}
    It can be derived from \cref{prop:kvtrace2aexec} and \cref{prop:aexec2kvtrace}.
\end{proof}

\begin{corollary} 
\label{cor:kvtrace2aexec}
$\CMs(\ET_{\top}) = \Set{\mkvs_{\aexec} }[ \aexec \text{ satisfies } \RP_{\LWW}]$.
\end{corollary}
\begin{proof}
    It follows by \cref{thm:kvtrace2aexec.app}.
\end{proof}



==> listofitems.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "listofitems"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\loiname                 {listofitems}                           %
\def\loiver                      {1.61}                              %
%                                                                    %
\def\loidate                  {2019/03/03}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% Author     : Christian Tellechea, Steven B. Segletes               %
% Status     : Maintained                                            %
% Maintainer : Christian Tellechea                                   %
% Email      : unbonpetit@netc.fr                                    %
%              steven.b.segletes.civ@mail.mil                        %
% Package URL: https://www.ctan.org/pkg/listofitems                  %
% Bug tracker: https://framagit.org/unbonpetit/listofitems/issues    %
% Repository : https://framagit.org/unbonpetit/listofitems/tree/master
% Copyright  : Christian Tellechea 2016-2019                         %
% Licence    : Released under the LaTeX Project Public License v1.3c %
%              or later, see http://www.latex-project.org/lppl.txt   %
% Files      : 1) listofitems.tex                                    %
%              2) listofitems.sty                                    %
%              3) listofitems-fr.tex                                 %
%              4) listofitems-fr.pdf                                 %
%              5) listofitems-en.tex                                 %
%              6) listofitems-en.pdf                                 %
%              7) README                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\ProvidesPackage\else
	\immediate\write -1 {%
	Package: \loidate\space v\loiver\space Grab items in lists using user-specified sep char (CT)}%
\fi

\expandafter\edef\csname loi_restorecatcode\endcsname{\catcode\number`\_=\number\catcode`\_\relax}
\catcode`\_11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% gestion des erreurs %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\PackageError
	\def\loi_error#1{\PackageError\loiname{#1}{Read the manual}}% pour LaTeX
\else
	\def\loi_error#1{\errmessage{Package \loiname\space Error: #1^^J}}% pour TeX
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% vérification de la présence de etex %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begingroup
\edef\__tempa{\meaning\eTeXversion}\edef\__tempb{\string\eTeXversion}%
\ifx\__tempa\__tempb
	\endgroup
\else
	\endgroup
	\loi_error{You are not using an eTeX engine, listofitems cannot work.}%
	\loi_restorecatcode\expandafter\endinput
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros auxiliaires %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chardef\loi_stop=0
\def\loi_quark{\loi_quark}
\long\def\loi_identity#1{#1}
\long\def\loi_gobarg#1{}
\long\def\loi_first#1#2{#1}
\long\def\loi_second#1#2{#2}
\long\def\loi_firsttonil#1#2\_nil{#1}
\long\def\loi_antefi#1#2\fi{#2\fi#1}
\long\def\loi_exparg#1#2{\expandafter\loi_exparg_a\expandafter{#2}{#1}}% \loi_exparg{<a>}{<b>} devient <a>{<*b>}
\long\def\loi_exparg_a#1#2{#2{#1}}
\long\def\loi_expafter#1#2{\expandafter\loi_expafter_a\expandafter{#2}{#1}}% \loi_expafter{<a>}{<b>} devient <a><*b>
\long\def\loi_expafter_a#1#2{#2#1}
\def\loi_macroname{\loi_ifinrange\escapechar[[0:255]]{\expandafter\loi_gobarg}{}\string}
\def\loi_argcsname#1#{\loi_argcsname_a{#1}}
\def\loi_argcsname_a#1#2{\loi_expafter{#1}{\csname#2\endcsname}}
\long\def\loi_addtomacro#1#2{\loi_exparg{\def#1}{#1#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macros de test %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\loi_ifnum#1{\ifnum#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifx#1{\ifx#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifempty#1{\loi_exparg\loi_ifx{\expandafter\relax\detokenize{#1}\relax}}
\def\loi_ifstar#1#2{\def\loi_ifstar_a{\loi_ifx{*\loi_nxttok}{\loi_first{#1}}{#2}}\futurelet\loi_nxttok\loi_ifstar_a}
\long\def\loi_ifstuffexpandable#1{\def\loi_tempa{#1}\loi_exparg{\def\loi_tempb}{#1}\expandafter\unless\loi_ifx{\loi_tempa\loi_tempb}}
\long\def\loi_ifcsexpandable#1{% #1 est-il constitué d'une sc _développable_ ?
	\loi_ifempty{#1}
		{\loi_second
		}
		{\loi_ifspacefirst{#1}
			{\loi_second% si espace en 1er, faux
			}
			{%
			\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\begingroup\escapechar`\_\def\_{#1}\expandafter\endgroup
					\csname loi_\if\expandafter\expandafter\expandafter\loi_firsttonil\expandafter\string\_\_nil\string _first\else second\fi\endcsname
						{\loi_ifstuffexpandable{#1}}
						{\loi_second}%
				}
				{\loi_second% si plusieurs tokens, faux
				}%
			}%
		}%
}
\def\loi_ifinrange#1[[#2:#3]]{\loi_ifnum{\numexpr(#1-#2)*(#1-#3)>0 }\loi_second\loi_first}
\def\loi_ifstring#1\in#2{% si la chaine #1 est contenue dans #2
	\def\loi_ifstring_a##1#1##2\_nil{\loi_ifempty{##2}\loi_second\loi_first}%
	\loi_ifstring_a#2#1\@nil% appel de la macro auxiliaire
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros \loi_foreach %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_cnt_foreach_nest \loi_cnt_foreach_nest=0
\def\end_foreach{\end_foreach}
\def\loi_def_foreachsep#1{%
	\long\def\loi_foreach##1\in##2##3{%
		\global\advance\loi_cnt_foreach_nest1
		\loi_argcsname\def{loop_code_\number\loi_cnt_foreach_nest}{##3}%
		\loi_foreach_a##1##2#1\end_foreach#1%
		\loi_argcsname\let{loop_code_\number\loi_cnt_foreach_nest}\empty
		\global\advance\loi_cnt_foreach_nest-1
	}%
	\long\def\loi_foreach_a##1##2#1{%
		\def##1{##2}%
		\loi_ifx{\end_foreach##1}
			{}
			{\csname loop_code_\number\loi_cnt_foreach_nest\endcsname% exécute le code
			\loi_foreach_a##1%
			}%
	}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% macros gérant l'appariement %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\defpair#1{%
	\let\loi_listofpair\empty
	\loi_ifempty{#1}
		{}
		{\defpair_a{}#1\loi_quark\loi_quark}%
}
\long\def\defpair_a#1#2#3{%
	\loi_ifx{\loi_quark#2}
		{\def\loi_sanitizelist##1,\_nil{\def\loi_listofpair{##1}}%
		\loi_sanitizelist#1\_nil
		}
		{\loi_if_validpair#2#3%
			{\long\def\loi_paired_a{#2}\long\def\loi_paired_b{#3}%
			\loi_ifx{\loi_paired_a\loi_paired_b}
				{\loi_error{Paired tokens must not be equal, the pair \detokenize{#2#3} is ignored}%
				\defpair_a{#1}%
				}
				{\defpair_a{#1#2#3,}%
				}%
			}
			{\loi_error{Invalid paired tokens, the pair "\detokenize{#2}" and "\detokenize{#3}" is ignored}%
			\defpair_a{#1}%
			}%
		}%
}
\long\def\loi_if_validpair#1#2{%
	\def\loi_validpair{1}%
	\loi_if_invalid_pairtoken{#1}{\def\loi_validpair{0}}%
	\loi_if_invalid_pairtoken{#2}{\def\loi_validpair{0}}%
	\loi_ifnum{\loi_validpair=1 }
}
\long\def\loi_if_invalid_pairtoken#1{%
	\loi_ifempty{#1}
		{\loi_identity
		}
		{\loi_ifspacefirst{#1}
			{\loi_identity
			}
			{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\ifcat\relax\noexpand#1\expandafter\loi_identity\else\expandafter\loi_gobarg\fi}
				{\loi_identity}% si plusieurs tokens, faux
			}%
		}%
}
\long\def\loi_count_occur#1\in#2:#3{% compte le nombre d'occurrences de #1 dans #2 et met le résultat dans la macro #3
	\long\def\loi_count_occur_a##1##2#1##3\_nil{%
		\loi_ifempty{##3}
			{\def#3{##1}}
			{\expandafter\loi_count_occur_a\number\numexpr##1+1\relax##3\_nil}%
	}%
	\loi_count_occur_a0#2#1\_nil
}
\long\def\loi_check_pair#1#2\in#3{% teste l'appariement de #1 et #2 dans #3
	\loi_ifempty{#3}
		{\loi_second
		}
		{\loi_count_occur#1\in#3:\loi_tempa
		\loi_count_occur#2\in#3:\loi_tempb
		\loi_ifnum{\loi_tempa=\loi_tempb\relax}%
		}%
}
\long\def\loi_grabpaired_expr#1#2#3#4#5{% #1=liste de paires  #2=expression  #3=séparateur   #4=résultat    #5=ce qui reste
	\let#4\empty
	\def\loi_remain{#2#3}%
	\loi_foreach\loi_pair\in{#1}{\expandafter\loi_grabpaired_expr_a\loi_pair{#3}#4}%
	\def\loi_remove_lastsep##1#3\_nil{\def#4{##1}}%
	\expandafter\loi_remove_lastsep#4\_nil
	\expandafter\long\expandafter\def\expandafter\loi_grab_remain#4##1\_nil{\loi_ifempty{##1}{\let#5\empty}{\loi_exparg{\def#5}{\loi_gobarg##1}}}%
	\loi_grab_remain#2\_nil
}
\long\def\loi_grabpaired_expr_a#1#2#3#4{% #1#2=paire en cours  #3=séparateur   #4=résultat
	\loi_exparg{\loi_check_pair#1#2\in}#4% si les paires sont appariées dans le résultat
		{}% passer à la paire suivante
		{\long\def\loi_grabpaired_expr_b##1#3##2\_nil{%
			\loi_addtomacro#4{##1#3}% ajouter au résultat ce qui est jusqu'au prochain séparateur
			\def\loi_remain{##2}%
			\loi_exparg{\loi_check_pair#1#2\in}{#4}
				{}
				{\loi_ifempty{##2}
					{\loi_error{"\detokenize{#1}" and "\detokenize{#2}" are not paired}}
					{\loi_grabpaired_expr_b##2\_nil}%
				}%
			}%
		\expandafter\loi_grabpaired_expr_b\loi_remain\_nil
		}%
}
\def\insidepair#1#2#3#4{% #1#2=paire  #3=expr  #4=macro reçevant le resultat
	\loi_if_validpair#1#2%
		{\loi_ifcsexpandable{#3}
			{\loi_exparg{\insidepair#1#2}{#3}#4%
			}
			{\loi_check_pair#1#2\in{#3}% si les paires sont appariées dans le résultat
				{\def\insidepair_a##1#1##2\_nil{\insidepair_b##2\_nil{#1}}%
				\def\insidepair_b##1#2##2\_nil##3{%
					\loi_check_pair#1#2\in{##3##1#2}
						{\loi_exparg{\def#4}{\loi_gobarg##3##1}}%
						{\insidepair_b##2\_nil{##3##1#2}}%
					}%
				\insidepair_a#3\_nil
				}
				{\loi_error{"\detokenize{#1}" and "\detokenize{#2}" are not paired in "#3"}%
				}%
			}%
		}
		{\loi_error{Invalid paired tokens "\detokenize{#1}" and "\detokenize{#2}", empty \string#4 returned}% et bim
		\let#4\empty% voilà, bien fait pour vos gueules
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \loi_fornum %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_fornum#1=#2to#3\do{%
	\edef#1{\number\numexpr#2}\edef\loi_sgncmp{\ifnum#1<\numexpr#3\relax>+\else<-\fi}%
	\expandafter\loi_fornum_a\csname loi_fornum_\string#1\expandafter\endcsname\expandafter{\number\numexpr#3\expandafter}\loi_sgncmp#1%
}
\long\def\loi_fornum_a#1#2#3#4#5#6{\def#1{\unless\ifnum#5#3#2\relax\loi_antefi{#6\edef#5{\number\numexpr#5#41\relax}#1}\fi}#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% macro retirant les espaces extrêmes %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\loi_ifspacefirst#1{\expandafter\loi_ifspacefirst_a\detokenize{#10} \_nil}
\long\def\loi_ifspacefirst_a#1 #2\_nil{\loi_ifempty{#1}}
\expandafter\def\expandafter\loi_gobspace\space{}
\def\loi_removefirstspaces{\romannumeral\loi_removefirstspaces_a}
\long\def\loi_removefirstspaces_a#1{\loi_ifspacefirst{#1}{\expandafter\loi_removefirstspaces_a\expandafter{\loi_gobspace#1}}{\loi_stop#1}}
\edef\loi_restorezerocatcode{\catcode0=\number\catcode0 \relax}
\catcode0 12
\long\def\loi_removelastspaces#1{\romannumeral\loi_removelastspaces_a#1^^00 ^^00\_nil}
\long\def\loi_removelastspaces_a#1 ^^00{\loi_removelastspaces_b#1^^00}
\long\def\loi_removelastspaces_b#1^^00#2\_nil{\loi_ifspacefirst{#2}{\loi_removelastspaces_a#1^^00 ^^00\_nil}{\loi_stop#1}}
\loi_restorezerocatcode
\long\def\loi_removeextremespaces#1{% #1=texte où les espaces extrêmes sont retirés
	\romannumeral\expandafter\expandafter\expandafter\loi_removelastspaces\expandafter\expandafter\expandafter
	{\expandafter\expandafter\expandafter\loi_stop\loi_removefirstspaces{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro publique \setsepchar %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\setsepchar{\futurelet\loi_nxttok\setsepchar_a}
\def\setsepchar_a{\loi_ifx{[\loi_nxttok}\setsepchar_b{\setsepchar_b[/]}}
\long\def\setsepchar_b[#1]#2{% #1=sepcar de <liste des sepcar>  #2=<liste des sepcar>
	\loi_ifempty{#1}
		{\loi_error{Empty separator not allowed, separator "/" used}%
		\setsepchar_b[/]{#2}%
		}
		{\def\loi_currentsep{#1}%
		\_removeextremespacesfalse
		\loi_nestcnt1 % réinitaliser niveau initial à 1
		\def\nestdepth{1}%
		\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
		\def\loi_listname{loi_listofsep}%
		\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
		\let\loi_listofpair_saved\loi_list_ofpair
		\let\loi_list_ofpair\empty
		\loi_ifempty{#2}
			{\loi_error{Empty list of separators not allowed, "," used}%
			\readlist_e1{,}%
			}
			{\readlist_e1{#2}%
			}%
		\loi_argcsname\let\nestdepth{loi_listofseplen[0]}%
		\loi_argcsname\let\loi_currentsep{loi_listofsep[1]}% 1er car de séparation
		\let\loi_listofpair\loi_listofpair_saved
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro normalisant l'index %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_normalizeindex#1#2#3{% #1=macroname  #2=liste d'index  #3=profondeur max --> renvoie {err}{indx norm}
	\loi_ifempty{#2}
		{\loi_stop{}{}}
		{\loi_normalizeindex_a1{}{#3}{#1}#2,\loi_quark,}%
}%
\def\loi_normalizeindex_a#1#2#3#4#5,{% #1=compteur de profondeur #2=index précédents  #3=profondeur max #4=macroname  #5=index courant
	\loi_ifx{\loi_quark#5}
		{\loi_normalizeindex_c#2\loi_quark% supprimer la dernière virgule
		}
		{\loi_ifnum{#1>#3 }
			{\loi_invalidindex{Too deeply nested index, index [.] retained}{#2}% si profondeur trop grande
			}
			{\loi_ifinrange\ifnum\numexpr#5<0 -1*\fi(#5)[[1:\csname #4len[#20]\endcsname]]% si abs(#5) hors de [1,len]
				{\loi_exparg\loi_normalizeindex_b{\number\numexpr#5\ifnum\numexpr#5<0 +\csname #4len[#20]\endcsname+1\fi}{#1}{#2}{#3}{#4}}
				{\loi_invalidindex{#5 is an invalid index, index [.] retained}{#2}}%
			}%
		}%
}
\def\loi_normalizeindex_b#1#2#3{\loi_exparg\loi_normalizeindex_a{\number\numexpr#2+1}{#3#1,}}% #1=index à rajouter  #2=compteur de profondeur #3=index précédents
\def\loi_normalizeindex_c#1,\loi_quark{\loi_stop{}{#1}}
\def\loi_invalidindex#1#2{\loi_ifempty{#2}{\loi_invalidindex_a{#1},}\loi_invalidindex_a{#1}{#2}}
\def\loi_invalidindex_a#1#2{\loi_invalidindex_b#1\loi_quark#2\loi_quark}
\def\loi_invalidindex_b#1[.]#2\loi_quark#3,\loi_quark#4\loi_quark,{\loi_stop{#1[#3]#2}{#3}}% #4= index ignorés

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro publique \readlist %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_nestcnt
\def\greadlist{\let\loi_def\gdef\let\loi_edef\xdef\def\loi_let{\global\let}\readlist_a}%
\def\readlist{\let\loi_def\def\let\loi_edef\edef\let\loi_let\let\readlist_a}
\def\readlist_a{%
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_b}{\_removeextremespacesfalse\readlist_b}%
}
\long\def\readlist_b#1#2{% #1=macro stockant les éléments  #2=liste des éléments
	\loi_ifcsexpandable{#2}
		{\loi_exparg{\readlist_b#1}{#2}%
		}
		{\loi_edef\loi_listname{\loi_macroname#1}%
		\loi_argcsname\loi_let{\loi_listname nest}\nestdepth
		\loi_argcsname\loi_def{\loi_listname[]}{#2}% la liste entière
		\loi_argcsname\loi_def{\loi_listname sep[]}{}% séparateur vide
		\loi_ifempty{#2}
			{\loi_def#1[##1]{}%
			\loi_argcsname\loi_def{\loi_listname len}{0}\loi_argcsname\loi_def{\loi_listname len[0]}{0}%
			\loi_error{Empty list ignored, nothing to do}%
			}
			{\loi_edef#1[##1]{\unexpanded{\romannumeral\expandafter\loi_checkindex\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname}}%
			\loi_argcsname\loi_edef{\loi_listname sep}[##1]{\unexpanded{\romannumeral\expandafter\loi_checkindex\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname sep}}%
			\readlist_c{#2}%
			\loi_argcsname\loi_argcsname\loi_let{\loi_listname len}{\loi_listname len[0]}% longueur du niveau 0
			}%
		}%
}
\def\loi_checkindex#1#2#3{%
	\expandafter\expandafter\expandafter\loi_stop\csname#3[#2]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}
\def\readlist_c{%
	\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
	\expandafter\readlist_d\loi_currentsep||\_nil
}
\long\def\readlist_d#1||#2\_nil#3{\readlist_e1{#3#1}}% #1=<sep courant simple>  #3=liste -> rajoute un élément vide pour le test \ifempty ci dessous
\long\def\readlist_e#1#2{% #1=compteur d'index  #2=liste d'éléments à examiner terminée par <sep courant simple> >>RIEN laissé après
	\loi_ifempty{#2}
		{\loi_argcsname\loi_edef{\loi_listname len[\csname loi_previndex[\number\loi_nestcnt]\endcsname0]}{\number\numexpr#1-1\relax}%
		\loi_argcsname\loi_let{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname\number\numexpr#1-1\relax]}\empty% le dernier <sep> est <vide> ##NEW v1.52
		\advance\loi_nestcnt-1
		\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
		}
		{\loi_expafter{\readlist_f{#2}{}}\loi_currentsep||\loi_quark||#2\_nil{#1}% aller isoler le 1er item
		}%
}
\long\def\readlist_f#1#2#3||{% #1=liste restante   #2=<dernier sep utilisé>  #3=<sep courant>
	\loi_ifx{\loi_quark#3}% on a épuisé tous les <séparateurs> ? RESTE à lire <expr+sep1>\_nil{<compteur>}
		{\loi_ifempty{#2}% si #2 vide, aucun <sep utilisé> n'a été trouvé, il reste à lire "<liste complète>\_nil"
			{\long\def\readlist_g##1\_nil##2{\loi_exparg{\readlist_h{##2}{}}{\loi_gobarg##1}{#2}}% ##2=compteur d'index
			}
			{\loi_ifx{\loi_listofpair\empty}% paires définies ?
				{\long\def\readlist_g##1#2##2\_nil##3{\loi_exparg{\readlist_h{##3}{##2}}{\loi_gobarg##1}{#2}}%
				}
				{\long\def\readlist_g##1\_nil##2{%
					\loi_exparg{\loi_exparg\loi_grabpaired_expr\loi_listofpair}{\loi_gobarg##1}{#2}\loi_grabpaired_result\loi_grabpaired_remain
					\loi_exparg{\loi_exparg{\readlist_h{##2}}{\loi_grabpaired_remain}}{\loi_grabpaired_result}{#2}}%
				}%
			}%
		\readlist_g\relax% le \relax meuble l'argument délimité
		}
		{\long\def\readlist_g##1#3##2\_nil{%
			\loi_ifempty{##2}% si <liste restante> ne contient pas le <sep courant>
				{\readlist_f{#1}{#2}% recommencer avec le même <sep utile>
				}%
				{\loi_ifx{\loi_listofpair\empty}% si pas de paires définies
					{\loi_exparg\readlist_f{\loi_gobarg##1#3}{#3}% raccourcir <liste restante> et <sep courant>:=<sep utile>% ##BUGFIX v1.53
					}%
					{\loi_exparg\loi_grabpaired_expr\loi_listofpair{#1}{#3}\loi_grabpaired_result\loi_grabpaired_remain
					\loi_exparg\readlist_f{\loi_grabpaired_result#3}{#3}%
					}%
				}%
			}%
		\readlist_g\relax#1#3\_nil% ##BUGFIX v1.53
		}%
}
\long\def\readlist_h#1#2#3{% #1=compteur d'index  #2=liste restante  #3=élément courant
	\loi_ifnum{0\loi_exparg\loi_ifspacefirst{\loi_currentsep}{}1\if_removeextremespaces1\fi=11 }% s'il faur retirer les espaces extrêmes
		{\loi_exparg{\loi_exparg{\readlist_i{#1}{#2}}}{\loi_removeextremespaces{#3}}}% redéfinir l'élément courant
		{\readlist_i{#1}{#2}{#3}}%
}
\long\def\readlist_i#1#2#3#4{% #1=compteur d'index  #2=liste restante  #3=élément courant   #4=sep utilisé
	\loi_ifnum{0\if_ignoreemptyitems1\fi\loi_ifempty{#3}1{}=11 }
		{\readlist_e{#1}{#2}% si l'on n'ignore pas les éléments vides
		}%
		{\loi_argcsname\loi_def{\loi_listname[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#3}% assignation de l'item ctuel à la macro
		\loi_argcsname\loi_def{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#4}% assignation du <sep> actuel à la macro \<macrolist>sep
		\loi_ifnum{\loi_nestcnt<\nestdepth\relax}% si imbrication max non atteinte
			{\advance\loi_nestcnt1
			\loi_argcsname\edef{loi_previndex[\number\loi_nestcnt]}{\csname loi_previndex[\number\numexpr\loi_nestcnt-1]\endcsname#1,}%
			\readlist_c{#3}% recommencer avec l'élément courant
			}
			{}%
		\loi_exparg\readlist_e{\number\numexpr#1+1}{#2}% puis chercher l'élément suivant dans la liste restante
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \listlen %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\listlen#1[#2]{%
	\romannumeral\loi_ifempty{#2}
		{\expandafter\expandafter\expandafter\loi_stop\csname\loi_macroname#1len[0]\endcsname}
		{\loi_exparg\listlen_a{\romannumeral-`\.\loi_macroname#1}{#2}}%
}
\def\listlen_a#1#2{% #1=macro name   #2=index non normalisé    prendre <profondeur max-1>
	\loi_exparg{\expandafter\listlen_b\romannumeral\loi_normalizeindex{#1}{#2}}{\number\numexpr\csname#1nest\endcsname-1}{#1}%
}
\def\listlen_b#1#2#3{% #1=err   #2=index normalisé  #3=macroname
	\expandafter\expandafter\expandafter\loi_stop\csname#3len[#2,0]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \foreachitem %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\foreachitem#1\in#2{%
	\edef\foreachitem_a{\noexpand\foreachitem_c\noexpand#1{\expandafter\noexpand\csname\loi_macroname#1cnt\endcsname}{\loi_macroname#2}}%
	\futurelet\loi_nxttok\foreachitem_b
}
\def\foreachitem_b{\loi_ifx{\loi_nxttok[}\foreachitem_a{\foreachitem_a[]}}
\def\foreachitem_c#1#2#3[#4]{% prendre <profondeur max-1>
	\loi_exparg{\expandafter\foreachitem_d\romannumeral\loi_normalizeindex{#3}{#4}}{\number\numexpr\csname#3nest\endcsname-1}#1{#2}{#3}%
}
\def\foreachitem_d#1#2{\loi_ifempty{#2}{\foreachitem_e{#1}{}}{\foreachitem_e{#1}{#2,}}}% #1=err  #2=index norm
\long\def\foreachitem_e#1#2#3#4#5#6{% #1=err  #2=index norm  #3=macroiter  #4=compteur associé  #5=nom de macrolist  #6=code
	\loi_ifnum{\csname#5len[#20]\endcsname>0 }
		{\loi_ifempty{#1}{}{\loi_error{#1}}%
		\loi_fornum#4=1to\csname#5len[#20]\endcsname\do{\loi_argcsname\let#3{#5[#2#4]}#6}%
		}
		{}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \showitem %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\showitems{\loi_ifstar{\let\showitems_cmd\detokenize\showitems_a}{\let\showitems_cmd\loi_identity\showitems_a}}
\def\showitems_a#1{\def\showitems_b{\showitems_d#1}\futurelet\loi_nxttok\showitems_c}
\def\showitems_c{\loi_ifx{\loi_nxttok[}\showitems_b{\showitems_b[]}}
\def\showitems_d#1[#2]{\foreachitem\showitems_ater\in#1[#2]{\showitemsmacro{\expandafter\showitems_cmd\expandafter{\showitems_ater}}}}
\unless\ifdefined\fbox
	\newdimen\fboxrule \newdimen\fboxsep \fboxrule=.4pt \fboxsep=3pt % réglages identiques à LaTeX
	\def\fbox#1{% imitation de la macro \fbox de LaTeX, voir pages 271 à 274 de "Apprendre à programmer en TeX"
		\hbox{%
			\vrule width\fboxrule
			\vtop{%
				\vbox{\hrule height\fboxrule \kern\fboxsep \hbox{\kern\fboxsep#1\kern\fboxsep}}%
				\kern\fboxsep \hrule height\fboxrule
			}\vrule width\fboxrule
		}%
	}
\fi
\def\showitemsmacro#1{% encadrement par défaut
	\begingroup\fboxsep=0.25pt \fboxrule=0.5pt \fbox{\strut#1}\endgroup
	\hskip0.25em\relax
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \itemtomacro %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\itemtomacro#1[#2]{% #1[#2]=item  non encore lu: #3=macro
	\edef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_a\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}\let
}
\def\gitemtomacro#1[#2]{% #1[#2]=item
	\xdef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_a\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}{\global\let}%
}
\def\itemtomacro_a#1#2#3#4{%
	\loi_ifempty{#1}{}{\loi_error{#1}}%
	\loi_argcsname#3#4{\loi_listname[#2]}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% réglages par défaut %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if_removeextremespaces
\newif\if_ignoreemptyitems
\let\ignoreemptyitems\_ignoreemptyitemstrue
\let\reademptyitems\_ignoreemptyitemsfalse
\setsepchar{,}
\defpair{}
\loi_def_foreachsep{,}
\reademptyitems

\loi_restorecatcode
\endinput

######################################################################
############################  Historique #############################
######################################################################

v1.0  19/8/2016
  - Première version publique

v1.1  01/09/2016
  - Stockage des séparateurs dans <macrolist>sep
  - bug corrigé dans \loi_restorecatcode

v1.2  22/10/2016
  - macros \greadlist et \gitemtomacro pour la globalité

v1.3  18/11/2016
  - bugs corrigés dans la gestion de la globalité

v1.4  05/10/2017
  - test \loi_ifprimitive ajouté au test \loi_ifcs
  - suppression de \loi_expafternil, création de \loi_expafter,
    modification de \loi_argcsname
  - correction d'un bug : \setsepchar{\par} ne provoque plus
    d'erreur. \loi_ifnum devient \long

v1.5  06/10/2017
  - correction d'un bug dans \loi_ifcs

v1.51 24/10/2017
  - correction d'un bug dans \loi_ifcs

v1.52 13/01/2018
  - le dernier séparateur est <vide>

v1.53 13/03/2018
  - correction d'un bug dans \readlist_g

v1.6 01/11/2018
  - possibilité d'appariement de tokens dans les items
  
v1.61 03/03/2019
    - la macro \loi_ifcs contient une erreur de conception.
      Il faut tester si le token est un sc && s'il est
      développable pour renvoyer vrai car il existe des sc
      non développables && qui ne sont _pas_ des primitives.
      Macro rebaptisée \loi_ifcsexpandable

==> logic/long-fork-proof.tex <==
\begin{figure}[!ht]
\hrule
\[
\intass :
\begin{array}[t]{@{} c @{\quad} c @{} }
\begin{rclarray}[t]
    \CB{L1} & : & \key_1 \fpW 1 \sep \null \fpA \cass{\CB{L1}}{\lrid} \\
\end{rclarray}
&
\begin{rclarray}[t]
    \CB{R1} & : & \key_2 \fpW 1 \sep \null \fpA \cass{\CB{R1}}{\lrid} \\
\end{rclarray}
\\
\begin{rclarray}[t]
    \CB{L2} & : & \key_1 \fpR 1 \sep \key_2 \fpR 0 \sep \key_3 \fpW 1 \sep \null \fpA \cass{\CB{L2}}{\lrid} \\
\end{rclarray}
&
\begin{rclarray}[t]
    \CB{R2} & : & \key_1 \fpR 0 \sep \key_2 \fpR 1  \sep \key_4 \fpW 1 \sep \null \fpA \cass{\CB{R2}}{\lrid} \\
\end{rclarray}  
\end{array}
\]


\hrule\vspace{5pt}
\centering
\scalebox{.9}{%
\(
\begin{session}
    \specline{ \cass{\CB{L1}}{\lrid} \sep \cass{\CB{L2}}{\lrid} \sep \cass{\CB{R1}}{\lrid} \sep \cass{\CB{R2}}{\lrid} \sep \boxass{\key_1 \pt 0 \sep \key_2 \pt 0 \sep \key_3 \pt 0 \sep \key_4 \pt 0}{\lrid}{\intass}  } \\ \\
\begin{array}{@{}l@{}}
\begin{parl}
\begin{session}
    \specline{ 
        \cass{\CB{L1}}{\lrid} \sep \boxass{\key_1 \pt 0 \sep \asstrue }{\lrid}{\intass}
    } \\
    \begin{transaction}
        \specline{ \key_1 \fpI 0 } \\
        \pmutate{\key_1}{1} ; \\
        \specline{ \key_1 \fpW 1 } \\
    \end{transaction} \\
    \specline{ 
        \boxass{\key_1 \pt 1 \sep \cass{\CB{L1}}{\lrid} \sep \asstrue }{\lrid}{\intass} \\
    } \\
\end{session}
&
\begin{session}
    \specline{ 
        \cass{\CB{R1}}{\lrid} \sep \boxass{\key_2 \pt 0 \sep \asstrue }{\lrid}{\intass} 
    } \\
    \begin{transaction}
        \specline{ \key_2 \fpI 0 } \\
        \pmutate{\key_2}{1} ; \\
        \specline{ \key_2 \fpW 1 } \\
    \end{transaction} \\
    \specline{ 
        \boxass{\key_2 \pt 1 \sep \cass{\CB{R1}}{\lrid} \sep \asstrue }{\lrid}{\intass} \\
    } \\
\end{session}
\end{parl} \\ \\
\qqqquad \qqqquad \begin{array}{@{} || c ||@{} c @{}}
\begin{session}
    \specline{ 
        \cass{\CB{L2}}{\lrid} \sep 
        \boxass{ 
            \left( 
                \begin{array}{@{}l@{}}
                    \key_1 \pt 0 \lor \cass{\CB{L1}}{\lrid} \sep {} \\
                    ( \key_1 \pt 0 \lor \key_1 \pt 1 ) \\
                \end{array}
            \right)
            \sep {} \\
            \left( 
                \begin{array}{@{}l@{}}
                    \key_2 \pt 0 \lor \cass{\CB{R1}}{\lrid} \sep{} \\
                    ( \key_2 \pt 0 \lor \key_2 \pt 1 ) \\
                \end{array}
            \right) \sep {} \\
            \key_3 \pt 0 \sep \key_4 \pt \anyval 
        }{\lrid}{\intass}  \\
        {} \lor \cass{\CB{L2}}{\lrid} \sep 
        \boxass{\key_1 \pt 1 \sep  \key_2 \pt 1 \sep  {} \\
            \key_3 \pt 0 \sep \key_4 \pt \anyval \sep {} \\
            \cass{\CB{R1}}{\lrid} \sep
            \cass{\CB{R2}}{\lrid} 
            \sep \cass{\CB{L1}}{\lrid} }{\lrid}{\intass} 
    } \\
    \begin{transaction}
        \specline{ 
            \exsts{n,m \in \Set{0,1}} \\
            \key_1 \fpI n \sep \key_2 \fpI m
            \sep \key_3 \fpI 0
        } \\
        \plookup{\pv{a}}{\key_1};
        \quad \plookup{\pv{b}}{\key_2};\\
        \pifs{ \pv{a} = 1 \land \pv{b} = 0 } 
        \passign{\key_3}{1} ; 
        \pife \\
        \specline{ 
            \exsts{n,m \in \Set{0,1}} \\
            \key_1 \fpR n \sep \key_2 \fpR m  \\
            {} \sep \mathtt{if} \ n = 1 \land m = 0 \\
            \ \mathtt{then} \ \key_3 \fpW 1 
            \ \mathtt{else} \ \key_3 \fpI 0
        } \\
    \end{transaction} \\
    \specline{ 
        \cass{\CB{L2}}{\lrid} \sep 
        \boxass{ 
            \left( 
                \begin{array}{@{}l@{}}
                    \key_1 \pt 0 \lor \cass{\CB{L1}}{\lrid} \sep {} \\
                    ( \key_1 \pt 0 \lor \key_1 \pt 1 ) \\
                \end{array}
            \right)
            \sep {} \\
            \left( 
                \begin{array}{@{}l@{}}
                    \key_2 \pt 0 \lor \cass{\CB{R1}}{\lrid} \sep{} \\
                    ( \key_2 \pt 0 \lor \key_2 \pt 1 ) \\
                \end{array}
            \right) \sep {} \\
            \key_3 \pt 0 \sep \key_4 \pt \anyval 
        }{\lrid}{\intass}  \\
        {} \lor \boxass{
            \key_1 \pt 1 \sep ( \key_2 \pt 0 \lor \key_2 \pt 1 ) \\ 
            {} \sep \key_3 \pt 1 \sep \key_4 \pt \anyval \sep {} \\
            \cass{\CB{R1}}{\lrid} \sep \cass{\CB{L1}}{\lrid} \sep \cass{\CB{L2}}{\lrid} }{\lrid}{\intass} \\
        {} \lor \cass{\CB{L2}}{\lrid} \sep 
        \boxass{\key_1 \pt 1 \sep  \key_2 \pt 1 \sep  {} \\
            \key_3 \pt 0 \sep \key_4 \pt \anyval \sep {} \\
            \cass{\CB{R1}}{\lrid} \sep
            \cass{\CB{R2}}{\lrid} 
            \sep \cass{\CB{L1}}{\lrid} }{\lrid}{\intass} 
    } \\
\end{session}
&
\begin{session}
    \specline{ 
        \cass{\CB{R2}}{\lrid} \sep 
        \boxass{ 
            \left( 
                \begin{array}{@{}l@{}}
                    \key_1 \pt 0 \lor \cass{\CB{L1}}{\lrid} \sep {} \\
                    ( \key_1 \pt 0 \lor \key_1 \pt 1 ) \\
                \end{array}
            \right)
            \sep {} \\
            \left( 
                \begin{array}{@{}l@{}}
                    \key_2 \pt 0 \lor \cass{\CB{R1}}{\lrid} \sep {} \\
                    ( \key_2 \pt 0 \lor \key_2 \pt 1 ) \\
                \end{array}
            \right) \sep {} \\
            \key_3 \pt \anyval \sep \key_4 \pt 0
        }{\lrid}{\intass}  \\
        {} \lor \cass{\CB{R2}}{\lrid} \sep 
        \boxass{
            \key_1 \pt 1 \sep  \key_2 \pt 1 \sep {} \\
            \key_3 \pt \anyval \sep \key_4 \pt 0 \sep {} \\
            \cass{\CB{R1}}{\lrid} \sep \cass{\CB{L1}}{\lrid} \sep \cass{\CB{L2}}{\lrid} }{\lrid}{\intass} 
    } \\
    \begin{transaction}
        \specline{ 
            \exsts{n,m \in \Set{0,1}} \\
            \key_1 \fpI n \sep \key_2 \fpI m
            \sep \key_4 \fpI 0
        } \\
        \plookup{\pv{c}}{\key_1};
        \quad \plookup{\pv{d}}{\key_2};\\
        \pifs{ \pv{c} = 0 \land \pv{d} = 1 } 
        \passign{\pv{f2}}{1} ; 
        \pife \\
        \specline{ 
            \exsts{n,m \in \Set{0,1}} \\
            \key_1 \fpR n \sep \key_2 \fpR m  \\
            {} \sep \mathtt{if} \ n = 0 \land m = 1 \\
            \ \mathtt{then} \ \key_4 \fpW 1 
            \ \mathtt{else} \ \key_4 \fpI 0
        } \\
    \end{transaction} \\
    \specline{ 
        \cass{\CB{R2}}{\lrid} \sep 
        \boxass{ 
            \left( 
                \begin{array}{@{}l@{}}
                    \key_1 \pt 0 \lor \cass{\CB{L1}}{\lrid} \sep {} \\
                    ( \key_1 \pt 0 \lor \key_1 \pt 1 ) \\
                \end{array}
            \right)
            \sep {} \\
            \left( 
                \begin{array}{@{}l@{}}
                    \key_2 \pt 0 \lor \cass{\CB{R1}}{\lrid} \sep {} \\
                    ( \key_2 \pt 0 \lor \key_2 \pt 1 ) \\
                \end{array}
            \right) \sep {} \\
            \key_3 \pt \anyval \sep \key_4 \pt 0
        }{\lrid}{\intass}  \\
        {} \lor \boxass{( \key_1 \pt 0 \lor \key_1 \pt 1 ) \sep \key_2 \pt 1 \\
            {} \sep \key_3 \pt \anyval \sep \key_4 \pt 1 \sep {} \\
        {} \cass{\CB{L1}}{\lrid} \sep \cass{\CB{R1}}{\lrid} \sep \cass{\CB{R2}}{\lrid} }{\lrid}{\intass}  \\
        {} \lor \cass{\CB{R2}}{\lrid} \sep 
        \boxass{
            \key_1 \pt 1 \sep  \key_2 \pt 1 \sep {} \\
            \key_3 \pt \anyval \sep \key_4 \pt 0 \sep {} \\
            \cass{\CB{R1}}{\lrid} \sep \cass{\CB{L1}}{\lrid} \sep \cass{\CB{L2}}{\lrid} }{\lrid}{\intass} 
    } \\
\end{session}
\end{array} \\
\end{array} \\ \\
\specline{ 
    \cass{\CB{L2}}{\lrid} \sep \boxass{
        \key_3 \pt 0 \sep \key_4 \pt 1 \sep 
        \cass{\CB{L1}}{\lrid} \sep \cass{\CB{R1}}{\lrid}
        \sep \cass{\CB{R2}}{\lrid} \sep \asstrue 
    }{\lrid}{\intass} \\
    {} \lor \cass{\CB{R2}}{\lrid} \sep \boxass{
        \key_3 \pt 1 \sep \key_4 \pt 0 \sep 
        \cass{\CB{L1}}{\lrid} \sep \cass{\CB{R1}}{\lrid} 
        \sep \cass{\CB{L2}}{\lrid} \sep \asstrue 
    }{\lrid}{\intass} \\
    {} \lor \cass{\CB{L2}}{\lrid} \sep \cass{\CB{R2}}{\lrid} 
    \sep \boxass{
        \key_3 \pt 0 \sep \key_4 \pt 0 
        \sep \cass{\CB{L1}}{\lrid} \sep \cass{\CB{R1}}{\lrid} 
        \sep \asstrue 
    }{\lrid}{\intass} \\
} \\
\end{session} 
\)%
}

\hrulefill

\caption{Sketch proofs for long fork under parallel snapshot isolation}
\label{fig:long-fork-proof}
\end{figure}


==> logic/prog_sound.tex <==
\subsection{Program Soundness}

We first define a trace via \( \pred{stepc}{\nat, \w, \w', \stk, \stk', \cmd, \ET} \) predicate (\cref{def:appendix-soundness-judgement-cmd}).
It asserts that given a world \( \w \) and a local stack \( \stk \), after \( \nat \) steps of rely steps and local executions, the \( \cmd \) reaches \( \pskip \) and the final world and stack are \( \w'\) and \( \stk' \).
\emph{The soundness judgement for commands} (\cref{def:soundness-judgement-cmd}) says that
for any terminated trace with the initial world \( \w \) satisfying the precondition \( \gpre \), the final world \( \w' \) induced  by \( \pred{stepc} \) should satisfy the postcondition \( \gpost \).

\begin{definition}[soundness judgement for commands]
\label{def:appendix-soundness-judgement-cmd}
\label{def:soundness-judgement-cmd}
\label{def:semantic-triple}
\label{def:triple-semantic}
\label{def:semantic-steps}
The \( \pred{stepc} \) predicate is defined as the follows:
\[
\begin{rclarray}
    \pred{stepc}{0,\w, \w', \stk, \stk',\pskip, \ET} & \defeq & 
    \begin{array}[t]{@{}l}
    \stk = \stk' \land \w = \w'
    \end{array} \\
    \pred{stepc}{\nat + 1,\w, \w', \stk, \stk', \cmd, \ET} & \defeq &
    \begin{array}[t]{@{}l}
        \exsts{ \mkvs, \mkvs'', \w''} \\
        \quad (\w,\w'') \in \Rely  
        \land (\mkvs, \stub ) = \clpsW{\w} \\
        \quad {} \land (\mkvs'', \stub ) = \clpsW{\w''} 
        \land \mkvs'' \in \CMs(\ET) \\
        \quad {} \land \pred{stepc}{\nat, \w'', \w', \stk, \stk', \cmd, \ET} \\
    \end{array} \\
    \pred{stepc}{\nat + 1,\w, \w', \stk, \stk', \cmd, \ET} & \defeq &
    \begin{array}[t]{@{}l}
        \exsts{\cl, \w'', \stk'', \cl, \cmd'} \\
        \quad (\clpsW{\w}, \stk), \cmd \toCMD{\ET} ( \clpsW{\w''}, \stk'' ), \cmd' \\
        \quad {} \land (\w, \w'') \in \Guar \\
        \quad {} \land \pred{stepc}{\nat, \w'', \w', \stk'', \stk', \cmd', \ET} \\
    \end{array}
\end{rclarray}
\]
The \emph{soundness judgement for commands} is as the follows:
\[
\begin{rclarray}
    \ET \tripleSemG{\gpre}{\cmd}{\gpost} & \defeq &
    \begin{array}[t]{@{}l@{}}
        \fora{ \w,\w', \stk, \stk', \lenv, \nat }   \\
        \quad \w \in \evalW[\lenv, \stk]{\gpre} 
        \land \pred{stepc}{\nat, \w, \w', \stk, \stk', \cmd, \ET} \\
        \qqquad \implies \w' \in \evalW[\lenv, \stk']{\gpost} 
    \end{array}
\end{rclarray}
\]
\end{definition}                                         

\begin{theorem}[soundness for commands]
\label{thm:command-soundness}
\label{thm:per-thread-soundness}
The \emph{soundness for commands} is:
\[
    \fora{\gpre, \cmd, \gpost, \ET}
    \tripleG{\gpre}{\cmd}{\gpost} 
    \implies 
    \ET \tripleSemG{\gpre}{\cmd}{\gpost} 
\]
\end{theorem}
\begin{proof}
It can be proved by induction on the derivations.

\begin{itemize}

\item \caseB{\rl{PRCommit}}
Assume pre- and post- conditions such that \( \tripleG{\gpre}{\ptrans{\trans}}{\gpost}  \).
It suffices to prove for any world \( \w \) that satisfies stable precondition, if the corresponding machine state \(\clpsW{\w'}\) can transfers to a new state \((\mkvs'',\vi'')\) via \rl{PCommit} (\cref{fig:program_semantics}), the final world should satisfy the stable postcondition \(\gpost\):
\begin{gather}
    \begin{array}{@{}l}
    \stable{\gpre, \ET}  
    \implies 
    \fora{\w, \w',\lenv, \stk}  
    \exsts{ \mkvs, \mkvs' }  \\
    \quad \w \in \evalW{\gpre} 
    \land (\w, \w') \in \Rely 
    \land (\mkvs, \stub) = \clpsW{\w} \\
    \qquad {} \land (\mkvs', \stub) = \clpsW{\w'} 
    \land \mkvs' \in \CMs(\ET)
    \implies \w' \in \evalW{\gpre} 
    \end{array} \tag{Stable Pre} \label{equ:stable-pre-condition} \\
    \nonumber \\
%
    \begin{array}{@{}l}
    \tripleL{\lpre}{\trans}{\lpost}
    \land \repartition{\gpre}{\gpost}{\lpre}{\lpost}
    \implies 
    \fora{\w, \w', \cl, \lenv, \stk, \stk'}  \\
    \quad \w \in \evalW{\gpre} 
    \land \cl \vdash (\eraseW{\w}, \stk), \ptrans{\trans}  
    \toCMD{\ET} (\eraseW{\w'}, \stk'), \pskip \\
    \qquad {} \land (\w, \w') \in \Guar 
    \implies \w' \in \evalW[\lenv, \stk']{\gpost} 
    \end{array} \tag{Commit} \label{equ:commit-transaction} \\
    \nonumber \\
%
    \begin{array}{@{}l}
    \stable{\gpost, \ET}  
    \implies 
    \fora{\w, \w',\lenv, \stk}  
    \exsts{ \mkvs, \mkvs' } \\
    \quad \w \in \evalW{\gpost} 
    \land (\w, \w') \in \Rely 
    \land (\mkvs, \stub) = \clpsW{\w} \\
    \qquad {} \land (\mkvs', \stub) = \clpsW{\w'}
    \land \mkvs' \in \CMs(\ET)
    \implies \w' \in \evalW{\gpost} 
    \end{array} \tag{Stable Post} \label{equ:stable-post-condition} 
\end{gather}

\begin{itemize}
\item Stable pre-condition.
The \( \stable{\gpre, \ET} \) (\cref{def:stable}) asserts any world \( \w \) that satisfies the pre-condition \( \gpre \), 
if the world can transfer to another world \( \w' \) through rely \( \Rely \), and if the transformation is allowed  by execution test \( \ET \), 
the new world \( \w' \) satisfies the precondition.
Thus It implies \cref{equ:stable-pre-condition}. 

\item Commit.
For any \( \w, \lenv, \stk, \mkvs, \vi \) such that \( \w \in \evalW{\gpre} \) and \( (\mkvs, \vi) = \eraseW{\w} \), by the first part of repartitioning,
there exists a snapshot \( \sn_\lpre\) and a residue \( \sn \) such that
\begin{equation}
\label{equ:local-pre-condition}
\sn_\lpre \composeH \sn = \snapshot[\mkvs, \vi] \land (\sn_\lpre, \unitO) \in \evalLS{\lpre}
\end{equation}
Because of the soundness for transactions (\cref{thm:transaction-soundness}) that for any initial stacks \( \stk \), logical environments \( \lenv \) and snapshots \( \sn \), 
if the states \( (\stk, \sn_\lpre, \unitO) \) satisfies the precondition \( \lpre \), the final states induced by the semantics \( (\stk', \sn_\lpost \composeH \sn, \fp) \) should satisfy the post-condition \( \lpost \).
\begin{equation}
\label{equ:local-transaction-sound}
\begin{array}{@{}l}
    (\stk, \sn_\lpre \composeH \sn, \unitO), \trans \toTRANS (\stk', \sn_\lpost \composeH \sn, \fp), \pskip
    \implies (\sn_\lpost, \fp) \in \evalLS[\lenv,\stk']{\lpost}
\end{array}
\end{equation}
The repartition \( \repartition{\gpre}{\gpost}{\lpre}{\lpost} \) also asserts that any world \( \w \) satisfying the pre-condition \( \gpre \), 
if the corresponding machine of the world \( (\mkvs, \vi) \) can transfer to a new state \(  (\mkvs', \vi') \) by committing the fingerprint \( \fp \),
there exists a new world \( \w' \) such that \( (\mkvs', \vi') = \eraseW{\w} \) and \( (\w, \w') \in \Guar \).
This new world should satisfy the postcondition \( \gpost \).
That is, for some \( \mkvs', \vi', \cl, \w' \),
\begin{equation}                                    
\label{equ:repartition}
\begin{array}{@{}l}
    \mkvs' \in \updateKV[\mkvs, \vi, \cl, \fp]
    \land \ET \vdash (\mkvs, \vi) \csat \fp : \vi'  \\
    \quad {} \land (\mkvs', \vi') = \eraseW{\w'} 
    \land (\w, \w') \in \Guar
    \implies \w' \in \evalW[\lenv, \stk']{\gpost}
\end{array}
\end{equation}
Combine \cref{equ:repartition} with \cref{equ:local-pre-condition} and \cref{equ:local-transaction-sound},
and we have the following:
\begin{equation}
\label{equ:combined-transaction-sound}
\begin{array}{@{}l}
    \w \in \evalW{\gpre}  
    \land (\mkvs, \vi) = \eraseW{\w} \\
    \quad {} \vdash (\stk, \snapshot[\mkvs, \vi], \unitO), \trans \toTRANS (\stk', \sn', \fp), \pskip  \\
    \quad {} \land \mkvs' \in \updateKV[\mkvs, \vi, \cl, \fp]
    \land \ET \vdash (\mkvs, \vi) \csat \fp : \vi'  \\
    \qquad {} \land (\mkvs', \vi') = \eraseW{\w'} 
    \land (\w, \w') \in \Guar
    \implies \w' \in \evalW[\lenv, \stk']{\gpost}
\end{array}
\end{equation}
Hence we prove \cref{equ:commit-transaction} by folding all the side conditions for a atomic transaction,
\[
\begin{array}{@{}l}
    \w \in \evalW{\gpre} 
    \land \cl \vdash (\eraseW{\w}, \stk), \ptrans{\trans} \toCMD{\ET} (\eraseW{\w'}, \stk'), \pskip \\
    \qqquad {} \land (\w, \w') \in \Guar 
    \implies \w' \in \evalW[\lenv, \stk']{\gpost}
\end{array}
\]

\item Stable post-condition.
It can be proven for the similar reason as \cref{equ:stable-pre-condition}.
\end{itemize}

\item \caseB{\rl{PRAss}}
We have \( \gpre \equiv \vx \dot= \lexpr\), \( \cmd \equiv \passign{\vx}{\expr}\) and \( \gpost \equiv \vx \dot= \expr\sub{\lexpr}{\vx}\) for some \( \vx, \lexpr \) and \( \expr \).
The precondition is interpreted to unit worlds \( \unitW = \evalW{\gpre} \), which is closed under rely.
If it takes one step to a new state where the stack is updated to \( \stk' = \stk\rmto{\vx}{\evalE{\expr}} \), it is easy to see that the logical value is evaluated to the same as before \( \evalLE[\lenv, \stk']{\lexpr} = \evalLE{\lexpr} \) and thus \( \evalLE[\lenv, \stk']{\expr\sub{\lexpr}{\vx}} = \evalLE[\lenv, \stk]{\expr} \).
We also know local assignment does not change the state of the world:
\[
    (\mkvs, \vi, \stk), \passign{\vx}{\expr} \toCMD{\stub} (\mkvs, \vi, \stk'), \pskip
\]
Last, for the similar reasons as \( \unitW = \evalW{\gpost}  \) the rely does not affect the postcondition.

\item \caseB{\rl{PRAssume}}
We have \( \gpre \equiv \gpost \equiv \expr \dot\neq 0\) and \( \cmd \equiv \passume{\expr}\) for some \( \vx \) and \( \expr \).
The precondition and postcondition are interpreted to unit worlds \( \unitW\).
The semantics for assume \( \passume{\expr} \) does not change the state of the world, so we have the proof.

\item \caseI{\rl{PRChoice}}
We have \( \cmd \equiv \cmd_1 \pchoice \cmd_2 \) for some \( \cmd_1 \) and \( \cmd_2 \) such that \( \tripleSemG{\gpre}{\cmd_1}{\gpost} \) and \( \tripleSemG{\gpre}{\cmd_2}{\gpost} \) for some \( \cmd_1 \) and \( \cmd_2 \).
Because the semantics for non-deterministic choice \( \cmd_1 \pchoice \cmd_2 \) does not change the state of the world, It is easy to see:
\[
    \tripleSemG{\gpre}{\cmd_1}{\gpost} \land \tripleSemG{\gpre}{\cmd_2}{\gpost} \implies \tripleSemG{\gpre}{\cmd_1 \pchoice \cmd_2}{\gpost}
\]

\item \caseI{\rl{PRSeq}}
We have \( \cmd \equiv \cmd_1 \pseq \cmd_2 \) for some \( \cmd_1 \) and \( \cmd_2 \) such that \( \tripleSemG{\gpre}{\cmd_1}{\gframe} \) and \( \tripleSemG{\gframe}{\cmd_2}{\gpost} \) for some \( \cmd_1, \cmd_2\) and \( \gframe \).
By the semantics  we know for any world \( \w \), stack \( \stk \) and execution test:
\[
    (\eraseW{\w}, \stk), \pskip \pseq \cmd_2 \toCMD{\ET} (\eraseW{\w}, \stk), \cmd_2
\]
It is easy to see:
\[
    \tripleSemG{\gpre}{\cmd_1 }{\gframe} \land \tripleSemG{\gframe}{\cmd_2}{\gpost} \implies \tripleSemG{\gpre}{\cmd_1 \pseq \cmd_2}{\gpost}
\]

\item \caseI{\rl{PRIter}}
By the definition of \( \pred{stepc}\), it suffice to prove:
\[
    \fora{\nat} \tripleG{\gpre}{\cmd^{\nat}}{\gpre} \implies \tripleSemG{\gpre}{\cmd^{\nat}}{\gpre} 
\]
where
\[
    \cmd^{0} \defeq \pskip \quad \cmd^{n + 1} \defeq \cmd \pseq \cmd^{n}
\]
We prove this by induction on the number \( \nat \).
When \( \nat = 0 \), it trivially holds.
If it holds when \( \nat = i\), let consider \( \nat = i + 1 \).
By the semantics  we know for any world \( \w \) and stack \( \stk \):
\[
    (\eraseW{\w}, \stk), \pskip \pseq \cmd \toCMD{\stub} (\eraseW{\w}, \stk), \cmd
\]
it is easy to see:
\[
    \tripleSemG{\gpre}{\cmd^{i}}{\gpre} \land \tripleSemG{\gpre}{\cmd}{\gpre} \implies \tripleSemG{\gpre}{\cmd^{i+1}}{\gpre} 
\]

\item \caseI{\rl{PRFrame}}
Given \( \tripleSemG{\gpre}{\cmd}{\gpost} \) and \( \stable{\gframe, \ET}\), we need to prove \( \tripleSemG{\gpre \sep \gframe }{\cmd}{\gpost \sep \gframe } \).
By \( \tripleSemG{\gpre}{\cmd}{\gpost} \), we know that for any trace defined by the \( \pred{stepc} \) predicate with an initial world \( \w \) satisfying the precondition \( \gpre \), the finial world \( \w' \) satisfies the postcondition \( \gpost \). 
Now we need to prove the frame does not invalidate the trace:
\[
\begin{array}[t]{@{}l}
    \fora{ \w,\w', \w_{f}, \w'', \stk, \stk', \lenv, \nat, \ET } \\
    \quad \pred{stepc}{\nat, \w, \w', \stk, \stk', \cmd, \ET} 
    \land \w' \in \evalW[\lenv, \stk']{\gpost}  
    \land \stable{\gframe, \ET} \\
    \qquad {} \land \pred{stepc}{\nat, \w \composeW \w_f, \w'', \stk, \stk', \cmd, \ET} 
    \land \w_f \in \evalW[\lenv, \stk]{\gframe} 
    \implies \w'' \in \evalW[\lenv, \stk']{\gframe \sep \gpost}
\end{array}
\]
We prove it by induction on the number \( \nat \).
\begin{itemize}
\item If \( \nat = 0 \),  we know \( \w = \w'\), \( \stk = \stk'\) and \( \cmd = \pskip \).
We can pick \( \w'' = \w \composeW \w_f\).

\item Assume it holds for \( \nat = i \) steps, let consider \( i + 1 \) steps.
Assume some initial worlds \( \w \), stacks \( \stk \) and logical environments \( \lenv \), and worlds from the frame \( \w_f \in \evalW[\lenv, \stk]{\gframe}\) such that \( (\w \composeW \w_f)\isdef \).
Given the definition of \( \pred{stepc}\) predicate, the next step may be a step of guarantee which change the command or a step of rely.

\begin{itemize}

\item First let consider a guarantee step.
Let \( \cmd' \) and \( \stk' \) be the new command and stack after the transformation \( (\w, \w') \in \Guar \) for some new world \( \w'\).
Assuming a world \( \w'' \) such that \( (\w \composeW \w_f, \w'') \in \Guar \), we want to prove \( \w''  = \w' \composeW \w_f'' \) for some worlds from the frame \( \w_f'' \in \evalW[\lenv, \stk']{\gframe} \).
Because of the side condition \( \func{fv}{\gframe} \cap \func{modify}{\cmd} = \emptyset \), the new stack \( \stk' \) does not affect the interpretation of the frame \(\evalW{\gframe} = \evalW[\lenv,\stk']{\gframe}\).
Because of the \cref{lem:appendix-locality-update} and the stabilisation of the frame, there exists a rely step \( (\w_f, \w_{f}') \in \Rely \) where the key-value store has been updated to match up with \( \w' \), yet the view remain the same, \ie \( \eraseW{\w_{f}'}\projection{1} = \eraseW{\w}\projection{1}\) and \( \eraseW{\w_f}\projection{2} = \eraseW{\w'_{f}}\projection{2}\).
Because the rely does not change the local capabilities, we know the local capabilities of \( \w'_{f}\) are compatible with the ones of \( \w' \), \ie \( (\w'\projection{1} \composeC \w'_{f}\projection{1})\isdef\).
We assume that the execution test satisfies at least monotonic read, so the view of \( \w'\) is greater than the view of \( \w \).
As the view shift rely allows arbitrarily to advance the view, there exists a world \( \w_f''\) by shifting the view from \( \w_f' \) such that \( (\w_f, \w_f'') \in \Rely \) and the view of \( \w_f'' \) matches with the view \( \w' \), therefore we have \( (\w' \composeW \w_f'')\isdef \).
Therefore, for any world transformation via guarantee \( (\w, \w') \in \Guar \), there exists \( \w_f, \w_f'' \in \evalW[\lenv,\stk']{\gframe}\)  such that \( (\w \composeW \w_f)\isdef\) and \( (\w' \composeW \w_f'')\isdef\).
By the definition of guarantee we have \( (\w \composeW \w_f, \w' \composeW \w''_f) \in \Guar \).
Finally, by applying \ih when \( \nat = i \), we can now fold the \( \pred{stepc} \) predicate for \( \nat = i + 1 \).

\item If it is a rely step, let assume \( (\w, \w') \in \Rely \) and \( (\w \composeW \w_f, \w'') \in \Rely \) for some world \( \w'' \)
and we want to prove \( \w''  = \w' \composeW \w_f'' \) for same \( \w_f'' \) such that \( \w_f'' \in \evalW[\lenv, \stk]{\gframe} \).
By \( (\w \composeW \w_f, \w'') \in \Rely \), the world transition is allowed by some capabilities, says \( \ca\), that are compatible with the local capabilities of \( \w \composeW \w_f \), \ie \( (\ca \composeC (\w\projection{1} \composeC \w_f\projection{1}) )\isdef \).
This means the capabilities \( \ca \) are disjointed with the local capabilities of \( \w\projection{1} \) and local capabilities of \( \w_f\projection{1}\) respectively.
Because of the stable of \( \gframe \), there is a world \( \w_f'' \) such that \( \w_f'' \in \evalW{\gframe}\) and \( \eraseW{\w_f''} = \eraseW{\w'} = \eraseW{\w''}\).
Because the rely and stabilisation do not alter the local capabilities, thus we prove \( \w'' = \w' \composeW \w_f'' \).
Finally, by applying \ih when \( \nat = i \), we can now fold the \( \pred{stepc} \) predicate for \( \nat = i + 1 \).
\end{itemize}
\end{itemize}
\end{itemize}

\end{proof}


\begin{lemma}[Locality of update]
\label{lem:locality-update}
\label{lem:appendix-locality-update}
When a client executes a transaction allowed by guarantee, the effect to the key-value store is included in the rely of other clients.
\[
\begin{array}{@{}l}
    \fora{\w_g, \w_g', \w_r, \mkvs} (\w_g\projection{1} \composeC \w_r\projection{1} )\isdef \\
    \quad {} \land (\mkvs, \stub) = \clpsW{\w_g} \land  (\mkvs, \stub) = \clpsW{\w_r} \land (\w_g, \w_g') \in \Guar  \\
    \qquad \implies \exsts{\w_r', \mkvs'} (\w_g'\projection{1} \composeC \w_r'\projection{1})\isdef \\
    \qqquad {} \land (\mkvs', \stub) = \clpsW{\w_g'} \land  (\mkvs', \stub) = \clps{\w_r'} \land (\w_r, \w_r') \in \Rely 
\end{array} 
\]
\end{lemma}
\begin{proof}
Assume two worlds \( \w_g \) and \( \w_r \) where the local capabilities are compatible \((\w_g\projection{1} \composeC \w_r\projection{1})\isdef\) and the key-value stores are the same, \ie \( \clpsW{\w_g}\projection{1} = \clpsW{\w_r}\projection{1} \).
If the first world can transfer to a new world \( \w_g \) allowed by the guarantee \( (\w_g, \w_g' ) \in \Guar \).
It means that for any region \( \rid \) that has been updated, there exists a \( \kap \) such that \( \kap \sqsubseteq \ca(\rid) \) which gives the permission.
Formally, let \( (\ca_g, \gs_g) = \w_g \) and \( (\ca_g', \gs_g') = \w_g' \):
\[
\begin{array}{@{}l}
    \fora{\rid} 
    \gs_g(\rid) = \gs_g'(\rid) \lor 
    \exsts{\mkvs, \mkvs', \vi, \vi', \ca_s, \ca_{s}', \intf, \kap} \\
    \qquad \gs_g(\rid) = (\mkvs, \vi, \ca_{s}, \intf) 
    \land \gs_g'(\rid) = (\mkvs', \vi', \ca_{s}', \intf)
    \land \kap \sqsubseteq \ca(\rid) \\
    \qquad {} \land ((\mkvs, \vi, \ca_{s}), (\mkvs', \vi', \ca_{s}')) \in \intf(\kap)
    \land (\ca_g \composeC \ca_s)^{\perp} = (\ca_g' \composeC \ca_s')^{\perp}
\end{array} 
\]
We now construct a world \( \w_r' = (\ca_r', \gs_r') \) that satisfies all the conditions.
First, because the guarantee preserves the orthogonal, we can take the same local capabilities as the \( \w_r \):
\begin{equation}
\label{equ:construct-local-ca}
    \ca_r' = \w_r'\projection{1}
\end{equation}
Then we take the same key-value store and shared capabilities as \( \w_g' \), but keep the view as the same in the \( \w_r \),
\begin{equation}
\label{equ:construct-gs}
\begin{array}{l}
    \fora{\rid} \exsts{\mkvs,\vi,\ca,\intf} \gs_r'(\rid) = (\mkvs, \vi, \ca, \intf) \\
    \qquad {} \land \gs_g'(\rid) = (\mkvs, \stub, \ca, \intf) \land \w'\projection{2}(\rid) = (\stub, \vi, \stub, \intf)
\end{array}
\end{equation}
Combining \cref{equ:construct-local-ca} and \cref{equ:construct-gs}, it is easy to see \( ( \w_r, \w_r' ) \in \relyU \) by \cref{def:rely-guarantee}, therefore \( ( \w_r, \w_r' ) \in \Rely \).
Given the way we construct \( \w_r' \), it directly implies all the conditions.
\end{proof}


\emph{The soundness for programs} (\cref{def:soundness-prog}) is a non-trivial proof as clients have the up-to-date kv-store because of the interleaving semantics but not the views.
Let world environment \( \wenv \) is worlds indexed by clients.
\emph{The soundness judgement for programs} (\cref{def:soundness-judgement-prog}) asserts that given a world environment \( \wenv \), an initial client environment \( \thdenv \), and a program \( \prog\), after \( \nat \)  steps where all clients reach \( \pskip \), the finial world environment and client environment are \( \wenv' \) and \( \thdenv' \).
Assuming that all clients start from the same world \( \w \) satisfying the overall precondition \( \gpre \), \emph{The soundness for programs} requires the finial world environment \( \wenv' \) defined by \( \pred{stepp} \) satisfying the postcondition \( \gpost \).

\begin{definition}[Soundness judgement for programs]
\label{def:soundness-judgement-prog}
Assume \emph{world environments} \( \wenv \in \Clients \parfinfun \World\), the \emph{soundness judgement for program} is defined as the follows:
\[
\begin{rclarray}
    \pred{stepp}{0,\wenv, \wenv', \thdenv, \thdenv',\prog, \ET} & \defeq &  
    \\
    \multicolumn{3}{@{}l}{%
    \qqquad 
    \begin{array}[t]{@{}l}
    \wenv = \wenv' 
    \land \thdenv = \thdenv' 
    \land \dom(\wenv) = \dom(\thdenv) = \dom(\prog) \\
    \quad {} \land  \left(\prod_{\cl \in \dom(\wenv')} \wenv'(\cl) \right)\isdef
    \land \fora{\cl \in \dom(\prog)} \prog(\cl) = \pskip
    \end{array}%
    }
    \\
    \pred{stepp}{ \nat + 1, \wenv, \wenv', \thdenv, \thdenv',\prog, \ET} & \defeq & \\
    \multicolumn{3}{@{}l}{%
    \qqquad 
    \begin{array}[t]{@{}l}
    \exsts{\wenv'', \thdenv'', \cl, \w, \w'} 
    \fora{\cl \in \dom(\wenv)} 
    (\wenv(\cl), \wenv(\cl)'') \in \Rely  \\
    \quad {} \land \pred{compatible}{\wenv''} 
    \land \pred{stepp}{ \nat, \wenv'', \wenv', \thdenv'', \thdenv',\prog, \ET} 
    \end{array}%
    }
    \\
    \pred{stepp}{ \nat + 1, \wenv, \wenv', \thdenv, \thdenv',\prog, \ET} & \defeq & \\
    \multicolumn{3}{@{}l}{%
    \qqquad 
    \begin{array}[t]{@{}l}
    \exsts{\wenv'', \thdenv'', \prog'', \cl}  
    \left(\wenv(\cl), \wenv''(\cl)\right) \in \Guar \\
    \quad {} \land \func{world2conf}{\wenv}, \thdenv, \prog \toPROG{}_{\ET} \func{world2conf}{\wenv''}, \thdenv'', \prog'' \\
    \quad {} \land \pred{compatible}{\wenv''} 
    \land \pred{stepp}{ \nat, \wenv'', \wenv', \thdenv'', \thdenv',\prog'', \ET} 
    \end{array}%
    }
    \\
\end{rclarray}
\]
where the \( \pred{compatible} \) asserts all clients have the same kv-store and shared capabilities but not necessary for views, and the \( \func{world2conf}\) collapses a world environment to a configuration:
\[
\begin{rclarray}
    \pred{compatible}{\wenv} & \defeq & 
    \begin{array}[t]{@{}l}
        \exsts{\wenv'}
        \left(\prod_{\cl \in \dom(\wenv')} \wenv'(\cl) \right)\isdef \\
        \qquad {} \land \fora{\cl \in \dom(\wenv)} (\wenv(\cl), \wenv'(\cl)) \in \relyV 
    \end{array} \\
    \func{world2conf}{\wenv} & \defeq & 
    \begin{cases}
        (\mkvs, \lambda \cl \ldotp \eraseW{\wenv(\cl)}\projection{2}) & \text{if } \fora{ \cl \in \dom(\wenv)} \eraseW{\wenv(\cl)}\projection{1} = \mkvs \\
        \text{undefined} & \text{otherwise}
    \end{cases} \\
\end{rclarray}
\]
\end{definition}

\begin{theorem}[Soundness for programs]
\label{def:soundness-prog}
For any program \( \prog \), if a initial world environment \( \wenv \) and a client environment \( \thdenv \) satisfy the precondition \( \gpre \), and for any world environment and client environment \( \wenv', \thdenv' \) induced by the \( \pred{stepp} \) predicate, the \( \wenv' \) satisfies the postcondition \( \gpost \):
\[
\begin{array}{@{}l}
\fora{\gpre, \gpost, \prog, \lenv, \ET, \stk, \w, \wenv, \wenv', \thdenv, \thdenv', \nat}  \exsts{\stk'}
    \tripleG{\gpre}{\prog}{\gpost} \\
    \quad {} \land \w \in \evalW{\gpre}
    \land \dom(\wenv) = \dom(\prog) = \dom(\thdenv)
    \land \w = \prod_{\cl \in \dom(\wenv)} \wenv(\cl) \\
    \quad {} \land \fora{\cl} \thdenv(\cl) = \stk
    \land \pred{steps}{\nat,\wenv, \wenv', \thdenv, \thdenv',\prog, \ET}  \\
    \qquad {} \implies \prod_{\cl \in \dom(\wenv')} \wenv'(\cl) \in \evalW[\lenv, \stk']{\gpost}
\end{array}
\] 
\end{theorem}
\begin{proof}
It can be proved by induction on the number of clients.

\begin{itemize}
\item \caseB{\( \prog = \Set{\txid \mapsto \cmd} \)}
If there is only one client, we want to prove:
\[
    \begin{array}{l}
    \pred{stepp}{\nat, \Set{\cl \mapsto \w},\Set{\cl \mapsto \w'}, \Set{\cl \mapsto \stk}, \Set{ \cl \mapsto \stk'}, \Set{\cl \mapsto \cmd}, \ET} \\
    \qqquad \implies \w' \in \evalW[\lenv, \stk']{\gpost}
\end{array}
\]
Because the \cref{lem:prgram-step-to-command-step} that the \( \pred{stepp} \) implies \( \pred{stepc}\), 
then because of the soundness for commands (\cref{thm:per-thread-soundness}) \( \tripleSemG{\gpre}{\cmd}{\gpost}\), we prove \( \w' \in \evalW[\lenv, \stk']{\gpost} \).

\caseI{\( \prog \ppar \cmd \)}
We want to prove that \( \stable{\gpre_1, \ET} \), \( \stable{\gpre_2, \ET} \), \( \tripleSemG{\gpre_{1}}{\prog}{ \gpost_{1} } \) and \( \tripleSemG{\gpre_{2}}{\cmd}{ \gpost_{2} } \) implies \( \tripleSemG{\gpre_{1} \sep \gpre_{2}}{\prog \ppar \cmd}{ \gpost_{1} \sep \gpost_{2} } \).
Let assume \( \wenv \) and \( \w \) such that \( \prod_{\cl \in \dom(\wenv)} \wenv(\cl) \in \evalW{\gpre_{1}} \) and \( \w \in \evalW{\gpre_{2}}\) for some \( \lenv \) and \( \stk \),
Because \( \gpre_{1} \sep \gpre_{2} \), we have \( \pred{compatible}{\wenv \uplus \Set{\cl \mapsto \w}}\).
Note that, since stacks are local for clients, it is safe to assume variables from different stacks are under different scopes and we will omit the stacks.
Give the \ih and the soundness result for commands \( \cmd \), we want to prove the follows:
\[
\begin{array}{@{}l}
    \fora{\nat, \wenv, \wenv', \thdenv, \thdenv', \w, \w', \stk, \stk', \cl, \ET}  \\
    \quad \pred{stepp}{\nat, \wenv, \wenv', \thdenv, \thdenv', \prog, \ET}  \\
    \quad {} \land \pred{stepc}{\nat, \w, \w', \stk, \stk', \cmd, \ET} 
    \land \pred{compatible}{\wenv \uplus \Set{\cl \mapsto \w}} \\
    \quad {} \land \prod_{\cl' \in \dom(\wenv') } \wenv'(\cl')  \in \evalW[\lenv, \stk']{\gpost_{1}} \land \w' \in \evalW[\lenv, \stk']{\gpost_{2}} \\
    \qquad \implies \exsts{\wenv'', \thdenv'', \stk'' }  \\
    \qquad \pred{stepp}{\nat, \wenv \uplus \Set{\cl \mapsto \w}, \wenv'', \thdenv \uplus \Set{\cl \mapsto \stk}, \thdenv'', \prog \uplus \Set{\cl \mapsto \cmd}, \ET}  \\
    \qqquad {} \land \prod_{\cl' \in \dom(\wenv'') } \wenv''(\cl')  \in \evalW[\lenv, \stk']{\gpost_{1} \sep \gpost_{2}}
\end{array}
\]
We prove it by induction on the number \( \nat \).
\begin{itemize}

    \item If \( \nat = 0\), it holds trivially by picking \( \wenv'' = \wenv \uplus \Set{\cl \mapsto \w} \) and \( \thdenv'' = \thdenv \uplus \Set{\cl \mapsto \stk}\).

    \item If it holds when \( \nat = i\), let consider \( \nat = i + 1\).
    There are three cases: \textbf{(i)} one client from \( \prog \) executes its commands; \textbf{(ii)} the client \( \cl \) executes its commands; and \textbf{(iii)} both take rely steps to cope with the environment.
    \begin{itemize}
        \item For the case that one client from \( \prog \) executes its commands, we unfold the definition of \( \pred{stepp} \) and assume that the \( \prog \) takes one step to a new \( \wenv_i\), \( \prog_i \) and \( \thdenv_i \):
        \[
        \begin{array}{@{}l}
            \exsts{\cl'} (\wenv(\cl'), \wenv_i(\cl')) \in \Guar \\ 
            \quad {} \land \func{world2conf}{\wenv}, \thdenv, \prog \toPROG{}_{\ET} \func{world2conf}{\wenv_i}, \thdenv_i, \prog_i  \\
            \quad {} \land \pred{compatible}{\wenv_i} \land \pred{steppp}{i, \wenv_i, \wenv', \thdenv_i, \thdenv', \prog_i, \ET}
        \end{array}
        \]
        Because the of the compatibility \( \pred{compatible}{\wenv \uplus \Set{\cl \mapsto \w}} \) and the \cref{lem:appendix-locality-update}, there exists a world \( \w_i\) via taking a rely step allowed by the \( \pred{stepc} \) predicate:
        \[
        \begin{array}{@{}l}
            (\w, \w_i) \in \Rely \land \pred{stepc}{i, \w'', \w', \stk, \stk', \cmd, \ET} \\
            \quad {} \land \pred{compatible}{\wenv_i \uplus \Set{\cl \mapsto \w_i}}
        \end{array}
        \]
        we now apply \ih and then can fold back \( \pred{stepp} \) when \( \nat = i + 1 \).
        \item Similarly, Let consider that the \( \cmd \) takes one step transferring the world to \( \w_i \) as \( (\w, \w_i) \in \Guar \).
        Because of \( \pred{compatible}{\wenv \uplus \Set{\cl \mapsto \w}} \) and the \cref{lem:appendix-locality-update}, there exists a world \( \wenv_i\) such that:
        \[
            \begin{array}{l}
            \fora{\cl' \in \dom(\wenv)} (\wenv(\cl'), \wenv_i(\cl')) \in \Rely \\
            \quad {} \land \pred{compatible}{\wenv_i} \land \pred{stepp}{ \nat, \wenv_i, \wenv', \thdenv, \thdenv',\prog, \ET} 
            \end{array}
        \]
        we now apply \ih and then can fold back \( \pred{stepp} \) when \( \nat = i + 1 \).
        \item Last, It is trivial true when both \( \prog\) and \( \cmd \) take a rely step as the local capabilities are compatible with each other.

    \end{itemize}
\end{itemize}
\end{itemize}
\end{proof}


\begin{lemma}
\label{lem:prgram-step-to-command-step}
Predicate \( \pred{stepp} \) implies  \( \pred{stepc} \).
\[
\begin{array}{@{}l}
    \fora{\nat, \w, \w', \stk, \stk', \cmd, \ET, \cl} \\
    \pred{stepp}{\nat, \Set{\cl \mapsto \w},\Set{\cl \mapsto \w'}, \Set{\cl \mapsto \stk}, \Set{ \cl \mapsto \stk'}, \Set{\cl \mapsto \cmd}, \ET}  \\ 
    \quad \implies \pred{stepc}{\nat, \w, \w', \stk, \stk', \cmd, \ET} \\
\end{array}
\]
\end{lemma}
\begin{proof}
We prove by induction on the number \( \nat \).

\begin{itemize}

\item \caseB{\(\nat = 0\)}
It is easy to see that \( \cmd = \pskip \), \( \w = \w'\) and \( \stk = \stk' \) by the definition of \(  \pred{stepp}\), so we have the proof for \( \pred{stepc} \).

\caseI{\nat = i + 1}
Assume it holds when \( \nat = i \), let consider \( \nat = i + 1 \).
If the \((i + 1)\)-\emph{th} step is a rely step, it trivially holds by applying the \ih and then folding back the \( \pred{stepc} \).
Let consider a guarantee step.
By the definition \( \pred{stepp}\), there exist a world \( \w'' \), a stack \( \stk'' \) and commands \( \cmd' \) such that:
\[
\begin{array}{@{}l@{}}
    (\w, \w'') \in \Guar  
    \exsts{\conf, \conf', \thdenv, \thdenv', \prog, \prog'} \\
    \quad \conf = \func{world2conf}{\Set{\cl \mapsto \w}}
    \land \thdenv =  \Set{\cl \mapsto \stk} 
    \land \prog = \Set{\cl \mapsto \cmd} \\
    \quad {} \conf' = \func{world2conf}{\Set{\cl \mapsto \w''}}
    \land \thdenv' =  \Set{\cl \mapsto \stk''} 
    \land \prog' = \Set{\cl \mapsto \cmd'} \\
    \quad {} \land  \conf, \thdenv , \prog \toPROG{}_{\ET} \conf', \thdenv' , \prog'   \\
    \quad {} \land \pred{stepp}{ i, \Set{\cl \mapsto \w''},\Set{\cl \mapsto \w'}, \Set{\cl \mapsto \stk''}, \Set{ \cl \mapsto \stk'}, \Set{\cl \mapsto \cmd'}, \ET}
\end{array}
\]
First by \ih, we know  \( \pred{steps}{ i, \w'', \w', \stk'', \stk', \cmd', \ET} \) holds.
Then because there is only one client, we know \( (\eraseW{\w}, \stk ), \cmd \toCMD{\ET} (\eraseW{\w''}, \stk'), \cmd' \).
Thus, by folding the predicate, we have that \( \pred{steps}{ i + 1, \w, \w', \stk, \stk', \cmd', \ET} \).
\end{itemize}
\end{proof}


==> logic/program.tex <==
\subsection{Reasoning programs}
\label{sec:reasoning-prog}

Each region has \emph{client-specified capabilities} \( \kap \in \Kaps \) that forms \emph{a partial commutative monoid (PCM)} (\cref{def:capabilities}).
To recall, \emph{a PCM} is a partially ordered set that is closed under a commutative binary operation \( \compose \) and has a set of unit elements \( \unitelem \).
The client-specified capabilities are lifted to \emph{capability composition function} \( \ca \in \Caps \) with their associated region identifiers (\cref{def:capabilities}).
For brevity, we often say \emph{capabilities} for \emph{capability composition function}.
The composition function for \emph{capabilities} \( \ca_l \composeC \ca_r \) is defined as compositing each region point-wise
and the units \( \unitC \) are functions where regions map to units of client-specified capabilities.

\begin{definition}[Capabilities]
\label{def:capabilities}
Assume a \emph{partial commutative monoid (PCM)} of \emph{client-specified capabilities} \( (\Kaps, \composeK, \unitK) \) with \( \kap \in \Kaps \), 
the composition \( \composeK \) and the units set \( \unitK \).
Given a set of \emph{region identifiers} \( \rid, \lrid \in \RegionID \), 
the \emph{capability composition function} or \emph{capabilities} is \( \ca \in \Caps \defeq \RegionID \parfun \Kaps \),
where the composition \( \composeC \) is defined as the follows:
\[
    \begin{rclarray}
        (\ca_{l} \composeC \ca_{r})(\rid) & \defeq  &
        \begin{cases}
            \ca_{l}(\rid) \composeK \ca_{r}(\rid) & \rid \in \dom(\ca_{l}) \cap \dom(\ca_{l}) \\
            \ca_{l}(\rid)  & \rid \in \dom(\ca_{l}) \setminus \dom(\ca_{l}) \\
            \ca_{r}(\rid) & \rid \in \dom(\ca_{r}) \setminus \dom(\ca_{l}) \\
            \text{undefined} & \text{otherwise} \\
        \end{cases}
    \end{rclarray}
\]
and the units set \( \unitC \defeq \Setcon{\ca}{\fora{\rid} \ca(\rid) \in \unitK } \).
A capability assertion is in the form of \( \cass{\kap(\vec{\lvar})}{\lrid} \in \CAst \).
The assertion is interpreted to a capability:
\[
\begin{rclarray}
    \evalC{\cass{\kap(\vec{\lvar})}{\lrid}} & \defeq & \Set{\lrid \mapsto \kap(\evalLE{\vec{\lvar}})} \\
\end{rclarray}
\]
\end{definition}

The \emph{capability assertions} are in the form of \( \cass{\kap(\vec{\lvar})}{\lrid} \) 
where \( \kap(\vec{\lvar}) \) is a client-specified syntactic capability parametrised by logical variables \( \vec{\lvar} \) and \( \lrid \) is the region identifier.
They are interpreted to some capabilities \( \Caps \) by interpreting the syntactic capabilities \( \kap(\vec{\lvar}) \).

Capabilities are resources that grant abilities to access the region.
That is, the \emph{interference} (\cref{def:intf}) of a region specifies the allowed fingerprints associated with certain capabilities,
and if a client holds those capabilities, it is allowed to perform those fingerprints.
Capabilities also can be used as ghost resources to track extra information and/or build protocols between clients.
For example in \cref{fig:write-skew-si-proof}, the capabilities \( \cass{\CB{L}}{\lrid} \) and \( \cass{\CB{L}}{\lrid} \) returns to shared region once being used,
so that other clients know the environment has executed transactions with fingerprints allowed by the capabilities.

Each shared region assertion is associated with a \emph{interference assertion} \( \intass \) to specify how the region can evolve (\cref{def:intf}).
\emph{A action} in the interference \( \exsts{\vec{\lvar}} \perm{\kap} : \bar{\assfp} \) says that 
if a client holds the capability \( \perm{\kap} \), it is allowed to execute a transaction and transfer capabilities with respect to \( \bar{\assfp} \).
The \emph{fingerprint and capability transferring assertions} \( \bar{\assfp} \) has fingerprint assertion (\cref{def:fingerprint-assertion}) and additionally assertions for transferring of capabilities, 
\ie adding capabilities to the shared region \( \null \fpA \cass{\kap}{\lrid} \), 
deleting capabilities from the shared region \( \null \fpD \cass{\kap}{\lrid} \) and updating the shared capabilities \( \cass{\kap(\vec{\lvar})}{\lrid} \fpU \cass{\kap(\vec{\lvar})}{\lrid} \). 
Those assertions \( \bar{\assfp} \) are interpreted as triples \( ( \assfp, \ca, \ca' ) \) of fingerprints \( \fp \), capabilities that moves into the region \( \ca \) and capabilities that moves out of the region \( \ca' \).
The existential quantification is for binding variables between the capability \( \kap \) and the assertions \( \bar{\assfp}\).

\emph{Interference assertions} are interpreted to \emph{interference environment}, \( \intf \in \Interference \) (\cref{def:intf}).
\emph{Interference environment} also \emph{interference} is a function from client-specified capabilities \( \kap \) to sets of possible transitions over shared states for a region, 
\ie tuples consisting of key-value stores, views, and (shared) capabilities (\cref{def:intf}). 
Given a interpretation of an action \( (\assfp, \ca_d, \ca_a) \in \evalF[\lenv',\stk]{\bar{\assfp}} \) and any initial state \( (\mkvs, \vi, \ca_r \composeC \ca_f ) \),
the final states \( (\mkvs',\vi', \ca_f \composeC \ca_a) \) are defined by committing the fingerprint \( \fp \) through \( \updateKV \) function,
updating the view \( \vi \sqsubseteq \vi' \), taking out \( \ca_r \) and adding \( \ca_a \).
Note that \( \ca_f \) are frames of capabilities as long as they are compatible before and after the update.
All the read values should match to the versions with respect to the view \( \vi \).
For technical reasons, the view \( \vi' \) after updating is any view greater than before.

\begin{definition}[Interference]
\label{def:intf}
The \emph{fingerprint and capability transferring assertions} is defined as:
\[
\begin{rclarray}    
    \bar{\assfp}, \bar{\assfp}' & ::= & 
    \assfp 
    \mid \null \fpA \cass{\kap(\vec{\lvar})}{\lrid}  
    \mid \null \fpD \cass{\kap(\vec{\lvar})}{\lrid} 
    \mid \cass{\kap(\vec{\lvar})}{\lrid} \fpU \cass{\kap(\vec{\lvar})}{\lrid} 
    \mid \bar{\assfp} \sep \bar{\assfp}'
\end{rclarray}
\] 
Given a logical environment $\lenv \in \LEnv$ (\cref{def:local_assertions}), a stack $\stk \in \Stacks$ and the  interpretation function for transactional assertions \( \evalLS[(.,.)]{.} \) (\cref{def:fingerprint-assertion}), the \emph{fingerprint and capability transferring assertions} is interpreted through function, $\evalF[(., .)]{.}: \FAst \times \LEnv \times \Stacks \parfun \Fingerprints \times \Caps \times \Caps$:
\[
\begin{rclarray}
    \evalF{ \assfp } & \defeq &
        \Setcon{(\fp, \ca, \ca')}{
            (\stub,\fp) \in \evalLS{\assfp} \land \ca, \ca' \in \unitC
        }  \\
    \evalF{\null \fpA \cass{\kap(\vec{\lvar})}{\lrid} } & \defeq & 
        \Setcon{(\unitO, \ca, \ca')}{
            \ca = \evalC{\cass{\kap(\vec{\lvar})}{\lrid}} \land \ca' \in \unitC
        } \\
    \evalF{\null \fpD \cass{\kap(\vec{\lvar})}{\lrid} } & \defeq &
        \Setcon{(\unitO, \ca, \ca')}{
            \ca \in \unitC \land \ca'  = \evalC{\cass{\kap(\vec{\lvar})}{\lrid}} 
        } \\
    \evalF{\cass{\kap(\vec{\lvar})}{\lrid} \fpU \cass{\kap'(\vec{\lvar}')}{\lrid} } & \defeq &
        \Setcon{(\unitO, \ca, \ca')}{
            \ca = \evalC{\cass{\kap(\vec{\lvar})}{\lrid}} \land \ca'  = \evalC{\cass{\kap'(\vec{\lvar}')}{\lrid}} 
        } \\
    \evalF{\assfp_{1} \sep \assfp_{2}} & \defeq & 
    \Setcon{%
        ( \fp_{1} \composeO \fp_{2}, \ca_{1} \composeC \ca_{2}, \ca'_{1} \composeC \ca'_{2} ) 
    }{%
        (\fp_{1}, \ca_{1}, \ca'_{1}) \in \evalF{\assfp_{1}}  \land{} \\ \quad  (\fp_{2}, \ca_{2}, \ca'_{2}) \in \evalF{\assfp_{2}}
    }\\

\end{rclarray}
\]
The grammar of \emph{interference assertions}, \( \intass \in \IAst \), is defined as:
\(
\begin{rclarray}
	\intass & ::=  & \emptyset \mid \Set{ \exsts{\vec{\lvar}} \perm{\kap} : \assfp } \cup \intass 
\end{rclarray}
\).
The \emph{interference environments} \( \intf \) is defined as the follows:
\[
\begin{rclarray}
    \intf \in \Interference & \defeq & \Kaps \to ( \MKVSs \times \Views \times \Caps ) \times  ( \MKVSs \times \Views \times \Caps )
\end{rclarray}
\]
The interference assertions are interpreted to interference environments via \emph{interference interpretation} function, $\evalI[(., .)]{.}: \IAst \times \LEnv \times \Stacks \to \Interference$:
\[
\begin{array}{@{}l}
	\evalI{\Set{ \exsts{\vec{\lvar}} \perm{\kap} : \assfp } \cup \intass }(\kap') \defeq \\
    	\qquad \left\{ 
            \begin{array}{@{}l @{\qqquad} l}
            \multicolumn{2}{@{}l@{}}{
                    \Setcon{
                        \begin{bracketarray}
                            (\mkvs, \vi, \ca_r \composeC \ca_f ), \\ 
                            (\mkvs',\vi', \ca_f \composeC \ca_a)
                        \end{bracketarray}
                    }{ 
                        \vi \in \Views(\mkvs) \\
                        \quad {} \land \exsts{\fp, \cl} 
                        ( \fp, \ca_{a}, \ca_{r} ) \in \evalF[\lenv',\stk]{\assfp} \\
                        \quad {} \land \mkvs' \in \updateKV[\mkvs, \vi, \cl, \fp] \\
                        \quad {} \land \pred{readFrom}{\mkvs, \vi, \fp}  \\
                        \quad {} \land \vi' \in \Views(\mkvs')
                    } 
                    \cup \evalI{\intass}(\kap')%
            } \\
            & \text{if there exist a logical environment} \ \lenv' \\
            & \text{by replacing} \ \vec{\lvar} \ \text{with some} \ \vec{\val} \ \text{\ie} \lenv' = \lenv\rmto{\vec{\lvar}}{\vec{\val}}, \\
            & \text{and under the new logical environment} \ \kap' = \evalI[\lenv', \stk]{\kap} \\
            \\
            \evalI{\intass}(\kap')        
            & \text{otherwise} \\
    	    \end{array}
        \right.  \\
\end{array}
\]
where the \( \pred{readFrom} \) asserts the fingerprint makes sense with respect to the view:
\[
\begin{rclarray}
    \pred{readFrom}{\mkvs, \vi, \fp} & \defeq & \fora{\key, \val} (\otR, \key, \val) \in \fp \implies \snapshot[\mkvs,\vi](\key) = \val
\end{rclarray}
\]
\end{definition}

A \emph{world} \( \w \in \World \) (\cref{def:world}) is a pair of \emph{local capabilities} \( \ca \) (\cref{def:capabilities}) and \emph{a shared state} \( \gs \).
The shared state is a function from region identifiers to quadruples consisting of key-value stores, views, shared capabilities and interference environments.
The composition functions for shared states \( \composeS \) asserts two shared states are identical.

\begin{definition}[Worlds]
\label{def:invariant-region}
\label{def:world}
Given the set of key-value stores $\MKVSs$ (\cref{def:his_heap}), views \( \Views \) (\cref{def:views}), capabilities \( \Caps\) (\cref{def:capabilities}) and region identifiers \( \RegionID \), the set of \emph{shared states} is \( \SStates \defeq \RegionID \parfun \MKVSs \times \Views \times \Caps \times \Interference \).
The \emph{shared state composition function}, $\composeS: \SStates \times \SStates \parfun \SStates$, is defined as $\composeS \defeq \composeEq$, where for all domains $\sort M$ and all $m, m' \in \sort M$:
%
\[
\begin{rclarray}
	m \composeEq m' &  \defeq  &
	\begin{cases}
		m & \text{if } m = m'\\
		\text{undefined} & \text{otherwise}
	\end{cases}
\end{rclarray}
\]
The set of \emph{worlds} \( \World \) is defined as the follows:
\[
\begin{rclarray}
	\world \in \World  & \defeq & 
    \Setcon{
        (\ca, \gs) 
    }{ 
        \ca \in \Caps \land \gs \in \SStates
        \land \exsts{ \mkvs, \vi, \ca' }   \\
        \quad (\mkvs, \vi, \ca') \in \func{collapse}[\gs] 
        \land \dom(\mkvs) = \Keys \\
        \quad {} \land \vi \in \Views(\mkvs) 
        \land \dom(\ca \composeC \ca') \subseteq \dom(\gs) \\
        \qquad {} \land \fora{\rid \in \dom(\gs)} 
        \exsts{\mkvs, \vi, \ca'', \intf}  \\
        \qquad \gs(\rid) = (\mkvs, \vi, \ca'', \intf) 
        \land ( \mkvs, \vi, \ca'' ) \in \func{inv}[\rid, \intf] \\
        \qquad {} \land  \left( \fora{ \key, i  }
        i \in  \vi( \key ) \implies  0 \leq i < \abs{ \mkvs(\key) } \right)
    }
\end{rclarray}
\]               
The \( \func{collapse}\) function is defined as the follows:
\[
\begin{rclarray}
    \func{collapse}[\emptyset] & \defeq & \Setcon{(\unitHH, \unitVI, \ca )}{ \ca \in \unitC } \\
    \func{collapse}[\Set{\rid \mapsto (\mkvs, \vi, \ca, \intf)} \uplus \gs ] & \defeq & 
        \Setcon{ 
            (\mkvs \composeHH \mkvs', \vi \compose \vi', \ca \composeC \ca') 
        }{ 
            (\mkvs', \vi', \ca') \in \func{collapse}[\gs] }\\
\end{rclarray}
\] 
where the composition for kv-store are standard disjointed union for functions \( \composeHH \defeq \uplus\).
Assume a global function \( \func{initCap} : \RegionID \to \Caps \) that returns the initial capabilities for a region.
The \( ( \mkvs, \vienv, \ca ) \in \func{inv}[\rid, \intf] \) iff:
\[
\begin{array}[t]{@{}l}
    (\mkvs, \vienv) \text{ is initial }
    \land \func{initCap}[\rid]  = \ca \\
    {} \lor \exsts{\mkvs', \vienv', \ca', \vi, \cl} 
    ( \mkvs' , \vienv', \ca' ) \in \func{inv}[\rid, \intf] \\
    \quad {} \land (( \mkvs' , \vienv'(\cl), \ca' ), ( \mkvs, \vi, \ca )) \in \intf(\kap) 
    \land \vienv = \vienv'\rmto{\cl'}{\vi}
\end{array}
\]
The \( ( \mkvs, \vi, \ca ) \in \func{inv}[\rid, \intf] \) is a short-hand for:
\[ 
\exsts{\vienv, \cl} \vi = \vienv(\cl) \land ( \mkvs, \vienv, \caset ) \in \func{inv}[\rid, \intf]
\]
% 
The \emph{world composition function}, $\composeW: \World \times \World \parfun \World$, is defined component-wise as: $\composeW \defeq (\composeC, \composeS)$.
The \emph{world unit set} is 
\[ \unitW \defeq \Setcon{(\ca, \gs)}{(\ca, \gs) \in \World \land \ca \in \unitC}
\]
The \emph{partial commutative monoid of worlds} is $(\World, \composeW, \unitW)$.
\end{definition}

The well-formed conditions for a world are:
\textbf{(i)} the state of every region is disjointed with each others (induced by the \(\func{collapse}\) function);
\textbf{(ii)} capabilities from regions are compatible with local capabilities and there is no capability of which the region identifier never appears in the shared state \ie \( \dom(\ca \composeC \ca') \in \dom(\gs) \); 
\textbf{(iii)} the state of a region \( (\mkvs, \vi, \ca'') \) satisfies the invariant of the region \( (\mkvs, \vi, \ca'') \in \func{inv}[\rid, \intf]\) and the domain of the view is the same as the domain of the key-value store, meaning they have exactly the same keys;
and \textbf{(iv)} the view of each region should be in the range of the key-value store.
In the \cref{def:world}, the \( \func[collapse] \) function erases the region identifiers and composites the states point-wise.
Because of the well-formedness, we introduce the \emph{erase function} \( \eraseW{.} : \World \to \MKVSs \times \Views \) that collapses a world to \emph{a unique pair of a key-value store and a view}:
\(
\begin{rclarray}
    \eraseW{(\ca,\gs)} & \defeq & (\mkvs, \vi)
\end{rclarray}
\),
where \( (\mkvs, \vi, \stub) \in \func{collapse}[\gs] \).

The \emph{program assertions} also \emph{assertions} (\cref{def:assertion}) have capability assertions \( \cass{\kap}{\lrid} \) for local capabilities, \emph{shared region assertions} also known as \emph{boxed assertions} \( \boxass{\bar{\lpre}}{\lrid}{\intass} \) for the shared states and standard separation logic assertions.
We assume the entire key-value store are shared, thus we do not have assertions related to key-value stores outside shared regions.

\begin{definition}[Program assertions]
\label{def:assertion}
\label{def:prog-assertion}
Given the set of logical expression \( \lexpr \in \LExpr\), the set of \emph{program assertions}, $\gpre, \gpost \in \Ast$, are defined by the following inductive grammar:
\[
\begin{rclarray}
    \bar{\lpre}, \bar{\lpost} & ::= & \assfalse \mid \asstrue \mid \bar{\lpre} \land \bar{\lpost} \mid \bar{\lpre} \lor \bar{\lpost} \mid \exsts{\lvar} \bar{\lpre} \mid \bar{\lpre} \implies \bar{\lpost} \mid \assemp \mid \cass{\kap}{\lrid} \mid \lexpr \pt \lexpr \mid \bar{\lpre} \sep \bar{\lpost} \\
	\gpre , \gpost & ::= & \assfalse \mid \asstrue \mid \gpre \land \gpost \mid \gpre \lor \gpost \mid \exsts{\lvar}\gpre \mid \gpre \implies \gpost \mid \assemp \mid \cass{\kap}{\lrid} \mid \boxass{\bar{\lpre}}{\lrid}{\intass} \mid \gpre \sep \gpost \\
\end{rclarray}
\]
%
where $\lvar, \lrid \in \LVar$, $\lexpr_1, \lexpr_2 \in \LExpr$ (\cref{def:local_assertions}), $\kap \in \Kaps$ (\cref{def:capabilities}) and $\intass \in \IAst$ (\cref{def:intf}).
Given a logical environment $\lenv \in \LEnv$ and a stack $\stk \in \Stacks$, the \emph{assertion interpretation} function, $\evalW[(., .)]{.}: \Ast \times \LEnv \times \Stacks \to \pset{\World}$, is defined as follows:
%
\[
\begin{rclarray}
	\evalW{\assfalse} & \defeq & \emptyset \\
	\evalW{\asstrue} & \defeq & \World \\
	\evalW{\gpre \land \gpost} & \defeq & \evalW{\gpre} \cap \evalW{\gpost} \\
	\evalW{\gpre \lor \gpost} & \defeq & \evalW{\gpre} \cup \evalW{\gpost} \\ 
	\evalW{\exsts{\lvar}  \gpre} & \defeq & \bigcup_{\val \in \textnormal{\Val}} \evalW[\lenv\rmto{\lvar}{\val}, \stk]{\gpre} \\
	\evalW{\gpre \implies \gpost} & \defeq & \Setcon{\w}{\w \in \evalW{\gpre} \implies \w \in \evalW{\gpost}} \\
	\evalW{\assemp} & \defeq & \unitW \\
	\evalW{\cass{\kap}{\lrid}} & \defeq & \Setcon{ (\Set{\lrid \mapsto \evalI{\kap}}, \gs) }{\gs \in \SStates} \\
	\evalW{ \boxass{\bar{\lpre}}{\lrid}{\intass} } & \defeq & 
    \Setcon{
        (\ca, \gs)
    }{         
        \exsts{\mkvs, \vi, \ca'}
        \ca \in \unitC \\
        \quad {} \land \gs(\lrid) = (\mkvs, \vi, \ca', \evalI{\intass}) 
        \land (\mkvs, \vi, \ca') \in \evalAUX{\bar{\lpre}} 
    } \\
	\evalW{ \gpre \sep \gpost } & \defeq & 
	\Setcon{
	   (\world_1 \composeW \world_2) 
    }{
       \world_1 \in \evalW{\gpre} \land \world_2 \in \evalW{\gpost}
	} \\
\end{rclarray}%
\]
The function \( \evalAUX[(., .)]{.} \) evaluates the assertions \( \bar{\lpre} \):
\[
\begin{rclarray}
    \evalAUX{\assfalse} & \defeq & \emptyset \\
    \evalAUX{\asstrue} & \defeq & \MKVSs \times \Views \times \Caps \\
    \evalAUX{\bar{\lpre} \land \bar{\lpost}} & \defeq & \evalAUX{\bar{\lpre}} \cap \evalAUX{\bar{\lpost}} \\ 
    \evalAUX{\bar{\lpre} \lor \bar{\lpost}} & \defeq & \evalAUX{\bar{\lpre}} \cup \evalAUX{\bar{\lpost}} \\ 
    \evalAUX{\exsts{\lvar} \bar{\lpre}} & \defeq & \bigcup_{\val \in \Val} \evalAUX[\lenv\rmto{\lvar}{\val}, \stk]{\bar{\lpre}} \\
    \evalAUX{\bar{\lpre} \implies \bar{\lpost}} & \defeq & \Setcon{ (\mkvs, \vi, \ca) }{ (\mkvs, \vi, \ca) \in \evalAUX{\bar{\lpre}} \implies (\mkvs, \vi, \ca) \in \evalAUX{\bar{\lpost}} }\\
    \evalAUX{\assemp} & \defeq & \Setcon{ (\unitHH, \unitVI, \ca) }{\ca \in \unitC } \\
    \evalAUX{\cass{\kap}{\lrid}} & \defeq & \Set{ (\unitHH, \unitVI, \Set{\lrid \mapsto \evalC{\kap}}) }\\
    \evalAUX{\lexpr_{1} \pt \lexpr_2} & \defeq & \Setcon{ (\mkvs, \vi, \ca) }{ \Set{ \evalLE{\lexpr_{1}} \mapsto \evalLE{\lexpr_{2}} } = \snapshot[\mkvs, \vi] \land \ca \in \unitC } \\
    \evalAUX{\bar{\lpre} \sep \bar{\lpost}} & \defeq & 
    \Setcon{ (\mkvs \composeHH \mkvs', \vi \composeVI \vi', \ca \composeC \ca') }{ (\mkvs, \vi, \ca) \in \evalAUX{\bar{\lpre}} \land (\mkvs', \vi', \ca') \in \evalAUX{\bar{\lpost}} } \\
\end{rclarray}%
\]
\end{definition}


The assertions inside regions \( \bar{\lpre} \) have capability assertions for shared capabilities, single-key assertions \( \lexpr \pt \lexpr \) and other standard separation logic assertions.
The single-key assertions \( \lexpr_1 \pt \lexpr_2 \) are interpreted to any pairs of kv-stores and views.
The view of each pair points to a version of the key \( \evalLE{\lexpr_1 }\) carrying value \( \evalLE{\lexpr_2}\).
The interpretation \( \evalAUX[(.,.)]{.} \) for the rest of \( \bar{\lpre} \) are standard.

Given \( \bar{\lpre} \) and its interpretation, shared region assertions are in the form of \( \boxass{\bar{\lpre}}{\lrid}{\intass} \).
They are interpreted to any world \( (\ca, \gs) \) where the local capabilities \( \ca \) is of unit elements,
the state of the region \( \lrid \) satisfies the assertion \( \bar{\lpre} \) and the interference environment of the region satisfies \( \intass \).
Because the composition of worlds is defined when the shared states are identical,
it means \( \boxass{\bar{\lpre}}{\lrid}{\intass} \sep \boxass{\bar{\lpost}}{\lrid}{\intass} \implies \boxass{\bar{\lpre} \land \bar{\lpost} }{\lrid}{\intass} \).

The \emph{rely} \( \Rely \) describes the allowed actions for the environment while the \emph{guarantee} \( \Guar \) are for the current client (\cref{def:rely-guarantee}).
They are defined as transitions over worlds.

\begin{definition}[Rely and guarantee]
\label{def:rely-guarantee}
Given the set of worlds $\World$ (\cref{def:world}), the \emph{update rely} relation, $\relyU \subseteq \World \times \World$, is defined as the follows:
\[	
    \begin{rclarray}
	\relyU & \defeq &
	\Setcon{
		((\ca_l,\gs), (\ca_l, \gs'))	
	}{
        \fora{\rid}
        \gs(\rid) = \gs'(\rid) \lor 
        \exsts{\kap, \mkvs, \mkvs', \vi_\rid, \vi_{e}, \vi_{e}', \ca, \ca_\rid, \ca_{\rid}', \intf}   \\
        \quad \gs(\rid) = (\mkvs, \vi_\rid, \ca_\rid, \intf)
        \land \gs'(\rid) = (\mkvs', \vi_{\rid}, \ca_{\rid}',\intf)  \\
        \quad {} \land ( \ca \composeC \ca_l \composeC \ca_r )\isdef
        \land \kap \sqsubseteq \ca(\rid)  \\ 
        \quad {} \land ( (\mkvs, \vi_e, \ca_\rid), (\mkvs', \vi_{e}', \ca_{\rid}') )  \in \intf(\kap)
	} \\
    \end{rclarray}
\]
The \emph{view shift rely} relation $\relyV \subseteq \World \times \World$, is defined as follows:
\[
    \begin{rclarray}
	\relyV & \defeq &
	\Setcon{
		((\ca_l,\gs), (\ca_l, \gs'))	
	}{
        \fora{\rid}
        \gs(\rid) = \gs'(\rid) \lor 
        \exsts{\mkvs, \vi, \vi'\ca, \ca, \intf} \\
        \quad \gs(\rid) = (\mkvs, \vi, \ca, \intf)
        \land \gs'(\rid) = (\mkvs, \vi', \ca, \intf) 
	} \\
    \end{rclarray}
\]
The \emph{rely} relation \( \Rely \) is the transitive closure of updates and view shift: \( \Rely \defeq {(\relyU \cup \relyV)}^{*} \).
The \emph{guarantee} relation, $\Guar \subseteq \World \times \World$, is defined as follows:
\[	
    \begin{rclarray}
	\Guar & \defeq &
	\Setcon{
		((\ca_l,\gs), (\ca_{l}', \gs'))	
	}{
        \fora{\rid}
        \gs(\rid) = \gs'(\rid) \lor {}
        \exsts{\kap, \mkvs, \mkvs', \vi_\rid, \vi_{\rid}', \ca_\rid, \ca_{\rid}', \intf}   \\
        \quad \gs(\rid) = (\mkvs, \vi_\rid, \ca_\rid,\intf)
        \land \gs'(\rid) = (\mkvs', \vi_{\rid}', \ca_{\rid}',\intf)  \\
        \quad \land \kap \sqsubseteq \ca_{l}(\rid)
        \land ( (\mkvs, \vi_\rid, \ca_\rid), (\mkvs', \vi_{\rid}', \ca_{\rid}') )  \in \intf(\kap) \\
        \quad \land (\ca_{l} \composeC \ca_\rid)^{\perp} = (\ca_{l}' \composeC \ca_{\rid}')^{\perp}
	} \\
    \end{rclarray}
\]
where for any element \( m \) from its domain \( \sort{M} \), the  \emph{orthogonal} is defined as:
\[
\begin{rclarray}
m^{\perp} & \defeq & \Setcon{m'}{(m \compose{} m')\isdef \land m' \in \sort{M}} 
\end{rclarray}
\]
\end{definition}

The \emph{rely} \( \Rely \) describes how the environment can change the state of the shared regions.
Given the local capabilities \( \ca_l \) and shared capabilities \( \ca_r \), the environment might own any capabilities \( \ca\) that are compatible, \ie \( (\ca \composeC \ca_l \composeC \ca_r)\isdef \).
Then the \emph{update rely} \( \relyU \) allows the environment to perform those actions associated with the capabilities \( \ca \) with their own view \( \vi_e \) to update the key-value store and shared capabilities.
Note that the \emph{update rely} does not change the views, since the views are actually local for clients.
Separately, the \emph{view shift rely} \( \relyV \) allows to advance the local view.

The \emph{guarantee} \( \Guar \) describes the allowed actions for the current client (\cref{def:rely-guarantee}).
The current client can perform actions associated with the local capabilities \( \ca_l \) to update the shared region and consequently the local capabilities.
Yet it should ensure no resource created or deleted through requiring that the \emph{orthogonal} of local capabilities and shared capabilities together remains unchanged.
The orthogonal of a capability \( \ca \) is a set of capabilities that are compatible with the capability \( \ca \).
The guarantee allows to update several regions, but each region can be updated at most once.


\begin{definition}[Stable]
\label{def:stable}
A set of worlds $\setworld \subseteq \World$ is \emph{stable}, written $\stable{\gpre, \ET}$, if and only if it is closed under the rely relation: 
\[
    \begin{rclarray}
        \stable{\gpre, \ET} & \defeq & 
        \begin{array}[t]{@{}l}
            \fora{\stk, \lenv, \w, \w', \mkvs, \mkvs', \vi, \vi', \vi''} 
            \exsts{\fp, \vi''} \\
            \quad \w \in \evalW{\gpre} 
            \land \ET \vdash (\mkvs, \vi) \csat \fp :  \vi''
            \land \vi'' \subseteq \vi' \\
            \quad {} \land (\w, \w') \in \Rely  
            \land (\mkvs, \vi) = \eraseW{\w} \\
            \quad {} \land (\mkvs', \vi') = \eraseW{\w'} 
            \implies \w' \in \evalW{\gpre}
        \end{array} \\
    \end{rclarray}
\]
\end{definition}

Assertions are \emph{stable} if they remain true against the rely (\cref{def:stable}).
Formally speaking, a set of worlds \( \evalW{\gpre} \) is stable under certain execution test \( \ET \) if the set is closed under rely relation \( (\w, \w') \in \Rely \) with the side conditions:
the new key-value store after a rely step is allowed by the consistency model induced by the execution test \( \mkvs' \in \CMs(\ET) \).

The rules for programs are in \cref{fig:rule-prog}.
The triple \( \tripleG{\gpre}{\prog}{\gpost} \) asserts that given any state satisfying the precondition \( \gpre \), if the program \( \prog \) terminates under the execution test \( \ET \), the state after satisfies the postcondition \( \gpost \).
The \rl{PRCommit} rule is the key rule.
It commits the local effect of a transaction \( \trans \) via \emph{repartitioning} \( \repartition{\gpre}{\gpost}{\lpre}{\lpost} \).
The repartitioning means:
\begin{itemize}
\item
for any possible world \( \w \) satisfying the precondition \( \gpre \), there exists a snapshot corresponding the world \( \snapshot[\mkvs, \vi] \) with empty fingerprint \( \unitO \) that overall satisfies the transactional precondition \( \lpre \);
\item
for any possible fingerprints  \( \fp \) satisfying the transactional postcondition \( \lpost \), there exists a world \( \w' \) satisfying the postcondition \( \gpost \) such that:
\begin{itemize}
\item 
the new key-value store in the new world \( \mkvs' \) is updated via committing the fingerprints \( \fp \) to \( \mkvs \);
\item
the new view \( \vi' \) is picked so that the update passes the execution test \( \ET \vdash (\mkvs,\vi) \csat \fp : \vi' \);
\item
and, the update is allowed by the guarantee \( (\w, \w') \in \Guar\).
\end{itemize}
\end{itemize}


\begin{figure}[t!]
\hrule\vspace{5pt}

\begin{mathpar}
    \inferrule[\rl{PRCommit}]{%
        \tripleL{\lpre}{\trans}{\lpost} 
        \\ \repartition{\gpre}{\gpost}{\lpre}{\lpost}
        \\\\ \stable{\gpre, \ET} 
        \\ \stable{\gpost, \ET} 
    }{%
        \tripleG{\gpre}{ \ptrans{\trans} }{\gpost}
    }
    \and
    \inferrule[\rl{PRPar}]{%
        \tripleG{ \gpre_{1} }{ \cmd_{1} }{ \gpost_{1} }
        \\ \tripleG{ \gpre_{2} }{ \cmd_{2} }{ \gpost_{2} } 
        \\\\ \stable{\gpre_{1}, \ET} 
        \\ \stable{\gpre_{2}, \ET} 
    }{%
        \tripleG{ \gpre_{1} \sep \gpre_{2} }{ \cmd_{1} \ppar \cmd_{2} }{ \gpost_{1} \sep \gpost_{2} }
    }
    \and
    \inferrule[\rl{PRAss}]{%
        \var \notin \func{fv}[\lexpr]
    }{%
        \tripleG{\var \dot= \lexpr }{ \passign{\var}{\expr} }{\var \dot= \expr\sub{\var}{\lexpr} }
    }
    \and
    \inferrule[\rl{PRAssume}]{ }{%
        \tripleG{ \expr \dot\neq 0 }{ \passume{\expr} }{ \expr \dot\neq 0 } 
    }
    \and
    \inferrule[\rl{PRChoice}]{%
        \tripleG{ \gpre }{ \cmd_{1} }{ \gpost } 
        \\ \tripleG{ \gpre }{ \cmd_{2} }{ \gpost } 
    }{%
        \tripleG{ \gpre }{ \cmd_{1} \pchoice \cmd_{2} }{ \gpost }
    }
    \and
    \inferrule[\rl{PRSeq}]{%
        \tripleG{ \gpre }{ \cmd_{1} }{ \gframe }
        \\ \tripleG{ \gframe }{ \cmd_{2} }{ \gpost }
    }{%
        \tripleG{ \gpre }{ \cmd_{1} \pseq \cmd_{2} }{ \gpost }
    }
    \and
    \inferrule[\rl{PRIter}]{%
        \tripleG{ \gpre }{ \cmd }{ \gpre } 
    }{%
        \tripleG{ \gpre }{ \cmd\prepeat }{ \gpre }
    }
    \and
    \inferrule[\rl{PRFrame}]{%
        \tripleG{ \gpre }{ \cmd }{ \gpost } 
        \\ \stable{\gframe, \ET}
        \\ \func{fv}[\gframe] \cap \func{modify}[\cmd] = \emptyset 
    }{%
        \tripleG{ \gpre \sep \gframe }{ \cmd }{ \gpost \sep \gframe }
    }
\end{mathpar}


\hrule\vspace{5pt}
\[
\begin{rclarray}
    \repartition{\gpre}{\gpost}{\lpre}{\lpost} & \defeq & 
    \begin{array}[t]{@{}l@{}}
        \fora{ \w, \mkvs, \vi, \lenv, \stk } 
        \w \in \evalW{\gpre} 
        \land (\mkvs, \vi) = \eraseW{\w}
        \implies  \\
        \quad \exsts{\sn_\lpre, \sn}
        \sn_\lpre \composeH \sn = \snapshot[\mkvs, \vi]
        \land (\sn, \unitO) \in \evalLS{\lpre}  \\
        \quad {} \land \fora{\w', \mkvs', \vi', \stk', \fp, \cl}  \\
        \qquad  (\stub, \fp) \in \evalLS[\lenv, \stk']{\lpost} 
        \land \mkvs' \in \updateKV[\mkvs, \vi, \cl, \fp] \\
        \qquad {} \land \ET \vdash (\mkvs, \vi) \csat \fp : \vi' 
        \land (\mkvs', \vi') = \eraseW{\w'} 
        \land (\w, \w') \in \Guar \\
        \qqqquad \implies \w' \in \evalW[\lenv, \stk']{\gpost}
    \end{array} 
\end{rclarray}                          
\]

\hrule\vspace{5pt}
\caption{The rules for programs}
\label{fig:rule-prog}
\end{figure}


==> logic/rule_graph.tex <==
\subsection{Rules for Local}

The proof rules are standard except \rl{TRDeref} and \rl{TRMutate}.
The \rl{TRDeref} rule add read fingerprint in finger-tracking set, only if there is no write finger-print.
This is because once a location has been re-written, the rest read are considered as local operations, while the finger-print only records those operations might have effect on global state.

\begin{figure}[t]
\hrule\vspace{5pt}
\sx{Need to be careful about the implication, esp. for fingerprint assertion.}
\[
    \infer[\rl{TRSkip}]{%
        \tripleL{\assemp }{ \pskip }{\assemp }
    }{}
\]

\[
    \infer[\rl{TRAss}]{%
        \tripleL{\txvar \dot= \lexpr }{ \passign{\txvar}{\expr} }{\txvar \dot= \expr\sub{\txvar}{\lexpr} }
    }{%
    \txvar \notin \func{fv}[\lexpr]
        && \txvar \in \TxVars  
    }
\]

\[
    \infer[\rl{TRDeref}]{%
        \tripleL{\expr \pt \lexpr \sep \fpF }{ \plookup{\txvar}{\expr} }{\txvar \dot= \lexpr \sep \expr \pt \lexpr \sep \fpto{\assfp'} }
    }{%
    \txvar \notin \func{fv}[\expr]
        && \txvar \notin \func{fv}[\lexpr]
        && \txvar \in \TxVars  
        && \assfp' = \assfp \addO (\otR, \expr, \lexpr)
    }
\]

\[
    \infer[\rl{TRMutate}]{%
        \tripleL{\expr_1 \pt \stub \sep \fpF }{ \pmutate{\expr_1}{\expr_2} }{ \expr_1 \pt \expr_2 \sep \fpto{\assfp'} } 
    }{
        \assfp' = \assfp \addO (\otW, \expr_{1}, \expr_{2})
    }
\]

\[
    \infer[\rl{TRAssume}]{%
        \tripleL{ \expr \doteq 0 }{ \passume{\expr} }{ \expr \doteq 0 } 
    }{}
\]

\[
    \infer[\rl{TRChoice}]{%
        \tripleL{ \lpre }{ \trans_{1} \pchoice \trans_{2} }{ \lpost }
    }{%
        \tripleL{ \lpre }{ \trans_{1} }{ \lpost } && 
        \tripleL{ \lpre }{ \trans_{2} }{ \lpost } 
    }
\]

\[
    \infer[\rl{TRSeq}]{%
        \tripleL{ \lpre }{ \trans_{1} \pseq \trans_{2} }{ \lpost }
    }{%
        \tripleL{ \lpre }{ \trans_{1} }{ \lframe }  && 
        \tripleL{ \lframe }{ \trans_{2} }{ \lpost }
    }
\]

\sx{check the loop invariant with fingerprint}

\[
    \infer[\rl{TRLoop}]{%
        \tripleL{ \lpre }{ \trans\prepeat }{ \lpre }
    }{%
        \tripleL{ \lpre }{ \trans }{ \lpre } 
    }
\]
 
\[
   \infer[\rl{TRFrame}]{%
       \tripleL{ \lpre \sep \lframe }{ \trans }{ \lpost \sep \lframe }
   }{%
       \tripleL{ \lpre }{ \trans }{ \lpost } 
   }
\]
\hrule\vspace{5pt}
\caption{The rules for transactions}
\label{fig:rule-trans}
 \end{figure}

\subsection{Rely and Guarantee}

\begin{definition}[Rely and guarantee]
\label{def:rely-guarantee}
The \( \func{allowed} \) function asserts that a event is allowed by the owned capabilities,
\[
\begin{rclarray}
    \func{allowed}[\fp, \ca, \gs] & \defeq & \fp = \unitE \\
    \func{allowed}[\fp \composeE \fp', \ca, \gs \uplus \Set{\rid \mapsto (\stub, \stub, \intf)}] & \defeq & 
    \exsts{\kap } \kap \sqsubseteq \ca(\rid)
    \land \fp \in \dom(\intf(\kap)) 
    \land \func{allowed}[\fp', \ca, \gs]
\end{rclarray}
\]
Given the set of worlds $\World$ (\cref{def:world}), the \emph{update rely} relation, $\relyU \subseteq \World \times \World$, is defined as follows,
\[	
    \begin{rclarray}
	\relyU & \defeq &
	\Set{
		((\ca, \gs), (\ca, \gs'))	
	}[
        \exsts{\fp,\aexec, \aexec'}  
        \func{allowed}[\fp, \ca, \gs]  \\
        \quad {} \land \aexec \in \clpsW{\gs} 
        \land \aexec' \in \clpsW{\gs'}
        \land (\aexec, \fp, \aexec') \in \func{transinv}[\gs]
	] \\
    \end{rclarray}
\]
The invariant of a shared state is a lift of the invariants of interferences of regions.
The \emph{rely} relation, $\RelyI \defeq \World \times \World$, is defined as follows:
\[
    \begin{rclarray}
         \RelyI &\defeq & \closure{\left(\relyU\right)} \\
    \end{rclarray}
\]
A set of fingerprint worlds $\setworld \subseteq \World$ is \emph{stable}, written $\stable{\setworld}$, if and only if it is closed under the rely relation: 
\[
    \begin{rclarray}
        \stable{\setworld} & \defeq & \fora{\w_{p}, \w_{q}}  \w_{p} \in \setworld \land (\w_{p}, \w_{q}) \in \RelyI \implies \w_{q} \in \setworld
    \end{rclarray}
\]
The \emph{update guarantee} relation, $\guarU: \World \times \World$, is defined as follows:
\[	
    \begin{rclarray}
	\guarU & \defeq &
	\Set{
		((\ca, \gs), (\ca, \gs'))	
	}[
        \exsts{\fp, \ca', \aexec, \aexec'}  
        (\ca' \composeC \ca)\isdef
        \land \func{allowed}[\fp, \ca, \gs]  \\
        \quad {} \land \aexec \in \clpsW{\gs} 
        \land \aexec' \in \clpsW{\gs'}
        \land (\aexec, \fp, \aexec') \in \func{transinv}[\gs]
	] \\
    \end{rclarray}
\]
The \emph{guarantee} relation, $\GuarI \subseteq \World \times \World$, is defined as follows:
\sx{take away of the closure}
\[
	\GuarI \defeq \guarU
\]
\end{definition}

\subsection{Rules for Global}

The \rl{PRCommit} rule lifts the local effect of transaction \( \trans \) to global level by first converting global state to (local) observable state and then propagating the local fingerprint to the global state.
The \( \pred{down} \) predicate asserts that the local predicate \( \lpre \) is a over-approximation of the valid observation that is given by the interference.
The \( \pred{up} \) predicate says the post-condition \( \gpost \) is the result by lifting the local fingerprints \( \assfp \) to pre-condition \( \gpre \).



\begin{figure}[t!]
\hrule\vspace{5pt}

\sx{not right, we want to say a transaction \( \trans \) can be abstracted to a fingerprint \( \assfp \)}

\[
    \infer[\rl{PRCommit}]{%
        \tripleG{\gpre}{ \ptrans{\trans} }{\gpost}
    }{%
        \begin{array}{c}
        \gpre \snap \lpre
        \quad \tripleL{\lpre \sep \fpass{}}{\trans}{\lpost \sep \fpF}
        \quad \rpt{\gpre}{\gpost}{\assfp} \\
        \stable{\gpre} 
        \quad \stable{\gpost} 
        \end{array}
    }
\]

\[
    \infer[\rl{PRAss}]{%
        \tripleG{\var \dot= \lexpr }{ \passign{\var}{\expr} }{\var \dot= \expr\sub{\var}{\lexpr} }
    }{%
        \var \notin \func{fv}[\lexpr]
        && \var \in \ThdVars  
    }
\]

\[
    \infer[\rl{PRAssume}]{%
        \tripleG{ \expr \doteq 0 }{ \passume{\expr} }{ \expr \doteq 0 } 
    }{}
\]

\[
    \infer[\rl{PRChoice}]{%
        \tripleG{ \gpre }{ \prog_{1} \pchoice \prog_{2} }{ \gpost }
    }{%
        \tripleG{ \gpre }{ \prog_{1} }{ \gpost } && 
        \tripleG{ \gpre }{ \prog_{2} }{ \gpost } 
    }
\]

\[
    \infer[\rl{TRSeq}]{%
        \tripleG{ \gpre }{ \prog_{1} \pseq \prog_{2} }{ \gpost }
    }{%
        \tripleG{ \gpre }{ \prog_{1} }{ \gframe }  && 
        \tripleG{ \gframe }{ \prog_{2} }{ \gpost }
    }
\]

\[
    \infer[\rl{TRLoop}]{%
        \tripleG{ \gpre }{ \prog\prepeat }{ \gpre }
    }{%
        \tripleG{ \gpre }{ \prog }{ \gpre } 
    }
\]
 
\[
   \infer[\rl{TRFrame}]{%
       \tripleG{ \gpre \sep \gframe }{ \prog }{ \gpost \sep \gframe }
   }{%
       \tripleG{ \gpre }{ \prog }{ \gpost } 
   }
\]
 
\[
   \infer[\rl{TRPar}]{%
       \tripleG{ \gpre_{1} \sep \gpre_{2} }{ \prog_{1} \ppar \prog_{2} }{ \gpost_{1} \sep \gpost_{2} }
   }{%
       \tripleG{ \gpre_{1} }{ \prog_{1} }{ \gpost_{1} }
       && \tripleG{ \gpre_{2} }{ \prog_{2} }{ \gpost_{2} }
   }
\]

\[
\begin{rclarray}
    \gpre \snap \lpre & \defeq & \fora{ \w, \sn } \w \in \evalW{\gpre} \land \pred{takeinv}{\w, \sn} \implies \sn \in \evalLS{\lpre}\\
    \pred{takeinv}{\gs, \sn} & \defeq & \gs = \emptyset \land \sn = \unitH \\
    \pred{takeinv}{\Set{\rid \mapsto (\stub, \snset, \intf)} \uplus \gs, \sn \composeH \sn'} & \defeq & \sn \in \snset \land \pred{takeinv}{\gs,\sn'}\\
    \rpt{\gpre}{\gpost}{\assfp} & \defeq & 
    \begin{array}[t]{@{}l@{}}
        \fora{\w, \w', \aexec, \aexec'} \\
        \quad \w \in \evalW{\gpre}
        \land \aexec \in \clpsW{\w}
        \land \func{reachable}{\aexec, \aexec', \stub, \evalF{\assfp}, \ET}  \\
        \quad {} \land \aexec' \in \clpsW{\w'}
        \land (\w, \w') \in \Guar 
        \implies \w' \in \evalW{\gpost}
    \end{array} \\
\end{rclarray}                          
\]

\sx{
    For LLW the propagate can be done by syntactically update those addresses that has been written.
}

\hrule\vspace{5pt}
\caption{The rules for programs}
\label{fig:rule-prog}
\end{figure}

Many consistency model use last write win resolution policy, such as snapshot isolation, therefore the repartition \( \rpt{\gpre}{\gpost}{\assfp} \) can be simplified by checking the guarantee and then syntactically propagating the write fingerprints.
Also in practice, many implementation of consistency model assume strong session constraint.

\begin{figure}
\hrule\vspace{5pt}

\[
   \infer[\rl{FRead}]{%
       \tripleF{ \lexpr \pt \lexpr' \mid \lexpr \pt \lexpr'' }{ \Set{(\otR, \lexpr, \lexpr'')} }{ \lexpr \pt \lexpr' \mid \lexpr \pt \lexpr''}
   }{}
\]

\[
   \infer[\rl{FWriteNS}]{%
       \tripleF{ \lexpr \pt \lexpr' \mid \lexpr \pt \lexpr'' }{ \Set{(\otW, \lexpr, \lexpr''')} }{ \lexpr \pt \lexpr''' \mid ( \lexpr \pt \lexpr'' \lor \lexpr \pt \lexpr''') }
   }{}
\]

\[
   \infer[\rl{FWriteS}]{%
       \tripleF{ \lexpr \pt \lexpr' \mid \lexpr \pt \lexpr'' }{ \Set{(\otW, \lexpr, \lexpr''')} }{ \lexpr \pt \lexpr''' \mid \lexpr \pt \lexpr'''}
   }{}
\]

\[
   \infer[\rl{FFrame}]{%
       \tripleF{ \lpre \sep \lframe  \mid \lpre' \sep \lframe' }{ \assfp }{ \lpost \sep \lframe \mid \lpost' \sep \lframe' }
   }{%
       \tripleF{ \lpre \mid \lpre' }{ \assfp }{ \lpost \mid \lpost' }
   }
\]

\[
   \infer[\rl{FContinue}]{%
       \tripleF{ \lpre \sep \lframe  \mid \lpre' \sep \lframe' }{ \assfp  \uplus \assfp' }{ \lpost \sep \lframe \mid \lpost' \sep \lframe' }
   }{%
       \tripleF{ \lpre \sep \lframe  \mid \lpre' \sep \lframe' }{ \assfp }{ \lpost \sep \lframe \mid \lpost' \sep \lframe' }
   }
\]

\[
\begin{rclarray}
    \rpt{\gpre}{\gpost}{\assfp} & \defeq & 
    \begin{array}[t]{@{}l}
    \fora{\w, \w', \sn, \sn', \lpre, \lpre', \lpost, \lpost'}
    \w \in \evalW{\gpre} \\
    \quad {} \land \pred{unbox}{\w\projection{2}, \sn}
    \land \sn \in \evalLS{\lpre} 
    \land \gpre \snap \lpre' \\
    \quad {} \land {} \tripleF{ \lpre \mid \lpre' }{ \assfp }{ \lpost | \lpost'} \\
    \quad {} \land \pred{unbox}{\w'\projection{2},\sn'}
    \land \sn' \in \evalLS{\lpost} 
    \land \gpost \snap \lpost' \\
    \quad \implies \w' \in \evalW{\gpost}
    \end{array} \\
    \pred{unbox}{\gs, \sn} & \defeq & \gs = \emptyset \land \sn = \unitH \\
    \pred{unbox}{\Set{\rid \mapsto (\sn, \stub, \stub)} \uplus \gs, \sn \composeH \sn' } & \defeq & \pred{unbox}{\gs, \sn'} \\
\end{rclarray}
\]

\hrule\vspace{5pt}
\caption{Simplified repartition for last write win}
\label{fig:rule-prog}
\end{figure}



==> logic/trans_sound.tex <==
\subsection{Transaction Soundness}

The \cref{thm:transaction-soundness} is the soundness of for transactions, where the most interesting two rules \rl{TRLookup} and \rl{TRMutate} can be derived from the \cref{lem:fingerprint-op}.
Note that the transactional semantics is defined on snapshots as total functions.
Thus in the \cref{thm:transaction-soundness}, it is safe to extend \( h \) with \( \sn'' \)  to make the snapshot a total function, as there is no allocation and deallocation.

\begin{theorem}[Transaction soundness]
\label{thm:transaction-soundness}
The transaction soundness is as follows:
\[
    \begin{array}{@{}l@{}}
        \fora{ \lpre, \trans, \lpost } \tripleL{\lpre}{\trans}{\lpost}
        \implies 
        \fora{\lenv, \stk, \stk', \sn_\lpre, \sn_\lpost, \sn \fp, \fp' }  \\
        \quad (\sn_\lpre, \fp) \in \evalLS[\lenv, \stk]{\lpre}
        \land \dom(\sn) = \Keys \setminus \dom(\sn) \\
        \quad {} \land \vdash (\stk, \sn_\lpre \composeH \sn, \fp ), \trans \toTRANS^{*}  (\stk', \sn_\lpost \composeH \sn, \fp' ), \pskip  \\
        \qqquad \implies (\sn', \fp') \in \evalLS[\lenv, \stk']{\lpost}
    \end{array}
\]
\end{theorem}
\begin{proof}
Induction on the derivations.

\begin{itemize}

\item \caseB{\rl{TRSkip}}
We have \(\trans \equiv \pskip\), \( \lpre \equiv \lpost \equiv \assemp \), thus \( \sn_{p} = \sn_{q} = \unitH \), \( \fp = \fp' \) and \( \stk = \stk' \), and then \( (\unitH,\unitO ) \in \evalLS[\lenv, \stk']{\assemp} \) holds.

\item \caseB{\rl{TRAss}}
We have \(\trans \equiv ( \passign{\var}{\expr} ) \), \( \lpre \equiv ( \var \doteq \lexpr ) \) and \( \lpost \equiv ( \var \doteq \expr\sub{\var}{\lexpr} ) \) 
for some \( \expr, \lexpr \) and \( \var \) such that \( \var \notin \func{fv}{\lexpr}\).
Given the transaction semantics (\cref{fig:thread_semantics}), it has \( \stk' = \stk\rmto{\var}{\val} \) where \( \val = \evalLE[\lenv, \stk]{\expr\sub{\var}{\lexpr}} \).
Since \( \var \notin \func{fv}{\lexpr} \), we know \( \evalLE[\lenv, \stk]{\lexpr} = \evalLE[\lenv, \stk']{\lexpr} \), and then \( \evalLE[\lenv, \stk]{\expr\sub{\var}{\lexpr}} = \evalLE[\lenv, \stk']{\expr\sub{\var}{\lexpr}} \).
This means the assertions related to stack hold even thought the stack changes.
Also because the snapshot and fingerprint remain unchanged, \ie \( \sn = \sn' \) and \( \fp = \fp' \), so we prove \( (\sn', \fp' ) \in \evalLS[\lenv, \stk']{\lpost} \).

\item \caseB{\rl{TRLookup}}
We have \(\trans \equiv ( \plookup{\var}{\expr} ) \) and four cases for pre- and post-conditions defined by the relation \( \toFP{\otR(\expr, \lexpr)}\).
In all the four cases, the stack is updated to \( \stk' = \stk\rmto{\var}{\val} \), yet since \( \var \notin \func{fv}{\lexpr}\), the logical value \( \lexpr \) and new logical address \( \expr\sub{\var}{\lexpr}\) are evaluated to the same value \( \val \) and address \( \key \) as before.
By \cref{lem:appendix-fingerprint-op}, we know that the final state of snapshot and fingerprint satisfy the postcondition.

\item \caseB{ \rl{TRMutate} }
We have  \( \trans \equiv (\pmutate{\expr_{1}}{\expr_{2}}) \) and four cases for pre- and post-conditions defined by the relation \( \toFP{\otW(\expr, \lexpr)}\). 
In all the four cases, the stack remains untouched and  by \cref{lem:appendix-fingerprint-op} the snapshot and fingerprint match the postcondition.

\item \caseI{\rl{TRChoice}}
We have  \(\trans \equiv \trans_{1} + \trans_{2} \), where \( \tripleL{\lpre}{\trans_{1}}{\lpost} \) and \( \tripleL{\lpre}{\trans_{2}}{\lpost} \) hold, for some \( \trans_{1}, \trans_{2}, \lpre, \lpost \).
Given the transaction semantics (\cref{fig:thread_semantics}), it either has 
\[ 
( \stk, \sn_\lpre \composeH \sn, \fp ), \trans_{1} \pchoice \trans_{2} \toTRANS ( \stk, \sn_\lpre \composeH \sn, \fp ), \trans_{1} 
\]
or  
\[ 
( \stk, \sn_\lpre \composeH \sn, \fp ), \trans_{1} \pchoice \trans_{2} \toTRANS ( \stk, \sn_\lpre \composeH \sn, \fp ), \trans_{2} 
\]
Let us pick \( \trans_{1} \) and  assume it can be reduced to \( \pskip \) from the initial state, \ie \( ( \stk, \sn_\lpre \composeH \sn, \fp ), \trans_{1}  \toTRANS^{*} ( \stk', \sn', \fp' ), \pskip \).
By the premiss of the rule \( \tripleL{\lpre}{\trans_{1}}{\lpost} \) and the \ih, 
there exists a \( \sn_\lpost \) such that \( \sn' = \sn_\lpost \composeH \sn \) and  \( (\sn_\lpost, \fp') \in \evalLE[\lenv, \stk']{\lpost} \).
Symmetrically, if we pick \( \trans_{2} \), it gives the same result.

\item \caseI{\rl{TRSeq}}
We have \( \trans \equiv \trans_{1} \pseq \trans_{2} \) where \( \tripleL{\lpre}{\trans_{1}}{\lframe} \) and \( \tripleL{\lframe}{\trans_{2}}{\lpost} \) hold, for some \( \trans_{1}, \trans_{2}, \lpre, \lpost, \lframe \).
Given the transaction semantics (\cref{fig:thread_semantics}), 
it has 
\[
    \begin{array}{l}
    \vdash ( \stk, \sn_\lpre \compose \sn, \fp ), \trans_{1} \pseq \trans_{2} \toTRANS^{*} ( \stk'', \sn'', \fp'' ), \pskip \pseq \trans_{1} \\
    \qqquad \toTRANS ( \stk'', \sn'', \fp'' ), \trans_{1} \toTRANS^{*} ( \stk', \sn', \fp' ), \pskip 
\end{array}
\] 
for a residue \( \sn \) and  some states \( (\stk', \sn', \fp'), (\stk'', \sn'', \fp'') \).
By the \ih that \( \tripleL{\lpre}{\trans_{1}}{\lframe} \) is sound,
there exists a snapshot \( \sn_\lframe \) such that \( \sn'' = \sn_\lframe \composeH \sn \) and \( (\sn_\lframe, \fp'') \in \evalLE[\lenv, \stk'']{\lframe} \).
The elimination of prefix \( \pskip \) does not change the state, so \( (\sn'', \fp'') \in \evalLE[\lenv, \stk'']{\lframe} \).
Then similarly, 
By the \ih that \( \tripleL{\lframe}{\trans_{2}}{\lpost} \) is sound,
there exists a snapshot \( \sn_\lpost \) such that \( \sn'' = \sn_\lpost \composeH \sn \) and \( (\sn_\lpost, \fp') \in \evalLE[\lenv, \stk']{\lpost} \).

\item \caseI{\rl{TRLoop}}
Since the triple is only partial correct, 
meaning that only when the transaction \( \trans \) terminates, it will reach a state satisfying the post-condition \( \lpost \).
It is sufficient to prove the following is sound:
\[
    \fora{\lpre, \trans, \nat > 0} \tripleL{\lpre}{\trans^{\nat}}{\lpre}
\]
where,
\[
    \trans^{0} \defeq  \pskip \qquad
    \trans^{\nat} \defeq  \trans \pseq \trans^{\nat - 1} 
\]

We prove that by induction on the number \( \nat \).
\begin{itemize}
    \item \caseB{\( \nat = 0 \)} It has been proven before \( \triple{\lpre}{\pskip}{\lpre} \).
    \item \caseI{\( \nat > 0 \)} We have 
    \[ 
        \begin{array}{l}
        \vdash (\stk, \sn_\lpre \composeH \sn, \fp), \trans \pseq \trans^{\nat - 1} \toTRANS^{*} \\
        \qqquad (\stk'', \sn'', \fp''), \trans^{\nat - 1} \toTRANS^{*} (\stk', \sn', \fp'), \pskip  
        \end{array}
    \]
    for a residue \( \sn \) and some states \( ( \stk', \sn', \fp' ), ( \stk'', \sn'', \fp'' ) \).
    This is similar to the \rl{PSeq} case.
\end{itemize}

\item \caseI{\rl{TRFrame}}
We need to prove \( \tripleL{\lpre \sep \lframe }{\trans}{\lpost \sep \lframe} \) is sound, 
given the soundness of  \( \tripleL{\lpre}{\trans}{\lpost} \).
Assume snapshots \( \sn_\lpre, \sn_\lpost, \sn_\lframe \), fingerprints \( \fp, \fp', \fp'' \) and stacks\( \stk, \stk' \) 
such that \( ( \sn_\lpre, \fp ) \in \evalLS[\lenv, \stk]{\lpre} \), \( ( \sn_\lframe, \fp' ) \in \evalLS[\lenv, \stk']{\lpost} \) and \( ( \sn_\lpost, \fp'' ) \in \evalLS[\lenv, \stk]{\lframe}\).
Since \( \lpre \sep \lframe \), the component-wise composition is defined, \ie \( (\sn_\lpre \composeH \sn_\lframe, \fp \composeO \fp'') \in \evalLS[\lenv, \stk]{\lpre \sep \lframe} \).
The keys from the snapshots and fingerprints are disjointed.
By the hypothesis that \( \tripleL{\lpre}{\trans}{\lpost} \) is sound, 
we know \( ( \stk, \sn_\lpre \composeH \sn, \fp ), \trans \toTRANS^{*} ( \stk', \sn_\lpost \composeH \sn, \fp' ), \pskip \) for some residues \( \sn \).
The snapshot after the execution contains the same resources as before, that is \( \dom(\sn_\lpre) = \dom(\sn_\lpost) \) and \( \dom(\fp') \subseteq \dom(\sn_\lpost) \).
We know the composition of \( \sn_\lpost \composeH \sn_\lframe \) and \( \fp' \composeO \fp''\) exists, 
so 
\[ 
    ( \stk, \sn_\lpre \composeH \sn_\lframe \composeH \sn', \fp \composeO \fp''), \trans \toTRANS^{*} ( \stk', \sn_\lpost \composeH \sn_\lframe \composeH \sn', \fp' \composeO \fp'' ), \pskip 
\]
for some residues \( \sn' \).
Note that \( \dom(\sn_\lframe \composeH \sn') = \dom(\sn) \).
Finally, because the transaction \( \trans \) does not modify any variable from the frame \( \lframe \), 
the update of stack does not change the evaluation of the frame, 
\( \evalLS[\lenv, \stk]{\lframe} = \evalLS[\lenv, \stk']{\lframe} \) which then gives us the result \( (\sn_\lpost \composeH \sn_\lframe, \fp' \composeO \fp'') \in \evalLS[\lenv, \stk']{\lpost \sep \lframe} \).
\end{itemize}
\end{proof}

\begin{lemma}
\label{lem:fingerprint-op}
\label{lem:appendix-fingerprint-op}
For \( \mathtt{O} \in \Set{\otR, \otW} \), the relation \( \toFP{\mathtt{O}(\key,\val')}\) is sound with respect to the operator \( \addO \):
\[
\begin{array}{@{}l}
    \fora{\lpre, \lpost, \lenv, \stk, \stk', \fp, \fp', \mathtt{O}, \key, \val} \\
    \quad \mathtt{O} \in \Set{\otR, \otW} 
    \land \lpre \toFP{\mathtt{O}(\key,\val)} \lpost
    \land (\stub, \fp) \in \evalLS{\lpre}
    \land (\stub, \fp') \in \evalLS{\lpost} \\
    \qqquad \implies \fp' = \fp \addO (\mathtt{O}, \key, \val)
\end{array}
\]
\end{lemma}
\begin{proof}
\begin{itemize}
    \item In this case, a read operation is added \( \fp' = \Set{(\otR, \key, \val)} \) and it is included in the interpretation of the post condition \( \lpost \equiv \key \fpR \val \).
If \( \lpre \equiv \key \fpR \val \) and \( \lpost \equiv \key \fpR \val \), 
since there is already a read operation in the fingerprint, adding a new read operation does not change the fingerprint, \ie \( \fp' = \Set{(\otR, \key, \val)} \addO (\otR, \key, \val ) = \Set{(\otR, \key, \val)} \).
This is exactly the post-condition.
It is sound for the rest two cases that  when \( \lpre \equiv \key \fpW \val \) and \( \lpost \equiv \key \fpW \val \), and when \( \lpre \equiv \key \fpRW (\lexpr,\val) \) and \( \lpost \equiv \key \fpRW (\lexpr,\val) \), as the fingerprint remains the same in the rest two cases.

\item When \( \mathtt{O} = \otW\), we also have four cases for pre- and post-conditions.
If \( \lpre \equiv \key \fpI \val' \) for some value \( \val' \), a new write operation is added to the initially empty fingerprint, that is, \( \fp' = \Set{(\otW, \key, \val)}\).
This is exactly the post-condition \( \lpost \equiv \key \fpW \val \).
If \( \lpre \equiv \key \fpW \val' \) for some \( \val' \), the fingerprint before execution is \( \fp = \Set{(\otW, \key, \val')}\).
Since the fingerprint only has the last write for the key because of the property of the \( \addO \) operator,
the fingerprint after is \( \fp' = \fp \addO (\otW, \key, \val) = \Set{(\otW, \key, \val)}\) which satisfies the postcondition \( \lpost \equiv \expr_{1} \fpW \expr_{2} \).
The remaining two cases follow the same argument as the fingerprint only have the last write.
\end{itemize}
\end{proof}


==> logic/transaction.tex <==
\subsection{Reasoning inside transactions}
\label{sec:reasoning-transaction}

Recall that a transaction takes a snapshot of the kv-store and commits the fingerprint by the end.
Because of the atomicity, only the \emph{first reads preceding any write} and the \emph{last writes} of keys are contained in the fingerprint.
All the intermediate reads and writes are not observable to other transactions and have no effect on the key-value store.
To capture the state of the local snapshot as well as the fingerprint, 
the \emph{transactional assertions} (\cref{def:local_assertions}) extend normal sequential separate logic assertions with read and/or write labels, 
\eg \( \vx \fpR 0 \), \( \vy \fpW 1 \) and \( \pv{z} \fpRW (0,1) \).


\begin{definition}[Transactional assertions]
\label{def:fingerprint-assertion}
\label{def:local_assertions}
\label{def:logical-expr}
Assume a countably infinite set of \emph{logical variables} $\lvar \in \LVar$.
The set of \emph{logical expressions} $\lexpr \in \LExpr$ is defined by the inductive grammar:
\(
\begin{rclarray}
   \lexpr & ::= & \val \mid \lvar \mid \var \mid \lexpr + \lexpr \mid  \dots 
\end{rclarray}
\)
where \(\val \in \Val\)  and \(\var \in \Vars\).
The \emph{logical expression evaluation} function, $\evalLE[(., .)]{.}:\LExpr \times \Stacks \times \LEnv\rightharpoonup \Val$, is defined inductively over the structure of logical expressions,
where the \emph{logical environments} \(\lenv \in \LEnv: \LVar \parfun \Val\) associates logical variables with values:
%
\[
\begin{array}{@{}c@{}}
    \begin{rclarray}
        \evalLE{\val} & \defeq & \val \\
    \end{rclarray}
    \quad
    \begin{rclarray}
        \evalLE{\lvar} & \defeq & \lenv(\lvar) \\
    \end{rclarray}
    \quad
    \begin{rclarray}
        \evalLE{\var} & \defeq & \stk(\var) \\
    \end{rclarray} 
    \quad
    \begin{rclarray}
        \evalLE{\lexpr_1 + \lexpr_2} & \defeq & \evalLE{\lexpr_1} + \evalLE{\lexpr_2} \\
    \end{rclarray}
    \dots
\end{array}
\]
The set of \emph{transactional assertions}, $\lpre,  \lpost \LAst$, is defined by the following grammars:
\[
\begin{rclarray}
	\assfp & ::= & \lexpr \fpI \lexpr \mid \lexpr \fpR \lexpr \mid \lexpr \fpW \lexpr \mid \lexpr \fpRW (\lexpr, \lexpr)  \\
	\lpre, \lpost & ::= & \assfalse \mid \asstrue \mid \lpre \land \lpost \mid \lpre \lor \lpost \mid \exsts{\lvar} \lpre \mid \lpre \implies \lpost
    \mid \assemp \mid \assfp \mid \lpre \sep \lpost  \\
\end{rclarray}	 
\]
The \emph{transactional assertion interpretation function}, $\evalLS[(.,.)]{.}: \LAst \times \LEnv \times \LAst \parfun \pset{\Snapshots \times \Fingerprints} $, is defined over the structure of local assertions, where the composition for snapshots \( \composeH \defeq \uplus \) is standard disjointed union on two functions and the composition for fingerprints \( \fp \composeO \fp' \defeq \fp \uplus \fp'\) when they contain different keys, \ie \( \fp\projection{2} \cap \fp'\projection{2} = \emptyset\):
\[
\begin{rclarray}
	\evalLS{\assfalse} & \defeq & \emptyset \\
	\evalLS{\asstrue} & \defeq & \Snapshots \times \Fingerprints \\
	\evalLS{\lpre \land \lpost} & \defeq & \evalLS{\lpre} \cap \evalLS{\lpost} \\
	\evalLS{\lpre \lor \lpost} & \defeq & \evalLS{\lpre} \cup \evalLS{\lpost} \\
	\evalLS{\exsts{\lvar} \lpre} & \defeq & \bigcup_{\val \in \textnormal{\Val}}\evalLS[\lenv\rmto{\lvar}{\val}, \stk]{\lpre}  \\
	\evalLS{\lpre \implies \lpost} & \defeq & \Setcon{(\sn, \fp)}{(\sn , \fp) \in \evalLS{\lpre} \implies (\sn , \fp) \in \evalLS{\lpost}}\\
	\evalLS{\assemp} & \defeq & \Set{ ( \unitH, \unitE) }  \\
	\evalLS{ \lexpr_1 \fpI \lexpr_2 } & \defeq & \Set{\left(\Set{\evalLE{\lexpr_1} \mapsto \evalLE{\lexpr_2} }, \unitO\right)} \\
	\evalLS{ \lexpr_1 \fpR \lexpr_2 } & \defeq & \Set{\left(\Set{\evalLE{\lexpr_1} \mapsto \evalLE{\lexpr_2} }, \Set{(\otR, \evalLE{\lexpr_1},\evalLE{\lexpr_2})}\right)} \\
	\evalLS{ \lexpr_1 \fpW \lexpr_2 } & \defeq & \Set{\left(\Set{\evalLE{\lexpr_1} \mapsto \evalLE{\lexpr_2} }, \Set{(\otW, \evalLE{\lexpr_1},\evalLE{\lexpr_2})}\right)} \\
	\evalLS{ \lexpr_1 \fpRW (\lexpr_2, \lexpr_3) } & \defeq & \Set{\left(\Set{\evalLE{\lexpr_1} \mapsto \evalLE{\lexpr_3} }, \Set{(\otR, \evalLE{\lexpr_1},\evalLE{\lexpr_2}), \\ \quad (\otW, \evalLE{\lexpr_1},\evalLE{\lexpr_3})}\right)} \\
	\evalLS{\lpre \sep \lpost} & \defeq & 
    \Setcon{
        (\sn_1 \composeH \sn_2, \fp_{1} \composeE \fp_{2})
    }{ 
        (\sn_{1},\fp_{1}) \in \evalLS{\lpre} 
        \land (\sn_{2}, \fp_{2} ) \in \evalLS{\lpost} 
    } 
\end{rclarray}%
\]
\end{definition}

The \emph{transactional assertions} (\cref{def:local_assertions}) have \( \assfalse \), \(\asstrue \), conjunction \( \land \), disjunction \( \lor \), existential quantification \( \exists \), implication \( \implies  \), empty \( \assemp \), fingerprint assertions \( \stub \stackrel{\stub}{\hookrightarrow} \stub \) and separation conjunction \( \sep \).
They describes the state of local snapshot used by a transaction and more importantly the fingerprint of the transaction.
They are interpreted to pairs of snapshots and fingerprints.

A \emph{fingerprint assertion} describes the possible global effect from a transaction.
It includes the default \(\lexpr_{1} \fpI \lexpr_{2} \), the \emph{first read preceding any write} \( \lexpr_{1} \fpR \lexpr_{2} \), \emph{last write} \( \lexpr_{1} \fpW \lexpr_{2} \) for the key \( \lexpr_{1} \) and the combination of them \( \lexpr_{1} \fpRW \lexpr_{2} \).
The \( \lexpr_{1} \fpI \lexpr_{2} \) means the only key \( \lexpr_{1} \) in the local snapshot has value \( \lexpr_{2} \),
and the key has no associated fingerprint.
The \( \lexpr_{1} \fpR \lexpr_{2} \) means the key has been read before any other write carrying value \( \lexpr_{2} \) and the current value for the key is also \( \lexpr_{2} \).
The \( \lexpr_{1} \fpW \lexpr_{2} \) means the key has been written at least once, and the last written value is \( \lexpr_{2} \).
Because read does not change the state of snapshot, and the write fingerprint corresponds to the last write for the key,
so the state of the snapshot matches the fingerprint for cases \( \lexpr_{1} \fpR \lexpr_{2} \) and  \( \lexpr_{1} \fpW \lexpr_{2} \).
Last, The combined fingerprint \( \lexpr_{1} \fpRW (\lexpr_{2}, \lexpr_{3}) \) means the key has been read and then written at least once, the first read fetched value \( \lexpr_{2} \), and the last written value and the current state of the local snapshot for the key are both \( \lexpr_{3} \).

Other transactional assertions have standard interpretations.
Note that the separation conjunction \( \sep \) asserts two local snapshots and fingerprints when the keys are disjointed.
Observe that program expressions $\Expr$ (\cref{fig:semantics}) are contained in logical expressions $\LExpr$ (\cref{def:local_assertions}), \ie $\Expr \subset \LExpr$. 

The proof rules for transactions (\cref{fig:rule-trans}) are standard except \rl{TRLookup} and \rl{TRMutate}.
The \rl{TRLookup} rule adds read label only if there is no write label.
Because once a key has been written, the following reads are local to the transaction.
However, the local read always needs to match the current state of snapshot.
Especially for the case when the precondition is \( \lexpr \fpRW (\lexpr'', \lexpr') \),
the current state of the key is the last written value \( \lexpr' \).
The\rl{TRMutate} rule changes the state of the key and more importantly adds write label.
For the case when the precondition is \( \lexpr \fpRW (\lexpr'', \lexpr') \), 
the rule changes the value \( \lexpr' \) to the new written value \( \lexpr''' \)
but keeps the old read value \( \lexpr'' \) the same.

\begin{figure}[!t]
\sx{Font for E}
\hrule
\begin{mathpar}
    \inferrule[\rl{TRLookup}]{%
        \var \notin \func{fv}{\lexpr}  
        \\ \lpre \toFP{\otR(\expr, \lexpr)} \lpost
    }{%
        \tripleL{ \lpre }{ \plookup{\var}{\expr} }{\var \dot= \lexpr \sep \lpost\sub{\var}{\lexpr} }
    }
    \and
    \inferrule[\rl{TRMutate}]{
        \lpre \toFP{\otW(\expr_{1},\expr_{2})} \lpost
    }{%
        \tripleL{ \lpre }{ \pmutate{\expr_1}{\expr_2} }{ \lpost } 
    }
    \and
    \inferrule[\rl{TRAss}]{
        \var \notin \func{fv}{\lexpr}
    }{%
        \tripleL{\var \dot= \lexpr }{ \passign{\var}{\expr} }{\var \dot= \expr\sub{\var}{\lexpr} }
    }
    \and
    \inferrule[\rl{TRAssume}]{ }{%
        \tripleL{ \expr \dot\neq 0 }{ \passume{\expr} }{ \expr \dot\neq 0 } 
    }
    \and
    \inferrule[\rl{TRChoice}]{%
        \tripleL{ \lpre }{ \trans_{1} }{ \lpost } 
        \\ \tripleL{ \lpre }{ \trans_{2} }{ \lpost } 
    }{%
        \tripleL{ \lpre }{ \trans_{1} \pchoice \trans_{2} }{ \lpost }
    }
    \and
    \inferrule[\rl{TRSeq}]{%
        \tripleL{ \lpre }{ \trans_{1} }{ \lframe }
        \\ \tripleL{ \lframe }{ \trans_{2} }{ \lpost }
    }{%
        \tripleL{ \lpre }{ \trans_{1} \pseq \trans_{2} }{ \lpost }
    }
    \and
    \inferrule[\rl{TRIter}]{%
        \tripleL{ \lpre }{ \trans }{ \lpre } 
    }{%
        \tripleL{ \lpre }{ \trans\prepeat }{ \lpre }
    }
    \and
    \inferrule[\rl{TRFrame}]{%
        \tripleL{ \lpre }{ \trans }{ \lpost } \and \func{fv}{\lframe} \cup \func{modify}{\trans} = \emptyset
    }{% 
        \tripleL{ \lpre \sep \lframe }{ \trans }{ \lpost \sep \lframe }
    }
\end{mathpar}


\hrule
\[
\begin{array}{@{} c @{\qquad} c @{}}
\begin{rclarray}
    \lexpr \fpI \lexpr' & \toFP{\otR(\lexpr,\lexpr')} & \lexpr \fpR \lexpr' \\
    \lexpr \fpR \lexpr' & \toFP{\otR(\lexpr,\lexpr')} & \lexpr \fpR \lexpr' \\
    \lexpr \fpW \lexpr' & \toFP{\otR(\lexpr,\lexpr')} & \lexpr \fpW \lexpr' \\
    \lexpr \fpRW (\lexpr'', \lexpr') & \toFP{\otR(\lexpr,\lexpr')} & \lexpr \fpRW (\lexpr'', \lexpr') \\
\end{rclarray}
&
\begin{rclarray}
    \lexpr \fpI \lexpr' & \toFP{\otW(\lexpr,\lexpr'')} & \lexpr \fpW \lexpr'' \\
    \lexpr \fpR \lexpr' & \toFP{\otW(\lexpr,\lexpr'')} & \lexpr \fpRW (\lexpr',\lexpr'') \\
    \lexpr \fpW \lexpr' & \toFP{\otW(\lexpr,\lexpr'')} & \lexpr \fpW \lexpr'' \\
    \lexpr \fpRW (\lexpr'', \lexpr') & \toFP{\otW(\lexpr,\lexpr''')} & \lexpr \fpRW (\lexpr'', \lexpr''') \\
\end{rclarray}
\end{array}
\]
\hrule
\caption{The rules for transactions}
\label{fig:rule-trans}
 \end{figure}




==> semantics/op-semantics.tex <==
\section{Operational Semantics of Key-Value Stores}

We define a simple programming language for client programs interacting with a kv-store.
Clients may only interact with a kv-store by issuing read and write requests via transactions. 
For simplicity, we abstract away from aborting transactions:
rather than assuming a transaction may abort due to a violation of the consistency guarantees given by the kv-store,
we only allow a transaction to execute if its effects are guaranteed to not violate the consistency model. 
This emulates the setting in which clients always restart a transaction if it aborts.


\subsubsection{Programming Language}

\emph{A program} \( \prog \) comprises a finite number of clients,
where each client is associated with a unique identifier \( \cl \in \Clients \), 
and executes a sequential \emph{command} $\cmd$, given by the following grammar:
\[
\begin{array}{@{} r @{\hspace{2pt}} l @{\hspace{30pt}} r @{\hspace{2pt}} l@{} }
	\cmd ::=  &
        \pskip \mid 
        \ptrans{\trans} \mid 
	    \cmdpri \mid  
        \cmd \pseq \cmd \mid 
        \cmd \pchoice \cmd \mid 
        \cmd \prepeat 
        
   & \cmdpri ::=  &
   		\passign{\txvar}{\expr} \mid 
   		\passume{\expr} \\
%   
	\trans ::= &
        \pskip \mid
        \transpri \mid 
        \trans \pseq \trans \mid
        \trans \pchoice \trans \mid
        \trans\prepeat    
	& \transpri ::= &
   		\cmdpri \mid
        \plookup{\txvar}{\expr} \mid
        \pmutate{\expr}{\expr} 
 \end{array} 
\]
%
Sequential commands include the standard constructs of $\pskip$, sequential composition ($\cmd \pseq \cmd$), non-deterministic choice ($\cmd \pchoice \cmd$), loops $\cmd\prepeat$, 
as well as \emph{transactions} ($\ptrans{\trans}$) and primitive commands. 
Primitive commands include variable assignments ($\passign{\txvar}{\expr}$) and assume statements ($\passume{\expr}$) used to encode conditionals,
and are split into transactional ones (the $\transpri$ clause) 
and non-transactional ones (the $\cmdpri$ clause).
Transactional primitive commands are used for reading and writing to kv-stores and 
can be invoked only within the boundaries of transactions (the $\ptrans{\trans}$ clause).
Non-transactional primitive commands are used for computations over client-local data
and can be invoked without restrictions.

For clarity, we often write \( \cmd_{1}\ppar \dots \ppar \cmd_{n}\) as syntactic sugar 
for a program \( \prog \) with $n$ implicit clients associated with identifiers, 
$\cl_1 \dots \cl_n$, where each client $\cl_i$ executes $\cmd_i$: 
\( \prog = \Set{\cl_{1} \mapsto \cmd_{1}, \dots, \cl_{n} \mapsto \cmd_{n}  }\).

As is standard, we assume a language of expressions built from values ($\val \in \Val$), 
and (client-local) \emph{program variables} $\Vars$, ranged over by $\pvar{x}, \pvar{y}, \cdots$. 
The evaluation $\evalE{\expr}$ of  expression $\expr$ is parametric in the (client-local) \emph{stack} 
$\stk \in \Stacks \defeq \Vars \to \Val$, mapping program variables to values. 
\[
\expr  ::= 
        \val \mid
        \var \mid
        \expr + \expr \mid
        \dots  
\qquad   
\evalE{\val}  =  \val \quad 
\evalE{\var} = \stk(\var)  \quad  
\evalE{\expr_{1} + \expr_{2}}  =  \evalE{\expr_{1}} + \evalE{\expr_{2}} \quad
\dots
\]


\subsubsection{Operational Semantics of Transactions}
Transactional commands in $\transpri$ are associated with a transition system: 
$\toLTS{\transpri} \subseteq (\Stacks \times \Snapshots) \times (\Stacks \times \Snapshots)$, 
describing how the snapshot and stack evolve upon executing $\transpri$:
% \cref{fig:semantics}.
\[
\begin{array}{rcl @{\qquad} rcl}
(\stk, \sn)  & \toLTS{\passign{\var}{\expr}}          & (\stk\rmto{\var}{\evalE{\expr}}, \sn)                  &
(\stk, \sn)  & \toLTS{\passume{\expr}}                & (\stk, \sn) \text{ where } \evalE{\expr} \neq 0        \\
(\stk, \sn)  & \toLTS{\plookup{\var}{\expr}}           & (\stk\rmto{\var}{\sn(\evalE{\expr})}, \sn)              &
(\stk, \sn)  & \toLTS{\pmutate{\expr_{1}}{\expr_{2}}} & (\stk, \sn\rmto{\evalE{\expr_{1}}}{\evalE{\expr_{2}}}) \\
\end{array}                                                                                               
\]

To compute the overall effect of a transaction,
we define a \emph{fingerprint function}, 
$\func{fp}{\stub} : \Stacks \times \Snapshots \times \transpri \rightarrow \Ops \cup \Ops$, extracting the operation of a primitive transactional command: 
%
\[
\begin{array}{rcl @{\quad} rcl}
\func{fp}{\stk, \sn, \passign{\var}{\expr}}          & \defeq & \emptyop                                     &
\func{fp}{\stk, \sn, \passume{\expr}}                & \defeq & \emptyop                                     \\
\func{fp}{\stk, \sn, \plookup{\var}{\expr}}           & \defeq & (\otR, \evalE{\expr}, \sn(\evalE{\expr}))     &
\func{fp}{\stk, \sn, \pmutate{\expr_{1}}{\expr_{2}}} & \defeq & (\otW, \evalE{\expr_{1}}, \evalE{\expr_{2}}) \\
\end{array}
\]
%and a \emph{fingerprint composition operator} \( \addO \).
Note that non-transactional primitive commands are associated with the empty operation $\varepsilon$,
as they only access the local stack and do not access the kv-store.

We further define a \emph{fingerprint composition operator}, \( \addO \), 
incrementally computing the fingerprint of a transaction, after executing each constituent primitive command. 
For instance, when executing $ \ptrans{\trans}$ with $\trans \defeq \transpri^1; \cdots ; \transpri^n$,
the effect of each $\transpri^i$ is calculated via the $\op_i = \func{fp}{-, -, \transpri^i}$ function, 
with the overall fingerprint given as the $\addO$-composition of the constituent effects: $\op_1 \addO \cdots \addO \op_n$. 

For each key $\key$, the composition operator \( \addO \) records
the first value a transaction reads (before a subsequent write) for $\key$, 
and the last value the transaction writes for $\key$.
This is in line with our assumption that transactions read from an atomic snapshot of the kv-store.
In particular, for each key $\key$, 
only the first read from $\key$ fetches its value from the kv-store,
and since clients observe either none or all effects of a transaction, 
only the last write to $\key$ is committed.
%
\begin{align*}
    \fp \addO (\otR, \key, \val)  & \defeq
    \begin{cases}
        \fp \cup \Set{(\otR, \key, \val)} & \text{if} \ \fora{l, v'} (l, \key, v') \notin \fp \\
        \fp &  \text{otherwise} \\
    \end{cases} 
    \fp \addO \emptyop  \defeq  \fp \\
    \fp \addO (\otW, \key, \val) & \defeq 
    \left( \fp \setminus \Set{(\otW, \key, \val')}[\val' \in \Val] \right) \cup \Set{(\otW, \key, \val)} 
\end{align*}
\]
%
\ifTechReport
    \input{\RootPath/semantics/semantics-fig.tex}
\else
\begin{figure}[t]
\hrulefill
\begin{mathpar}
    \inferrule[\rl{TPrimitive}]{%
        (\stk, \sn) \toLTS{\transpri} (\stk', \sn')
        \\ \op = \func{fp}{\stk, \sn, \transpri}
    }{%
        (\stk, \sn, \fp) , \transpri \ \toTRANS \  (\stk', \sn', \fp \addO \op) , \pskip 
    }
    \\
    \inferrule[\rl{TChoice}]{
        i \in \Set{1,2}
    }{%
        (\stk, \sn, \fp) , \trans_{1} \pchoice \trans_{2} \ \toTRANS \  (\stk, \sn, \fp) , \trans_{i}
    }
    \and
    \inferrule[\rl{TIter}]{ }{%
        (\stk, \sn, \fp),  \trans\prepeat \ \toTRANS \  (\stk, \sn, \fp), \pskip \pchoice (\trans \pseq \trans\prepeat)
    } 
    \and
    \inferrule[\rl{TSeqSkip}]{ }{%
        (\stk, \sn, \fp), \pskip \pseq \trans \ \toTRANS \  (\stk, \sn, \fp), \trans
    }
    \and
    \inferrule[\rl{TSeq}]{%
        (\stk, \sn, \fp), \trans_{1} \ \toTRANS \  (\stk', \sn', \fp'), \trans_{1}'
    }{%
        (\stk, \sn, \fp), \trans_{1} \pseq \trans_{2} \ \toTRANS \  (\stk', \sn', \fp'), \trans_{1}' \pseq \trans_{2}
    }
\end{mathpar}
\hrulefill
\[
    \inferrule[\rl{PCommit}]{%
        \vi \viewleq  \vi''
        \qquad \sn = \snapshot[\mkvs,\vi'']
        \qquad \txid \in \nextTxid(\cl, \mkvs)
        \\\\ (\stk, \sn, \emptyset), \trans \ \toTRANS^{*} \  (\stk', \stub,  \fp) , \pskip
        \\ \ET \vdash (\mkvs, \vi'') \csat \fp : \vi'
    }{%
        \cl \vdash ( \mkvs, \vi, \stk ), \ptrans{\trans} \ \toCMD{(\cl, \vi'', \fp)}_{\ET} \ ( \updateKV[\mkvs, \vi, \txid, \fp],\vi', \stk' ) , \pskip
    }
\]
\[
    \inferrule[\rl{PPrimitive}]{
        \stk \toLTS{\cmdpri} \stk'
    }{%
    \cl \vdash ( \mkvs, \vi, \stk ) , \cmdpri \ \toCMD{(\cl,\iota)}_{\ET} \  ( \mkvs, \vi, \stk' ) , \pskip
    }
\]
\hrulefill
\[
    \inferrule[\rl{PProg}]{%
         \cl \vdash ( \mkvs, \vi, \thdenv(\cl) ) , \prog(\cl), \ \toCMD{\lambda}_{\ET} \  ( \mkvs', \vi', \stk' ) , \cmd'  
    }{%
         (\mkvs, \vienv\rmto{\cl}{\vi}, \thdenv ), \prog  \ \toCMD{\lambda}_{\ET} \  ( \mkvs', \vienv\rmto{\cl}{\vi'}, \thdenv\rmto{\cl}{\stk'} ) , \prog\rmto{\cl}{\cmd'} ) 
    }
\]
\hrulefill
\caption{Selected operational semantics rules for transactions (above); sequential commands (middle); and programs (below)}
\label{fig:semantics}
\end{figure}
\fi

In the top part of \cref{fig:semantics} we present a few selected rules of the operational semantics of transactional code (within the transaction boundaries in $\ptrans{}$). 
We refer the reader to \cref{sec:full-semantics} for the full operational semantics.
Transactional rules are of the form $(\stk, \sn, \fp), \toTRANS (\stk', \sn', \fp'), \trans'$, 
stating that when the fingerprint accumulated so far is recorded in $\fp$, 
executing $\trans$ for one step transforms the client-local stack $\stk$ 
and snapshot $\sn$ %(used to fetch the values of read operations),
to $\stk'$ and $\sn'$, respectively, with the extended fingerprint $\fp'$, and continuation $\trans'$.
The \rl{TSeq} rule is in a standard format; 
the \rl{TPrimitive}  models the execution of primitive transactional commands.
When $(\stk, \sn)$ is transformed to $(\stk', \sn')$ via the transition system $\toLTS{\transpri}$,
$\func{fp}{\stk, \sn, \transpri} = \op$, and the fingerprint recorded so far is given by $\fp$, 
then executing $\transpri$ transforms $(\stk, \sn)$ to $(\stk', \sn')$, with the fingerprint updated to $\fp \addO \op$ (to incorporate the effect of $\transpri$), with continuation $\pskip$. 

\subsubsection{Operational Semantics of Commands}
In \cref{fig:semantics} we present a select number of \emph{(sequential) command operational semantics}.
We refer the reader to \cref{sec:full-semantics} for the full operational semantics.
Command transitions are of the form $\cl \vdash (\mkvs, \vi, \stk), \cmd \ \toCMD{\lambda}_{\ET} \ (\mkvs', \vi', \stk') , \cmd'$, 
stating that given the kv-store $\mkvs$, view $\vi$ and stack $\stk$, client $\cl$ may execute command $\cmd$ for one step under $\ET$, update the kv-store to $\mkvs'$, the stack to $\stk'$, and the command to its continuation $\cmd'$, with label $\lambda$.
A transition label $\lambda$ is either
\begin{enumerate*}
	\item of the form $(\cl, \iota)$, denoting that the transition involved 
client-local computation that did not require access to the kv-store (\eg primitive commands $\cmdpri$; or
	\item of the form $(\cl, \vi, \fp)$, denoting that client $\cl$ commits a transaction with fingerprint $\fp$ under the view $\vi$.
\end{enumerate*}
Note that the operational semantics of commands are parametric in the choice of execution test $\ET$, 
and thus the choice of the underlying consistency model.


With the exception of the \rl{PCommit} rule, the remaining command transitions are standard and behave as expected. 
For instance, the \rl{PPrimitive} rule models the execution of a non-transactional primitive command $\cmdpri$, where the $\stk \toLTS{\cmdpri} \stk'$ transition describes how the stack of a client 
evolve upon executing $\cmdpri$:
\[
\begin{array}{rcl @{\qquad} rcl}
\stk  & \toLTS{\passign{\var}{\expr}} & \stk\rmto{\var}{\evalE{\expr}} &
\stk  & \toLTS{\passume{\expr}} & \stk \text{ where } \evalE{\expr} \neq 0 \\
\end{array}                                                                                               
\]
%
%
The \rl{PCommit} rule models the execution of a transaction $\ptrans{\trans}$, under the execution test $\ET$. 
The first premise of \rl{PCommit} states that the current view $\vi$ of the executing command maybe advanced to a newer atomic view $\vi''$ (see \cref{def:views}). 
The semantics only allows to advance the view to latest versions, which corresponds to \emph{monotonic read} \cite{.......}.
Given the new view $\vi''$, the transaction proceeds by obtaining a snapshot $\sn$ of the kv-store $\mkvs$, and executing $\trans$ locally to completion ($\pskip$), updating the stack to $\stk'$, while accumulating the fingerprint $\fp$. Note that the resulting snapshot is ignored (denoted by $\stub$) as the effect of the transaction is recorded in the fingerprint $\fp$. 
%

The transaction is now ready to commit and may propagate its changes to $\mkvs$.
To this end, a \emph{fresh} transaction identifier $\txid \in \nextTxid(\cl, \mkvs)$ (defined shortly) is picked
to identify the completed transaction, and the changes performed by $\txid$ are propagated to $\mkvs$. 
This is done via the $\func{updateMKVS}{\mkvs, \vi, \txid, \fp}$ function (defined shortly) to update $\mkvs$. 
%The fresh identifier $\txid$ is given by the $t \in \nextTxid(\cl, \mkvs)$ function defined shortly.
Once the kv-store is updated, the client subsequently updates its view to $\vi'$ with respect to its fingerprint. 
Lastly, to ensure that the effect of the transaction (its fingerprint  $\fp$) is permitted by the underlying consistency model, 
the last premise requires that the updates be permitted by the execution test $\ET$, \ie \( (\mkvs, \vi'') \csat \fp : \vi'\).

The $\nextTxid(\cl, \mkvs)$ returns the set of transactions identifiers associated with $\cl$ that are fresh with respect to $\mkvs$: 
$\nextTxid(\cl, \mkvs) \defeq \Set{\txid_{\cl}^{n}}[\fora{m} \txid_{\cl}^{m} \in \mkvs \implies m < n ]$.
Note that when $\txid_\cl^n = \nextTxid(\cl, \mkvs)$ in the premise of \rl{PCommit}, then $\txid_\cl^n$ is greater than any transaction identifier 
(with respect to session order $\toEDGE{\SO}$) 
of the form $\txid_{\cl}^{i}$ appearing in $\mkvs$,
as to reflect the fact that $\txid_\cl^n$ is the most recent transaction executed by $\cl$.

%
The \( \updateKV \) function is defined below, where $\lcat$ denotes list concatenation; 
and when $\vilist = \ver_0, \cdots, \ver_n$ and $i=0,\cdots,n$, 
$\vilist\rmto{i}{\ver}$ denotes the updated list 
$\vilist' = \ver_0, \cdots, \ver_{i-1}, \ver, \ver_{i+1}, \cdots, \ver_{n}$. 
%
%
%
%
\begin{align*}         
    \updateKV[\mkvs, \vi, \txid, \emptyset] &\defeq \mkvs \\
    \updateKV[\mkvs, \vi, \txid, \fp \uplus \Set{(\otR, \key, \stub)}] & \defeq 
    \begin{multlined}[t]
        \texttt{let} \ (\val, \txid', \txidset) = \mkvs(\key, \max_{<}(\vi(\key))), \\
        \vilist = \mkvs(\key)\rmto{\max_{<}(\vi(\key))}{(\val, \txid', \txidset \uplus \Set{ \txid })}\\
        \texttt{in} \ \updateKV[\mkvs\rmto{\key}{\vilist}, \vi, \txid, \fp]
    \end{multlined} \\
    \updateKV[\mkvs, \vi, \txid, \fp \uplus \Set{(\otW, \key, \val)}]& \defeq &  
    \begin{multlined}[t]
        \texttt{let } \mkvs' = \mkvs\rmto{\key}{ \mkvs(\key) \lcat (\val, \txid, \emptyset) } \\
        \quad \texttt{in } \updateKV[\mkvs', \vi, \txid, \fp]
    \end{multlined} \\
\end{align*}
%
%
For every read operation $(\otR, \key, \stub)$ in fingerprint $\fp$,
since a transaction reads the values of keys from 
the atomic snapshot determined by the view of the client, 
the version read by $\txid$ for key $\key$ corresponds to $\mkvs(\key, \max_{<}(\vi(\key)))$.
As such, to commit the transaction, 
the reader set of the version $\mkvs(\key, \max_{<}(\vi(\key)))$ is extended with a new reader $\txid_\cl^n$.
Similarly, for every write operation $(\otW, \key, \val)$ in fingerprint $\fp$, 
the list of versions $\mkvs(\key)$ is extended with a new version $(\val, \txid, \emptyset)$, 
denoting that $\txid_\cl^n$ is the writer of this version which has no readers as of yet. 

Note that the assumption that 
versions of a given key are totally ordered and consistent with the order in which 
transactions commit is standard, 
which corresponds to last-write-win resolution policy \cite{adya,framework-concur,seebelieve}. 
Moreover, under the assumption that fingerprints contain at most one read and one write 
operation per key, and the identifier is fresh $\txid \notin \mkvs$%
\footnote{%
We write $\txid \in \mkvs$ when there exists a key 
$\key$ and an index $i=0,\cdots, \lvert \mkvs(\key) \rvert -1$ such that $\txid \in \Set{\wtOf(\mkvs(\key, i)} \cup \rsOf(\mkvs(\key, i))$.}, 
the $\updateKV$ is well-defined.

\subsubsection{Operational Semantics of Programs}

The \emph{operational semantics of programs} are given at the bottom of \cref{fig:semantics}. 
Programs transitions are of the form $(\conf,  \thdenv, \prog) \ \toPROG{\lambda}_{\ET} (\conf',  \thdenv', \prog')$,
stating that given the configuration $\conf$ and the \emph{client environment} $\thdenv$, executing program $\prog$ for one step under $\ET$, updates the configuration to $\conf'$, the client environment to $\thdenv'$, and the program to its continuation $\prog'$. 
A \emph{client environment}, $\thdenv \in \ThdEnv$, is a mapping from client identifiers to pairs of stacks and views. 
We assume that the clients in the domain of client environments are are those in the domain of the program throughout the execution: 
$\dom(\thdenv) = \dom(\prog)$.
Program transitions are simply defined in terms of the transitions of their constituent client commands.
This in turn yields the standard interleaving semantics for concurrent programs. 
That is, a client performs a reduction in an atomic step, without affecting other clients.


